Asymptotic Differential Algebra and Model Theory of Transseries

We develop here the algebra of the differential field of transseries and of related valued differential fields. This book contains in particular our recently obtained decisive positive results on the model theory of these structures.

==> mt-9-1.tex <==
\section{Asymptotic Fields and Asymptotic Couples}\label{As-Fields,As-Couples}

\noindent
In the first subsection we define asymptotic fields and differential-valued
fields, in the second subsection we
show how to visualize an asymptotic couple, in the third subsection
we introduce the asymptotic couple of an asymptotic field,
and in the last subsection we define comparability classes.


\subsection*{Asymptotic fields} 
An {\bf asymptotic differential field}, or just {\bf asymptotic field\/}, 
is a valued differential field $K$  such that for all 
$f,g\in K^\times$ with $f,g\prec 1$,
\begin{itemize}
\item[(A)] $f\prec g \Longleftrightarrow f'\prec g'$.
\end{itemize}
If in addition we have for all $f,g\in K^\times$ with $f,g\prec 1$,
\begin{itemize}
\item[(H)] $f\prec g \Longrightarrow f^\dagger\succeq g^\dagger$,
\end{itemize}
then we say that $K$ is an {\bf $H$-asymptotic field\/} \label{p:H-asymptotic field} or an asymptotic field
of {\bf $H$-type.} Our main interest is in $H$-asymptotic fields, 
but many things go through without the $H$-type assumption.
An {\bf asymptotic extension} of an asymptotic field $K$ is by definition a valued differential field extension of $K$ that is asymptotic.  

\index{extension!asymptotic}
\index{asymptotic extension}
\index{valued differential field!asymptotic}
\index{field!asymptotic}
\index{asymptotic field}
\index{asymptotic field!of $H$-type}
\index{$H$-asymptotic field}

\begin{lemma}\label{neatderas} Let $K$ be a valued differential field such that 
$C\subseteq \mathcal{O}$, $\der \smallo\subseteq \smallo$, and $\der$ is 
neatly surjective. Then $K$ is asymptotic.
\end{lemma}
\begin{proof} From $C\subseteq \mathcal{O}$ we obtain $C\cap \smallo=\{0\}$, so
the restriction of $\der$ to $\smallo$ is injective. From $\der \smallo\subseteq \smallo$ we obtain a strictly increasing map 
$v_{Y'}=v_{\der}: \Gamma \to \Gamma$ with $v_{\der}(0)=0$. 
Let $f,g\in \smallo^{\ne}$.
Then $f', g'\in \smallo^{\ne}$, so $v_{\der}(vf)=v(f')$ and $v_{\der}(vg)=v(g')$ by
the neat surjectivity of $\der$.
Thus $f\prec g\Longleftrightarrow f'\prec g'$. 
\end{proof}

\noindent
Suppose $K$ is an asymptotic field. Then
$C\cap \smallo=\{0\}$: if $0\ne c\in C\cap \smallo$, 
then $c^2\prec c\prec 1$, so $0=(c^2)'\prec c'=0$ by
(A), which is impossible. Thus the valuation $v$ is trivial on $C$, and
the map $\varepsilon\mapsto\varepsilon'\colon \smallo\to K$ is injective.
In particular, $C\subseteq \mathcal{O}$ and 
the residue map $a \mapsto \bar{a}\colon \mathcal{O} \to \k$ is injective on 
$C$.
The following three conditions on $K$ are clearly equivalent: \begin{enumerate}
\item $\mathcal{O}=C+\smallo$;
\item $\{\bar{a}:\ a\in C\}=\k$;
\item for all $f\asymp 1$ in $K$ there exists $c\in C$ with $f\sim c$.
\end{enumerate}
\noindent
We say that $K$ is {\bf differential-valued\/} (or {\bf $\d$-valued}, for short) if it satisfies these 
three
(equivalent) conditions. The next lemma is clear from (3) above.

\label{p:dv}
\index{field!differential-valued}
%\index{field!$H$-differential-valued}
\index{differential-valued}
\index{valued differential field!differential-valued}
%\index{$H$-differential-valued field}
%\index{valued differential field!$H$-differential-valued}

\begin{lemma}\label{dv}
If $L$ is an asymptotic extension of a $\d$-valued field $K$ with
$\res(K)=\res(L)$, then $L$ is $\d$-valued, with $C_L=C$. 
\end{lemma}


\noindent
%Differential-valued fields of $H$-type are also called 
%{\em $H$-differential-valued fields}. 
Our final results in Chapter~\ref{ch:QE} concern 
just $\d$-valued fields of $H$-type such as $\mathbb{T}$, but towards this goal 
we need the wider setting of $H$-asymptotic fields 
where we can coarsen and pass to suitable
differential subfields at our convenience.



\begin{figure}[h!]
\begin{picture}(300,200)

\put(0,0){\line(0,1){200}}
\put(0,0){\line(1,0){300}}

\put(20,20){\line(0,1){160}}
\put(20,20){\line(1,0){260}}

\put(40,40){\line(0,1){120}}
\put(40,40){\line(1,0){220}}

\put(60,60){\line(0,1){80}}
\put(60,60){\line(1,0){180}}

\put(0,200){\line(1,0){300}}
\put(20,180){\line(1,0){260}}
\put(40,160){\line(1,0){220}}
\put(60,140){\line(1,0){180}}

\put(300,0){\line(0,1){200}}
\put(280,20){\line(0,1){160}}
\put(260,40){\line(0,1){120}}
\put(240,60){\line(0,1){80}}

\multiput(80,80)(0,4){10}{\line(0,1){2.5}}
\multiput(218.5,80)(0,4){10}{\line(0,1){2.5}}
\multiput(80,80)(4,0){35}{\line(1,0){2.5}}

\multiput(218.5,119)(-4,0){35}{\line(-1,0){2.5}}


\put(10,5){valued differential fields}
\put(30,25){asymptotic fields}
\put(50,45){$\d$-valued fields}
\put(70,65){$\d$-valued fields of $H$-type}
\put(90,85){$H$-fields}

\end{picture}
\caption{Classes of valued differential fields.}
\label{fig:classes of valued differential fields}
\end{figure}

\medskip\noindent
The figure above indicates the inclusion relations among some
classes of valued differential fields, with the class of $H$-fields from Section~\ref{Asymptotic-Fields-Section} below as
the smallest class; strictly speaking, $H$-fields are more than just valued differential fields, since they also carry an ordering.

Any differential subfield of an asymptotic field $K$
with the restricted dominance relation is itself
an asymptotic field. If $K$ is an asymptotic
field and $\phi\in K^{\times}$, then its compositional conjugate
$K^\phi$ with the same dominance relation remains an 
asymptotic field with the same constant field. (These two statements 
remain true with {\em $H$-asymptotic\/} in place of {\em asymptotic}.) 
If $K$ is a 
$\d$-valued field and $\phi\in K^{\times}$, then 
$K^\phi$ (with same dominance relation) remains $\d$-valued.

An asymptotic field is said to be {\bf asymptotically maximal} if it has no proper immediate asymptotic field extension. Likewise, 
an asymptotic field is said to be {\bf asymptotically $\d$-algebraically maximal} 
if it has no proper immediate $\d$-algebraic asymptotic field extension. By Zorn, any asymptotic field has an asymptotically maximal
immediate asymptotic field extension, and also an asymptotically $\d$-algebraically maximal immediate $\d$-algebraic asymptotic field extension.
%These notion will become important in Chapter~\ref{ch:newtonian %fields}.

\label{p:asymptotically maximal}
\label{p:asymptotically d-algebraically maximal}
\index{asymptotically!maximal}
\index{asymptotically!$\d$-algebraically maximal}
\index{asymptotic field!asymptotically maximal}
\index{asymptotic field!$\d$-algebraically maximal}

\subsection*{Asymptotic couples} We defined asymptotic couples
in Section~\ref{sec:ascouples}. Consider an asymptotic couple $(\Gamma, \psi)$.
For reasons that will become clear in the next subsection we also 
use the notation
$$ \alpha^\dagger:= \psi(\alpha), \qquad \alpha':= \alpha + \psi(\alpha) \qquad (\alpha \in \Gamma^{\ne}).$$
Of course this is only used when $\psi$ is understood from
the context. Thus $\alpha'>\beta^\dagger$ for $\alpha\in \Gamma^{>},\ \beta\in \Gamma^{\ne}$. The following subsets of $\Gamma$ play special roles:
\begin{align*}  (\Gamma^{\ne})'\ &:=\ \{\gamma':\ \gamma\in \Gamma^{\ne}\}, 
\qquad (\Gamma^{>})'\ :=\ \{\gamma':\ \gamma\in \Gamma^{>}\},\\
   \Psi\ &:=\ \psi(\Gamma^{\ne})\ =\ \{\gamma^\dagger:\ \gamma\in \Gamma^{\ne}\}\ =\ \{\gamma^\dagger:\ \gamma\in \Gamma^{>}\}.
\end{align*}
We call $\Psi$ the $\Psi$-set of $(\Gamma,\psi)$, and 
set $\alpha^\dagger:=\infty\in \Gamma_{\infty}$ for
$\alpha=0\in \Gamma$.  
\input{mt-psipic.tex}
%(This set is denoted by $\Psi$ in \cite{ }, { }, { }, { }.) 
\noindent
Figure~\ref{psipic} gives a rough idea of the graphs of $\gamma'$ and $\gamma^\dagger$
as functions of $\gamma\in \Gamma^{\ne}$. We have found this picture very 
helpful in getting a ``feel'' for asymptotic couples. 
It suggests for example that $\gamma'$ is 
strictly increasing on $\Gamma^{\ne}$, and this is part (3) of Lemma~\ref{BasicProperties}.
It also suggests that $\gamma'$ has the intermediate value property on~$\Gamma^{>}$ as well as on $\Gamma^{<}$. This is the case for 
$H$-asymptotic couples by Lemma~\ref{ivp} below, but not for all asymptotic 
couples; see {\em Example 2.8} in 
\cite{AvdD2}.   
The picture is really meant just for
$H$-asymptotic couples, where $\gamma^\dagger$ is increasing for $\gamma<0$ and
decreasing for $\gamma>0$. Of course, we are unable to make the picture show,
for $H$-asymptotic $(\Gamma, \psi)$, that
$\psi$ is constant on each archimedean class $[\alpha]$, 
$\alpha\in \Gamma^{\ne}$.  

\nomenclature[T]{$\Psi$}{$\psi(\Gamma^{\neq})$}
\nomenclature[T]{$\gamma'$}{$\gamma'=\gamma+\psi(\gamma)$, for $\gamma\neq 0$}
\nomenclature[T]{$\gamma^\dagger$}{$\gamma^\dagger=\psi(\gamma)$, for $\gamma\neq 0$}


  



\subsection*{The asymptotic couple of an asymptotic field}
Let $K$ be an asymptotic 
field. It is clear that then $vg'$ is uniquely determined by $vg$
for $g\in K^\times$ and $vg\ne 0$, that is, the derivation of $K$ induces a function
$$\gamma \mapsto \gamma'\ \colon\ \Gamma^{\ne} \to \Gamma   \qquad \text{($\gamma=vg$, $\gamma'=vg'$, 
 $g$ as above)}$$ 
on its value group $\Gamma$. We also consider the logarithmic-derivative analogue:
$$ \gamma \mapsto \gamma^{\dagger}:= \gamma'- \gamma\ \colon\ \Gamma^{\ne} \to \Gamma,$$
that is, $\gamma^\dagger=v(g^\dagger)$ for $g$ as above.
The asymptotic couple of $K$ is just
the value group of $K$ equipped with this induced operation 
$\gamma \mapsto \gamma^{\dagger}$. To justify this terminology, we characterize asymptotic fields as follows:

\begin{prop}\label{CharacterizationAsymptoticFields}
Let $K$ be a differential field with dominance relation $\preceq$. Then the
following are equivalent:
\begin{enumerate}
\item $K$ is an asymptotic field.
\item There is an asymptotic couple $(\Gamma, \psi)$ with
$\Gamma:=v(K^\times)$ such that for 
all $g\in K^\times$ with $g\nasymp 1$ we have
$\psi(vg)=v(g^\dagger)$.
\item If $f,g\in K^\times$ with
$f,g\nasymp 1$, then $f\preceq g \Longleftrightarrow f'\preceq g'$.
\item If $f,g\in K^\times$, then
$$\begin{cases}
&f\prec 1,\ g\nasymp 1 \quad\Rightarrow\quad f'\prec g^\dagger,\\
&f\asymp 1,\ g\nasymp 1 \quad\Rightarrow\quad f'\preceq g^\dagger.
\end{cases}$$
\end{enumerate}
\end{prop}
\begin{proof}
We first show the equivalence of (2) and (4). Suppose that (2) holds.
The first implication of (4) is clear. For the second implication, 
let $f,g\in K^\times$, $f\asymp 1$, $g\nasymp 1$.
We have $g^\dagger\asymp (fg)^\dagger=f^\dagger+g^\dagger$.
Hence $f'\asymp f^\dagger\preceq g^\dagger$.
Conversely, suppose that (4) holds. Let $f,g\in K^\times$ with $f\asymp g
\prec 1$. Then
$f^\dagger - g^\dagger = (f/g)^\dagger \asymp (f/g)'$ with $f/g\asymp 1$,
so $f^\dagger-g^\dagger \preceq f^\dagger$ and 
$f^\dagger-g^\dagger\preceq g^\dagger$
by the second implication of (4). It follows that $f^\dagger\asymp g^\dagger$.
Thus $v(f^\dagger)$ only depends on $vf$, for $f\in K^{\times}$ with 
$f\nasymp 1$.
The first implication of (4) now yields (2).

Note that 
(2)~$\Rightarrow$~(3) is a consequence of Lemma~\ref{BasicProperties},~(3),
and (3)~$\Rightarrow$~(1) is trivial. Lemma~\ref{CharAsymptoticCouples} gives (1)~$\Rightarrow$~(2).
\end{proof}


\noindent
If $K$ is an asymptotic field, we call $(\Gamma,\psi)$ as
defined in (2) of Proposition~\ref{CharacterizationAsymptoticFields} 
the {\bf asymptotic couple of $K$}. An asymptotic field is of $H$-type iff
its asymptotic couple is of $H$-type. If $(\Gamma,\psi)$ is the 
asymptotic couple of the asymptotic field $K$ and $a\in K^{\times}$, 
then $(\Gamma, \psi^a)$ with $\psi^a:= \psi-va$ is the asymptotic couple 
of $K^a$.

\index{asymptotic couple!of an asymptotic field}
\index{asymptotic field!asymptotic couple}
\index{asymptotic couple!shift}

\begin{cor}\label{CharacterizationAsymptoticFields-Corollary}
Let $K$ be an asymptotic field and $f,g\in K$. Then
\begin{enumerate}
\item if $f\prec g\nasymp 1$, then $f'\prec g'$;
\item if $f\preceq g\nasymp 1$, then $f\sim g \Longleftrightarrow f'\sim g'$;
\item if $f\preceq g\nasymp 1$ and $g'\preceq g$, then $f^{(n)}\preceq g'$
for all $n\ge 1$;
\item if $f\asymp 1$ and $0\neq g\nasymp 1$, then
$f^\dagger\not\sim g^\dagger$.
\end{enumerate}
\end{cor}
\begin{proof}
For (1), if $f\prec g$ and $f,g\nasymp 1$, then $f'\prec g'$
by Proposition~\ref{CharacterizationAsymptoticFields},~(3), 
and if $1\asymp f\prec g$, then $f'\preceq g^\dagger=g'/g
\prec g'$ by Proposition~\ref{CharacterizationAsymptoticFields},~(4). 
For (2), suppose that~$g\nasymp 1$.
If $f\sim g$, then $1\nasymp g\succ f-g$, so $g'\succ f'-g'$ by (1),
i.e.,~$f'\sim g'$. Conversely, suppose that $f\preceq g\nasymp 1$ and 
$f'\sim g'$. If $f-g\nasymp 1$
then  Proposition~\ref{CharacterizationAsymptoticFields},~(3), yields
$f \sim g$. 
If $f-g\asymp 1$, then  $g\succ 1$, and thus $f-g\asymp 1\prec g$.
Part (3) follows by induction on $n$ from (1) and
Proposition~\ref{CharacterizationAsymptoticFields},~(3).
As to (4), if  $f\asymp 1$ and $0\neq g\nasymp 1$, then
$g/f\asymp g\nasymp 1$, so 
$(g/f)^\dagger=g^\dagger-f^\dagger \asymp
g^\dagger$, hence~$f^\dagger\not\sim g^\dagger$.
%Part (5) follows from
%(4) in Proposition~\ref{CharacterizationAsymptoticFields}.
\end{proof}

\noindent
In the next two corollaries we assume that $K$ is an asymptotic field.


\begin{cor}\label{c1} The derivation of $K$ is continuous.
\end{cor}
\begin{proof} If $\Gamma=\{0\}$, then the
valuation topology on $K$ is discrete and so $\der$
is continuous. Assume $\Gamma \ne \{0\}$,
and take $g\in K^\times$ with $g\succ 1$. Then $a:= g'\ne 0$, and
so $\der \smallo \subseteq a\smallo$ by Corollary~\ref{CharacterizationAsymptoticFields-Corollary}. Thus $\der$ is continuous by Lemma~\ref{cd2}.
\end{proof}

\noindent
As a consequence of Corollary~\ref{c1} and Lemma~\ref{ExtendingDerivation}, 
the completion  $K^{\operatorname{c}}$ of our asymptotic field $K$ 
is naturally a valued differential field, but more is true:


\begin{cor}\label{completingasymp} The valued differential field $K^{\operatorname{c}}$ is an asymptotic field. If $K$ is $\d$-valued, then so is $K^{\operatorname{c}}$.
\end{cor}
\begin{proof} 
We claim that~$K^{\operatorname{c}}$ is asymptotic with the same asymptotic couple
$(\Gamma, \psi)$ as $K$, and to show this
we use (2) of Proposition~\ref{CharacterizationAsymptoticFields}. Let 
$f\in K^{\operatorname{c}}$ and
$0\ne f\nasymp 1$. Density of $K$ in $K^{\operatorname{c}}$ gives $g\in K$ with
$f\sim g$ and $f'\sim g'$. Then $\psi(vf)=\psi(vg)=v(g^\dagger)=v(f^\dagger)$. This proves our claim. If $K$ is even $\d$-valued, then so is~$K^{\operatorname{c}}$ by Lemma~\ref{dv},
since $\res{K}=\res{K^{\operatorname{c}}}$. 
\end{proof}

\index{completion!of an asymptotic field}
\index{asymptotic field!completion}

\noindent
We say that an asymptotic couple $(\Gamma, \psi)$ has 
{\bf  asymptotic integration }
if $$\Gamma=(\Gamma^{\ne})'.$$ An asymptotic field is said to 
have {\bf asymptotic integration\/} if its asymptotic couple has asymptotic integration.
The reason for this terminology is that if $K$ is a $\d$-valued field,
then $K$ has asymptotic integration iff for all $a\in K^\times$ there is
$b\in K$ such that $a\sim b'$. 

\label{p:asymptotic integration}
\index{asymptotic integration!}
\index{asymptotic field!with asymptotic integration}
\index{asymptotic couple!with asymptotic integration}

\subsection*{Comparability and groundedness} Let
$K$ be an asymptotic field.
On the set~$K^\times$ we
define the binary relations $\comp$,~$\flatter$,~$\flattereq$ as follows:
\begin{align*}
f\comp g \quad &:\Longleftrightarrow\quad f^\dagger \asymp g^\dagger, \\
f\flatter g \quad &:\Longleftrightarrow\quad f^\dagger \prec g^\dagger, \\
f\flattereq g \quad &:\Longleftrightarrow\quad f^\dagger \preceq g^\dagger.
\end{align*}
For the meaning of $\flattereq$ in
Hardy fields, see Corollary~\ref{hardyflateq}. Note: these relations on $K^\times$ do not change when passing from $K$ to a compositional conjugate $K^{\phi}$ with~$\phi\in K^\times$. 
For $f,g\in K^\times$ with $f,g\nasymp 1$ we say that
$f$ and~$g$ are {\bf comparable} if $f\comp g$,  and we say that
$f$ is {\bf flatter} than $g$ if 
$f\flatter g$. 
 Comparability
is an equivalence relation on $\{f\in K^\times: f\nasymp 1\}$. The equivalence
class of an element~$f$ from this set is called its {\bf comparability class},
written as $\Cl(f)$. The relation $\flatter$ induces a linear ordering
on the set of comparability classes by 
$$\Cl(f)<\Cl(g)\ :\Longleftrightarrow\
f\flatter g.$$ Let $(\Gamma,\psi)$ be the asymptotic couple of $K$. Then for $f\in K^\times$ with $f\nasymp 1$ we have:
$\Cl(f)$ is the smallest comparability class of $K$ iff $\psi(vf)$ is the largest element of~$\Psi$. Thus $K$ has a smallest comparability class iff $\Psi$ has a largest element. Note also that if $K$ is of $H$-type and
$f,g\in K$, then $1\prec f\preceq g \Rightarrow f\flattereq g$. We define the asymptotic field $K$ to be {\bf grounded}
if $K$ has a smallest comparability class, equivalently,
$\Psi$ has a largest element; an asymptotic field that is not grounded is called {\bf ungrounded}. 

\label{p:grounded asymptotic field}
\nomenclature[R]{$f\comp g$}{$f$ and $g$ are comparable}
\nomenclature[R]{$f\flatter g$}{$f$ is flatter than $g$}
\nomenclature[R]{$f\flattereq g$}{$f$ is flatter than or comparable with $g$}
\nomenclature[Rx]{$\Cl(f)$}{comparability class of $f$}
\index{comparability class}
\index{comparable}
\index{flatter}
\index{asymptotic field!grounded}
\index{grounded!asymptotic field}




==> mt-9-10.tex <==


\section{Miscellaneous Facts about Asymptotic Fields}
\label{Miscellaneous Facts about Asymptotic Fields}

\noindent
This section indicates some possible and impossible features
of asymptotic fields. Only Lemma~\ref{sine cosine} will be
used later. 
Can a differentially closed field 
have a nontrivial valuation making it an asymptotic field? This was 
answered negatively by Scanlon~\cite{Scanlon08}. The solution given 
here, inspired by
Rosenlicht~\cite{Rosenlicht2}, is a little different. Scanlon used the 
logarithmic derivative map of an elliptic curve. The 
differential-algebraic properties of this map are used here 
for another purpose:
to construct asymptotic fields that cannot be obtained 
by coarsening pre-$\d$-valued fields, and to construct an
algebraically closed $\d$-valued field of $H$-type that is not an
algebraic closure of a real closed $\d$-valued field. We finish with
the result that~$\T$ as a subset of $\T[\imag]$ is definable in
the differential field $\T[\imag]$. 






\subsection*{Differentially closed fields cannot be asymptotic} 
In this subsection $K$ is a differential field, with constant field $C$, and
$y$ ranges over $K$.  

\index{differential field!differentially closed}
\index{closed!differentially}

\begin{prop}\label{Scanlon-Prop} If $K$ is differentially closed, 
then there is no valuation ring $\cal{O}\neq K$ of $K$ with 
$\der \cal{O} \subseteq  \cal{O}$. 
\end{prop}
\begin{proof} Let $K$ be differentially closed
and suppose for a contradiction that $\cal{O}\neq K$ is a
valuation ring of $K$ with $\der\cal{O}\subseteq \cal{O}$. Since $K$ remains
 differentially closed upon replacing $\der$
by $a\der$ with $a\in  \smallo^{\neq}$, we can assume
$\der \cal{O}\subseteq \smallo$. Take $y$ such that $y+(y')^2=y^3$ and $y\ne y^3$.
The argument below uses the second part of Lemma~\ref{Cohn-Lemma} several times.
If $y\succ 1$, then $y+(y')^2 \prec y^3$, a contradiction. Thus $y\in \cal{O}$, and so
$y\equiv y^3\bmod \smallo$, hence $y\equiv -1$, $0$, or $1 \bmod \smallo$. The case $y\equiv 0 \bmod \smallo$ is impossible, since $y\ne 0$ gives $(y')^2 \prec y$ and $y^3\prec y$. If $y\equiv \-1 \bmod \smallo$, set $y=z+1$, and
we get a similar contradiction from $-2z + (z')^2 =z^3+3z^2$ and $0\ne z\prec 1$,
and the case $y\equiv -1 \bmod \smallo$ is likewise impossible.    
\end{proof}


\subsection*{The logarithmic derivative map on an elliptic curve}
In this subsection $K$ is a differential field with constant field $C$. 
Let $c\in C$, $c\neq 0,1$, and put
$$P(X) := X(X-1)(X-c) = X^3 - (c+1)X^2 +cX \in C[X].$$
Consider the projective plane curve $E$ defined over $C$ by the equation
$$Y^2Z = X^3 - (c+1)X^2Z + cXZ^2.$$
The affine part of $E$ (in standard coordinates) is given by $Y^2=P(X)$, and
$E$ is an elliptic curve whose group law
has $(0:1:0)$, the unique point at infinity on $E$, as its zero element. 
 
We define the logarithmic derivative map $\ell_E \colon E(K)\to K$ as follows:
$$\ell_E(0:1:0):=0, \quad \ell_E(x:y:1) := x'/y\ \text{ if }y\ne 0, \quad
\ell_E(x:0:1):= 0.$$ By Lemma~2 on p.~805 
of \cite{Kolchin-GTDF}, 
the map $\ell_E$ is a group homomorphism from $E(K)$ to the additive group 
of $K$; its kernel is $E(C)$. 

\begin{lemma}\label{ell_E maps into O}
Let $\cal{O}$ be a valuation ring of $K$ such that $\der \smallo \subseteq \smallo$ and $c,c-1\in \cal{O}\setminus  \smallo$. 
Then $\ell_E\big(E(K)\big)\subseteq \cal{O}$. 
\end{lemma}
\begin{proof}
Let $x,y\in K$ with $(x:y:1)\in E(K)$. If $y=0$, then 
$\ell_E(x:y:1)=0\in \cal{O}$. Assume $y\neq 0$; 
we need to show $x'/y\preceq 1$. We distinguish two cases. 
Suppose first that $x\preceq 1$; then $y^2= P(x) \preceq 1$, hence 
$y\preceq 1$. Differentiating both sides of the equality $y^2=P(x)$ we 
obtain $2yy'=P'(x)\cdot x'$. Hence if $P'(x)\asymp 1$ then 
$x'/y \asymp 2y'\preceq 1$. Otherwise $P'(x)\prec 1$ and therefore 
$y^2=P(x)\asymp 1$, since the reduced polynomial 
$\bar{P}(X)\in (\res K)[X]$ has no multiple zeros; hence 
$x'/y \asymp x'\preceq 1$. 
Now suppose that $x\succ 1$. Then $y^2=P(x)\asymp x^3$ and $(x')^2 \preceq x^3$ 
by Lemma~\ref{Cohn-Lemma}, therefore $x'/y\preceq 1$.
\end{proof}


\begin{cor} If $\ell_E\colon E(K)\to K$ is surjective, then $K$ has no nontrivial 
valuation making it an asymptotic field.
\end{cor}

\noindent
For use in the next subsection we prove:

\begin{prop}\label{making ell_E surjective}
Suppose $C$ is algebraically closed. There exists a differential field 
extension $L$ of $K$, $\d$-algebraic over $K$ with $C_L=C$, 
such that
\begin{enumerate}
\item $\ell_E\colon E(L)\to L$ is surjective \textup{(}so $L$ has 
no non\-trivial valuation making it an asymptotic 
field\textup{)};
\item for each $y\in L^\times$ with $y^\dagger\in C^\times$ there exists $n>0$
with $y^n\in K$.
\end{enumerate}
\end{prop}

\noindent
The main work goes into proving the next two lemmas, in both of which
$C$ is assumed to be algebraically closed.

\begin{lemma}
There is no group homomorphism $E(C)\to C^\times$ with finite kernel.
\end{lemma}
\begin{proof}
Suppose 
$\varphi\colon E(C)\to C^\times$ is a group homomorphism with 
$k:=\abs{\ker\varphi}<\infty$. For an additive abelian group $G$ 
and $n>0$, put
$G[n] := \{g\in G:ng=0\}$, a subgroup of $G$. Then, for $n>0$, $E(C)[n]$ is 
finite with $\abs{E(C)[n]}=n^2$, see \cite{Silverman}, 
Theorem~VI.6.1, and 
$\varphi\big(E(C)[n]\big)\subseteq \{\zeta\in C^\times: \zeta^n=1\}$. 
Take a prime number $p$ not dividing $k$. Then $\varphi|E(C)[p]$
%\colon E(C)[p\to \{\zeta\in C^\times: \zeta^p=1\}$ 
is injective, contradicting $\abs{\{\zeta\in C^\times: \zeta^p=1\}}\leq p$.
\end{proof}

\begin{lemma}\label{power of y}
Let $a\in K^\times$, and let $f$ be an element in a differential field 
extension of $K$ with the same constant field $C$ as $K$, satisfying 
$(f')^2=a^2P(f)\neq 0$. Let $y$ be a nonzero element of the differential 
field $K\langle f\rangle=K(f,f')$ with $y^\dagger\in C^\times$. Then 
$y^n\in K$ for some $n>0$.
\end{lemma}
\begin{proof}
From Section~\ref{Differential Fields and Differential Polynomials} recall that given a differential field extension $L$ of $K$, we denote by 
$\Aut_\der(L|K)$ the group of differential automorphisms of $L$ which are 
the identity on $K$. 
Suppose for a contradiction that $y^n\notin K$ for all $n>0$. Then $y$ is 
transcendental over $K$, so $f$ is transcendental over $K$. 
%From $y^\dagger \in C^\times$ we obtain that 
Also $\sigma(y)/y\in C^\times$ for every $\sigma\in\Aut_\der\big(K(y)|K\big)$,
and the map 
\begin{equation}\label{isomorphism with multiplicative group}
\sigma\mapsto \sigma(y)/y\colon\Aut_\der\big(K(y)|K\big)\to C^\times
\end{equation}
is a group isomorphism \cite[p.~803]{Kolchin-GTDF}.
Writing the group operation on $E(K)$ additively, we have for
$\sigma\in\Aut_\der\big(K\langle f\rangle|K\big)$,
$$p_\sigma := \big(\sigma(f):\sigma(f'/a):1\big) - (f:f'/a:1)\in E(C),$$
and the map 
\begin{equation}\label{embedding into E(C)}
\sigma\mapsto p_\sigma\colon \Aut_\der\big(K\langle f\rangle|K\big)\to E(C)
\end{equation} 
is an injective group homomorphism \cite[p.~807]{Kolchin-GTDF}. The 
homomorphism 
\begin{equation}\label{restriction homomorphism}
\sigma\mapsto{\sigma\restrict K(y)}\colon
\Aut_\der\big(K\langle f\rangle|K\big)\to\Aut_\der\big(K(y)|K\big)
\end{equation}
is surjective by \cite[Theorem~3 on p.~797]{Kolchin-GTDF}; in particular, 
$\Aut_\der\big(K\langle f\rangle|K\big)$ is infinite. Hence 
the map \eqref{embedding into E(C)} is an 
isomorphism, by \cite[p.~807]{Kolchin-GTDF}. Moreover, the kernel of 
\eqref{restriction homomorphism} is finite by \cite[p.~796, Theorem~2]{Kolchin-GTDF}. Composing the inverse of the map~\eqref{embedding into E(C)} 
with~\eqref{restriction homomorphism} and~\eqref{isomorphism with 
multiplicative group} yields a homomorphism $E(C)\to C^\times$ with finite 
kernel; this is impossible by the previous lemma.
\end{proof}

\noindent
To prove Proposition~\ref{making ell_E surjective}, fix a differential 
closure $K^{\operatorname{dc}}$ of $K$; then
 $K^{\operatorname{dc}}$  is $\d$-algebraic over $K$ and  $C_{K^{\operatorname{dc}}}=C$.
(See Section~\ref{sec:DCF}.) By Zorn we can take a differential subfield
$L$ of $K^{\operatorname{dc}}$ 
containing $K$ which is maximal with respect to the
property that for each $y\in L^\times$ 
with $y^\dagger\in C^\times$ there exists $n>0$ with $y^n\in K$.
Then $\ell_E\big(E(L)\big)=L$. To see this, let $a\in L^\times$ and take 
$f\in K^\times$ with $(f')^2=a^2P(f)\neq 0$. Suppose that $y$ is a nonzero
element of $L\langle f\rangle$ such that $y^\dagger\in C^\times$. 
Lemma~\ref{power of y} (applied to $L$ in place of $K$) yields an 
$n>0$ with $y^n\in L$; since $(y^n)^\dagger=ny^\dagger\in C^\times$, we
have $y^{nm}\in K$ for some $m>0$. So $L\langle f\rangle=L$ by
maximality of $L$; in particular 
$f\in L$ and thus $(f:f'/a:1)\in E(L)$ with
$\ell_E(f:f'/a:1)=a$. \qed


\subsection*{An asymptotic field that is not a coarsening of a 
pre-$\d$-valued field}

Let~$\k$ be a differential field
such that $a'+na\ne 0$ for all $a\in \k^\times$ and $n\geq 1$. Equip~$\k\(( t\)) $ with the valuation $v$ that has $\k[[t]]$ as its valuation ring,
and with the unique derivation extending that 
of $\k$ such that $t'=t$ and $\k[[t]]'\subseteq \k[[t]]$. 
Then $\k\(( t\)) $ is an asymptotic field.  (To see this, 
note that 
$(at^n)'=(a'+na)t^n$ for $a\in \k^\times$ and $n\geq 1$.)
It has small derivation, with $\Psi=\{0\}$ (so its asymptotic
couple is of $H$-type); its differential residue field is
$\k$, and its constant field is $C_\k$. The valued differential subfield 
$K:=\k(t)$ of $\k\(( t\)) $ is an asymptotic field with valuation ring 
$\cal{O}=\k[t]_{(t)}$. If $\k$ has an element $b$ with $b'\ne 0$,
then $vb=vb'=0$, so $K$ is not pre-$\d$-valued in that case.

\begin{lemma}\label{asd}
Suppose $\k$ has an element $b$ with $b'\neq 0$, and $\k$ has no 
nontrivial valuation making it a pre-$\d$-valued field. 
Then $\k(t)$ has no valuation $v_1$ with $v_1(t)>0$ that makes $\k(t)$ a 
pre-$\d$-valued field. 
%such that $t\in\cal O_1$, $t^{-1}\notin\cal O_1$. 
\end{lemma}
\begin{proof}
Suppose $v_1$ is a valuation on $\k(t)$ with $v_1(t)>0$ that makes $\k(t)$ a 
pre-$\d$-valued field. Let $\cal{O}_1$ be the valuation ring of $v_1$.
Then $\cal{O}_1\cap\k$ is a valuation ring of $\k$ making $\k$ a 
pre-$\d$-valued field, so $\cal{O}_1\cap \k=\k$. 
Then $\cal{O}_1=\k[t]_{(t)}=\cal{O}$, which 
contradicts the observation preceding the lemma.
\end{proof}

\noindent
If $\k$ satisfies the hypothesis of the lemma, then
$K$ cannot be obtained by coarsening a pre-differential valuation of $\k(t)$:
there is no valuation $v_1\colon \k(t)^\times\to\Gamma_1$ 
making~$\k(t)$ a pre-$\d$-valued field such that for some
convex subgroup $\Delta$ of $\Gamma_1$ the coarsened valuation
$\dot{v}_1\colon \k(t)^\times \to \Gamma_1/\Delta$ has valuation ring $\cal{O}$. 


\medskip\noindent
To obtain a differential field $\k$ satisfying the 
requirements above we first take any algebraically closed field $C$ 
of characteristic zero. Let 
$C(x)$ be a field extension of $C$ with $x$ transcendental over $C$,
equipped with the unique derivation with constant field $C$ and $x'=1$.
Proposition~\ref{making ell_E surjective} yields a differential 
field extension $\k$ of $C(x)$ such that
for every $y\in\k^\times$ with $y^\dagger\in C^\times$ there exists $n>0$ 
with $y^n\in C(x)$, and such that $\k$ has no nontrivial 
valuation making it an asymptotic field. 
Since there is no $y\in C(x)^\times$ with $y^\dagger\in C^\times$ 
(by Corollary~\ref{cor:no new exps under integration}), 
there is no $y\in\k^\times$ with $y^\dagger\in C^\times$. 
Hence, as required, $a'+na\ne 0$ for all $a\in \k^\times$ and $n\geq 1$, 
$C_\k\neq \k$, and~$\k$ has no nontrivial valuation making it 
a pre-$\d$-valued field. Thus the asymptotic field $K$ defined just 
before Lemma~\ref{asd} cannot be obtained by coarsening a 
pre-differential valuation.



\subsection*{An algebraically closed $\d$-valued field 
that is not an algebraic closure of a real closed $\d$-valued field}
Every algebraically closed field $L$ of characteristic zero has a real 
closed subfield $K$ such that $L=K(\imag)$, where $\imag^2=-1$. This suggests the 
following question: 

\medskip\noindent
{\it Let $L$ be an algebraically closed 
$\d$-valued field of $H$-type; 
is there a real closed $\d$-valued subfield $K$ of $L$ such that 
$L=K(\imag)$?}\/  

\medskip\noindent
We show that the answer is 
negative for $L$ as in Corollary~\ref{newcor}.
This result follows from the next lemma, also used later in this
section.
%Section~\ref{Exceptional Values and Multiplicities}. 
%\marginpar{Reference to be filled in later.}

\begin{lemma}\label{sine cosine}
Suppose $K$ is a real closed $\d$-valued field with an element
$a\in K^\times$ satisfying $a \succ \der \smallo$. 
Then the algebraic
closure $K(\imag)$ of $K$, where $\imag^2=-1$, has no nonzero
element $y$ such that $y^\dagger=a\imag$.
\end{lemma}
\begin{proof} The residue field of $K$ is isomorphic to $C$, hence
real closed, so $K^{\preceq 1}$ is convex in $K$  by Theorem~\ref{thm:KW}.
%Note first that there is no $h\in K^\times$ with $h\sim i$ or $h\sim -i$.
Suppose $y\in K(\imag)^\times$ satisfies $y^\dagger=a\imag$. 
We have $y=f+g\imag$ with $f,g\in K$; think of 
$y$ as $\ex^{\imag\int{a}}$ and of $f$ and $g$ as $\cos \int{a}$ and $\sin \int{a}$. 
So 
$f'=-ag$ and $g'=af$, hence $f,g\neq 0$ and
$$(f^2+g^2)'=2ff'+2gg'=0.$$
Therefore $f^2+g^2\in C^\times$, so $f\preceq 1$ and $g\preceq 1$, and
either $f\succeq 1$ or $g\succeq 1$. Suppose $f\succeq 1$. (The case 
$g\succeq 1$ is similar.)  Since $g'=af\succeq a\succ b'$ for 
all $b\in K^{\preceq 1}$, we have
$g\succ 1$, a contradiction.
\end{proof}


\begin{cor}
If $L$ is a $\d$-valued field with small derivation
and an element $y\in L^\times$ such that  $y^\dagger=\imag$,  $\imag^2=-1$,
then $L$ has no real closed 
$\d$-valued subfield $K$ with $L=K(\imag)$.
\end{cor} 


\subsection*{Definability of $\T$ in $\T[\imag]$} It is well-known that
$\R$ as a subset of $\C=\R[\imag]$ is not definable (even allowing parameters) in the field $\C$ of complex numbers; see~\ref{cor:ACF sm}. In stark contrast, the {\em differential\/} field structure of $\T[\imag]$ is strong enough to define~$\T$:

\begin{prop}\label{prop:defining T} The subset $\T$ of $\T[\imag]$ is definable in the
differential field $\T[\imag]$.
\end{prop} 
\begin{proof} Below, ``definable'' means definable without parameters in the differential field $\T[\imag]$. Let $\mathcal{O}$ be the valuation ring of $\T$
with maximal ideal $\smallo$. Then $\mathcal{O}+\mathcal{O}\imag$
is the valuation ring of $\T[\imag]$ with maximal ideal $\smallo + \smallo \imag$. We begin with noting the definability of $\R$, as a consequence of Lemma~\ref{sine cosine}:
$$\R\ =\ \big\{y\in \T[\imag]:\ \text{$y'=0$ and $y=f^\dagger$  for some 
$f\in \T[\imag]^\times$}\big\}.$$
Indeed, this lemma gives the more
precise result $(\T[\imag]^\times)^\dagger \subseteq \T+\imag \der\smallo$. We claim that $(\T[\imag]^\times)^\dagger = \T+\imag \der\smallo$. To see this, note that for $b\in \smallo$ we have
$$\sin b\ :=\  b-\frac{b^3}{6} + \frac{b^5}{120} -\dots\in \T, \qquad \cos b\ :=\ 1-\frac{b^2}{2} + \frac{b^4}{24} -\dots\in \T^{\ne}$$
with $(\sin b)'=b'\cos b$ and $(\cos b)'=-b'\sin b$, and so
$$f\ :=\ \exp(\imag b)\ :=\ \cos b + \imag \sin b\in \T[\imag]^\times$$ satisfies
$f^\dagger= ib'$. Hence $\imag \der \smallo\subseteq (\T[\imag]^\times)^\dagger$, and thus $\T+ \imag \der \smallo\subseteq (\T[\imag]^\times)^\dagger$, and the claim follows. Think of $\T+\imag \der \smallo$ as a thin strip around the ``real axis'' $\T$ in the ``complex
plane'' $\T[\imag]$. Intersecting $\T+\imag \der \smallo$ with
its multiple $\imag(\T+\imag \der\smallo)$ yields the definable
set $\der\smallo + \imag\der\smallo$, and taking integrals gives
the definability of
$\mathcal{O} + \mathcal{O}\imag$, and of its maximal ideal $\smallo + \smallo\imag$.
Hence
$(\T[\imag]^\times)^\dagger+ (\smallo + \smallo\imag)=\T + \smallo\imag$ is definable. Thus $\mathcal{O} + \smallo\imag=(\mathcal{O}+\mathcal{O}\imag)\cap (\T+ \smallo\imag)$ is definable. It is easy to check that for $f\in \mathcal{O}+\smallo\imag$, 
$$f\cdot (\T+\smallo \imag)\ \subseteq\ \T+\smallo\imag\ \Longleftrightarrow\ f\in \mathcal{O},$$
so $\mathcal{O}$ is definable, and therefore its
fraction field $\T$ in $\T[\imag]$ is definable.
%$\T= \bigcap_{f\in \mathcal{O}^{\ne}} f\cdot (\T+\smallo \imag)$ is definable.
\end{proof}

















==> mt-9-2.tex <==

\section{$H$-Asymptotic Couples}\label{AbstractAsymptoticCouples}

\noindent 
In this section our main interest is in $H$-asymptotic couples rather 
than arbitrary asymptotic couples.  
We begin with proving further basic facts about asymptotic couples.
Next we recall an intermediate value property for suitable functions on 
ordered abelian groups, and apply this to $H$-asymptotic couples. We also 
introduce a contraction map and the so-called $\psi$-maps on suitable 
$H$-asymptotic couples.
We finish with some embedding lemmas on asymptotic couples, and
with a look at the device of coarsening asymptotic couples and 
asymptotic fields. {\em Throughout this section  $(\Gamma,\psi)$ is an 
asymptotic couple}, not necessarily of $H$-type. 
 
\index{$H$-asymptotic couple}

\subsection*{Further basic facts on asymptotic couples}
In this subsection $\alpha$,~$\beta$,~$\gamma$ range over $\Gamma$. Recall that 
$\Psi\  <\  (\Gamma^{>})'$.  

\begin{lemma}\label{asy1} There is at most one $\beta$ such that
$$ \Psi\  < \beta\  < (\Gamma^{>})'.$$
If $\Psi$ has a largest element, there is no such $\beta$.
\end{lemma}
\begin{proof} If $\Psi\  \le \alpha < \beta\  < (\Gamma^{>})'$,
then $\gamma:= \beta-\alpha>0$ gives 
$$ \gamma^\dagger \le \alpha =\beta-\gamma < \gamma'-\gamma=\gamma^\dagger,$$ 
a contradiction. 
\end{proof}

\noindent
An element $\beta$ as in Lemma~\ref{asy1} is called a {\bf gap} in 
$(\Gamma, \psi)$.
If $K$ is an asymptotic field with asymptotic couple $(\Gamma,\psi)$, 
then such an element is also called a gap in $K$. 

\index{gap!in an asymptotic couple}
\index{gap!in an asymptotic field}
\index{asymptotic couple!gap}
\index{asymptotic field!gap}

\begin{lemma}\label{GapLemma} Suppose $K$ is an asymptotic field. Then:
\begin{enumerate}
\item $K$ has at most one gap;
\item if $\Psi$ has a largest element, then $K$ has no gap;
\item if $L$ is an $H$-asymptotic field extension of $K$ such that $\Gamma^{<}$ is
cofinal in $\Gamma_L^{<}$, then a gap in $K$ remains a gap in $L$;
\item if $K$ is the union of a directed family $(K_i)$ of asymptotic subfields
such that no $K_i$ has a gap, then $K$ has no gap. 
\end{enumerate} 
\end{lemma}






\begin{lemma}\label{cofin} If $\Gamma\ne \{0\}$, then $(\Gamma^{>})'$ is cofinal in $\Gamma$, and $(\Gamma^{<})'$ is coinitial
in $\Gamma$. 
\end{lemma}  
\begin{proof} Assume $\Gamma\ne \{0\}$. Shifting $\psi$ does not affect
the conclusion of the lemma, so we can arrange that $\beta^\dagger \ge 0$ for some $\beta>0$, and thus $(\Gamma^{>})'>0$. Let $\gamma>0$; we have to find $\alpha>0$ such that
$\alpha'\ge \gamma$. It is easy to check that
$\alpha:= 2\gamma$ works. This proves the desired cofinality.

Next, let $\gamma<0$; we have to find $\alpha<0$ such that $\alpha'\le \gamma$.
Again, $\alpha:= 2\gamma$ works if $\gamma' \le 0$, and this can be arranged by
decreasing $\gamma$ so that
$-\gamma > \Psi$. 
\end{proof}  


\noindent
Call $(\Gamma, \psi)$ {\bf grounded} if $\Psi$ has a largest element, and {\bf ungrounded} otherwise. So an asymptotic field is grounded iff its asymptotic couple is grounded. 
We say that $(\Gamma,\psi)$ {\bf has small derivation} if $\gamma'>0$
whenever $\gamma>0$. So an asymptotic field has small derivation iff its asymptotic couple has small derivation.

\label{p:grounded as couple/small der}
\index{asymptotic couple!with small derivation}
\index{asymptotic field!with small derivation}
\index{asymptotic couple!grounded}
\index{grounded!asymptotic couple}

\begin{lemma}\label{PresInf-Lemma} 
$(\Gamma,\psi)$  has small derivation iff there is no
$\gamma<0$ with $\Psi \le \gamma$.
\end{lemma}
\begin{proof} Suppose $\Gamma$ has a least positive 
element $1$; then $1'=\min (\Gamma^{>})'$. 
If $(\Gamma,\psi)$ does not have small derivation, then
$\Psi < 1'\le 0$, so $\Psi \le -1$.
Conversely, if $\Psi \le -1$, then {\em either\/} 
$-1\in \Psi$, so $-1$ is the largest element
of $\Psi$, and hence $1'=0$ by Lemma~\ref{asy1},  {\em or\/} 
$\Psi < -1$, and then also $1'\le 0$ by Lemma~\ref{asy1}.

Next, assume that $\Gamma$ does not have a least positive element. 
If $\gamma< 0$ is 
such that $\Psi \le \gamma$, then take $\beta$ with
$\gamma < \beta < 0$, and note that by Lemma~\ref{asy1} there is $\alpha>0$
with $\alpha'\le 0$. Conversely, if $\alpha>0$ and $\alpha'\le 0$, then we can 
take $\beta$ such that $0 < \beta < \alpha$, and then
$\Psi \le \gamma:=\beta'<0$.
\end{proof}


\noindent
Recall that $\Q\Gamma$ denotes the
ordered divisible hull of $\Gamma$. 
%Put $\Q\Gamma^{>}:= (\Q\Gamma)^{>}$.

\begin{lemma}\label{PresInf-Lemma2} Suppose that $(\Gamma,\psi)$ has small
derivation. Then:
\begin{enumerate}
\item $(\Q\Gamma, \psi)$  has small derivation;
\item $\gamma^\dagger \le \gamma\ \Rightarrow\ \gamma^\dagger > -\gamma/n$ for all $n\ge 1$; 
\item $\gamma^\dagger > \gamma\ \Rightarrow\ 
\gamma^\dagger > \gamma/n$ for all $n\ge 1$;
\item $\gamma^\dagger \leq 0\ \Rightarrow\ 
\gamma^\dagger=o(\gamma)$.
\end{enumerate}
\end{lemma}
\begin{proof}
If $\Gamma^{>}$ has no least element, then $\Gamma^{>}$ is coinitial
in $(\Q\Gamma)^{>}$, therefore $(\Gamma^{>})'$ is
coinitial in $((\Q\Gamma)^{>})'$, which yields (1).
If $\Gamma^{>}$ has a least
element $\alpha$, then $\alpha'\geq\alpha > 0$, and
thus $((\Q\Gamma)^{>})'>\alpha^\dagger\geq 0$.
 
Let $n\ge 1$ in the rest of the proof. Suppose that $\gamma^\dagger\leq \gamma$. Then 
$$(-\gamma)'\ =\  -\gamma + \gamma^\dagger\ \le\ 0,$$
so $\gamma > 0$. Applying (1) yields
$(\gamma/n)+
\gamma^\dagger=(\gamma/n)+(\gamma/n)^\dagger>0$,
which yields (2).  For (3),
assume $\gamma^\dagger>\gamma$. 
If $\gamma<0$, then
$(-\gamma/n)+ \gamma^\dagger
=(-\gamma/n)+ (-\gamma/n)^\dagger>0$ 
by (1), so
$\gamma^\dagger > \gamma/n$.
If $\gamma\ge 0$, then $\gamma^\dagger > \gamma\ge \gamma/n$.
This proves (3). Part (4) follows from (2) by taking $\gamma>0$.
\end{proof}

\noindent
Next some technical facts that are needed occasionally.

\begin{lemma}\label{lem:phipsi} Let 
$\alpha$,~$\beta$,~$\gamma$ be given. Then: 
\begin{enumerate}
\item if $\alpha < \beta < (\Gamma^{>})'$, then 
$\psi(\beta-\alpha)> \alpha$;
\item if $\beta\ne 0$, $\alpha=\beta'$, $\gamma\neq\alpha$, and 
$\gamma\geq \beta^\dagger$, then $\psi(\alpha-\gamma)\leq\gamma$.
\end{enumerate} 
\end{lemma}
\begin{proof} For (1), use that $\alpha < \beta < (\Gamma^{>})'$
gives 
$\beta < (\beta-\alpha)'=(\beta-\alpha) + \psi(\beta-\alpha)$.
For (2), let $\beta\ne 0$, $\alpha=\beta'$, $\gamma\neq\alpha$, and
$\gamma\geq\beta^\dagger$.
Then $\alpha-\gamma=\beta+\beta^\dagger-\gamma\leq\beta$ with 
$\alpha-\gamma\ne 0$ and $\beta\neq 0$ and hence 
$(\alpha-\gamma)'\le \beta'$, that is,
$$\alpha-\gamma+\psi(\alpha-\gamma)\ \leq\ \alpha,$$
 and thus $\psi(\alpha-\gamma)\leq\gamma$, as claimed.
\end{proof}

\noindent
From (1) in the preceding lemma we immediately obtain: 

\begin{cor}\label{1+o(1)}
Suppose $(\Gamma,\psi)$ is of $H$-type and $0<\alpha=\psi(\alpha)\leq \beta<(\Gamma^>)'$. Then $\beta=\alpha+o(\alpha)$.
\end{cor}

\noindent
From Section~\ref{sec:ordered sets} recall that 
$\Psi^{\downarrow}=\{\alpha\ :\ \text{$\alpha \le \beta$ for some 
$\beta\in \Psi$}\}$. 



\begin{lemma}\label{hasc} Suppose $(\Gamma,\psi)$ is $H$-asymptotic and ungrounded. Let $\alpha\in \Psi^{\downarrow}$. Then there are $\gamma_0\in \Psi^{>\alpha}$ and $\delta_0\in (\Gamma^>)'$ such that
the map
$$ \gamma \mapsto \psi(\gamma-\alpha)\ \colon\ \Gamma \to \Gamma_{\infty}$$
is constant on the set $[\gamma_0,\delta_0]:=\{\gamma:\gamma_0\leq\gamma\leq\delta_0\}$, with value $>\alpha$.
\end{lemma}
\begin{proof} Take $\beta_0\in \Gamma^{>}$ so small that 
$\psi(\beta_0)> \alpha$ and
$[\beta_0] < \big[\psi(\beta_0)-\alpha\big]$,
and set $\gamma_0:=\psi(\beta_0)$ and $\delta_0:=\beta_0'$.
Then
$$[\gamma_0-\alpha]\ =\  \big[\psi(\beta_0)-\alpha\big]\ 
=\ \big[\beta_0+\psi(\beta_0)-\alpha\big]\ 
=\ [\delta_0-\alpha],$$
so $\psi(\gamma_0-\alpha)=\psi(\delta_0-\alpha)$.
Since the map $\gamma\mapsto\psi(\gamma-\alpha)\colon \Gamma^{>\alpha}\to\Gamma$ is decreasing,
$\gamma_0$ and $\delta_0$ have the desired property. The map takes value
$>\alpha$ by Lemma~\ref{lem:phipsi}.  
\end{proof} 

\begin{remark}
With $(\Gamma,\psi)$ and $\alpha$, $\gamma_0$, $\delta_0$ as in Lemma~\ref{hasc} and any $H$-asymptotic couple $(\Gamma_1,\psi_1)$ extending $(\Gamma,\psi)$, the map $\gamma_1 \mapsto \psi_1(\gamma_1-\alpha)$
is constant on $[\gamma_0,\delta_0]_{\Gamma_1}$.
\end{remark}

\noindent
Let $(\Gamma,\psi)$ and $\alpha$ be as in Lemma~\ref{hasc}. Then we
let $\psi(*-\alpha)$ denote the
value of $\psi(\gamma-\alpha)$ for all large enough $\gamma\in \Psi$.  
\nomenclature[T]{$\psi(*-\alpha)$}{value of $\psi(\gamma-\alpha)$ for all large enough $\gamma\in \Psi$}

\begin{cor}\label{corhasc} Let $(\Gamma,\psi)$ be as in 
Lemma~\ref{hasc}. If $\alpha\in \Psi^{\downarrow}$, then
$\alpha < \psi(*-\alpha)$. If
$\alpha, \beta\in \Psi^{\downarrow}$ and 
$\alpha\le \beta$, then  $\psi(*-\alpha)\le \psi(*-\beta)$.
\end{cor}



\subsection*{Steady and slow functions on $H$-asymptotic couples} 
{\em In this subsection $(\Gamma,\psi)$ is of $H$-type}, and 
$\alpha$, $\beta$, $\gamma$ 
range over $\Gamma$. Our first goal is to show:

\begin{lemma}\label{ivp} The functions 
$$\gamma \mapsto \gamma'\colon \Gamma^{>} \to \Gamma, \qquad \gamma \mapsto \gamma'\colon
\Gamma^{<} \to \Gamma$$
have the intermediate value property. \textup{(}Recall from Lemma~\ref{BasicProperties} that these functions are strictly
increasing.\textup{)}
\end{lemma}

\noindent
The proof is based on the results about steady and slow functions from Section~\ref{sec:oag}. From this section we recall some terminology.
Let $v\colon \Gamma \to S_{\infty}$ be a convex valuation on the ordered abelian group $\Gamma$.
Then  
$v\alpha > v\beta\ \Rightarrow\ \alpha=o(\beta)$. We can replace here 
``$\Rightarrow$'' by ``$\Longleftrightarrow$'' by taking for $v$
the standard valuation
$\gamma \mapsto [\gamma]\colon \Gamma \to [\Gamma]$, which assigns to each $\gamma$ its archimedean class
$[\gamma]$, with the reversed natural ordering on $[\Gamma]$ so as to make $[0]$ its largest element. 
Also important for us is the valuation $\psi\colon \Gamma \to \Gamma_{\infty}$. 
We let $o_v(\beta)$ stand for any element $\alpha$ with $v\alpha> v\beta$.
 
Let $U$ be a nonempty convex subset of $\Gamma$. In Section~\ref{sec:oag} we defined a function $i\colon U \to \Gamma$ to be $v$-steady if $i$ has the intermediate value property and
$i(x)-i(y)=x-y + o_{v}(x-y)$ for all distinct $x,y\in U$.  
We also defined a function $\eta\colon U \to \Gamma$ to be  $v$-slow on the right if for all $x,y,z\in U$,
\begin{enumerate}
\item[(s1)]$\eta(x)-\eta(y)=o_v(x-y)$ if $x\ne y$;
\item[(s2)] $\eta(y)=\eta(z)$ if $x<y<z$ and $z-y=o_v(z-x)$.
\end{enumerate} 
In the same way we defined $\eta\colon U \to G$ to be $v$-slow on the left, except that in clause (s2) we replace
``$x<y<z$'' by ``$x>y>z$''. 
By Lemma~\ref{sloste}, the sum of a $v$-steady function $U\to\Gamma$ and a $v$-slow (on the right or on the left) function $U\to\Gamma$ is $v$-steady.

\begin{proof}[Proof of Lemma~\ref{ivp}]
With $v$ the standard valuation, the  identity function on 
$\Gamma^{>}$ is clearly $v$-steady. Also, the restriction of $\psi$ to
$\Gamma^{>}$ is $v$-slow on the right: part (2) of Lemma~\ref{BasicProperties} shows
that (s1) is satisfied, and the $H$-type assumption implies easily that
(s2) is satisfied. Thus by Lemma~\ref{sloste} the map 
$$\gamma \mapsto \gamma'=\gamma+\psi(\gamma)\ \colon\  \Gamma^{>} \to \Gamma$$ is $v$-steady; in particular, it has the intermediate value property. The other part of Lemma~\ref{ivp} follows in the same way,
with $\Gamma^{<}$ and ``$v$-slow on the left'' in place of~$\Gamma^{>}$ and
``$v$-slow on the right''.
\end{proof}



\begin{lemma}\label{have1} For all $\gamma$ we have:
$\ \gamma \in (\Gamma^{<})'\ \Longleftrightarrow\ \gamma < \psi(\alpha) \text{ for some }\alpha > 0$. \newline 
If $\Psi^{>0}\ne \emptyset$, then there is a unique element
$1\in \Gamma^{>}$ with $\psi(1)=1$.
\end{lemma}
\begin{proof} If $\gamma=(-\alpha)'$, $\alpha>0$, then $\gamma =\psi(\alpha)-\alpha< \psi(\alpha)$. Thus the forward direction of the equivalence holds. For the other direction we first note that by Lemma~\ref{ivp} the strictly decreasing function 
$$\alpha\mapsto
\psi(\alpha)-\alpha=(-\alpha)'\ \colon\ \Gamma^{>}\to\Gamma$$ 
has the intermediate value property. Let $\gamma$ be given, and suppose 
$\gamma< \psi(\alpha)$ for some
$\alpha>0$. By decreasing $\alpha>0$, we can only increase $\psi(\alpha)$, so
for sufficiently small $\alpha>0$ we have $\gamma \le \psi(\alpha) -\alpha=(-\alpha)'$,
and so by the intermediate value property of the function above, we get 
$\gamma\in (\Gamma^{<})'$.

Suppose now that $\Psi^{>0}\ne \emptyset$. Then the function above
takes a nonnegative value for sufficiently small $\alpha>0$, and negative values for sufficiently large $\alpha>0$, so there is
a unique element $1$ of $\Gamma^{>}$ at which this function takes the value $0$,
that is, $\psi(1)=1$. 
\end{proof}

\noindent
If $\Psi^{>0}\ne \emptyset$, then the element $1$ as in Lemma~\ref{have1} serves as a unit of length, and we
identify $\Z$ with the subgroup $\Z\cdot 1$ of $\Gamma$ via 
$k\mapsto k\cdot 1$. 

\begin{cor}\label{trich} $(\Gamma, \psi)$ has exactly one of the following three properties: \begin{enumerate}
\item[(i)] there is $\beta$ such that $\Psi< \beta < (\Gamma^{>})'$, that is, $(\Gamma, \psi)$ has a gap;
\item[(ii)] $\Psi$ has a largest element, that is, $(\Gamma, \psi)$ is grounded;
\item[(iii)] $\Gamma=(\Gamma^{\ne})'$, that is, $(\Gamma, \psi)$ has asymptotic integration.
\end{enumerate}
Moreover, $\Gamma$ has at most one element outside $(\Gamma^{\ne})'$.
\end{cor}
\begin{proof} We know from Lemma~\ref{asy1} that (i) and (ii) exclude each other. Also,
$\beta$ as in (i) cannot be in $(\Gamma^{<})'$, since
$(-\gamma)'=\gamma^\dagger - \gamma < \gamma^\dagger$ for $\gamma>0$. For the same reason,
if $\Psi$ has a largest element, this element cannot be in $(\Gamma^{<})'$. Thus (i) as well as (ii) excludes (iii). If we are neither in case (i) nor in case (ii), then it follows
from Lemma~\ref{have1} that we are in case (iii). The final statement is now an easy
consequence, using also Lemma~\ref{have1}.
\end{proof}

\noindent
The order in which the three possibilities are listed is natural: The trivial 
$H$-asymptotic couple with $\Gamma= \{0\}$ falls under (i), with $\beta=0$.
When $\Gamma$ is not trivial, but divisible and of finite dimension as a vector space
over $\Q$, then $\Psi$ is nonempty and finite, and so we are in case (ii).
Case (iii) typically requires a more infinitary construction: for example, the asymptotic couple of $\mathbb{T}$ falls under (iii). 
Note that $\sup \Psi = \beta$ in case (i), and that $\Psi$ has no
supremum in $\Gamma_{\infty}$ in case (iii). 

\begin{lemma}\label{lem:as int}
$(\Gamma^{\neq})'=((\Q\Gamma)^{\neq})'\cap\Gamma$.
\end{lemma}
\begin{proof} Suppose $\beta\notin (\Gamma^{\neq})'$; it suffices to
show that then $\beta\notin((\Q\Gamma)^{\neq})'$. The assumption $\beta\notin(\Gamma^{\neq})'$ means that $\beta$ is a gap in $(\Gamma, \psi)$ or $\beta=\max \Psi$. If $\beta$ is a gap in $(\Gamma, \psi)$, then $[\Gamma^{\neq}]$ has no smallest element, so $\Gamma^>$ is coinitial in $(\Q\Gamma)^>$, and thus $\beta$ is also a gap in $(\Q\Gamma,\psi)$, which
gives $\beta\notin((\Q\Gamma)^{\neq})'$. If $\beta=\max\Psi$, then
$\Psi=\psi((\Q\Gamma)^{\ne})$ gives $\beta=\max\psi((\Q\Gamma)^{\neq})$, and thus $\beta\notin((\Q\Gamma)^{\neq})'$.
\end{proof}

\noindent
Note that $(\Gamma, \psi)$ is grounded iff $(\Q\Gamma, \psi)$ is grounded. 
By the previous lemma, if $(\Q\Gamma,\psi)$ has asymptotic integration, then so does $(\Gamma,\psi)$. However, there are $(\Gamma,\psi)$ with asymptotic integration where $(\Q\Gamma, \psi)$ does not have asymptotic integration; see \cite[Example~12.9]{AvdD3}. %\marginpar{but needs work to see this gives an example}
This situation needs to be dealt with in parts of Section~\ref{sec:LO-cuts} where the next lemma will be used. This lemma concerns the special role of the set $2\Psi=\{2\psi(\gamma):\gamma\neq 0\}$ in that section. 

\begin{lemma}\label{lem:split gamma}
Suppose $(\Gamma,\psi)$ has asymptotic integration, and let $\gamma$ be given. Then the following conditions are equivalent:
\begin{enumerate}
\item $\gamma$ is a supremum of $2\Psi$ in the ordered set $\Gamma$;
\item $\gamma>2\Psi$, and there are no $\alpha,\beta>\Psi$ with $\alpha+\beta=\gamma$;
\item $\frac{1}{2}\gamma$ is a supremum of $\Psi$ in the ordered set $\Q\Gamma$;
\item $\frac{1}{2}\gamma$ is a gap in $(\Q\Gamma,\psi)$.
\end{enumerate}
\end{lemma}
\begin{proof} Assume $\gamma=\sup 2\Psi$, and
$\alpha,\beta>\Psi$ satisfy $\alpha+\beta=\gamma$.
Take $\alpha_1\in\Gamma$ with $\Psi < \alpha_1 < \alpha$.
Then $2\Psi < \alpha_1+\beta < \gamma$, contradicting (1).
This gives (1)~$\Rightarrow$~(2).

To get (2)~$\Rightarrow$~(3), we prove the contrapositive. So assume
$\frac{1}{2}\gamma$ is not a gap in $(\Q\Gamma,\psi)$.
Then either $\Psi\not<\frac{1}{2}\gamma$ or $\frac{1}{2}\gamma\not<  \big( (\Q\Gamma)^>\big){}'$.
If $\Psi\not<\frac{1}{2}\gamma$, then $\gamma\not>2\Psi$. Suppose  
$\frac{1}{2}\gamma\not<  \big( (\Q\Gamma)^>\big){}'$. Since $\Gamma^>$ is coinitial in $(\Q\Gamma)^>$, we have 
$\delta\in\Gamma^>$ with $\frac{1}{2}\gamma \geq \delta'$.
Then $\gamma-\delta'\geq \frac{1}{2}\gamma>\Psi$, so $\alpha:=\delta'$ and $\beta:=\gamma-\alpha$ 
satisfy $\alpha,\beta>\Psi$ and $\alpha+\beta=\gamma$.

The implication  (3)~$\Rightarrow$~(4) follows from Lem\-ma~\ref{asy1}, and
(4)~$\Rightarrow$~(1) is clear.
 \end{proof}

\noindent
The $H$-asymptotic couple $(\Gamma,\psi)$ is said to have {\bf rational asymptotic integration} if $(\Q\Gamma,\psi)$ has asymptotic integration, and an $H$-asymptotic field is said to have rational asymptotic integration if its asymptotic couple has rational asymptotic integration.

\label{p:rational as int}
\index{asymptotic couple!with rational asymptotic integration}
\index{asymptotic field!with rational asymptotic integration}
\index{asymptotic integration!rational}
\index{rational!asymptotic integration}

\begin{lemma}\label{psim} Suppose $(\Gamma, \psi)$ has small derivation. Then the function $\psi|\Gamma^{>}$ is $\psi$-slow on the right. Define
$$\psi_{-}\colon \Gamma \to \Gamma, \qquad
\psi_{-}(\gamma):=\min\bigl(\psi(\gamma),0\bigr).$$ 
Then $\psi_{-}|\Gamma^{\ge 0}$ is $\psi$-slow on the right.
\end{lemma}
\begin{proof} First, $\psi|\Gamma^{>}$ satisfies (s1): let $0 < \alpha < \beta$; we wish to show that then $\psi(\psi(\alpha)-\psi(\beta))> \psi(\alpha-\beta)$. The case $\psi(\alpha)=\psi(\beta)$ is obvious, so we can
assume $\psi(\alpha)> \psi(\beta)$. Then $\psi(\alpha-\beta)=\psi(\beta)$, and so the desired result follows from Lemma~\ref{BasicProperties},~(1). To see that $\psi|\Gamma^{>}$ satisfies (s2),
let $0 < \alpha<\beta<\gamma$, with 
$\psi(\gamma-\beta)> \psi(\gamma-\alpha)$, and suppose
$\psi(\beta)\neq \psi(\gamma)$. So $\psi(\alpha)\geq\psi(\beta)>\psi(\gamma)$ 
and $\psi(\alpha-\beta)=\psi(\alpha-\gamma)$,
hence $\psi(\gamma)=\psi(\gamma-\alpha)=\psi(\alpha-\beta)\geq\psi(\beta)$, 
a contradiction. This establishes the claim about $\psi|\Gamma^{>}$.
 Hence by Lemma~\ref{LatticeOrdered} the function $\psi_{-}|\Gamma^{>}$ is $\psi$-slow on the right.
Thus to prove the claim about $\psi_{-}|\Gamma^{\ge 0}$,
it is enough to show the following: Let
$\beta,\gamma >0$; then \begin{enumerate}
\item $ \psi_{-}(\beta)=o_{\psi}(\beta)$;
\item $\big(\beta < \gamma \text{ and }\gamma - \beta=o_{\psi}(\gamma)\big)\
\Rightarrow\ \psi_{-}(\beta)=\psi_{-}(\gamma)$.
\end{enumerate}
Since (1) holds trivially if $\psi(\beta)\ge 0$, assume $\psi(\beta)<0$. Then 
$$\psi(\Gamma^{\ne})\ =\ \psi\big((\Q\Gamma)^{\ne}\big), \qquad \textstyle{\frac{1}{2}}\psi(\beta)\ <\ 0,$$ 
so Lemmas~\ref{PresInf-Lemma} and 
\ref{PresInf-Lemma2} provide an $\alpha\ne 0$ such that
$\psi(\beta) < \frac{1}{2}\psi(\beta) < \psi(\alpha)$, and thus
$|\psi(\beta)-\psi(\alpha)|>\frac{1}{2}|\psi(\beta)|$. Together with
Lemma~\ref{BasicProperties},~(1), this gives
$$ \psi\big(\psi(\beta)\big)\ \ge\ 
\psi\big(\psi(\beta)-\psi(\alpha)\big)\ >\ \psi(\beta),$$
so $\psi(\beta)=\psi_{-}(\beta) = o_{\psi}(\beta)$. Item (2): if $\beta<\gamma$
and
$\psi(\gamma - \beta)>\psi(\gamma)$, then 
$$0\ <\ \gamma - \beta\ <\ \beta < \gamma, \qquad \psi(\gamma-\beta)\ >\ \psi(\gamma)\ =\ 
\psi\big(\gamma-(\gamma-\beta)\big),$$ 
%- \beta) = o_{\psi}(\beta),$$ 
so $\psi_{-}(\beta)=\psi_{-}(\gamma)$ where we use that $\psi_{-}|\Gamma^{>}$ 
is $\psi$-slow on the right.
\end{proof}


\noindent
With the same assumptions on $(\Gamma, \psi)$ as in 
this lemma, it follows by symmetry that $\psi_{-}|\Gamma^{\le 0}$ is $\psi$-slow on the left. 
Note that if $(\Gamma,\psi)$ is the asymptotic couple of an $H$-asymptotic field $K$ with small derivation,  
then $\psi_-(\gamma)=\min\big(\psi(\gamma),0\big)=\psile(\gamma)$ for $\gamma\neq 0$,
where $\psile$ is as
in Section~\ref{sec:dvvg}.



\subsection*{Contraction} {\em In this subsection $(\Gamma,\psi)$ is 
$H$-asymptotic and ungrounded}, and we let $\alpha$,~$\beta$,~$\gamma$
range over $\Gamma$. So we are in 
case (i) or case (iii) of Corollary~\ref{trich}. By Lemma~\ref{have1} we 
can define the so-called contraction map $\chi\colon \Gamma^{<} \to \Gamma^{<}$ 
by $\chi(\alpha)'=\alpha^\dagger$. It has the following basic properties:

\begin{lemma}\label{contracting} Let $\alpha, \beta<0$. Then: \begin{enumerate}
\item the map $\chi$ is increasing: $\alpha < \beta\ \Longrightarrow\ \chi(\alpha)\le \chi(\beta)$;
\item $\alpha^\dagger=\beta^\dagger\ \Longrightarrow\ \chi(\alpha)=\chi(\beta)$;
\item $\chi(\alpha)=o_{\psi}(\alpha)$, and thus $\chi(\alpha)=o(\alpha)$; 
\item $\alpha \ne \beta\ \Longrightarrow\ \chi(\alpha)-\chi(\beta)=o(\alpha-\beta)$.
\end{enumerate}
Moreover, $\chi$, while defined in terms of $\psi$, does not 
change upon replacing $\psi$ by a shift $\psi + \gamma$. If $(\Gamma, \psi)$ has small derivation, then 
$$ \alpha^\dagger< 0,\ \psi(\alpha^\dagger)<0\ \Rightarrow\ \alpha^\dagger=o(\alpha),\ \psi(\alpha^\dagger) = o(\alpha^\dagger),\   \chi(\alpha)=\alpha^\dagger-\psi(\alpha^\dagger).$$
\end{lemma}
\begin{proof} Properties (1) and (2) hold because the map 
$\alpha \mapsto \alpha'$ is strictly increasing and the map $\alpha \mapsto \alpha^\dagger$ is increasing (where $\alpha<0$). To get (3), we note that
$$\chi(\alpha)<0, \qquad \chi(\alpha)'\ =\ \chi(\alpha)+ \chi(\alpha)^\dagger\ =\ \alpha^\dagger,$$
so $\chi(\alpha)^\dagger > \alpha^\dagger$.  As to (4), this follows from (2) if $\alpha^\dagger=\beta^\dagger$. If $\alpha^\dagger < \beta^\dagger$,
then $\beta=o(\alpha)$, so $\chi(\alpha)=o(\alpha-\beta)$ and
$\chi(\beta)=o(\alpha-\beta)$ by (3), so 
$\chi(\alpha)-\chi(\beta)=o(\alpha-\beta)$. 

The invariance of $\chi$ under shifts follows easily from the definition of $\chi$. 
The last statement is easily deduced from Lemma~\ref{PresInf-Lemma2},~(4).
\end{proof}


%It is also contracting in the sense that
%$\chi(\alpha)=o_{\psi}(\alpha)$, and thus $\chi(\alpha)=o(\alpha)$, for
%$\alpha<0$. 
%A useful feature of $\chi$ is that while it depends on $\psi$, it does not 
%change upon replacing $\psi$ by a shift $\psi + \gamma$. Nevertheless, 
%if $(\Gamma, \psi)$ has small derivation, then for all $\alpha$,
%$$ \alpha< 0,\ \alpha^\dagger< 0,\ \psi(\alpha^\dagger)<0\ \Rightarrow\ 
%\alpha^\dagger=o(\alpha),\ \psi(\alpha^\dagger) = o(\alpha^\dagger),\   %
%\chi(\alpha)=\alpha^\dagger-\psi(\alpha^\dagger),$$
%as is easily deduced from Lemma~\ref{PresInf-Lemma2},~(4). 
%The dependence of $\chi$ on $\psi$ holds also in the sense that 
%if $\psi(\alpha)=\psi(\beta)$
%with $\alpha,\beta<0$, then $\chi(\alpha)=\chi(\beta)$.  

\index{contraction}
\index{asymptotic couple!contraction}
\nomenclature[T]{$\chi$}{contraction map of an $H$-asymptotic couple}

\begin{lemma}\label{Deltacontract}  Let $\Delta$ be a subgroup of $\Gamma$ with $\psi(\Delta^{\ne}) \subseteq \Delta$, and suppose $\alpha\in \Delta^{<}$ is such that $\alpha^\dagger$ is not maximal in $\psi(\Delta^{\ne})$. Then $\chi(\alpha)\in \Delta$.
\end{lemma}
\begin{proof} By the assumptions on $\Delta$ and $\alpha$ we can take $\beta\in \Delta^{<}$ such that $\beta' =\alpha^\dagger$.
Then $\beta=\chi(\alpha)$.
\end{proof}

\noindent
The next result will soon be needed in Section~\ref{Applicationtodifferentialpolynomials}. 

\begin{lemma}\label{evtcon} 
%Assume $\Gamma\ne\{0\}$ is divisible. 
Assume $\Gamma\ne \{0\}$ and $d, e_0, e_1,\dots, e_n\in \Z$ are not all $0$, and let $\alpha\in \Gamma$. Then there exists a $\beta<0$ such that:
\begin{align*} \text{either for all }\gamma\in (\beta,0),\ \alpha + d\psi(\gamma) + e_0\gamma+ e_1\chi(\gamma) + \cdots + e_n\chi^n(\gamma)\ &<\  0,\\
\text{or for all }\gamma\in (\beta,0),\
\alpha + d\psi(\gamma) + e_0\gamma+ e_1\chi(\gamma) + \cdots + e_n\chi^n(\gamma)\ &>\  0.
\end{align*}
\end{lemma}
\begin{proof} Since $\Gamma^{<}$ is cofinal in $(\Q\Gamma)^{<}$ we can pass to the divisible hull and arrange that
 $\Gamma$ is divisible.  
Consider first the case that $(\Gamma, \psi)$ has  asymptotic 
integration.

\medskip\noindent {\sc Subcase 1.}~{\it $d > 0$.} Then $\alpha + d\psi(\gamma)$ is 
increasing as a function of $\gamma<0$, and 
$\{\alpha+d\psi(\gamma):\ \gamma<0\}$ has no supremum in $\Gamma$ (using
divisibility of $\Gamma$). Thus we have $\beta\in \Gamma^{<}$ and $\epsilon\in \Gamma^{>}$ such that either $\alpha+d\psi(\gamma) < -\epsilon$ for all $\gamma\in (\beta,0)$, or  $\alpha+d\psi(\gamma) > \epsilon$ for all $\gamma\in (\beta,0)$.
By increasing $\beta$ if necessary, we have also 
$|e_0\gamma+ e_1\chi(\gamma) + \cdots + e_n\chi^n(\gamma)| < \epsilon/2$
for all $\gamma\in (\beta,0)$, and so this $\beta$ does the job.

\medskip\noindent {\sc Subcase 2.}~{\it $d < 0$.} This follows by symmetry from Subcase~1.

\medskip\noindent {\sc Subcase 3.}~{\it $d = 0$.} If $\alpha\ne 0$, then the desired result
follows since for all $\gamma<0$,
$$|e_0\gamma+ e_1\chi(\gamma) + \cdots + e_n\chi^n(\gamma)|\ <\ \big(|e_0|+1\big)|\gamma|.$$
If $\alpha=0$, then we take $i$ least with
$e_i\ne 0$ and use that $e_i\chi^i(\gamma)$ is the dominant term
in the sum $e_0\gamma+ e_1\chi(\gamma) + \cdots + e_n\chi^n(\gamma)$ for $\gamma<0$.

\medskip\noindent
This concludes the asymptotic integration case. Before we continue, we 
make a general observation: for $\delta\in \Gamma$ the shift 
$(\Gamma, \psi-\delta)$
has the same $\chi$-map as $(\Gamma,\psi)$, and
$\alpha + d\psi(\gamma)=(\alpha+d\delta) + d(\psi-\delta)(\gamma)$
for $\gamma<0$, so we may replace $(\Gamma, \psi)$ by its shift 
$(\Gamma, \psi-\delta)$, keeping the same $d,e_0,\dots, e_n$ and replacing
$\alpha$ by $\alpha+d\delta$. The remaining case is that $\Psi$ has
a supremum in $\Gamma$. Then we arrange by shifting that this supremum is
$0$, so $\sup \Psi=0\notin \Psi$. If $\alpha\ne 0$, the desired result follows
from
$$|d\psi(\gamma) + e_0\gamma+ e_1\chi(\gamma) + \cdots + e_n\chi^n(\gamma)|\ <\ 
   (|e_0|+1)|\gamma| \qquad (\gamma< 0),$$
which in turn depends on Lemma~\ref{PresInf-Lemma2} (4).
Suppose $\alpha=0$. If also $d=0$, then we reach the desired
result by arguing as in Subcase 3 above, so assume $d\ne 0$. If $e_0\ne 0$,
then we use that $e_0\gamma$ is the dominant term in the sum 
$$d\psi(\gamma) + e_0\gamma+ e_1\chi(\gamma) + \cdots + e_n\chi^n(\gamma).$$
So we can assume $\alpha=0$, $d\ne 0$, $e_0=0$. In this case we proceed by
induction on $n$. If $n=0$, the desired result holds, so let $n\ge 1$. 
Using $\psi(\gamma)=\chi(\gamma)+ \psi(\chi(\gamma))$ and setting
$\gamma^*:=\chi(\gamma)$ for $\gamma<0$, we have
$$ d\psi(\gamma) + e_1\chi(\gamma) + \cdots + e_n\chi^n(\gamma)\ =\
d\psi(\gamma^*) + (d+e_1)\gamma^*  +\sum_{i=1}^{n-1}e_{i+1}\chi^i(\gamma^*),$$
and so a suitable inductive hypothesis takes care of this.
\end{proof}

\noindent
By Lemma~\ref{have1} the image of the strictly increasing map 
$\gamma\mapsto \gamma+\psi(\gamma)\colon \Gamma^{<}\to\Gamma$ is a
cofinal subset of $\Psi^\downarrow$. In contrast to this, we have:

\begin{lemma}\label{lem:not cofinal in Psi}
Suppose $(\Gamma, \psi)$ has asymptotic integration and $\Gamma$ is divisible. Let $\alpha\in \Gamma$, $d_0\in \N^{\ge 1}$, $d\in\N^{\ge 2}$ and the map 
$i\colon \Gamma^<\to \Gamma$ be such that for all $\gamma<0$,
$$i(\gamma)\ =\ \alpha+d_0\,\gamma+d\,\psi(\gamma)+\epsilon(\gamma)\quad\text{with $\epsilon(\gamma)=o(\gamma)$,}$$
and $i$ is increasing. 
Then there are $\beta<0$ and 
$\gamma_0\in \Psi$ and $\delta_0\in (\Gamma^{>})'$ such that the $i$-image
of the interval $(\beta,0)$ is disjoint from the interval $(\gamma_0,\delta_0)$.
\end{lemma}
\begin{proof} 
If $i(\beta)>\Psi$ for some $\beta<0$, we take such $\beta$ such that $i(\beta)\in (\Gamma^{>})'$, and then the lemma holds with $\delta_0:= i(\beta)$ and any $\gamma_0\in \Psi$.
So we can assume that $i(\Gamma^{<})\subseteq \Psi^{\downarrow}$, and
it remains to show that $i(\Gamma^<)$ is  not cofinal in $\Psi^\downarrow$.
Towards a contradiction, suppose $i(\Gamma^<)$ is  cofinal in 
$\Psi^\downarrow$. Pick $\alpha_0\in \Gamma$ such that for
all $\gamma<0$,
$$i(\gamma)-\alpha_0\ =\ d_0\gamma + d(\psi(\gamma)-\alpha_0)+ \epsilon(\gamma),$$
in other words, $(1-d)\alpha_0 = \alpha$. 
Replacing $(\Gamma,\psi)$ by its shift $(\Gamma,\psi-\alpha_0)$ and $i$ by the map $i-\alpha_0$, we arrange that $\alpha=0$. We now distinguish two cases.

\case[1]{$(\Gamma,\psi)$ has small derivation.} Then $\Psi\cap \Gamma^{>}\ne \emptyset$, so we have $1\in \Gamma^>$ with $\psi(1)=1$. Identifying $\Q$ with its image under
$r\mapsto r\cdot 1\colon\Q\to\Gamma$, we get
$\frac{3}{2}=\frac{1}{2}+\psi\left(\frac{1}{2}\right)>\Psi$.
Let $-1\leq \gamma<0$. Then $\psi(\gamma) \ge \psi(-1) =1$ and 
$\epsilon(\gamma)> \gamma$, hence
$$i(\gamma)\ =\ d_0\,\gamma+d\,\psi(\gamma)+\epsilon(\gamma)\ >\ (d_0+1)\gamma+d.$$
Taking in addition $\gamma\geq\frac{1}{d_0+1}\left(\frac{3}{2}-d\right)$, we get
$i(\gamma) > \left(\textstyle\frac{3}{2}-d\right)+d=\textstyle\frac{3}{2}$, 
so $i(\gamma)\notin\Psi^\downarrow$, and we have a contradiction.

\case[2] {$(\Gamma, \psi)$ does not have small derivation.} Then by Lemma~\ref{PresInf-Lemma} we can take
$\delta>0$ such that $\Psi \le  -\delta$. For $\gamma<0$ we have 
\begin{align*} i(\gamma)\ &=\ \psi(\gamma) + \big(d_0\gamma + (d-1) \psi(\gamma) + \epsilon(\gamma)\big), \text{ and}\\ 
 d_0\gamma + (d-1) \psi(\gamma) + \epsilon(\gamma)\ &\le\ \psi(\gamma)\ \le \ -\delta,
 \end{align*}
so the $i$-image of $\Gamma^{<}$ is contained in $(\Psi-\delta)^{\downarrow}$, which is contained $\Psi^{\downarrow}$ but not cofinal in it, since $\psi(\delta)> \Psi-\delta$. 
\end{proof} 

%\noindent
%We cannot drop in the lemma above the assumption that $(\Gamma, \psi)$
%has asymptotic integration. 

\begin{cor}\label{cor:not cofinal in Psi} Suppose $(\Gamma, \psi)$ has rational asymptotic integration. Let $\alpha\in \Gamma$ and 
$d_0\in \N^{\ge 1}$, $d\in \N^{\ge 2}$, $e_1,\dots, e_n\in \Z$. 
Let $i\colon \Gamma^<\to\Gamma$ be given by
\begin{equation}\label{eq:def of i}
i(\gamma)\ =\ \alpha+ d_0\,\gamma + d\psi(\gamma) +  \sum_{i=1}^{n} e_i\,\chi^{i}(\gamma).
\end{equation}
Then $i$ is strictly increasing, and there are $\beta<0$ and 
$\gamma_0\in \Psi$ and $\delta_0\in (\Gamma^{>})'$ such that the $i$-image
of the interval $(\beta,0)$ is disjoint from the interval $(\gamma_0,\delta_0)$.
\end{cor}
\begin{proof} By passing to the divisible hull of $\Gamma$ and extending $i$ according to \eqref{eq:def of i}, we arrange that $\Gamma$ is divisible.
Clearly $i$ is strictly increasing by Lemma~\ref{contracting}, (4).
Thus Lemma~\ref{lem:not cofinal in Psi} applies.
\end{proof}

 


%\begin{cor}\label{cor:not cofinal in Psi} Suppose 
%$(\Gamma, \psi)$ has rational asymptotic integration. 
%Let $\alpha\in\Gamma$ and  $d_0,d_1,\dots, d_{r}\in \N$, 
%$d_0\geq 1$, $d_1+\cdots+d_r\geq 2$. 
%Let $i\colon \Gamma^<\to\Gamma$ be given by
%\begin{equation}\label{eq:def of i}
%i(\gamma)\ =\ \alpha+ d_0\,\gamma +  \sum_{i=1}^{r} d_i\,\psi%% 
%   \big(\chi^{i-1}(\gamma)\big)
%\end{equation}
%Then $i$ is strictly increasing, and there are $\beta<0$ and 
%$\gamma_0\in \Psi$ and $\delta_0\in (\Gamma^{>})'$ such that 
%the $i$-image of the interval $(\beta,0)$ is disjoint from the interval 
%$(\gamma_0,\delta_0)$.
%\end{cor}
%\begin{proof} By passing to the divisible hull of $\Gamma$ and 
%extending $i$ according to \eqref{eq:def of i}, we arrange that 
%$\Gamma$ is divisible.
%Clearly $i$ is strictly increasing. Induction on $m$ gives 
%$\psi(\chi^m(\gamma))=\psi(\gamma)-\sum_{i=1}^m\chi^i(\gamma)$ for 
%$\gamma<0$. With $d:=d_1+\cdots+d_r$ and $e_i:=d_{i+1}+\cdots+d_r$ 
%for $i=1,\dots,r-1$, we obtain: 
%$$i(\gamma) \ =\ \alpha+ d_0\,\gamma + d\,\psi(\gamma) - 
%\sum_{i=1}^{r-1} e_i\,\chi^{i}(\gamma) \qquad (\gamma<0).$$
%Thus Lemma~\ref{lem:not cofinal in Psi} applies.
%\end{proof}

 

\subsection*{Some facts about $\psi$-functions} {\em In this subsection $(\Gamma, \psi)$ is of $H$-type with small derivation, $\Gamma\ne \{0\}$ and $\Gamma$ is divisible}; $\alpha$,~$\beta$,~$\gamma$ range over $\Gamma$. We set
$$\Gamma_{\psi}\ :=\  \big\{\gamma:\ \text{$\psi^n(\gamma)<0$  for all $n\ge 1$}\big\},$$
so $\psi(\Gamma_{\psi})\subseteq \Gamma_{\psi}^{<0}=
-\Gamma_{\psi}^{>0}$, and $\Gamma_{\psi}^{<0}$ is downward closed: if
$\alpha \le \beta\in \Gamma_{\psi}^{<0}$, then $\psi(\alpha) \le \psi(\beta)$, and so by induction $\alpha\in \Gamma_{\psi}^{<0}$. In particular, $\Gamma_{\psi}^{<0}$ is a convex (possibly empty)
subset of $\Gamma^{<}$. Note also that for $\gamma\in \Gamma_{\psi}$ we have
$$\psi^{n+1}(\gamma)\ =\ o(\psi^n(\gamma)).$$
Let $\alpha$ be given as well as natural numbers $r$
and $d,d_1\dots, d_r$. Then we have a function $i=i_{\alpha, d,d_1,\dots, d_r}\colon \Gamma_{\psi} \to \Gamma$,
$$
i(\gamma)\ :=\ \alpha + d\gamma + d_1\psi(\gamma) + \dots + d_r\psi^r(\gamma),
$$
and we call $i$ a {\bf $\psi$-function of slope $d$ and order $r$}, and also a {\bf $\psi$-function of type $(\alpha,d,r)$\/} if we want to specify $\alpha$.
By part (1) of Lemma~\ref{BasicProperties}, if
$\alpha$,~$\beta$ are distinct and nonzero, then $\psi\big(\psi(\alpha)-\psi(\beta)\big)> \psi(\alpha -\beta)$, that is, 
$$\psi(\alpha)-\psi(\beta)\ =\ o_{\psi}(\alpha-\beta).$$ It follows that 
the function 
$$\gamma \mapsto  d_1\psi(\gamma) + \dots + d_r\psi^r(\gamma)\ \colon\ \Gamma_{\psi} \to \Gamma$$
is $\psi$-slow on the left when restricted to $\Gamma_{\psi}^{<0}$ and $\psi$-slow
on the right when restricted to $\Gamma_{\psi}^{>0}$. Also, if $d>0$, then
for all distinct
$x,y\in \Gamma_{\psi}$,
$$i(x)-i(y)\ =\ d(x-y)+o_{\psi}(x-y)$$ and so $i$ is 
strictly increasing, and $i$ has the intermediate value property on
$\Gamma_{\psi}^{<0}$ as well as on $\Gamma_{\psi}^{>0}$. The next result
is needed in Section~\ref{Applicationtodifferentialpolynomials}. 

\index{$\psi$-function}
\index{$H$-asymptotic couple!$\psi$-function}
\index{slope!$\psi$-function}
\index{order!$\psi$-function}
\index{type!$\psi$-function}

\begin{lemma}\label{ps2}
Let $i$, $j$ be $\psi$-functions of slopes $d> e$. Then either
$i< j$ on $\Gamma_{\psi}^{<0}$, or there is a unique 
$\beta\in \Gamma_{\psi}^{<0}$ such that $i(\beta)=j(\beta)$; in the latter
case, $i(\gamma)>j(\gamma)$ if $\beta < \gamma \in \Gamma_{\psi}^{<0}$. Likewise, either $i>j$ on 
$\Gamma_{\psi}^{>0}$, or there is a unique 
$\beta\in \Gamma_{\psi}^{>0}$ such that $i(\beta)=j(\beta)$; in the latter
case, $i(\gamma) <j(\gamma)$ if $\beta > \gamma\in  \Gamma_{\psi}^{>0}$. 
\end{lemma}
\begin{proof} Use that $i-j$ is strictly increasing, and that it has the intermediate value property on $\Gamma_{\psi}^{<0}$ as well as on $\Gamma_{\psi}^{>0}$.
\end{proof}





\subsection*{Embedding lemmas for $H$-asymptotic couples} 
Let $(\Gamma, \psi)$ and $(\Gamma_1, \psi_1)$ be asymptotic couples. An
{\bf embedding} $$h \colon\ (\Gamma,\psi)
\to (\Gamma_1,\psi_1)$$ is an embedding $h \colon\Gamma\to\Gamma_1$
of ordered abelian groups
such that $$ h\bigl(\psi(\gamma)\bigr)\ =\ \psi_1\bigl(h(\gamma)\bigr)\ 
\text{ for $\gamma\in\Gamma^{\ne}$.}$$
If $\Gamma\subseteq \Gamma_1$ and the inclusion $\Gamma\hookrightarrow\Gamma_1$ is 
an embedding $(\Gamma,\psi)
\to (\Gamma_1,\psi_1)$, then we call~$(\Gamma_1,\psi_1)$ an {\bf extension} of $(\Gamma,\psi)$.
Most of the embedding results in this subsection come from \cite{AvdD2}, 
but the restriction below
to asymptotic couples of $H$-type makes things a bit simpler and more coherent.

\index{asymptotic couple!embedding}
\index{asymptotic couple!extension}
\index{embedding!of asymptotic couples}
\index{extension!of asymptotic couples}

\medskip\noindent
{\em In the rest of this subsection
$(\Gamma,\psi)$ and $(\Gamma_1, \psi_1)$ are
asymptotic couples of $H$-type}. Recall that 
then $\psi$ is constant on archimedean classes of $\Gamma$: for 
$\alpha,\beta\in\Gamma^{\ne}$ with $[\alpha]=[\beta]$ we have $\psi(\alpha)=
\psi(\beta)$. 
%The next lemma is Lemma~2.14 in \cite{AvdD2}.
 
\begin{lemma}\label{extension4}
Let $i\colon\Gamma\to G$ be an embedding of ordered abelian groups inducing
a bijection $[\Gamma]\to [G]$. Then there is a
unique function $\psi_G\colon G^{\ne} \to G$ such that~$(G,\psi_G)$
is an $H$-asymptotic couple and $i\colon (\Gamma, \psi) \to (G,\psi_G)$ is an
embedding. 
%and $i\bigl(\psi(\gamma)\bigr)=\psi_1\bigl(i(\gamma)\bigr)$ for all 
%$\gamma\in\Gamma^{\ne}$. 
\end{lemma}
\begin{proof} Define $\psi_G(g):= i\bigl(\psi(\gamma)\bigr)$ for $g\in G^{\ne}$ and
$\gamma\in \Gamma^{\ne}$ with $[g]=[i(\gamma)]$. Then $\psi_G\colon G^{\ne} \to G$ is easily seen to have the required property.
\end{proof}

\noindent
The next
lemma and its proof show how to remove a gap. 

\begin{lemma}\label{extension1}
Let $\beta$ be a gap in $(\Gamma, \psi)$. Then there is an 
$H$-asymptotic couple $(\Gamma+\Z \alpha,
\psi^{\alpha})$ extending $(\Gamma,\psi)$ such that \begin{enumerate}
\item $\alpha>0$ and $\alpha'=\beta$;
\item if $i\colon (\Gamma,\psi)\to (\Gamma_1,\psi_1)$ is an embedding and $\alpha_1\in\Gamma_1$, $\alpha_1>0$, $\alpha_1'=i(\beta)$, then
$i$ extends uniquely to an embedding $j\colon\bigl(\Gamma+\Z \alpha,
\psi^{\alpha}\bigr)\to (\Gamma_1,\psi_1)$ with $j(\alpha)=\alpha_1$.
\end{enumerate}
\end{lemma}
\begin{proof} Suppose $(\Gamma+\Z \alpha,
\psi^{\alpha})$ is an asymptotic couple that extends $(\Gamma,\psi)$ and
satisfies (1). At this point we do not assume $(\Gamma+\Z \alpha, \psi^{\alpha})$ to be of $H$-type. Then $\alpha'< (\Gamma^{>})'$ gives 
$0 <\alpha< \Gamma^{>}$. Since $\Psi$ has no largest element, 
$[\Gamma^{\ne}]$ has no least element, so $0 < n\alpha < \Gamma^{>}$ 
for all~$n\ge 1$, in particular,
$\Gamma + \Z\alpha=\Gamma\oplus \Z\alpha$. Hence
$$\psi^{\alpha}(\alpha)\ =\ \alpha'-\alpha\ =\ \beta-\alpha\ >\ \Psi,$$ 
and thus for all $\gamma\in \Gamma$ and $k\in \Z$ with $\gamma+k\alpha\ne 0$, 
\begin{equation}\label{eq:psialpha}
\psi^{\alpha}(\gamma+k \alpha)\ =\ \begin{cases}
\psi(\gamma), &\text{if $\gamma\neq 0$,}\\
\beta-\alpha, &\text{otherwise.}
\end{cases} 
\end{equation}
It follows easily that $(\Gamma+\Z\alpha, \psi^{\alpha})$ is of $H$-type,
and has the universal property~(2). All this assumes the existence
of an asymptotic couple $(\Gamma+\Z\alpha, \psi^{\alpha})$ that extends~$(\Gamma, \psi)$
and satisfies (1), but the above also suggests how to construct it. 
For details we refer to the proof of Lemma~2.10 in~\cite{AvdD2}, which is just our lemma for arbitrary asymptotic couples instead of $H$-asymptotic couples. 
\end{proof}

\noindent
The universal property (2) determines $(\Gamma+\Z \alpha, \psi^{\alpha})$ up to isomorphism over $(\Gamma, \psi)$.
Note also that 
$[\Gamma+\Z\alpha]=[\Gamma] \cup \{[\alpha]\}$, so for $\Psi^{\alpha}:=\psi^{\alpha}\big((\Gamma+\Z\alpha)^{\ne}\big)$ we have:
\begin{equation}\label{eq:Psialpha} \Psi^{\alpha}\ =\ \Psi\cup\{\beta-\alpha\}, \qquad \beta-\alpha\ =\ \max\Psi^{\alpha}.
\end{equation}
Lemma~\ref{extension1} goes through with $\alpha < 0$ and $\alpha_1 <0$ in place of $\alpha >0$ and $\alpha_1 > 0$, respectively. In the setting of this modified lemma
we have $\Gamma^{<} < n\alpha < 0$
for all $n\ge 1$, and \eqref{eq:psialpha} goes through for $\gamma\in \Gamma$ and $k\in \Z$ with $\gamma + k\alpha \ne 0$, and \eqref{eq:Psialpha} goes through. So we have really two ways to
remove a gap, and this is a pervasive {\em fork in the road.}\/ In any case,
removal of a gap as above leads to a grounded $H$-asymptotic couple, and this is the situation we consider next. 

\begin{lemma}\label{extas2} Assume $\Psi$ has a largest element $\beta$. 
Then there is an 
$H$-asymptotic couple $(\Gamma+\Z \alpha,
\psi^{\alpha})$ extending $(\Gamma,\psi)$ with $\alpha\ne 0$, $\alpha'=\beta$, such that for any embedding $i\colon (\Gamma,\psi)\to (\Gamma_1,\psi_1)$ and any $\alpha_1\in\Gamma_1^{\ne}$ with $\alpha_1'=i(\beta)$ there is a unique extension of $i$ to an embedding $j\colon\bigl(\Gamma+\Z \alpha,
\psi^{\alpha}\bigr)\to (\Gamma_1,\psi_1)$ with $j(\alpha)=\alpha_1$.
\end{lemma}
\begin{proof} Suppose $(\Gamma+\Z \alpha,
\psi^{\alpha})$ is an $H$-asymptotic couple extending $(\Gamma,\psi)$ with
$\alpha\ne 0$, $\alpha'=\beta$. Then $\alpha< 0$ and so $\psi^{\alpha}(\alpha)= \beta-\alpha > \Psi$. Hence
$\Gamma^{<} < n\alpha < 0$ for all~$n\ge 1$, in particular,
$\Gamma + \Z\alpha=\Gamma\oplus \Z\alpha$, and \eqref{eq:psialpha} holds
for all $\gamma\in \Gamma$ and $k\in \Z$ with $\gamma+k\alpha\ne 0$. 
It follows easily that $(\Gamma+\Z\alpha, \psi^{\alpha})$ has the
required universal property. All this assumes the existence
of an $H$-asymptotic couple $(\Gamma+\Z\alpha, \psi^{\alpha})$ extending 
$(\Gamma, \psi)$ with $\alpha\ne 0$, $\alpha'=\beta$, but the above also suggests how to construct it. We leave the details to the reader. That the resulting construction leads to an asymptotic couple $(\Gamma+\Z\alpha, \psi^{\alpha})$ of $H$-type
follows from \eqref{eq:psialpha}.  
\end{proof}

\noindent
Lemma~\ref{extas2} is a variant of Lemma~2.12 in~\cite{AvdD2}.

\medskip\noindent
Let $(\Gamma+\Z\alpha, \psi^{\alpha})$ be as in Lemma~\ref{extas2}. Then
$[\Gamma+\Z\alpha]=[\Gamma] \cup \{[\alpha]\}$, so \eqref{eq:Psialpha}
holds for $\Psi^{\alpha}:=\psi^{\alpha}\big((\Gamma+\Z\alpha)^{\ne}\big)$.
Thus our new $\Psi$-set $\Psi^{\alpha}$ still has a maximum, but
this maximum is larger than the maximum $\beta$ of the original $\Psi$-set
$\Psi$. By iterating this construction indefinitely,
taking a union, and passing to the divisible hull, we obtain a divisible
$H$-asymptotic couple with asymptotic integration. Once we have a divisible $H$-asymptotic couple with asymptotic integration, we can create an extension
with a gap as follows:


 \begin{lemma}~\label{addgap} Suppose $(\Gamma, \psi)$ has asymptotic 
integration and $\Gamma$ is divisible. 
Then there is an $H$-asymptotic couple 
$(\Gamma+ \Q\beta, \psi_{\beta})$ extending $(\Gamma, \psi)$ such that:
 \begin{enumerate}
\item $\Psi< \beta < (\Gamma^{>})'$;
\item for any divisible $(\Gamma_1, \psi_1)$ extending 
$(\Gamma, \psi)$ and $\beta_1\in \Gamma_1$ with  $\Psi< \beta_1 < (\Gamma^{>})'$
there is a unique embedding 
$(\Gamma+ \Q\beta, \psi_{\beta})\to (\Gamma_1, \psi_1)$ of asymptotic 
couples that is the 
identity on $\Gamma$ and sends $\beta$ to $\beta_1$. 
\end{enumerate}
\end{lemma}
\begin{proof} Since $\Psi$ has no largest element, we can take an 
elementary ex\-ten\-sion $(\Gamma^*, \psi^*)$ of
$(\Gamma,\psi)$ with an element $\beta\in \Gamma^*$ such that
$\Psi< \beta < (\Gamma^{>})'$. Moreover, for each $\alpha\in \Gamma^{>}$ we have
$\alpha^\dagger < \beta < \alpha'$ and $\alpha'-\alpha^\dagger= \alpha$, so
$\Gamma$ is dense in $\Gamma+ \Q \beta$ by Lemma~\ref{gendense}. 
Hence $[\Gamma+\Q \beta]=[\Gamma]$, and thus 
$\psi^*$ maps $(\Gamma+\Q \beta)^{\ne}$ into $\Psi$, and with~$\psi_{\beta}$
the restriction of $\psi^*$ to $(\Gamma+\Q \beta)^{\ne}$ we have an 
$H$-asymptotic 
couple $(\Gamma+ \Q\beta, \psi_{\beta})$ extending $(\Gamma, \psi)$
satisfying (1). Let $(\Gamma_1, \psi_1)$ be a divisible $H$-asymptotic couple extending 
$(\Gamma, \psi)$ and $\beta_1\in \Gamma_1$, $\Psi< \beta_1 < (\Gamma^{>})'$.
By the universal property of Lemma~\ref{uniorvec} we have a unique
embedding $\Gamma+ \Q\beta \to \Gamma_1$
of ordered vector spaces over $\Q$ that is the identity on $\Gamma$ and sends
$\beta$ to $\beta_1$. It is routine to check that this embedding is also
an embedding $(\Gamma+ \Q\beta, \psi_{\beta})\to (\Gamma_1, \psi_1)$ 
of asymptotic couples.  
\end{proof}

\noindent
Let $(\Gamma, \psi)$ be divisible with asymptotic
integration and let $(\Gamma+ \Q\beta, \psi_{\beta})$ be an 
$H$-asymptotic couple as in Lemma~\ref{addgap}. If 
$(\Gamma + \Q\alpha, \psi_{\alpha})$ is also a divisible $H$-asymptotic couple 
extending $(\Gamma, \psi)$ with $\Psi< \alpha < (\Gamma^{>})'$, then
by (2) we have an isomorphism 
$(\Gamma+ \Q\beta, \psi_{\beta})\to (\Gamma+ \Q\alpha, \psi_{\alpha})$ 
of asymptotic couples
that is the identity on $\Gamma$ and sends $\beta$ to $\alpha$.
In this sense, $(\Gamma + \Q\beta, \psi_{\beta})$ is unique up to isomorphism
over~$(\Gamma, \psi)$. Thus the construction of $(\Gamma+ \Q\beta, \psi_{\beta})$
in the proof of Lemma~\ref{addgap} gives the following extra information,
with $\Psi_{\beta}$ the set of values of $\psi_{\beta}$ on 
$(\Gamma+ \Q\beta)^{\ne}$: 

\begin{cor}\label{addgapcor} The set $\Gamma$ is dense 
in the ordered abelian group 
$\Gamma+ \Q\beta$, so 
$[\Gamma] = [\Gamma+ \Q\beta]$, 
$\Psi_{\beta}=\Psi$ and $\beta$ is a gap in 
$(\Gamma+ \Q\beta, \psi_{\beta})$.  
\end{cor}



\noindent
Here is a version of Lemma~\ref{addgap} for possibly non-divisible $\Gamma$:

\begin{cor}\label{addgapmore}
Suppose $(\Gamma,\psi)$ has rational asymptotic integration. Then there is an $H$-asymptotic couple $(\Gamma +\Z\beta,\psi_\beta)$ extending $(\Gamma,\psi)$ such that:
\begin{enumerate}
\item $\Psi<\beta<(\Gamma^>)'$, $k\beta\notin \Gamma$ for all nonzero $k\in \Z$, and $[\Gamma+\Z\beta]=[\Gamma]$;
\item for any $(\Gamma_1,\psi_1)$ extending $(\Gamma,\psi)$ and any 
 $\beta_1\in\Gamma_1$ with $\Psi<\beta_1<(\Gamma^>)'$ there is a unique  embedding $(\Gamma\oplus\Z\beta,\psi_\beta)\to (\Gamma_1,\psi_1)$ of asymptotic couples that is the identity on $\Gamma$ and sends $\beta$ to
 $\beta_1$. 
\end{enumerate}
Moreover, $\beta$ is a gap in $(\Gamma +\Z\beta,\psi_\beta)$ for  any such 
extension of $(\Gamma, \psi)$. 
 \end{cor}
\begin{proof}
By assumption, $(\Q\Gamma,\psi)$ has asymptotic integration, so we can take an $H$-asymptotic couple
$(\Q\Gamma+\Q\beta,\psi_\beta)$ extending $(\Q\Gamma,\psi)$ and satisfying (1) and (2) in Lemma~\ref{addgap},
with $(\Q\Gamma,\psi)$ replacing $(\Gamma,\psi)$. Note that $k\beta\notin \Gamma$ for all $k\in \Z^{\ne}$.
By Corollary~\ref{addgapcor} we have $\psi_{\beta}\big((\Gamma+\Z\beta)^{\ne}\big)=\Psi$.
Denoting the restriction of $\psi_{\beta}$ to $(\Gamma+\Z\beta)^{\ne}$
also by $\psi_{\beta}$ we obtain therefore
an $H$-asymptotic couple $(\Gamma\oplus\Z\beta,\psi_{\beta})$ extending
$(\Gamma,\psi)$ satisfying (1) and (2) in the present corollary.
\end{proof}


\noindent 
From Section~\ref{sec:ordered sets} recall that a cut in an 
ordered set $S$ is simply a downward closed subset of $S$, and an element $a$ of an ordered set extending $S$ is said to
realize the cut $C$ in $S$ if $C<a<S\setminus C$.
Next a result that combines Lemma~2.15 of 
\cite{AvdD2} and 
a remark that follows the proof of that lemma. 

\begin{lemma}\label{extension5}
Let $C$ be a cut in $[\Gamma^{\ne}]$ and let $\beta\!\in\!\Gamma$ be such that
$\beta\!\!<\!\!(\Gamma^{>})'$,
$\gamma^\dagger \leq\beta$ for all $\gamma\in\Gamma^{\ne}$ with $[\gamma]\notin C$,
and $\beta\leq \delta^\dagger$ for all $\delta\in\Gamma^{\ne}$ with $[\delta]\in C$. 
Then there 
exists an $H$-asymptotic couple $(\Gamma\oplus\Z\alpha,\psi^\alpha)$ 
extending
$(\Gamma,\psi)$, with $\alpha>0$, such that:
\begin{enumerate}
\item $[\alpha]\notin [\Gamma^{\ne}]$ realizes the cut $C$ in $[\Gamma^{\ne}]$, 
$\psi^\alpha(\alpha)=\beta$;
\item given any embedding $i$ of $(\Gamma,\psi)$ into an $H$-asymptotic couple
$(\Gamma_1,\psi_1)$ 
and any element $\alpha_1\in \Gamma_1^{>}$ such that $[\alpha_1]\notin
\bigl[i(\Gamma^{\ne})\bigr]$ realizes the cut $\bigl\{\bigl[i(\delta)\bigr]:
[\delta]\in C\bigr\}$
in $\bigl[i(\Gamma^{\ne})\bigr]$ and $\psi_1(\alpha_1)=i(\beta)$, there is
a unique extension of $i$ to an embedding $j\colon 
(\Gamma\oplus\Z\alpha,\psi^\alpha)\to (\Gamma_1,\psi_1)$ with $j(\alpha)=
\alpha_1$.
\end{enumerate}
If $(\Gamma, \psi)$ has asymptotic integration, then
$(\Gamma\oplus \Z\alpha, \psi^\alpha)$ has asymptotic integration.
\end{lemma}

\noindent
For $C=\emptyset$ and $\beta$ a gap in $(\Gamma, \psi)$, this gives:

\begin{cor} Let $\beta\in \Gamma$ be a gap in $(\Gamma, \psi)$. Then there exists an $H$-asymptotic couple $(\Gamma+\Z\alpha,\psi^\alpha)$ 
extending $(\Gamma,\psi)$, such that:
\begin{enumerate}
\item $0 < n\alpha < \Gamma^{>}$ for all $n\ge 1$, and 
$\psi^\alpha(\alpha)=\beta$;
\item for any embedding $i$ of $(\Gamma,\psi)$ into an $H$-asymptotic couple
$(\Gamma_1,\psi_1)$ 
and any $\alpha_1\in \Gamma_1^{>}$ with $\psi_1(\alpha_1)=i(\beta)$, there is
a unique extension of $i$ to an embedding $j\colon 
(\Gamma+\Z\alpha,\psi^\alpha)\to (\Gamma_1,\psi_1)$ with $j(\alpha)=
\alpha_1$.
\end{enumerate}
\end{cor} 

\subsection*{Coarsening} 
Given also an asymptotic couple $(\Gamma_1,\psi_1)$, a {\bf morphism} 
$$h\colon (\Gamma,\psi)\to (\Gamma_1,\psi_1)$$ is a $\le$-preserving morphism
$h\colon\Gamma\to\Gamma_1$ of abelian groups such that
$$ h\bigl(\psi(\gamma)\bigr)= \psi_1\bigl(h(\gamma)\bigr) \text{ for all }\gamma\in
\Gamma\setminus\ker h.$$
Let $\Delta$ be a convex subgroup of $\Gamma$. Then we have the ordered quotient
group $\dot{\Gamma}:=\Gamma/\Delta$: if $\gamma \ge 0$ in $\Gamma$,
then $\dot{\gamma}:=\gamma + \Delta\ge 0$ in $\dot{\Gamma}$. 
Lemma~\ref{Coarsening-Prop} below yields an asymptotic couple 
$(\dot{\Gamma}, \dot{\psi})$.
  
\index{morphism!of asymptotic couples}
\index{asymptotic couple!morphism}
\nomenclature[T]{$(\dot{\Gamma}, \dot{\psi})$}{coarsening of $(\Gamma,\psi)$ by a convex subgroup}

\begin{lemma}\label{Coarsening-Prop}
There is a unique map 
$\dot{\psi}=\psi_\Delta \colon\ \dot{\Gamma}^{\ne}\to \dot{\Gamma}$
such that $(\dot{\Gamma}, \dot{\psi})$ is an asymptotic couple and
$\gamma\mapsto \dot{\gamma} \colon \Gamma \to \dot{\Gamma}$ is a 
morphism $(\Gamma,\psi) \to
(\dot{\Gamma}, \dot{\psi})$. It is given by
$$\dot{\psi}(\dot{\gamma})\ =\ \psi(\gamma) + \Delta \qquad\text{for 
$\gamma\in
\Gamma\setminus\Delta$.}$$ 
If $\Delta \neq \{0\}$, then 
$\Psi_\Delta:=\dot{\psi}\bigl(\dot{\Gamma}^{\ne})$ has 
supremum $\psi(\delta)+\Delta$, where
$\delta\in\Delta^{\ne}$ is arbitrary.
If $(\Gamma,\psi)$ has small derivation, then 
$(\dot{\Gamma}, \dot{\psi})$ has small derivation.
If $(\Gamma,\psi)$ is $H$-asymptotic, then 
$(\dot{\Gamma}, \dot{\psi})$ is $H$-asymptotic.
\end{lemma}
\begin{proof}
It suffices to prove existence. In what follows,
let $\alpha,\beta\in\Gamma^{\ne}$ and $\alpha \neq \beta$; then by part (2) of
Lemma~\ref{BasicProperties}, we have
$\bigl[\psi(\alpha)-\psi(\beta)\bigr]<[\alpha-\beta]$.
Hence, if $\alpha-\beta\in\Delta$, then
$\psi(\alpha)-\psi(\beta)\in\Delta$. Therefore we have a map
$$\dot{\psi}\colon \dot{\Gamma}^{\ne}\to \dot{\Gamma} , \quad
\dot{\gamma} \mapsto\psi(\gamma) + \Delta \quad 
(\gamma\in \Gamma \setminus \Delta).$$
If $\beta-\alpha>\Delta$, then
$\beta'-\alpha'=\bigl(\beta+\psi(\beta)\bigr)-\bigl(\alpha+\psi(\alpha)\bigr)>\Delta$, and
thus by Lemma~\ref{CharAsymptoticCouples},  $(\dot{\Gamma},\dot{\psi})$
is an asymptotic couple. 
To prove the claim about $\Psi_{\Delta}$, 
assume in addition that $\alpha\in \Delta$, $\alpha>0$, and $\beta>\Delta$. 
Then $\bigl(\beta+\psi(\beta)\bigr)-\psi(\alpha)>\Delta$, so in $\dot{\Gamma}$,
$$\psi(\alpha) + \Delta\ <\  \beta' + \Delta\ =\ (\beta+\Delta)'.$$
Moreover,  $\psi(\beta) < \alpha + \psi(\alpha)\in \psi(\alpha) + \Delta$, so  
$\Psi_{\Delta} \leq \psi(\alpha)+\Delta$. 

If $(\Gamma,\psi)$ has small derivation, then $\alpha>\Delta$ implies
$\alpha'=\alpha+ \alpha^\dagger > \Delta$ by Lemma~\ref{PresInf-Lemma2}, (4), 
and so $(\dot{\Gamma}, \dot{\psi})$ has small derivation.  
\end{proof}

\noindent
In connection with coarsening we sometimes use the following lemma.

\begin{lemma}\label{asymp-lemma1}
Assume $\Delta \ne \{0\}$. The following conditions are equivalent:
\begin{enumerate}
\item $\psi(\Delta^{ \ne})\cap\Delta\neq\emptyset$;
\item $\psi(\Delta^{\ne})\subseteq\Delta$;
\item $(\Delta^{\ne})'\cap\Delta \neq\emptyset$;
\item $(\Delta^{\ne})'\subseteq\Delta$.
\end{enumerate}
If $(\Gamma,\psi)$ is of $H$-type and \textup{(1)} holds, then $\Psi^{> 0}\subseteq \Delta$.
\end{lemma}
\begin{proof}
Let $\delta\in\Delta^{\ne}$ be such that $\delta^\dagger\in\Delta$. Then we have for
$\delta_1\in\Delta^{\ne}$: $$\abs{\delta^\dagger-\delta_1^\dagger}\leq\abs{\delta-
\delta_1}\in\Delta,$$ so $\delta_1^\dagger\in\Delta$. The equivalences easily
follow. Now assume $(\Gamma,\psi)$ is of $H$-type, (1) holds, and
$\Psi^{>0}\neq \emptyset$.
Then $(\Delta, \psi|\Delta^{\ne})$ is an $H$-asymptotic couple with
$\psi(\delta)>0$ for some $\delta\in \Delta^{\ne}$, so by Lemma~\ref{have1} the unique element $1\in \Gamma^{>}$ with $\psi(1)=1$ lies in $\Delta$.
Then $\Psi^{>0}< 1+1\in \Delta$, and thus $\Psi^{>0}\subseteq \Delta$. 
\end{proof}

\noindent
Now let $K$ be an asymptotic field with valuation $v$ and
asymptotic couple $(\Gamma, \psi)$. The convex subgroup $\Delta$ of
$\Gamma$ then leads to the coarsening of $v$ by $\Delta$:
$$\dot{v}=v_\Delta \colon\
K^\times\to\dot{\Gamma}=\dot{v}(K^\times),\qquad \dot{v}(f):=v(f) + \Delta.$$
The dominance relation on $K$ corresponding to the coarsened
valuation $\dot{v}$ is denoted by $\dotpreceq$ or $\preceq_\Delta$, so 
$f\preceq g \Rightarrow f \dotpreceq g$ for $f,g\in K$. (See Section~\ref{sec:decomposition}.)  Let $(K, {\dotpreceq})$ be the valued differential
field $K$ with $v$ replaced by $\dot{v}$.  

\begin{cor}\label{coarsen}
The valued differential field $(K,{\dotpreceq})$ has the following properties: 
\begin{enumerate}
\item $(K,{\dotpreceq})$ is
an asymptotic field with asymptotic couple $(\dot{\Gamma},\dot{\psi})$;
\item if $a,b\in K$, $a, b\not\asymp 1$, then $a \dotprec b\ \Longleftrightarrow\ a' \dotprec b'$.
\end{enumerate}
\end{cor}
\begin{proof} For (1), use Lemma~\ref{Coarsening-Prop} and 
Proposition~\ref{CharacterizationAsymptoticFields}. For (2),
let $a,b\in K$ and $a, b\nasymp 1$. Then $a\prec b \Longleftrightarrow 
a' \prec b'$. Set $\alpha=va$, $\beta=vb$, so
$va'=\alpha + \alpha^\dagger$ and $vb'=\beta+ \beta^\dagger$. Now
Lemma~\ref{BasicProperties}, (2), gives
$a \dotprec b\ \Longleftrightarrow\ a' \dotprec b'$.  
\end{proof}



\subsection*{Notes and comments} Much of this section (not all of it) stems from~\cite{AvdD, AvdD2, AvdD3}. A more explicit version of Lemma~\ref{hasc} is due to A. Gehret~\cite{Geh}. 
Ordered abelian groups with a contraction map are studied in~\cite{FVK-chi1, FVK-chi2}
and \cite[Appendix~A]{Kuhlmann00}; see also~\cite[Section~5]{psiremarks}.




==> mt-9-3.tex <==
\section{Application to Differential Polynomials}\label{Applicationtodifferentialpolynomials}

\noindent
{\em In this section $K$ is an $H$-asymptotic field with divisible value group
$\Gamma\ne \{0\}$}. We let~$\beta$ and $\gamma$ range over 
$\Gamma$. We also fix a differential polynomial $P\in K\{Y\}^{\ne}$ of 
order~$r$. We shall use here the $\psi$-functions from 
Section~\ref{AbstractAsymptoticCouples}
to describe the behavior of $vP(y)$ for small $vy<0$.    
 

\subsection*{Special case} The inductive proof of the key lemma~\ref{ps6a}
goes as follows: if $P$ is inhomogeneous, consider the homogeneous parts of 
$P$; reduce the homogeneous case of positive order to that of lower 
order by taking the Riccati transform.



\begin{lemma}\label{ps6a} Assume $\der\smallo\subseteq \smallo$. Let $B$ be a nonempty convex subset of $\Gamma^{<}$ 
such that $\psi(B)\subseteq B$ \textup{(}so $B\subseteq \Gamma_{\psi}^{<0}$\textup{)}.  Then there are 
$\beta\in B$ and a $\psi$-function $i=i_{\alpha,d,d_1,\dots, d_r}$ 
such that $P_d\ne 0$, and for all $y\in K$ with $vy \in B^{>\beta}$:  \begin{enumerate}
\item $P(y)\sim P_d(y)$; and $P_d(y)\succ P_e(y)$ whenever $e\in \N$, $e\ne d$;
\item $vP(y)\ =\ i(vy)$;
\item $d_j\le d\cdot r!$ for $j=1,\dots,r$. 
\end{enumerate}
\end{lemma}
\begin{proof} We proceed by induction on $r$.
For $r=0$ and homogeneous $P=aY^d$, $a\in K^\times$, the desired result 
holds with any $\beta\in B$ and $i=i_{\alpha,d}$, $\alpha=va$. Assume it holds 
whenever $P$ (of order $r$) is homogeneous. Suppose now that 
$P$ of order~$r$ is not
necessarily homogeneous, and let $P_{d_0},\dots, P_{d_k}$ with $d_0 < \dots < d_k$
be the nonzero homogeneous parts of $P$. 
Take $\beta\in B$
and $\psi$-functions $i_0,\dots, i_k$ with
$i_p=i_{\alpha_p,d_{p},d_{p,1},\dots, d_{p,r}}$ and
$d_{p,1},\dots, d_{p,r}\le d_pr!$ for $p=0,\dots,k$, and
$$vP_{d_0}(y)=i_0(vy), \dots,  vP_{d_k}(y)=i_k(vy)\ \text{ whenever $y\in K$, $vy \in B^{>\beta}$,} $$ 
and such that for all distinct $p,q\in \{0,\dots,k\}$, 
either $i_p> i_q$ on $B^{>\beta}$, or $i_p < i_q $ on~$B^{>\beta}$.
This gives $p\in  \{0,\dots,k\}$ such that for all $y\in K$  
with $vy \in B^{>\beta}$,
$$P(y)\sim P_{d_p}(y), \qquad P_{d_p}(y)\succ P_e(y) \text{ whenever
 $e\in \N$, $e\ne d_p$.}$$
Suppose $H\in K\{Y\}$ has order $r+1$, and is homogeneous of
degree $d$. Put $G:= \Ric(H)$, so $G$ is of order $r$, $v(G)=v(H)$,
and $\deg G\le \wt(H) \le (r+1)d$.
Take $\beta$ and $i_p$ as above for $G$ in the role of $P$, and note that 
$vH(y)=dvy + i_p(\psi(vy))$ for all $y\in K$ with $vy \in B^{>\beta}$.
Thus the lemma holds for $H$ instead of $P$. 
\end{proof}

\noindent
The same induction on $r$ shows that in Lemma~\ref{ps6a}, if $P\in C\{Y\}^{\ne}$
and $P$ is homogeneous of degree $d$, then we can take $i$ to be of type 
$(0,d,r)$. For later use it is important to find out more about the values of
$\alpha$ and $d$ in Lemma~\ref{ps6a} for general $P$. 
The next lemma provides such
information for special $K$ and $B$. 

\begin{lemma}\label{vpy} Suppose $\sup \Psi = 0$ and $0\notin \Psi$. Set 
$B:=\Gamma^{<}$; so $\psi(B)\subseteq B$. Then there are $\beta<0$ and a $\psi$-function $i=i_{\alpha,d,d_1,\dots, d_r}$ with the properties
described in Lemma~\ref{ps6a} such that in addition $\alpha=v(P)$ and 
$d=\max\{e\in \N:\ v(P)=v(P_e)\}$. 
\end{lemma}
\begin{proof} Follow the proof of Lemma~\ref{ps6a}, taking into account 
that $\Gamma_{\psi}=\Gamma^{\ne}$, and that for any $\psi$-functions $i_1=i_{\alpha_1,d,d_1,\dots, d_m}$ and $i_2=i_{\alpha_2,e,e_1,\dots, e_n}$, if
either $\alpha_1 < \alpha_2$, or
$\alpha_1=\alpha_2$ and $d>e$, then $i_1 < i_2$ on some interval $(\beta,0)$ with $\beta < 0$.
\end{proof} 

\begin{cor}\label{vpyc}  Suppose $\sup \Psi = 0$ and $0\notin \Psi$.
Assume also that $P\succ P_0$. 
Then there is $\beta<0$
such that $P(y_1) \succ P(y_2) \succ P(z)$ whenever $y_1, y_2,z\in K$ and 
$\beta < vy_1 < vy_2 < vz=0$. 
\end{cor}
\begin{proof} Take $\beta$ and $i=i_{\alpha,d,d_1,\dots, d_r}$ as in 
Lemma~\ref{vpy} above. Since $P\ne 0$ and $P\succ P_0$ we have $d\ge 1$, 
and so the desired result holds for this $\beta$. 
\end{proof}

\subsection*{A useful coarsening} In order to better pin down 
the value of $\alpha$ in Lemma~\ref{ps6a} we 
introduce a coarsening that gives a reduction to
the case $\sup \Psi=0\notin \Psi$. This will be used in the proof of 
Proposition~\ref{alpha=vev}. {\em In this subsection we assume 
$\der\smallo\subseteq \smallo$}.

\medskip\noindent
Let $B$ be a nonempty convex subset of $\Gamma^{<}$ such that 
$\psi(B)\subseteq B$, just as in Lemma~\ref{ps6a} \textup{(}so $B\subseteq \Gamma_{\psi}^{<}$\textup{)}. 
Then we have the convex subgroup 
$$\Delta=\Delta(B)\ :=\ \big\{\gamma:\  \psi(\gamma)> \psi(B)\big\}$$
of $\Gamma$. Note that also $\Delta= \{\gamma:\  
\psi(\gamma)> B\}$. We are now going to
use the coarsening $\dot{v}=v_{\Delta}$ of $v$ by $\Delta$. Recall from the
end of Section~\ref{AbstractAsymptoticCouples} that
$K$ with $\dot{v}$ is an $H$-asymptotic field with asymptotic couple 
$(\dot{\Gamma}, \dot{\psi})$ and $\Psi_{\Delta}:=\dot{\psi}(\dot{\Gamma}^{\ne})$. 

\begin{lemma}\label{alphadelta}  Let $\alpha$ be as in Lemma~\ref{ps6a}. Then 
$\dot{\alpha}=\dot{v}(P)$. Moreover, if $P\dotsucc P_0$, then there is $\beta\in B$ such that 
$P(y_1) \dotsucc P(y_2) \dotsucc P(z)$
whenever $y_1, y_2 ,z\in K$ and 
$vy_1, vy_2\in B^{>\beta}$, $v(z)\in \Delta$, $y_1\dotsucc y_2$.
\end{lemma}
\begin{proof} We first show that $\Delta=\{\gamma: B<-|\gamma|\}$.  
If $\beta\in B$ and $\gamma\in \Delta^{<}$, 
then $\psi(\beta) < \psi(\gamma)$, so $\beta < \gamma$. This gives
$B<\Delta$. Next, assume $\gamma\in \Gamma^{<}$ and $B<\gamma$. Then
$\beta < \psi(\beta)  \le \psi(\gamma)$ for all $\beta\in B$, so
$\gamma\in \Delta$. This proves our claim about $\Delta$.

Note that $\dot{\Gamma}=\Gamma/\Delta$ is
divisible, and $\dot{B}$ is a convex subset of $\dot{\Gamma}^{<}$
with $[\dot{\beta}, \dot{0})\subseteq \dot{B}$ for all $\beta\in B$.
So for $\beta\in B$ we have $\beta < \psi(\beta)\in B$, so 
$\dot{\beta} \le \dot{\psi}(\dot{\beta})=\psi(\beta)+\Delta < \dot{0}$.
Thus $\dot{0}\notin\Psi_{\Delta}$ and $\sup \Psi_{\Delta}=\dot{0}$.
We can now apply 
Lemma~\ref{vpy} and Corollary~\ref{vpyc} to $K$ equipped with $\dot{v}$,
and this gives the desired result.
\end{proof}






\subsection*{Reduction to the special case}
{\em In this subsection $K$ is ungrounded}.
 So we have the contraction map $\chi\colon \Gamma^{<} \to \Gamma^{<}$. We now consider a convex nonempty set~$B\subseteq \Gamma^{<}$ 
that satisfies a {\em weaker\/} condition than in Lemma~\ref{ps6a}, 
namely, $\chi(B)\subseteq B$. For example, this holds for $B=\Gamma^{<}$. 
(In this subsection we do not assume $\der\smallo\subseteq \smallo$.)

\begin{prop}\label{ps6b} There are
$\alpha\in \Gamma$ and $\beta\in B$, and $d_0, d_1,\dots, d_r\in \N$ such that
$d_0\le \deg P$, and for all $y\in K$,
$$vy\in B^{>\beta}\ \Longrightarrow\ vP(y)\ =\ \alpha+ d_0vy + \sum_{i=1}^r d_i\psi\big(\chi^{i-1}(vy)\big).$$
If $P(0)=0$ we can take $d_0\ge 1$. If $P$ is homogeneous, we can take 
$d_0=\deg P$.
\end{prop}
\begin{proof} Consider first the special case that  $\der\smallo\subseteq \smallo$ and  $\psi(B)<0$. Then $\psi(B)\subseteq B$: given $\gamma\in B$ we have $\psi(\gamma)<0$ and $\chi(\gamma)\in B$ and so $\psi(\chi(\gamma))<0$, hence
$$\gamma < \psi(\gamma)=\chi(\gamma)+\psi(\chi(\gamma))< \chi(\gamma)\in B,$$
and thus $\psi(\gamma)\in B$ since $B$ is convex. Also $\chi(\gamma)=\psi(\gamma)-\psi^2(\gamma)$ for $\gamma\in B$, by earlier remarks. 
This gives $\psi(\gamma)< \chi(\gamma) < \psi(\gamma)/2$ for
$\gamma\in B$,  and thus $\psi^2(\gamma)=\psi(\chi(\gamma))$ for
such $\gamma$, and thus by induction on $m$,
$$\psi^m(\gamma)=\psi(\chi^{m-1}(\gamma)), \qquad(\gamma\in B,\ m\ge 1).$$
This yields the desired result in view of Lemma~\ref{ps6a}. 

\medskip\noindent
The general case is reduced to this special case by
compositional conjugation. In this connection recall that, unlike
$\psi$, the contraction map $\chi$ is invariant under compositional conjugation.
Take an elementary extension $L$ of $K$ with an element~$\theta\in L^\times$
such that $\psi(B)< v\theta < (\Gamma_L^{>})'$ (so $L^{\theta}$ has
small derivation). 
Let $B_L$ be the convex hull of $B$ in
$\Gamma_L$. Then $\chi(B_L)\subseteq B_L$ and $\psi^\theta(B_L) < 0$, so we are
in the special case considered before, with $P^\theta$, $B_L$, and $L^\theta$ in place of $P$,
$B$, and $K$. This gives $\alpha_0\in \Gamma_L$, $\beta\in B$, and $d_0,\dots, d_r\in \N$, $d_0\le \deg P^{\theta}$, such that for all $y\in L$, 
$$ vy\in B_L^{> \beta}\ \Longrightarrow\  vP^{\theta}(y)\ =\ 
\alpha_0+ d_0vy + \sum_{i=1}^{r} d_i\psi^\theta\big(\chi^{i-1}(vy)\big), $$
and thus with $d:= d_1 +\dots + d_r$ we have for all $y\in L$ with 
$vy\in B_L^{> \beta}$, 
$$  vP(y)\ =\ vP^{\theta}(y)\ =\ (\alpha_0-dv\theta) + d_0vy + \sum_{i=1}^{r} d_i\psi\big(\chi^{i-1}(vy)\big).$$
This holds in particular for $y\in K$ with $vy\in B^{> \beta}$, and so 
$\alpha:=\alpha_0-dv\theta\in \Gamma$. 
\end{proof}

\noindent
By taking $B=\Gamma^{<}$ in Proposition~\ref{ps6b}, we obtain the existence of
some $\beta<0$ such that $P(y)\ne 0$ for all $y\in K$ with $\beta<vy <0$. 


\begin{cor}\label{ps6e} Suppose $P(0)=0$. Then there are $\beta<0$ and a strictly increasing function $i\colon (\beta,0) \to \Gamma$ with the intermediate value property such that $vP(y)=i(vy)$ for all $y\in K$ with 
$\beta < vy <0$. 
\end{cor}
\begin{proof} With $B=\Gamma^{<}$ and notations from the proof of Proposition~\ref{ps6b}, the function
$$i\colon B_L \to \Gamma_L, \quad i(\beta):=\alpha + d_0\beta + \sum_{i=1}^r d_i\psi\big(\chi^{i-1}(\beta)\big)$$
is strictly increasing and has the intermediate value property.
Now use that $(\Gamma_L, \psi_L)$ is an elementary extension of $(\Gamma,\psi)$.
\end{proof}


\noindent
We have $\psi(\chi^m(\gamma))=\psi(\gamma)-\sum_{i=1}^m \chi^i(\gamma)$ for 
$\gamma<0$.
This yields a formulation of Proposition~\ref{ps6b} for
$B=\Gamma^{<}$ that is more illuminating for $vy$ tending to $0$:

\begin{cor}\label{ps6c} There are 
$\alpha\in \Gamma$ and $d,d_0,e_1,\dots, e_{r-1}\in \N$ with $d_0\le \deg P$, $d\ge e_1\ge \dots \ge e_{r-1}$, such that for some $\beta<0$ we have, for all $y\in K$,
$$\beta < vy < 0\ \Longrightarrow\  vP(y)\ =\ \alpha+ d\psi(vy) + d_0vy  - \sum_{i=1}^{r-1} e_i\chi^{i}(vy).$$ 
If $P(0)=0$ we can take here $d_0\ge 1$. If $P$ is homogeneous, we can take $d_0=\deg P$.
\end{cor}

\noindent 
Here we adopt the convention that $\sum_{i=1}^{r-1} e_i\chi^{i}(\gamma) = 0$ for 
$r\le 1$ and $\gamma <0$. With~$\alpha$ and $d_0,\dots,d_r$ as in 
Proposition~\ref{ps6b} for $B=\Gamma^{<}$ we can take in  
Corollary~\ref{ps6c} the same values for $\alpha$ and $d_0$, and $d=d_1+\dots + d_r,\  e_i=d_{i+1}+ \dots + d_r$. Note:
$$y\in K,\ vy<0 \ \Longrightarrow\ \sum_{i=1}^{r-1} e_i\chi^{i}(vy) = o_{\psi}(vy).$$
By Lemma~\ref{evtcon} there is a unique tuple 
$(\alpha, d, d_0, e_1,\dots, e_{r-1})$ as in Corollary~\ref{ps6c}. 
Here is a slight extension of Corollary~\ref{ps6e}:

\begin{cor}\label{ps6f} Suppose $P(a)=0$, $a\in K$. Then for any $\gamma$ there are $\beta<\gamma$ and a strictly increasing $i\colon (\beta,\gamma) \to \Gamma$ with the intermediate value property such that $vP(a+y)=i(vy)$ for all $y\in K$ with 
$\beta < vy <\gamma$. 
\end{cor}
\begin{proof} Take $g\in K$ with $vg=\gamma$, put $Q:= P_{+a,\times g}=P(a+gY)$,
and apply Corollary~\ref{ps6e} to $Q$ in the role of $P$.
\end{proof}


\subsection*{Notes and comments} The material in this section is mostly new and plays a key role in the next chapter.


==> mt-9-4.tex <==



\section{Hardy Fields and $H$-Fields}\label{Asymptotic-Fields-Section}


\noindent
Hardy fields are $H$-asymptotic fields of a classical origin, and
will often serve as examples and counter-examples. Accordingly
we begin this section
with a brief discussion of Hardy fields, which are not just 
asymptotic fields
but also carry a natural ordering. By abstraction this leads to the 
notions of $H$-field and pre-$H$-field. 
The transseries field $\mathbb{T}$ with its natural ordering is an example of
a {\em Liouville closed\/} $H$-field, and 
we devote a
subsection to summarizing some facts from \cite{AvdD2,AvdD3} about 
Liouville closed $H$-fields. 

\medskip\noindent
Some terminology: When a valued differential field $K$ is given, then an {\em extension of~$K$\/} is a valued differential field extension of $K$. Likewise, an {\em extension\/} of an ordered valued differential field $K$ is an ordered valued differential field extension of $K$. The term ``embedding'' is used in a similar way:
when $K$ and $L$ are given as valued differential fields, then an
{\em embedding\/} of $K$ into $L$ is an embedding of valued differential fields, and when $K$ and $L$ are given as ordered valued 
differential fields, then an
{\em embedding\/} of $K$ into $L$ is an embedding of ordered valued differential fields. 


\index{extension!of valued differential fields}
\index{extension!of ordered valued differential fields}

\subsection*{Hardy fields}
Basic references on this subject are \cite[Appendice]{Bourbaki} and \cite{Rosenlicht4}, which also include proofs omitted here.
Let $\mathcal{G}$ be the ring
of germs at $+\infty$ of real valued functions with domain a subset of $\R$
containing an interval $(a, +\infty)$, $a\in \R$; the domain and the interval may vary 
and the ring operations are defined pointwise. Call a germ $g\in \mathcal{G}$ {\em differentiable\/} if it is the germ of
a differentiable (and thus continuous) function $(a,+\infty)\to \R$ for some $a\in \R$;
in that case $g'\in \mathcal{G}$ denotes the germ of the derivative of that function.
If $g\in \mathcal{G}$ is the germ of a real valued function 
on some interval $(a, +\infty)$, $a\in \R$, then we simplify notation
by letting $g$ also denote this function if the resulting ambiguity is harmless.
With this convention, given a property $P$ of real numbers
and $g\in \mathcal{G}$ we say that $P(g(t))$ holds eventually if $P(g(t))$ holds for all sufficiently large real $t$. 
We identify each real number $r$ with the germ at $+\infty$ of the function 
$\R\to \R$ that takes the constant value $r$. This  makes the field $\R$ into a subring of $\mathcal{G}$.

\medskip\noindent
We define a {\bf Hardy field\/} to be a subring $K$ of $\mathcal{G}$ such that $K$ is a field, all $g\in K$ are differentiable, and $g'\in K$ for all $g\in K$.
For example, given polynomials 
$p(x), q(x)\in \R[x]$ with $q\ne 0$, let us identify the rational function 
$p(x)/q(x)\in \R(x)$
with the germ at $+\infty$ of $t \mapsto p(t)/q(t)$, for $t\in \R$ with $q(t)\ne 0$. This makes the rational function field $\R(x)$ into a Hardy field, with
$x$ the germ of the identity function on $\R$. Note also that
$\R$ is a Hardy field, and so is any subfield of $\R$.  

\index{germs}
\index{Hardy field}
\index{field!Hardy}

Let $K$ be a Hardy field. We consider $K$ as a differential field with derivation~$g\mapsto g'$. It has constant field $C=K\cap \R$. We make 
$K$ an ordered field by defining for $g\in K$: 
$$g>0\ \Longleftrightarrow\ \text{$g(t) > 0$, eventually.}$$
Thus $C$ is a common ordered subfield of $K$ and of $\R$. There is a unique Hardy field $K(\R)\subseteq \mathcal{G}$ generated as a field over $K$ by $\R$. It has $\R$ as its constant field.
There is a
unique real closed Hardy field extension $K^{\text{rc}}$ of $K$ that is
algebraic over~$K$ (and thus a real closure of the ordered field $K$).
For $f\in K$ we have Hardy field extensions~$K(e^f)$ and~$K(g)$ where
$g$ is any {\em integral\/} of $f$, that is, $g\in \mathcal{G}$
is differentiable and~$g'=f$. Thus for $f\in K^{>}$ we get a Hardy field $K(\log f)$, since $(\log f)'=f^\dagger\in K$.
Our Hardy field $K$ is a valued field 
with valuation ring
$$ \mathcal{O}\ =\ \big\{g\in K:\ \text{$|g|\le n$ for some $n$}\big\}\ =\ \big\{g\in K:\ \text{$|g| \le c$ for some $c\in C$}\big\}.$$
This makes $K$ an $H$-asymptotic field; if $C=\R$, then $K$ is even 
$\d$-valued.

\begin{cor}\label{hardyflateq} Let $K$ be a Hardy field and $f,g\in K$, $f,g\succ 1$. Then
$$f\flattereq g\ \Longleftrightarrow\ |f|\le |g|^n \text{ for some }n.$$
\end{cor}
\begin{proof} Assume $f\flattereq g$. Then  $f^\dagger\preceq g^\dagger$, that is, $(\log{|f|})'\preceq (\log{|g|})'$.
Working in a Hardy field extension of $K$ containing $\log{|f|}$ and $\log{|g|}$ we have $\log{|f|}\succ 1$ and $\log{|g|}\succ 1$, so $\log{|f|}\preceq \log{|g|}$,
that is, $\log{|f|}\le n\log{|g|}$ for some $n$, and thus 
$|f|\le |g|^n$ for some $n$. The converse follows by reversing
this reasoning.
\end{proof}

\subsubsection*{Example of a Hardy field that is not $\d$-valued}
The Hardy subfield $\Q(x)$ of $\R(x)$ is also $\d$-valued with
constant field $\Q$, but its algebraic extension 
$$\Q\left(\sqrt{2+x^{-1}}\,\right)    \qquad\text{(a subfield of $\R(x)^{\text{rc}}$)}$$ 
is a Hardy field with
the same constant field $\Q$, but with $\sqrt{2}$ in the residue field.
Thus $\Q\left(\sqrt{2+x^{-1}}\,\right)$ is not $\d$-valued, even 
though it is a valued differential subfield of the $\d$-valued Hardy field $\R(x)^{\text{rc}}$.

\subsection*{Pre-differential-valued fields} Our goal is a good model theory
for the
valued differential field $\mathbb{T}$, but this
requires attention also to substructures of the structures of interest.
In this connection the previous subsection has an instructive example: 
a valued differential 
subfield of a $\d$-valued field that is not itself $\d$-valued. 
Any valued differential subfield of a $\d$-valued field is of course
asymptotic,
but actually has the stronger property of being pre-$\d$-valued: a {\bf pre-differential-valued field\/}  (for short: {\bf pre-$\d$-valued field}) is a
valued differential field $K$ such that

\begin{list}{*}{\setlength\leftmargin{3em}}
\item[(PDV)] for all $f\in K$ and $g\in K^\times$, if $f\preceq 1$, $g\prec 1$, then $f'\prec g^\dagger$.
\end{list}
Thus any differential field with the trivial valuation is a pre-$\d$-valued field. Here is an easy consequence of the definition of {\em pre-$\d$-valued}:

\begin{lemma} If $K$ is a pre-$\d$-valued field and $f,g\in K^\times$, $f\asymp g\not\asymp 1$, then 
$f^\dagger\sim g^\dagger$.
\end{lemma}

\noindent
The next lemma from  \cite{Rosenlicht2} characterizes 
pre-$\d$-valued fields as exactly the valued differential fields whose
valuation is trivial on the constant field and that obey a 
valuation-theoretic version of l'Hospital's Rule:
 
\label{p:pdv}
\index{valued differential field!pre-differential-valued}
\index{pre-differential-valued field}
\index{field!pre-differential-valued}

\begin{lemma}\label{lem:char pdv}
Let $K$ be a valued differential field. Then the following are equivalent:
\begin{enumerate}
\item $K$ is pre-$\d$-valued;
\item for all $f\in K$ and $h\in K^\times$, if $f\preceq 1\prec h$, then $f'\prec h^\dagger$;
\item $C\subseteq\mathcal O$, and for all $f,g\in K^\times$:
$$f\preceq g\prec 1 \quad\Rightarrow\quad \frac{f}{g}-\frac{f'}{g'}\prec 1;$$
\item $C\subseteq\mathcal O$, and for all $f,g\in K^\times$:
$$1\prec f\preceq g \quad\Rightarrow\quad \frac{f}{g}-\frac{f'}{g'}\prec 1.$$
\end{enumerate}
\end{lemma}
\begin{proof}
The equivalence of (1) and (2) is immediate, taking $g=1/h$ and using $g^\dagger=-h^\dagger$.
Suppose $K$ is pre-$\d$-valued. Then $K$ is asymptotic by (2) and 
(PDV), in view of the equivalence $(1)\Leftrightarrow(4)$ of 
Proposition~\ref{CharacterizationAsymptoticFields}. 
Hence $C\subseteq\mathcal O$. Let $f,g\in K^\times$ and $f\preceq g\prec 1$. 
Then $g'\ne 0$, and
$$\frac{f}{g}-\frac{f'}{g'}\ =\ \frac{fg' - f'g}{gg'}\ =\ -\frac{(f/g)'}{g^\dagger}.$$
As $f/g\preceq 1$ and $g\prec 1$, this gives $(f/g)'\prec g^\dagger$, and
we have shown (1)~$\Rightarrow$~(3).
To prove (3)~$\Rightarrow$~(4), suppose (3) holds, and let $f,g\in K$ with $1\prec f\preceq g$
and set $a:=1/g$, $b:=1/f$. Then $a\preceq b\prec 1$, hence $a^2/b \preceq a\prec 1$. Also,
$$\frac{f}{g}-\frac{f'}{g'}\ =\ \frac{1/b}{1/a}-\frac{(1/b)'}{(1/a)'}\ =\ \frac{a}{b}-\frac{a^2b'}{b^2a'}\ =\
\frac{(a^2/b)'}{a'}-\frac{a^2/b}{a},$$
which is infinitesimal by (3).
Finally, we show  (4)~$\Rightarrow$~(2).
Suppose (4) holds, and let $f\in K$, $h\in K^\times$ with $f\preceq 1\prec h$.
We want to show that $f'\prec h^\dagger$; for this, replacing $f$ by $f+1$ if necessary, we may assume that
$f\asymp 1$. Then $1\prec fh\asymp h$, so 
$$f'\frac{h}{h'}\ =\ \frac{(fh)'}{h'}- \frac{fh}{h}\ \prec\ 1$$
by (4), and therefore $f'\prec h^\dagger$.
\end{proof} 

\noindent
As noted in the proof, pre-$\d$-valued fields are asymptotic.
If $K$ is a pre-$\d$-valued field, then so is
any compositional conjugate $K^{\phi},\ \phi\in K^\times$.

\begin{cor}\label{asymp-predif} If $K$ is an ungrounded asymptotic field, 
then $K$ is pre-$\d$-valued.
\end{cor}
\begin{proof} This follows from 
Proposition~\ref{CharacterizationAsymptoticFields}, part (4).
\end{proof}

\noindent
In particular, if $K$ is an $H$-asymptotic field with asymptotic integration, 
then $K$ is pre-$\d$-valued, by Corollaries~\ref{trich} and 
~\ref{asymp-predif}.


\begin{example}
Let $\k$ be a differential field, and consider the Hahn field $\k\(( t^\Q\)) $.
Let $g\in \k\(( t^{\Q}\)) $ and make 
$\k\(( t^{\Q}\)) $ into a differential field extension of $\k$ by
$$\left(\sum a_{q}t^{q}\right)'\ =\ \sum a_{q}'t^q + \left(\sum qa_q t^{q-1}\right)g\qquad\text{(so $t'=g$.)}$$
Suppose $vg< 1$. Then $\k\(( t^\Q\)) $ is pre-$\d$-valued: just note
that for $f\in \k\(( t^\Q\)) ^\times$ we have $v(f')=vf+vg-1$ if $vf\neq 0$, and $v(f')>vg-1$ if $vf = 0$.
\end{example}

\index{hull!differential-valued}
\nomenclature[Z]{$\operatorname{dv}(K)$}{differential-valued hull of  $K$}

\noindent
Let $K$ be a pre-$\d$-valued field. Theorem~4.4 in \cite{AvdD2}
provides a $\d$-valued extension~$\operatorname{dv}(K)$ of $K$ 
that embeds uniquely over $K$ into any $\d$-valued extension of $K$. 
This universal property determines $\operatorname{dv}(K)$ up to 
unique isomorphism over $K$ of valued differential field extensions
of~$K$. We call $\operatorname{dv}(K)$ the {\bf differential-valued hull}
of~$K$. 
The proof of Theorem~4.4 in \cite{AvdD2} provides extra information: \begin{enumerate}
\item[(i)] $\res(K)=\res(\operatorname{dv}(K))$;
\item[(ii)] $\operatorname{dv}(K)=K(D)$ where $D$ is the constant field of $\operatorname{dv}(K)$;
\item[(iii)] $\operatorname{dv}(K)$ is
$\d$-algebraic over $K$, as a consequence of (ii).
\end{enumerate}
Corollary~4.5 in \cite{AvdD2} describes $\Gamma_{\operatorname{dv}(K)}$. We state it
here for $K$ of $H$-type: 


\begin{cor}\label{cor:value group of dv(K)}
Suppose $K$ is a pre-$\d$-valued field of $H$-type.
\begin{enumerate}
\item If $K$ has no gap, then $\Gamma_{\operatorname{dv}(K)}=\Gamma$.
\item If $K$ has a gap $\beta$ and there is no $b\asymp 1$ in $K$ with
$v(b')=\beta$, then $\Gamma_{\operatorname{dv}(K)}=\Gamma$.
\item Suppose $K$ has a gap $\beta$ and $b\asymp 1$ in $K$ satisfies
$v(b')=\beta$. Let $a$ be the unique element of
$\operatorname{dv}(K)$ with $a'=b'$ and $a\prec 1$. Then 
the asymptotic couple of $\operatorname{dv}(K)$ is 
$(\Gamma+\Z\alpha,\psi^\alpha)$ as
in Lemma~\ref{extension1}, with $\alpha:=va$.
\end{enumerate}
In particular, $\operatorname{dv}(K)$ is of $H$-type, by Lemma~\ref{extension1}. 
%Moreover, if $K$ has no
%gap, then $\operatorname{dv}(K)$ is an immediate extension of $K$. 
\end{cor}

\noindent
If $K$ is $\d$-valued of $H$-type with a gap $\beta$, then 
we are in case~(2) of Corollary~\ref{cor:value group of dv(K)}: there is no $b\asymp 1$ with $v(b')=\beta$. 
Examples~\ref{ex:pdv with gap, 1} and \ref{ex:pdv with gap, 2} below yield pre-$\d$-valued fields of $H$-type satisfying 
the hypothesis in part (3).

\medskip\noindent
In Section~\ref{sec:LO-cuts} we shall need the following:

\begin{lemma}\label{alggapcase} Let $K$ be a pre-$\d$-valued field of $H$-type
with asymptotic integration. Let $L$ be a pre-$\d$-valued field extension of $K$ of $H$-type and suppose $L$ is
algebraic over~$K$ and has a gap $\beta$.
Then there is no
$b\asymp 1$ in $L$ with $v(b')=\beta$. 
\end{lemma}
\begin{proof} Identify $\operatorname{dv}(K)$ with a valued differential subfield
of $\operatorname{dv}(L)$ via the embedding $\operatorname{dv}(K)\to \operatorname{dv}(L)$ that extends the
inclusion $K \to L$. Now $\operatorname{dv}(K)$ is an immediate extension of
$K$ by Corollary~\ref{cor:value group of dv(K)}, and $\operatorname{dv}(L)$ is algebraic over $\operatorname{dv}(K)$
by items (i) and (ii) preceding that corollary. It follows that
$\Gamma_{\operatorname{dv}(L)}/\Gamma$ is a torsion group, and so
$\Gamma_{\operatorname{dv}(L)}/\Gamma_L$ is a torsion group.
Now apply part (3) of Corollary~\ref{cor:value group of dv(K)} to $L$ in the role of $K$.
\end{proof} 





\subsection*{$H$-fields and pre-$H$-fields} 
In Hardy fields the ordering and derivation interact. To capture the 
elementary properties of this interaction we define an {\bf $H$-field\/} 
as an ordered differential field $K$ such that:
\begin{list}{*}{\setlength\leftmargin{3em}}
\item[(HF1)] for all $f\in K$, if $f>C$, then $f'>0$;
\item[(HF2)] $\cal{O}=C+\smallo$ where 
$\mathcal{O}= \{g\in K:\text{$\abs{g} \le c$ for some $c\in C$}\}$ and $\smallo$ is the maximal ideal of the convex subring $\cal{O}$ of $K$.
\end{list} 
Hardy fields with constant field $\R$ are $H$-fields. Also, $\mathbb{T}$ with its usual ordering and derivation is an $H$-field.

\index{$H$-field}
\index{ordered differential field!$H$-field}
\label{p:H-field}

Let $K$ be an $H$-field.  We regard
$K$ as an ordered valued differential field by taking the valuation given by the valuation ring $\cal{O}$ defined in (HF2). Then $K$ is 
$\d$-valued of $H$-type, and if 
$a,b\in K^\times$
and $a \succ b$, then $a^\dagger > b^\dagger$. Any compositional conjugate $K^{\phi}$ with 
$\phi\in K^{>}$ is an $H$-field (with the same ordering). The real closure of an 
$H$-field is an $H$-field. We refer to \cite{AvdD2} and \cite{AvdD3} 
for these basic facts and others related to $H$-fields that we are going to 
mention. Note that in an 
$H$-field the ordering determines the valuation, but in our experience
the valuation is the more robust and useful feature. Nevertheless, 
the ordering deserves attention. 

Our main goal is to develop a model theory of the particular $H$-field
$\mathbb{T}$, but this requires considering $H$-fields in general, 
and substructures of $H$-fields. The example at the end of the 
subsection on Hardy fields shows that a differential 
subfield of an $H$-field with the induced ordering and valuation is not
always an $H$-field; it is, however, always a pre-$H$-field in the following 
sense.

\label{p:pre-H-field}

A {\bf pre-$H$-field\/} is an ordered pre-$\d$-valued field $K$ whose
ordering, valuation, and derivation are related as follows: 
\begin{list}{*}{\setlength\leftmargin{3em}}
\item[(PHF1)] the valuation ring $\cal{O}$ is convex with respect to 
the ordering;
\item[(PHF2)] for all $f\in K$, if $f>\cal{O}$, then $f'>0$.
\end{list}
Thus pre-$H$-fields are asymptotic differential fields. If $K$ is a pre-$H$-field, then so is any compositional conjugate $K^{\phi}$ with $\phi\in K^{>}$. 
Hardy fields are pre-$H$-fields. 
Any ordered differential field with the trivial valuation is a pre-$H$-field.
We always consider $H$-fields as ordered valued differential fields, so
in particular as pre-$H$-fields. It is easy to check that
that for any pre-$H$-field $K$,
$$ K \text{ is an $H$-field}\ \Longleftrightarrow\ K \text{ is $\d$-valued}.$$
The next lemma is often used
and elaborates on 
Corollary~\ref{lem:ordering immediate ext}.

\index{pre-$H$-field}
\index{ordered differential field!pre-$H$-field}

\begin{lemma}\label{prehimm} Let $K$ be a pre-$H$-field and $L$ an immediate asymptotic field
extension of $K$. Then $L$ has a unique field ordering extending that of $K$ 
in which $\mathcal{O}_L$ is convex. With this ordering $L$ is a pre-$H$-field 
and $\mathcal{O}_L$ is the convex hull of $\mathcal{O}$ in $L$.
If $K$ is an $H$-field, then so is $L$ with this ordering.
\end{lemma} 

\noindent
This is a slight extension of Corollary~3.2 in~\cite{AvdD2} with the same proof.
If $K$ is a pre-$H$-field, then we always consider any immediate asymptotic 
extension of $K$ as a pre-$H$-field according to Lemma~\ref{prehimm}.
In view of Corollary~\ref{completingasymp} we get:

\begin{cor}\label{completinghfields} If $K$ is a pre-$H$-field, so is its completion $K^{\operatorname{c}}$. If $K$ is an $H$-field, so is its completion $K^{\operatorname{c}}$.
\end{cor}   

\medskip
\noindent
A key fact about pre-$H$-fields is that they can be canonically extended
to $H$-fields, and so they are of $H$-type. Here are the details. Let $K$ be a pre-$H$-field. As a pre-$\d$-valued field, $K$ has a differential-valued hull $\operatorname{dv}(K)$.
The proof of Corollary~4.6 in~\cite{AvdD2} provides 
a unique field ordering on $\operatorname{dv}(K)$ extending that of~$K$ in which the valuation ring of $\operatorname{dv}(K)$ is convex. 
Let $H(K)$ be $\operatorname{dv}(K)$ equipped with this ordering. Then $H(K)$ is an
$H$-field, it extends $K$ as an ordered valued differential field, and it embeds uniquely over $K$ into any $H$-field extension of $K$.
See Section~4 in~\cite{AvdD2} for proofs of these claims. 
Of course this universal property determines $H(K)$ up to unique isomorphism
(of ordered valued differential fields) over $K$.  We call $H(K)$ the {\bf $H$-field hull} of $K$. 

\index{hull!$H$-field}
\nomenclature[Z]{$H(K)$}{$H$-field hull of the pre-$H$-field $K$}

\medskip\noindent
Let $K$ be a pre-$H$-field. Then we equip the differential 
field extension $K[\imag]$ of $K$ with the valuation ring 
$\mathcal {O} + \mathcal{O}\imag$ of $K[\imag]$; see Lemma~\ref{imagconvex}.
This makes $K[\imag]$ a valued differential
field extension of $K$ with the same value group as $K$, and we have
$v(a+b\imag) = \min(va, vb)$ for all $a,b\in K$. Moreover:

\begin{lemma} The valued differential field $K[\imag]$ is pre-$\d$-valued and of $H$-type. 
If~$K$ is an $H$-field, then $K[\imag]$ is $\d$-valued. 
\end{lemma}
\begin{proof} Let $g\in K[\imag]^\times$, $g=a+b\imag,\ a,b\in K$. Then 
$g\bar{g}= a^2+ b^2$, so $g^\dagger + {\bar{g}}^\dagger= (a^2+b^2)^\dagger$,
which in view of $g^\dagger \asymp  {\bar{g}}^\dagger$ gives
$g^\dagger \succeq (a^2+b^2)^\dagger$.
As $K$ is pre-$\d$-valued, it follows easily that
$K[\imag]$ is pre-$\d$-valued. Since $K$ and $K[\imag]$ have the 
same asymptotic couple, $K[\imag]$ is of $H$-type. For the last claim of the lemma, use that the constant field of $K[\imag]$ is $C+C\imag$. 
\end{proof}


\noindent
Even if our main interest is in the model theory of the $H$-field 
$\mathbb{T}$ it is sometimes useful to work in algebraically closed 
extensions like
$\mathbb{T}[\imag]$ that are not $H$-fields 
but still $\d$-valued of $H$-type. 

\subsection*{Constant field extension}
Differential-valued fields and $H$-fields are well-be\-haved under constant field extensions. To make this precise,
let $K$ be a $\d$-valued field, and let $L$ be an extension
field of $K$ with a subfield $D\supseteq C$ such that~$K$ and~$D$ are linearly
disjoint over~$C$ and $L=K(D)$. For a proof of the following fact, see \cite[Theorem 3]{Rosenlicht2}:

\begin{prop}\label{prop:constant field ext}
There is a unique derivation on $L$ that extends the one of~$K$ and is
trivial
on $D$; this derivation has $D$ as its constant field. There is also a unique
valuation of $L$ that extends the valuation of $K$ and is trivial on $D$;
this valuation of $L$ has the same value group as $K$.
Equipped with this derivation and valuation, $L$ is $\d$-valued.
\end{prop}

\noindent
In the proposition below, proved in \cite[Proposition~9.1]{AvdD3}, we consider $L$ as being equipped with the
derivation and valuation discussed in the previous proposition.

\begin{prop}\label{prop:Hconstants}
Let $K$ and $D$ also be equipped with orderings that
make $K$ an $H$-field for the given derivation and valuation of $K$, and
$D$ an ordered field extension of $C$. Then there is a unique field ordering
of $L$ extending the orderings of~$K$ and $D$ in which the valuation ring
of $L$ is convex. With this ordering $L$ is an $H$-field for the
derivation and valuation of $L$.
\end{prop}

\begin{cor}\label{cor:dconstantsval} Let $F$ be a pre-$H$-field, $E$ a differential subfield of $F$, and $F=E(C_F)$. Then  
$v(F^\times)=v(E^\times)+\Z\alpha$ for some 
$\alpha\in v(F^\times)$.
\end{cor}
\begin{proof} Extending $F$ to its $H$-field hull
we arrange that $F$ is an $H$-field. Next, consider $E$
as a pre-$H$-subfield of $F$ and identify its $H$-field hull $H(E)$ with an $H$-subfield of $F$ via its embedding over $E$ into $F$. Then $H(E)$ and $C_F$ are linearly disjoint over $C_{H(E)}$ by a remark preceding Lemma~\ref{lem:lin disjoint over constants}.
It remains to note that $v(F^\times)=v(H(E)^\times)$ by Proposition~\ref{prop:constant field ext}, and that
$v(H(E)^\times)=v(E^\times)+\Z\alpha$ for some 
$\alpha\in v(H(E)^\times)$, by Corollary~\ref{cor:value group of dv(K)}. 
\end{proof}




\subsection*{Liouville closed $H$-fields} See \cite{AvdD2}
for proofs of most facts mentioned in this subsection.
A pre-$H$-field $K$ is said to be
{\bf Liouville closed\/} if it is a real closed $H$-field and for each $a\in K$ there exist
$y,z\in K$ such that $y'=a$ and $z\ne 0$, $z^\dagger =a$; note that then
any equation $y'+ay=b$ with $a,b\in K$ has a solution in $K^\times$.
The $H$-field~$\mathbb{T}$ is Liouville closed. If $K$ is a Liouville closed $H$-field and $\phi\in K^{>}$, then $K^{\phi}$ is a Liouville closed $H$-field. For use in Section~\ref{sec:special sets} we mention two easy results: 

\label{p:Liouville closed}

\begin{lemma}\label{intersectliou} Let $K$ and $L$ be Liouville closed $H$-subfields
of an $H$-field $M$ such that $C_L=C_M$. Then $K\cap L$ is a Liouville
closed $H$-subfield of $M$. 
\end{lemma}
\begin{proof} It is easy to check that $K\cap L$ is a real closed 
$H$-subfield
of $M$ with constant field $C=C_K$. Let $a\in K\cap L$. First, take
$f\in K$ and $g\in L$ such that $f'=a=g'$. Then $f-g\in C_M$, so
$f-g\in L$, and thus $f\in K\cap L$. Next, take $f\in K^\times$ and
$g\in L^\times$ such that $f^\dagger=a=g^\dagger$. Then
$f/g\in C_M$, so $f/g\in L$, and thus $f\in K\cap L$.
\end{proof}

\noindent
The next lemma is \cite[Lemma~6.3,~(2)]{AvdD2}:

\begin{lemma}\label{intersectlioumany} If $K$ is a Liouville closed 
$H$-field and $(K_i)_{i\in I}$ $(I\ne \emptyset)$ is a family of Liouville closed $H$-subfields of $K$, all with the same constants as $K$, then $\bigcap_i K_i$ is a Liouville closed $H$-subfield of $K$.
\end{lemma} 

\noindent
The next result is \cite[Lemma~10.2]{AvdD3}. It will be used in Section~\ref{sec:reldifhens}.

\begin{lemma}\label{lioucompletion} If $K$ is a Liouville closed $H$-field, then so is its completion $K^{\operatorname{c}}$.
\end{lemma}


\index{$H$-field!Liouville closed}
\index{Liouville closed $H$-field}
\index{logarithm!on an asymptotic field}

\noindent
Let $K$ be a Liouville closed $H$-field. Then $K$ has asymptotic integration, 
and so its asymptotic couple $(\Gamma, \psi)$ 
has a contraction map $\chi\colon \Gamma^{<} \to \Gamma^{<}$. This 
contraction map is induced by a logarithm map on $K^{>}$ as follows. 
Choosing for each
$a\in K^{>}$ a ``logarithm'' $\Log(a)\in K$, that is, 
$\Log(a)'=a^{\dagger}$, we have 
$$\chi(\alpha)=v\big(\Log(a)\,\big)\ \text{ 
whenever $\alpha\in \Gamma^{<}$, $\alpha=va$, $a\in K^{>}$.}$$ 
A {\bf Liouville extension} of a
differential field $K$ is a differential field extension $L$ of $K$ such that $C_L$ is algebraic
over $C$ and for each $a\in L$ there are
$t_1,\dots,t_n\in L$ with $a\in K(t_1,\dots,t_n)$ and for $i=1,\dots,n$, 
\begin{enumerate}
\item[(i)] $t_i$ is algebraic over $K(t_1,\dots,t_{i-1})$, or
\item[(ii)] $t_i'\in K(t_1,\dots,t_{i-1})$, or 
\item[(iii)] $t_i\ne 0$ and $t_i^\dagger \in K(t_1,\dots,t_{i-1})$.
\end{enumerate}
A {\bf Liouville closure} of an $H$-field $K$ is a
Liouville closed $H$-field extension $L$ of $K$ such that 
 $L$ is a Liouville extension of $K$.
For a Hardy field $K\supseteq \R$ we define 
$\operatorname{Li}(K)$ as the smallest
Hardy field extension of $K$ that is real closed and 
closed under exponentiation and integration; then $\operatorname{Li}(K)$ is a 
Liouville closure of $K$.
The main result of \cite{AvdD2} is as follows:  

\index{differential field!Liouville extension}
\index{extension!Liouville}
\index{Liouville extension}
\index{closure!Liouville}
\index{$H$-field!Liouville closure}
\nomenclature[Z]{$\operatorname{Li}(K)$}{Liouville closure of the Hardy field $K\supseteq \R$}

\begin{theorem}\label{thm:Liouville closures}
Let $K$ be an $H$-field. Then one of the following occurs: 
\begin{enumerate}
\item[\rom{(I)}] $K$ has exactly one Liouville closure up to isomorphism over $K$,
\item[\rom{(II)}] $K$ has exactly two Liouville closures up to isomorphism over $K$.
\end{enumerate}
\end{theorem}

\noindent
Moreover, the following holds for an $H$-field $K$ with asymptotic couple $(\Gamma,\psi)$:
\begin{enumerate}
\item[(1)]  If $K$ is grounded, then Case (I) of 
the theorem occurs. But (I) can also occur in other ways.
\item[(2)]  If $K$ has a gap, then Case (II) of the theorem occurs. More precisely, if $\Psi < \beta < (\Gamma^{>})'$,
then in one Liouville closure $L_1$ of $K$, all 
$s\in K$ with $v(s)=\beta$ have the form $b'$ with  
$b\succ 1$, while in another Liouville closure $L_2$ of $K$ 
all $s\in K$ with $v(s)=\beta$ have the form $b'$
with $b\prec 1$.
\item[(3)] The situation of (2) is {\it the}\/  
fork in the road towards a Liouville closure: (II) is equivalent to the
existence of a Liouville 
$H$-field extension of $K$ with a gap.
\item[(4)] Any embedding of $K$ into a Liouville closed $H$-field
$M$ can be extended to an embedding of some Liouville closure of $K$ into $M$.
\end{enumerate}

\subsection*{Notes and comments} Theorem 6.7 in \cite{AvdD2} is an application of the results above and says that any
embedding of a Hardy field $H\supseteq \R$ into $\T$ which is the identity on $\R$ extends to an embedding of $\operatorname{Li}(H)$ into
$\T$; here ``embedding'' is in the sense of ordered valued differential fields. In the first sentence of 
{\em Generalities on Liouville closed $H$-fields}
in Section~6 of \cite{AvdD2},
{\em solution in $K$\/} should be 
{\em solution in $K^{\times}$}.

The $H$-field derivations on Hahn fields $\R\(( t^\Gamma\)) $ that are constructed in \cite{AvdD3, KuMa2} respect infinite sums; 
see also the survey~\cite{Ma}. 
 
 Recently we noticed that \cite{Kulchinovskii98,Kulchinovskii99} contains a variant of the concept of $H$-field and an analogue of Corollary~\ref{completinghfields}.



==> mt-9-5.tex <==
  


\section{Basic Facts about Asymptotic Fields}\label{Asymptotic-Fields-Basic-Facts}

\noindent
We now return to asymptotic fields in general, in connection
with issues around small derivation, 
$\d$-henselianity, coarsening, and
specialization.
{\em Throughout this section $K$ is an asymptotic field with
asymptotic couple $(\Gamma,\psi)$, valuation ring $\mathcal O$, maximal ideal $\smallo$ of $\mathcal O$,
and residue field~$\k=\mathcal O/\smallo$}. 

\subsection*{The case of a small derivation}
Recall that the derivation of a valued differential field is said to be small
if the derivative of every infinitesimal is infinitesimal.
Any asymptotic field has a compositional conjugate with small derivation, so this enables us to reduce 
problems to the case where the derivation is small. 

\medskip\noindent
Suppose $K$ has small derivation~$\der$.
By Lemma~\ref{closed under der}, not only do we have 
$\der \smallo\subseteq \smallo$, but even 
$\der\mathcal{O}\subseteq \mathcal{O}$, and so $\der$ 
induces a derivation on %the residue field 
$\k$.
As we saw in Sections~\ref{The Gaussian Valuation} and~\ref{sec:ldopv}
this allows us to associate to $P\in K\{Y\}^{\ne}$ and 
$A\in K[\der]^{\ne}$ functions $v_P\colon \Gamma \to \Gamma$ and
$v_A\colon \Gamma \to \Gamma$ such that  
$$v_P(\gamma)=v(P_{\times g}),  \qquad v_A(\gamma)=v(Ag) \qquad(g\in K^\times,\ vg=\gamma).$$ 
For example, for $A=\der$ we have
$$v_\der(\gamma)\ =\ \min(\gamma, \gamma') \text{ if  
$\gamma\in \Gamma^{\ne}$,} \qquad v_\der(0)\ =\ 0.$$
%Section~\ref{pafae} shows that the algebraic 
%closure of any asymptotic field
%is asymptotic; here the algebraic closure is equipped with 
%the unique derivation extending the given one, and any %valuation extending the given one. In view of
%part~(1) of Lemma~\ref{PresInf-Lemma2} it follows that the
%algebraic closure of $K$ has small derivation. 
An asymptotic field has small derivation iff its asymptotic couple has. Thus:

\begin{lemma} If $K$ has small derivation and $L$ is
an asymptotic field extension of~$K$ with $\Gamma_L=\Gamma$, then $L$ has small
derivation. 
\end{lemma}

\noindent
When referring to $\sup \Psi$ we mean the supremum of $\Psi$
in the ordered set $\Gamma_{\infty}$, and the condition
$\sup \Psi=\alpha$ (for $\alpha\in \Gamma_{\infty}$) includes the requirement that $\sup \Psi$ exists. 
Note that if $\sup \Psi=0$, then $K$ has small
derivation. While $\sup \Psi=0$ is a strong restriction, it is often
useful to reduce to this case. (If
$\Gamma=\{0\}$, then $\Psi=\emptyset$, so $\sup \Psi =0$.)
In the next two lemmas we describe situations where $\sup \Psi=0$ holds. The first lemma is in the spirit of
Lemma~\ref{obun}. 

\begin{lemma}\label{ndsupPsi=0} Suppose $K$ has small derivation and the differential residue field $\k$ has nontrivial derivation. Then $\sup \Psi=0$. 
\end{lemma} 
\begin{proof} Take $f\asymp 1$ in $K$ such that $f'\asymp 1$.
Then $g^\dagger\succeq 1$ for all $g\in K^\times$ with $g\not\asymp 1$,
by Proposition~\ref{CharacterizationAsymptoticFields}, and thus
$\Psi\le 0$. It remains to use Lemma~\ref{PresInf-Lemma}. 
\end{proof}



%The next two lemmas relate the
%condition $\sup \Psi=0$ to $\der$ being neatly surjective. 

\begin{lemma}\label{supPsi=0} Suppose $\der\smallo =\smallo$. Then 
$(\Gamma^{>})'= \Gamma^{>}$, and thus $\sup \Psi=0$. Also,
$C$ maps onto the constant field $C_{\k}$ of 
$\k$ under the residue map $\mathcal{O} \to \k$.  
\end{lemma}

\noindent 
This is an easy consequence of~\ref{asy1}.
The condition $\der \smallo =\smallo$ is satisfied when $K$ has small derivation and $\der$ is neatly surjective. The following partial 
converse to Lemma~\ref{supPsi=0} 
is useful in verifying the hypothesis of~\ref{nslinsur}.
 

\begin{lemma}\label{sup=0neatsur} Suppose $\sup \Psi=0$, $C$ maps onto the constant field $C_{\k}$ of 
$\k$ under the residue map $\mathcal{O} \to \k$, and $\der K = K$. Then 
$\der$ is neatly surjective.
% there is for each
%$b\in K^\times$ an $a\in K^\times$ such that $a'=b$ and $v_{\der}(va)=vb$.
\end{lemma} 
\begin{proof} The condition $\sup \Psi=0$ gives $v_{\der}(\gamma) = \gamma'$ 
for all $\gamma\in \Gamma$, where 
$0'=0\in \Gamma$ by convention. Hence the only  
nonobvious case is when $a, b\in K^\times$,
$a'=b$ and $a\asymp 1$, $b\prec 1$. Then the image $\bar{a}$ of $a$ in $\k$
satisfies $\bar{a}'=0$, so $\bar{a}=\bar{c}$ with $c\in C$, by our 
assumption on the constant field of $\k$. Hence $(a-c)'=b$ and $a-c\prec 1$,
so  $v_{\der}(v(a-c))=vb$, as desired.
\end{proof}

\noindent
In cases like $K=\mathbb{T}$ where $\sup \Psi=0$ fails, it is often useful to arrange it by compositional conjugation and coarsening. 
%with $\Gamma\neq\{0\}$.

\begin{lemma}\label{impreservesas} Suppose $\sup \Psi =0$ and $L$ is an immediate
valued differential field extension
of $K$ with small derivation. Then $L$ is asymptotic.
\end{lemma}
\begin{proof} We use the equivalence of
(1) and (2) in Proposition~\ref{CharacterizationAsymptoticFields}. Let $b\in L^\times$ be such that $b\nasymp 1$. Take $a\in K^\times$ with
$b=a(1+\varepsilon)$, $\varepsilon\prec 1$. Then 
$b^\dagger =a^\dagger + \frac{\varepsilon'}{1+\varepsilon}$ 
with $a^\dagger \succeq 1$ and 
$\frac{\varepsilon'}{1+\varepsilon}\prec  1$, so 
$b^\dagger \sim a^\dagger$, and thus $\psi(vb)=\psi(va)=v(a^\dagger)=v(b^\dagger)$. 
\end{proof}




\begin{lemma}\label{smallunramasymp}
Suppose $\sup\Psi=0\notin\Psi$, and
$L$ is a valued differential field extension of $K$ with small derivation and $\Gamma_L=\Gamma$.
Then $L$ is pre-$\d$-valued. 
\end{lemma}
\begin{proof}
Since $L$ has small derivation, we have $f'\preceq 1$ for all $f\preceq 1$
in $L$. So it is enough to show that $g^\dagger\succ 1$ whenever $g\in L^\times$ and $g\not\asymp 1$.
For such~$g$, take $a\in K^\times$ and $u\in L^\times$ with $g=au$ and $u\asymp 1$. Then $g^\dagger=a^\dagger+u^\dagger$ with $u^\dagger\asymp u'\preceq 1 \prec a^\dagger$ and hence $g^\dagger\sim a^\dagger\succ 1$.
\end{proof}

\noindent
Note: 
$\sup \Psi=0\notin \Psi \Longleftrightarrow 0\in \Gamma \text{ is a gap in }K$.
Thus to get a $K$ with $\Gamma\ne \{0\}$ and $\sup \Psi=0\notin \Psi$ we can 
start with any asymptotic field with a gap and nontrivial valuation---Corollary~\ref{cor:embedintogap} yields $H$-fields with this
property---and then arrange by compositional conjugation that this gap is $0$.

\begin{exampleNumbered}\label{ex:pdv with gap, 1}
Suppose $\sup\Psi=0\notin\Psi$. Let $a$ in a differential field extension of $K$ be transcendental over $K$ with $a'=1$; equip~$K(a)$ with the valuation in
Theorem~\ref{resext} for $F:=Y'$. Then by Lemma~\ref{smallunramasymp} the valued differential field $K(a)$ is pre-$\d$-valued with value group $\Gamma$
and $a\asymp 1$. If in addition~$K$ is of $H$-type, then $K(a)$,~$0$,~$a$ satisfy the conditions on $K$,~$\beta$,~$b$ in part~(3) of Corollary~\ref{cor:value group of dv(K)}.
\end{exampleNumbered}
 

\noindent
In view of Corollary~\ref{cor:resext} we obtain from 
Lemma~\ref{smallunramasymp}:

\begin{cor}\label{resextpred}
If $\sup\Psi=0\notin\Psi$ and
$\k_L$ is a differential field extension of~$\k$, then $K$ has a
pre-$\d$-valued field extension $L$ with small derivation, the same
value group as $K$, and differential residue field isomorphic to $\k_L$ over $\k$.
\end{cor}

\noindent
The assumption $\sup \Psi=0\notin \Psi$ in Lemma~\ref{smallunramasymp} may seem overly restrictive, but is in fact appropriate in view of the next two lemmas.

\begin{lemma}\label{lem:K<Y> asymptotic} Suppose $\der\smallo\subseteq \smallo$ and $K\<Y\>$ with its gaussian valuation is asymptotic. Then $\sup\Psi=0$. If $K\<Y\>$ with this valuation is pre-$\d$-valued, then $0\notin\Psi$.
\end{lemma}
\begin{proof} We have $Y\asymp 1$ in $K\<Y\>$, so
$f'\prec 1\asymp Y'\preceq g^\dagger$ for all $f,g\in K^\times$ with $f\prec 1$ and $g\not\asymp 1$, by the equivalence of (1) and (4) in 
Proposition~\ref{CharacterizationAsymptoticFields}. Thus $\sup\Psi=0$.
If $K\<Y\>$ is pre-$\d$-valued, then $f'\prec 1\asymp Y'\prec g^\dagger$ for all $f,g\in K^\times$ with $f\prec 1$ and $g\not\asymp 1$, and thus $0\notin \Psi$.
\end{proof}


\begin{lemma} Assume $\der\smallo\subseteq \smallo$.
Let $K\<a\>$ be as in Theorem~\ref{resext} 
with minimal annihilator $F$ of $a$ over $K$ of order $r\geq 1$, and
$\overline{F}\notin \k^\times  Y'$. 
If $K\<a\>$ is asymptotic, then $\sup\Psi=0$. If $K\<a\>$ is pre-$\d$-valued, then $0\notin\Psi$.
\end{lemma}
\begin{proof} We have $a\asymp 1$. We claim that $a'\asymp 1$.
This claim clearly holds for $r\ge 2$, and also when $r=1$ and 
$F$ has degree $\ge 2$ in $Y'$. Suppose $r=1$ and $F$ has degree~$1$ in $Y'$. Then $F=IY'+G$ with
$I, G\in \mathcal{O}[Y],\ vI=0$.  The assumption on $\overline{F}$ and its irreducibility in $\k\{Y\}$ yields $vG=0$, and so again $a'\asymp 1$. With the claim established, argue
as in the proof of Lemma~\ref{lem:K<Y> asymptotic} with $a$ replacing $Y$.
\end{proof}

\noindent
We now turn to the case $\max \Psi=0$:

\begin{lemma}\label{KgroundedLasymp} Assume $\max \Psi=0$.
Let $L$ be a valued differential field extension of $K$ with small derivation, $\Gamma_L=\Gamma$, and $(\k_L^\times)^\dagger\cap \k \subseteq (\k^\times)^\dagger$. Then $L$ is asymptotic.
\end{lemma}
\begin{proof} Let $g\in L^\times$, $g\prec 1$. By Proposition~\ref{CharacterizationAsymptoticFields} it is enough show that $v(g^\dagger)=\psi(vg)$.
We have $u\in L$, $f\in K$
such that $g=uf$, $u\asymp 1$, and $f\asymp g$. 
Then $g^\dagger = u^\dagger +f^\dagger$,
and  $u^\dagger\preceq 1$, $f^\dagger\succeq 1$.
If $u^\dagger \prec 1$ or $f^\dagger \succ 1$, then $v(g^\dagger)=v(f^\dagger)=\psi(vf)=\psi(vg)$. 
It remains to consider the case that $u^\dagger\asymp 1$ and
$f^\dagger\asymp 1$. If $u^\dagger + f^\dagger\asymp 1$, we
have again $v(g^\dagger)=v(f^\dagger)=\psi(vf)=\psi(vg)$,
so assume $u^\dagger + f^\dagger\prec 1$. Then
$\bar{u}^\dagger\in (\k_L^\times)^\dagger\cap \k$, and so
we have $\phi\in K$ such that 
$\phi\asymp 1$ and $u^\dagger \sim \phi^\dagger$. Then
$0\ne \phi f\prec 1$ and $(\phi f)^\dagger=\phi^\dagger + f^\dagger \prec 1$, contradicting $\max \Psi=0$. 
\end{proof} 


\begin{cor} Suppose that $\sup \Psi=0$. Then $K\<Y\>$ equipped  with its gaussian valuation is asymptotic.
\end{cor}
\begin{proof} If $0\notin \Psi$, apply Lemma~\ref{smallunramasymp}. If $0\in \Psi$, then $\max \Psi=0$,
and we can apply Lemma~\ref{KgroundedLasymp} to $L=K\<Y\>$,
and Corollary~\ref{gaussdagger} with $\k$ in the role of $K$.
\end{proof}




\subsection*{Differential-henselian asymptotic fields}
{\em In this subsection we assume that $K$ has small derivation. Let
$\k$ be its differential residue field}. Recall that if $K$ is $1$-differential-henselian, then $\mathcal{O}$ is $1$-linearly surjective.
Thus by the next lemma, if~$K$ is $1$-differential-henselian, then
$\sup \Psi=0$. 


\begin{lemma}\label{dhns3} Suppose $\mathcal{O}$ is $1$-linearly surjective. Then $\der\smallo=\smallo$, 
$\sup \Psi = 0$, and the field embedding 
$a\mapsto \bar{a}\colon C \to C_{\k}$ is bijective.
\end{lemma}
\begin{proof} From $v(\der)=0$ we get $v_{\der}(\Gamma^{>})=\Gamma^{>}$ by the Equalizer Theorem. Since $\mathcal{O}$ is $1$-linearly surjective, $\der$ is neatly surjective, so $\der\smallo=\smallo$. Now use Lemma~\ref{supPsi=0}.
\end{proof} 


\noindent
Since $\sup \Psi = 0$ fails for $\mathbb{T}$, this asymptotic field 
is not $\d$-henselian. Chapter~\ref{ch:newtdirun} and Lemma~\ref{diffnewt}, however, show that $\mathbb{T}$ becomes $\d$-henselian if we coarsen its valuation by any convex subgroup of $\Gamma_{\T}$ that contains $v(x)$.

 
%\begin{lemma}\label{dhres} Suppose $K$ is 
%$n$-differential-henselian, $n\ge 1$, and
%identify $C$ and $C_{\k}$ via the field isomorphism 
%$a\mapsto \bar{a}%\colon C \to C_{\k}$.
%Let $A\in K[\der]$ have order $\le n$, with $vA=0$. Then the map
%$$ a \mapsto \overline{a} \colon\ \mathcal{O}\cap \ker A\ \to\ 
%\ker \bar{A}$$
%is $C$-linear and surjective.
%\end{lemma}
%\begin{proof} Let $A=a_0 + a_1\der+ \dots + a_n\der^n$ with 
%$a_0,\dots, a_n\in K$. Set $$P(Y)\ :=\ a_0Y+ \dots + a_nY^{(n)}.$$ 
%Suppose $a\in \mathcal{O}$, $v(a)=0$ and 
%$\overline{A}(\overline{a})=0$. Then $P$ is in dh-position 
%at $a$, so we have $y\in \mathcal{O}$ such that
%$P(y)=0$ and $\overline{y}=\overline{a}$. Then $A(y)=0$.
%\end{proof}  

\begin{cor}\label{asexistdhenselization} Assume $\k$ is linearly surjective. Then $K$ has an immediate asymptotic field extension $L$ such that: \begin{enumerate}
\item $L$ is $\d$-algebraic over $K$;
\item $L$ has small derivation and is $\d$-henselian;
\item no proper differential subfield of $L$ containing $K$ is $\d$-henselian.
\end{enumerate}
\end{cor}
\begin{proof} Corollary~\ref{henimm} yields an immediate valued differential field extension $F$ of $K$ with small derivation such that $F$ is $\d$-henselian. Then $F$ is asymptotic by Lemma~\ref{impreservesas}. 
By keeping only the elements of 
$F$ that are $\d$-algebraic over $K$ we arrange that $F$ is  $\d$-algebraic over $K$. 

 Let $L$ be the intersection inside
$F$ of the collection of all differential subfields~$E$ of $F$ that
contain $K$ and are $\d$-henselian. 
Proposition~\ref{noextrazeros} applied to the
extensions $E\subseteq F$ shows that $L$ has the desired property.
\end{proof} 

\noindent
We conjecture that there is only one $L$ as in 
Corollary~\ref{asexistdhenselization}, up to isomorphism over 
$K$. For any $r\in \N$, Corollary~\ref{asexistdhenselization}
goes through with ``linearly surjective'' and ``$\d$-henselian'' replaced by
``$r$-linearly surjective'' and ``$r$-$\d$-henselian''.  

\medskip\noindent
We already mentioned the significant constraint $\sup \Psi=0$
on $\d$-henselian $K$. This condition is necessary for
$K$ to be merely {\em embeddable\/} into a 
$\d$-henselian asymptotic field; is it also sufficient? 
Here is a partial answer.

\begin{cor}\label{aspsidh} Suppose $\sup \Psi=0\notin \Psi$.
Then $K$ has a $\d$-henselian pre-$\d$-valued field extension $L$ with $\Gamma_L=\Gamma$.
\end{cor}
\begin{proof} Since $\k$ can be extended to a
linearly surjective differential field, Corollary~\ref{resextpred} yields a pre-$\d$-valued field extension $E$ of $K$ with small derivation, the same
value group as $K$, and linearly surjective differential residue field $\k_E\supseteq \k$. Then Corollary~\ref{cor2diftrzda} and Lemma~\ref{smallunramasymp} yield
an immediate spherically complete pre-$\d$-valued field extension $L$ of $E$; any such $L$ is $\d$-henselian.
\end{proof}

\noindent
If $\max \Psi=0$, then $K$ also has a $\d$-henselian asymptotic field extension with the same value group, by Lemma~\ref{KgroundedLasymp} together with some facts about the {\em linear surjective closure of a differential field\/}, a notion to be developed in the next volume. 

%This raises two questions: 
%\begin{enumerate}
%\item[(i)] Are there $\d$-henselian $K$ with 
%$\Gamma\ne \{0\}$ and $0\notin \Psi$? 
%\item[(ii)] Are there $\d$-henselian $K$ with $0\in \Psi$?
%\end{enumerate}
%Both questions have a positive answer, as we now indicate.

%\marginpar{commented out material below has been checked}
%For (ii) we start with a $\d$-henselian $K$ such that 
%$\Gamma\ne \{0\}$ and $0\notin \Psi$. 
%Take $\gamma\in \Psi$, and set
%$\delta:= \gamma^\dagger$, so 
%$\gamma < \delta < 0$ and $\delta=o(\gamma)$. Set 
%$$\Delta\ :=\ \{\alpha\in \Gamma:\ |\alpha|\le n|\delta| 
%\text{ for some }n\}.$$ Then $\Delta$ is a convex 
%subgroup of $\Gamma$ and $\delta, \delta^\dagger\in \Delta$. 
%Also $\gamma\notin \Delta$ and $\gamma^\dagger\in \Delta$, 
%so the $\Psi$-set $\Psi_{\Delta}$ of the $\Delta$-coarsening %of $K$ has largest element $0\in \Gamma/\Delta$, and 
%this $%\Delta$-coarsening of
%$K$ is asymptotic and $\d$-henselian, by 
%Corollary~\ref{coarsen} and Lemma~\ref{inva3}.   




\subsection*{More on coarsening} The asymptotic fields that play a role 
in later chapters and that 
are not pre-$\d$-valued are 
obtained by coarsening the valuation of a 
pre-$\d$-valued field. This raises the question whether
every asymptotic field arises by coarsening the valuation of a
pre-$\d$-valued field. In Section~\ref{Miscellaneous Facts about Asymptotic Fields} we show that this is 
not the case. The next result answers another question:  
when is a coarsening of an asymptotic field pre-$\d$-valued? 

Let $\Delta$ be a convex subgroup of 
$\Gamma$. Using the same notations as at the end of Section~\ref{AbstractAsymptoticCouples},  
we have the $\Delta$-coarsening
$(K,{\dotpreceq})$, which is again an asymptotic field. 


\begin{prop}\label{Coarsenings-Pdv}
Suppose that $\{0\} \ne \Delta\neq\Gamma$. The following are equivalent:
\begin{enumerate}
\item $(K,\dotpreceq)$ is a pre-$\d$-valued field;
\item the subset $\Psi_{\Delta}$ of $\dot{\Gamma}$ does not have a largest element;
\item $\psi(\gamma)-\psi(\delta)\notin\Delta$ for all $\gamma\in\Gamma
\setminus\Delta$, $\delta\in\Delta^{\ne}$;
\item $\psi(\gamma)-\psi(\delta) < \Delta$ for all $\gamma\in\Gamma
\setminus\Delta$, $\delta\in\Delta^{\ne}$.
\end{enumerate}
\end{prop}
\begin{proof}
The implication (4)~$\Rightarrow$~(3) is trivial,
(3)~$\Rightarrow$~(2) follows by Lemma~\ref{Coarsening-Prop}, and
(2)~$\Rightarrow$~(1) by 
Corollary~\ref{asymp-predif}.
To show (1)~$\Rightarrow$~(4), let
$(K,\dotpreceq)$ be pre-$\d$-valued, and let
 $\gamma\in\Gamma$, $\gamma >\Delta$, $\delta\in\Delta^{\ne}$. 
Then $\gamma=vg$, $\delta=
vf$ with $f,g\in K^\times$, so
$\dot{v}(f') > \dot{v}( g^\dag)$, hence $\Delta>v(g^\dagger)-v(f')=
\psi(\gamma)-\bigl(\delta+\psi(\delta)\bigr)$. Thus
 $\psi(\gamma)-\psi(\delta) < \Delta$. 
\end{proof}

\noindent
In view of Lemma~\ref{asymp-lemma1} this yields: 

\begin{cor}\label{Coarsenings-Pdv, application}
Suppose $\psi(\Delta^{\neq})\cap\Delta\neq\emptyset$. Then
$$\text{$(K,{\dotpreceq})$ is pre-$\d$-valued} \quad\Longleftrightarrow\quad 
\psi(\Gamma\setminus\Delta)\ \subseteq\ \Gamma\setminus\Delta.$$
\end{cor}

\noindent
This gives new cases where the hypothesis of part~(3) of Corollary~\ref{cor:value group of dv(K)} is satisfied:

\begin{exampleNumbered}\label{ex:pdv with gap, 2} Assume $K$ is of $H$-type and $1\in\Gamma^>$ satisfies $\psi(1)=1$. Set
$$\Delta\ :=\ \big\{\gamma\in\Gamma :\ \text{$\psi^n(\gamma) \geq 0$ for some $n\geq 1$} \big\}.$$
Then $\Delta$ is a convex subgroup of $\Gamma$ with 
$1\in\psi(\Delta^{\neq})\cap\Delta$, and $\psi(\Gamma\setminus\Delta)\subseteq\Gamma\setminus\Delta$.
Hence
 $(K,{\dotpreceq})$ is pre-$\d$-valued by Corollary~\ref{Coarsenings-Pdv, application}. Moreover, any $b\in K^\times$ with $1\nasymp b\dotasymp 1$ yields a gap 
 $\dot v(b')=\dot v(b^\dagger)=\psi\big(v(b)\big)+\Delta$ of $(K,{\dotpreceq})$, by Lemma~\ref{Coarsening-Prop} and the equivalence 
 of (1) and (2) in
Proposition~\ref{Coarsenings-Pdv}. Since $\Delta\ne \{0\}$, such $b$ exist, so the hypothesis of part~(3) of Corollary~\ref{cor:value group of dv(K)} holds 
for $(K,{\dotpreceq})$ in place of $K$.

If $K$ is an  $\aleph_0$-saturated elementary extension  of $\T$,  then 
$\Delta\neq\Gamma$ for this $\Delta$, since for each $n\geq 1$ and
$\gamma:= v\big(\exp^{n+1}(x)\big)$ we have $\psi^m(\gamma)<0$ for $m=1,\dots,n$.
\end{exampleNumbered} 



\subsection*{Specialization of asymptotic fields}
{\em Let $K$ have small derivation, and let~$\Delta$ be a convex subgroup
of $\Gamma=v(K^\times)$}. 
It follows from Corollary~\ref{cor:Cohn-Lemma} 
that
the valuation ring $\dot{\mathcal{O}}$ of the coarsening 
$\dot{v}=v_{\Delta}\colon K^\times \to \dot{\Gamma}$ of~$v$  
and the maximal ideal $\dot{\smallo}$
of~$\dot{\mathcal{O}}$
are closed under $\der$. Note that if $\sup \Psi=0$, then 
$\psi(\Delta^{\ne}) \subseteq \Delta$ and $\sup \psi(\Delta^{\ne})=0$ in $\Delta$, by Lemma~\ref{PresInf-Lemma2},~(4).


\medskip\noindent
{\em In the rest of this subsection we assume that 
$\psi(\Delta^{\ne}) \subseteq \Delta$}.
The residue 
field $\dot K= \dot{\mathcal{O}}/\dot{\smallo}$
of $\dot{\mathcal{O}}$ with its induced valuation 
$v\colon \dot K^\times \to \Delta$
and the induced derivation is then an asymptotic field
with asymptotic couple $(\Delta,\psi|\Delta^{\ne})$. (This follows from 
the equivalence of (1) and (2) in 
Proposition~\ref{CharacterizationAsymptoticFields}.) Moreover, $\dot K$ 
has small derivation, the field isomorphism 
$\res(K) \to \res(\dot K)$ from 
Section~\ref{sec:decomposition} is a differential field isomorphism, and if $K$ is
of $H$-type, then so is $\dot{K}$.
We identify $C$ with a subfield of $C_{\dot K}$ via the 
field embedding $c\mapsto\dot c\colon C\to C_{\dot K}$.

\begin{lemma}\label{Specialization of asymptotic fields}
Suppose $K$ is pre-$\d$-valued. Then $\dot K$ is 
pre-$\d$-valued. 
If $K$ is $\d$-valued, then $\dot K$ is $\d$-valued
with $C_{\dot K}=C$.
\end{lemma}
\begin{proof}
Let $f\in \cal{O}$ and 
$g\in \smallo\setminus \dot{\smallo}$, so 
$\dot f\in {\cal O}_{\dot K}$ and
$\dot g \in \smallo_{\dot K}\setminus\{0\}$. Then $vg\in \Delta^{\ne}$, so
$vg'\in \Delta$, hence  
$v(\dot {f}') \geq v(f')>v(g^\dagger)=
v({\dot g}^\dagger)$, so
$\dot K$ is pre-$\d$-valued. Now assume that 
$K$ is $\d$-valued. 
Then the natural map $C_{\dot K}\subseteq {\cal O}_{\dot K}\to \res(\dot K)$
restricts to an isomorphism $C\to\res(K)$ and hence is an
isomorphism $C_{\dot K}\cong\res(\dot K)$, since $\res(K)=\res(\dot K)$. Therefore $\dot K$ is
$\d$-valued with $C_{\dot K}=C$.
\end{proof}

\begin{lemma}\label{specasymptint} Suppose $K$ has asymptotic integration and $\Delta\ne \{0\}$.
Then $\dot{K}$ has asymptotic integration.
\end{lemma}
\begin{proof} Take $\alpha\in \Delta^{\ne}$, and note that $\alpha+\psi(\alpha)\in \Delta$. Let $\delta\in \Delta$, $\delta\ne \alpha+\psi(\alpha)$, and take $\beta\in \Gamma^{\ne}$ with $\beta + \psi(\beta)=\delta$. Then by 
Lemma~\ref{BasicProperties}, (2),  
$$\big(\alpha + \psi(\alpha)\big)-\big(\beta+\psi(\beta)\big)=\alpha-\beta + o(\alpha-\beta)\in \Delta,$$
so $\alpha-\beta\in \Delta$, and thus $\beta\in \Delta$. 
\end{proof}



\index{closed!under integration}
\index{closed!under logarithms}
\index{differential field!closed under integration}
\index{differential field!closed under logarithms}

\noindent
We say that the differential field $F$ is {\bf closed under integration}
if for every $f\in F$ there is a $y\in F$ with $y'=f$, and we say that
$F$ is {\bf closed under logarithms} if for every $f\in F^\times$ 
there is a $y\in F$ with $y'=f^\dagger$. So if $F$ is closed under
integration, then $F$ is closed under logarithms. Every Liouville closed
$H$-field is closed under integration.
If the differential field $F$ is closed under integration 
(closed under logarithms)
and $\phi\in F^\times$, then $F^\phi$ is closed under integration
(closed under logarithms, respectively). 

\begin{lemma} Suppose $\Delta\ne \{0\}$.
If $K$ is closed under integration, then so is $\dot{K}$. If $K$ is
closed under logarithms, then so is $\dot{K}$.
\end{lemma}
\begin{proof}
Take $\delta\in\Delta^{\ne}$; then $\psi(\delta)\in\Delta$.
Suppose $K$ is closed under integration, and
let $f\in \dot{\cal{O}}$. We need to find $y\in\dot{\cal{O}}$ with $y'-f\in
\dot{\smallo}$. If $vf>\Delta$, then we may take $y:=0$, so we may assume
$vf\in\Delta$. Take $y\in K$ with $y'=f$; we claim that $y\in\dot{\cal{O}}$.
Suppose $y\notin \dot{\cal{O}}$. Then $\gamma:=vy<\Delta$, 
in particular 
$[\gamma]>[\delta]$
and hence $\big[\psi(\gamma)-\psi(\delta)\big]<[\gamma-\delta]=[\gamma]$ by
Lemma~\ref{BasicProperties}, (2). 
Since $\gamma+\psi(\gamma)=vf\in
\Delta$, we therefore have $[\gamma]=\big[\gamma+\psi(\gamma)-\psi(\delta)\big]\in [\Delta]$ and hence $\gamma\in\Delta$, a contradiction. 
Thus $\dot{K}$ is closed under integration.
Similarly one shows that if $K$ is
closed under logarithms, then so is $\dot{K}$.
\end{proof} 

\noindent
Let $L$ be an asymptotic field extension of $K$  with small derivation. 
Let $\Delta_L$ be the convex hull of $\Delta$ in $\Gamma_L$, and let
$$ \dot{\mathcal{O}}_L:=
  \{y\in L: vy\ge \delta \text{ for some }\delta\in \Delta_L\}
$$
be the valuation ring of the corresponding coarsening 
$\dot{v}\colon L^\times \to \dot{\Gamma}_L= \Gamma_L/\Delta_L$.  
Then $\dot{\mathcal{O}}_L$ and its maximal ideal 
$\dot{\smallo}_L$
are closed under the derivation $\der$ of $L$. Note that 
$\dot{\mathcal{O}}_L$ lies over $\dot{\mathcal{O}}$. Let 
$\dot L:=  \dot{\mathcal{O}}_L/\dot{\smallo}_L$ be the residue 
field of $\dot{\mathcal{O}}_L$, equipped with the induced valuation
$v\colon {\dot L}^\times \to \Delta_L$. We have
$\psi_L(\Delta_L^{\ne}) \subseteq \Delta_L$, so the field 
$\dot L$ with its valuation $v$
and the induced derivation is an asymptotic field
with asymptotic couple $(\Delta_L,\psi_L|\Delta_L^{\ne})$. With the usual
identifications we have $\dot K\subseteq \dot L$, not only 
as (residue) fields, 
but also as asymptotic fields. 


\subsection*{Flattening} For certain {\em definable} ways of coarsening we 
use special notation and terminology, borrowed from \cite{JvdH}. These
particular coarsenings are called flattenings and 
will be very useful in Chapters~\ref{ch:The Dominant Part and the Newton Polynomial} and ~\ref{ch:newtonian fields}. 
{\em Assume $K$ is of $H$-type, and let 
$\gamma$ range over $\Gamma$}.
We have the convex subgroup 
$$\Gamma^\flat\ :=\ 
\bigl\{\gamma :\  \psi(\gamma)>0\bigr\}$$
of $\Gamma$. 
For example, if $K=\mathbb T$, then
$$\Gamma^\flat\ =\ \{vh:\  h\in K^\times,\ h\flatter \ex^x\}.$$
Let
$$v^\flat\ \colon\ K^\times\to \Gamma^\sharp
\qquad\text{where $\ \Gamma^\sharp\ :=\ \Gamma/\Gamma^\flat$}$$ 
be the coarsening of the valuation $v$ by $\Gamma^\flat$, with associated dominance relation $\preceq^\flat$ on $K$, and valuation ring $\mathcal{O}^\flat$. We call the valuation $v^\flat$ the {\bf flattening} of $v$. 
Note that the definition of $\Gamma^\flat$ depends on the derivation of $K$.

\index{flattening}
\index{valuation!flattening}
\nomenclature[Z]{$\Gamma^\flat$}{$\{\gamma:\psi(\gamma)>0\}$}
\nomenclature[Z]{$v^\flat$}{flattening of the valuation $v$ of an $H$-asymptotic field}
\nomenclature[Rx]{$\preceq^\flat$}{dominance relation associated to $v^\flat$}
\nomenclature[Z]{$\Gamma^\sharp$}{$\Gamma^\sharp=\Gamma/\Gamma^\flat$}

Let $\phi\in K^\times$, and use a subscript $\phi$ to indicate the flattened objects $\Gamma^\flat_\phi$, $v^\flat_\phi$, $\preceq^\flat_\phi$, $\prec^\flat_\phi$, $\asymp^\flat_\phi$, and $\simflat_\phi$ associated to the asymptotic field $K^\phi$. In particular
$$\Gamma^\flat_\phi\ =\  \big\{ \gamma :\  
\psi(\gamma) > v\phi \big\}.$$
Clearly $\Gamma^\flat_\phi=\{0\}$ iff
$v\phi\notin \big(\Gamma^{<}\big)'$, and $\Gamma^\flat_\phi=\Gamma$
iff $\Psi>v\phi$. The flattening $v^\flat_\phi$ of the valuation $v$ on 
$K^{\phi}$ will be useful for ungrounded
$K$ and $v\phi\in \Psi^{\downarrow}$. In that case, 
with $v\phi$ increasing cofinally in $\Psi^{\downarrow}$, the convex subgroup
$\Gamma^\flat_\phi$ of $\Gamma$ becomes arbitrarily small, and so
$v^\flat_\phi$ (with value group $\Gamma/\Gamma^\flat_{\phi}$) approximates $v$ in some sense. 

We denote the gaussian extension of
$v^\flat_{\phi}$ to $K^\phi\<Y\>$ also by $v^\flat_{\phi}$. The binary relations $\preceq^\flat_\phi$, $\prec^\flat_\phi$, $\asymp^\flat_\phi$, and $\simflat_\phi$,
on $K$ extend likewise, with the same notations, to binary relations on $K^{\phi}\<Y\>$. As $K\<Y\>$ and 
$K^{\phi}\<Y\>$ have the same underlying field, we also use
the same notations for elements of $K\<Y\>$; for example, 
given $f\in K$ and $P\in K\<Y\>$, $f\preceq^\flat_\phi P$ means that $v^\flat_{\phi}(f) \ge v^\flat_{\phi}(P)$ in $\Gamma/\Gamma^\flat_{\phi}$, where in the latter inequality
$f$ and $P$ are taken as elements of $K^\phi\subseteq K^\phi\<Y\>$ and 
$K^{\phi}\<Y\>$, respectively. 




\nomenclature[Z]{$\Gamma^\flat_\phi$}{$\{\gamma:\psi(\gamma)>v\phi\}$}
\nomenclature[Z]{$v^\flat_\phi$}{flattening of the valuation $v$ of $K^\phi$}
\nomenclature[Rx]{$\preceq^\flat_\phi$}{dominance relation associated to $v^\flat_\phi$}

\begin{lemma}
Suppose $\Phi\in K^\times$ with $\Phi\nasymp 1$ and 
$\Phi^\dagger\asymp\phi$, and $f,g\in K$. Then
\begin{align*}
f\preceq^\flat_\phi g &\quad\Longleftrightarrow\quad v^\flat_\phi(f)\geq v^\flat_\phi(g) 
\quad\Longleftrightarrow\quad \text{$f\preceq hg$ for some $h\in K^\times$ with $h\flatter\Phi$,}\\
f\prec^\flat_\phi g &\quad\Longleftrightarrow\quad v^\flat_\phi(f)> v^\flat_\phi(g) 
\quad\Longleftrightarrow\quad \text{$f\prec hg$ for all $h\in K^\times$ with $h\flatter\Phi$,}\\
f\asymp^\flat_\phi g &\quad\Longleftrightarrow\quad v^\flat_\phi(f)=v^\flat_\phi(g) 
\quad\Longleftrightarrow\quad \text{$f\asymp hg$  for some $h\in K^\times$ with $h\flatter \Phi$.}
\end{align*}
\end{lemma}
\begin{proof}
These equivalences follow from their validity for $g=1$, and in that case
we argue as follows:
\begin{align*}
f\preceq^\flat_\phi 1 &\quad\Longleftrightarrow\quad \text{$vf\geq vh$
for some $h\in K^\times$ with $vh\in\Gamma^\flat_\phi$} \\
&\quad\Longleftrightarrow\quad \text{$f\preceq h$ for some $h\in K^\times$ with $h\flatter \Phi$,}
\end{align*}
where we use that $1\flatter \Phi$ to get the last equivalence when $vh=0$.
We proceed likewise with $f\prec^\flat_\phi 1$ and $f\asymp^\flat_\phi 1$, treating the case $vh=0$ separately. 
\end{proof}

\noindent
The
valuation ring of $v^\flat_\phi$ is
$$\cal{O}^\flat_\phi\ =\ \big\{ f\in K:\  \text{$vf\geq 0$ or $v(f')>vf + v\phi$} \big\},$$
with maximal ideal 
$$\smallo^\flat_\phi\ =\ \big\{ f\in K:\  \text{$vf>0$ and $v(f')\leq vf + v\phi$} \big\}.$$
Note that if $\Gamma^\flat=\{0\}$, then the canonical map $\Gamma\to\Gamma^\sharp$ is an isomorphism
of ordered groups via which $\Gamma$ is identified with $\Gamma^\sharp$.
If $\Gamma^\flat\neq\{0\}$, then $K$ has small derivation and 
there exists a unique positive element $1$ in
$\Gamma^\flat$ with $\psi(1)=1$, so $\psi\big((\Gamma^\flat)^{\ne}\big)\subseteq\Gamma^\flat$
by Lemma~\ref{asymp-lemma1}, (1). Note also that if $\Gamma^\flat\neq\{0\}$, 
%and $\Gamma^\flat\neq \Gamma$, 
then by Lemma~\ref{Coarsening-Prop} we have
$\sup \Psi^\flat=0$ in $\Gamma^\sharp$, where
$$\Psi^\flat:= \big\{v^\flat(f^\dagger):\ f\in K^\times,\ f\not\asymp^\flat 1\big\}.$$
If $\Gamma^\flat\neq\{0\}$, then 
we denote the asymptotic residue field of $v^\flat$ by
$K^\flat := \cal{O}^\flat/\smallo^\flat$, with asymptotic couple  
$(\Gamma^\flat,\psi|\Gamma^\flat)$. 


\nomenclature[Z]{$\cal{O}^\flat_\phi$}{valuation ring of $v^\flat_\phi$}
\nomenclature[Z]{$\smallo^\flat_\phi$}{maximal ideal of the valuation ring of $v^\flat_\phi$}


\medskip\noindent
Let $\Phi\in K^\times$ with $\Phi\nasymp 1$. The binary relations 
$\preceq^\flat_{\Phi^\dagger}$, $\prec^\flat_{\Phi^\dagger}$, $\asymp^\flat_{\Phi^\dagger}$ on $K$, and on $K\<Y\>$,  are often denoted by
$\preceq_{\Phi}$, $\prec_{\Phi}$, $\asymp_{\Phi}$, respectively. Thus
for $f,g\in K$: 
\begin{align*}
f\preceq_\Phi g &\quad\Longleftrightarrow\quad  \text{$f\preceq hg$ for some $h\in K^\times$ with $h\flatter\Phi$,}\\
f\prec_\Phi g &\quad\Longleftrightarrow\quad    \text{$f\prec hg$ for all $h\in K^\times$ with $h\flatter\Phi$,}\\
f\asymp_\Phi g &\quad\Longleftrightarrow\quad \text{$f\asymp hg$  for some $h\in K^\times$ with $h\flatter \Phi$.}
\end{align*}
An advantage of this notation is that the relations $\preceq_{\Phi}$, $\prec_{\Phi}$, $\asymp_{\Phi}$ do not change in passing from $K$ to
a compositional conjugate $K^\phi$ ($\phi\in K^\times$). Note that $\Phi\nasymp_\Phi 1$ by Corollary~\ref{CharacterizationAsymptoticFields-Corollary}, (4), and if $\Phi\prec 1$, then $\Phi\prec_{\Phi} 1$. Also, for $f\nasymp 1$ in $K^{\times}$,
$$f\ \asymp_\Phi\ 1\ \Longleftrightarrow\ f\ \flatter\ \Phi.$$ 
Here are some further rules:

\nomenclature[Rx]{$\preceq_\Phi$}{dominance relation $\preceq^\flat_{\Phi^\dagger}$, for $\Phi\in K^\times$, $\Phi\nasymp 1$}

\begin{lemma}\label{symflat} Let $f,g\in K^\times,\ f, g\nasymp 1,\  f\prec_{g} g$. Then $f\prec_{f} g$.
\end{lemma}
\begin{proof} We have $f/g\prec^{\flat}_{g^\dagger} 1$, so $\psi(vf - vg)\le \psi(vg)$, hence $\psi(vf-vg)\le \psi(vf)$, which in view of $vf> vg$ yields $f/g\prec^{\flat}_{f^\dagger} 1$, so $f\prec_{f} g$.
\end{proof}

\begin{lemma}\label{lem:flat equivalence}
Let $\Phi_1,\Phi_2\in K^\times$ with $\Phi_1,\Phi_2\nasymp 1$ and $\Phi_1 \flattereq \Phi_2$. Then for $f,g\in K$:
$$f\preceq_{\Phi_1} g  \ \Rightarrow\ f\preceq_{\Phi_2} g\qquad\text{and}\qquad
f\prec_{\Phi_2} g \ \Rightarrow\  f\prec_{\Phi_1} g.$$
\end{lemma}

\begin{lemma}\label{cor:flat equivalence}
Suppose $\Phi\in K^\times$, $\Phi \nasymp^\flat 1$. 
Then for all $f,g\in K$:
$$f\preceq^\flat g  \ \Rightarrow\ f\preceq_{\Phi} g\qquad\text{and}\qquad
f\prec_{\Phi} g \ \Rightarrow\  f\prec^\flat g.$$
\end{lemma}
\begin{proof} The second part follows from the first. To prove the first part, arrange $f\neq 0$ and $g=1$.
Assume $f\preceq^{\flat} 1$. Then $f\preceq 1$ or 
$f^\dagger \prec 1$. From
$\Phi \nasymp^\flat 1$ we get $\Phi^\dagger \succeq 1$, so
$f\preceq 1$ or $f^{\dagger}\prec \Phi^\dagger$, and thus $f\preceq_{\Phi}1$.
\end{proof}

%\noindent
%Let $\Phi\in K^\times$, $\Phi\not\asymp 1$.
%Given $f,g\in K$, the truth value of each of the conditions
%$$f\asymp^{\flat}g,\ f\preceq^{\flat} g,\ f\prec^{\flat} g,\ $f\asymp_{\Phi}g,\ f\preceq_{\Phi} g,\ f\prec_{\Phi} g$$
%depends only on the pair $(vf, vg)$. This allows us 
%to extend each of
%the binary relations $\asymp^{\flat}$, $\preceq^{\flat}$, 
%$\prec^{\flat}$, 
%$\asymp_{\Phi}$, $\preceq_{\Phi}$,
%$\prec_{\Phi}$ on $K$ to a binary relation on $K\{Y\}$, 
%to be denoted by the same symbol: for $P,Q\in K\{Y\}$, we %declare $P\asymp^{\flat} Q$ to mean $f\asymp^{\flat} g$
%with $f,g\in K$ such that $vP=vf$, $vQ=vg$, and 
%likewise with the other relations.

\noindent
In the next lemma and its corollaries below
we assume that $K$ is ungrounded and has small derivation. Also $P\in K\{Y\}^{\neq}$ and $g\in K^\times$, $g\nasymp 1$.


\begin{lemma}\label{lem:Pg flat equivalence}
Suppose $P$ is homogeneous of degree $d$.  Then 
$P_{\times g} \asymp_g P\,g^d$.
\end{lemma}
\begin{proof}
If $g^\dagger\preceq 1$, then $P_{\times g}\asymp Pg^d$ by Lemma~\ref{vplemma}. 
If $g^\dagger\succ 1$, then $g^{\dagger\dagger}\prec g^\dagger$ by~(4) of Lemma~\ref{PresInf-Lemma2}, and thus
$P_{\times g} \asymp_g Pg^d$ by Proposition~\ref{ps1}.
\end{proof}

\begin{cor}\label{cor:Pg flat equivalence, 1}
Suppose $g\prec 1$ and $d:=\dv(P)=\val(P)$. 
Then
$$P_{\times g}\ \asymp_g  P\,g^d.$$ 
\end{cor}
\begin{proof}
We have $P_i\preceq P_d$ for $i\ge d$, and $g\prec_g 1$, hence
$P_i\,g^i\prec_g P_d\,g^d$ for $i>d$, and the claim follows from
Lemma~\ref{lem:Pg flat equivalence}.
\end{proof}

\noindent
For $F\in K\{Y\}$ and $d\in\N$ we put 
$$F_{\leq d}\ :=\ F_0+F_1+\cdots+F_d, \qquad F_{>d}\ :=\ F-F_{\leq d}.$$
With this notation, we have:

\begin{cor}\label{cor:Pg flat equivalence, 2}
Suppose $g\succ 1$ and $d:=\ddeg(P)=\ddeg(P_{\times g})$. Then $$gP_{>d}\ \preceq_g\  P.$$
\end{cor}
\begin{proof} The case $P_{>d}=0$ being trivial, assume $P_{>d}\ne 0$.
Take $i>d$ such that $P_i \asymp P_{>d}$. Then by Lemma~\ref{lem:Pg flat equivalence} and $g\succ 1$ we have
$$(P_{\times g})_i\ =\ (P_i)_{\times g}\ \asymp_g\ P_i\,g^i\ \succeq\ P_i\,g^{d+1}\ \asymp\ g^{d+1}P_{>d}$$ and so
$(P_{\times g})_{>d} \succeq_g  g^{d+1}P_{>d}$. Since $\ddeg(P_{\times g})=d$, we have  
$(P_{\times g})_d\succeq  (P_{\times g})_{>d}$, and by Lemma~\ref{lem:Pg flat equivalence} again,
$(P_{\times g})_d = (P_d)_{\times g} \asymp_g g^dP_d$. Since $\ddeg(P)=d$, we have $P\asymp P_d$, so
$$ g^dP\ \asymp\ g^dP_d\ \asymp_g\ (P_{\times g})_d\ \succeq\ (P_{\times g})_{>d}\ \succeq_g\ g^{d+1}P_{>d},$$ and thus
$P\succeq_g gP_{>d}$ as claimed.
\end{proof}

\begin{cor}\label{cor:Pg flat equivalence, 3}
Let $f\in K^\times$ be such that $f\nasymp 1$ and $f\flatter g$. Then $P_{\times f} \asymp_g P$.
\end{cor}
\begin{proof}
Take $d\in\N$ with $P_{\times f}\asymp (P_d)_{\times f}$.
Lemma~\ref{lem:Pg flat equivalence} gives 
$(P_d)_{\times f}\asymp_f P_df^d$, so 
$P_{\times f} \asymp_f P_d\, f^d$, which by Lemma~\ref{lem:flat equivalence} yields $P_{\times f}\asymp_g P_df^d$. From
$f\flatter g$ we also get $f\asymp_g 1$, so
$P_d\, f^d \asymp_g P_d \preceq P$, hence $P_{\times f}\preceq_g P$. Applying the same
argument to $P_{\times f}$, $f^{-1}$ in place of $P$, $f$ yields $P=(P_{\times f})_{\times f^{-1}}\preceq_g P_{\times f}$.
\end{proof}






==> mt-9-6.tex <==



\section{Algebraic Extensions of Asymptotic Fields}
\label{pafae}
 
\noindent
In this section we prove analogues for asymptotic fields of
results in Section~\ref{sec:algebraicext} on algebraic extensions of 
valued differential fields with small derivation.  

\subsection*{Immediate algebraic extensions} {\em In this subsection we fix a valued differential field $L$ with a subfield $K$.
We consider $K$ as a valued subfield of $L$ with valuation ring
$\mathcal{O}$, maximal ideal $\smallo$ of $\mathcal{O}$,
and value group $\Gamma$}. 
In order for $L$ to be asymptotic it is of course necessary that 
for all $f,g\in K^\times$ with $f,g\prec 1$ we have
$$f\prec g\quad \Longleftrightarrow\quad f'\prec g'.$$
Call $K$ {\bf asymptotic in  $L$} if this condition is satisfied. 
Below we prove:

\index{valued differential field!asymptotic in}

\begin{prop}\label{pa5} Suppose $K$ is asymptotic in $L$ and $L$ 
is an immediate 
algebraic extension of $K$. Then $L$ is asymptotic.
\end{prop}

\noindent
For later use it is important that in this proposition 
we do not require $K$ to be closed under the derivation of $L$. 
First some remarks and a lemma.
Suppose $K$ is asymptotic in $L$, and set $C:=\{a\in K:\ a'=0\}$, a subfield
of $K$. Then
$C\cap \smallo =\{0\}$ by the same argument as for
asymptotic fields. Thus the valuation $v$ is trivial on~$C$, and
the map $\varepsilon\mapsto\varepsilon'\colon \smallo\to L$ is injective.
A variant of Proposition~\ref{CharacterizationAsymptoticFields} goes through with the same proof:

\begin{lemma}\label{pa1} Suppose $v(L^\times)=v(K^\times) (=\Gamma)$.
Then the following are equivalent:
\begin{enumerate}
\item $K$ is asymptotic in $L$;
\item there is an asymptotic couple $(\Gamma,\psi)$ 
such that for all $f\in K^\times$ with $f\nasymp 1$ we have
$\psi(vf)=v(f^\dagger)$;
\item if $f,g\in K^\times$ with
$f,g\nasymp 1$, then $f\preceq g \Longleftrightarrow f'\preceq g'$.
\item if $f,g\in K^\times$, then:
$$\begin{cases}
&f\prec 1,\ g\nasymp 1 \quad\Rightarrow\quad f'\prec g^\dagger,\\
&f\asymp 1,\ g\nasymp 1 \quad\Rightarrow\quad f'\preceq g^\dagger.
\end{cases}$$
\end{enumerate}
\end{lemma}

\noindent
If $K$ is asymptotic in $L$ and $v(L^\times)=v(K^\times)$, then we call $(\Gamma, \psi)$ as defined in 
(2) of the lemma above the {\bf asymptotic couple of $K$ in $L$},  so
$$ \Psi\ :=\ \psi(\Gamma^{\ne})\ =\ \bigl\{v(g^{\dagger}): 1 \nasymp g\in K^{\times}\bigr\}.$$


\begin{proof}[Proof of Proposition~\ref{pa5}] 
Let $(\Gamma,\psi)$ be the
asymptotic couple of $K$ in $L$. We shall prove that $L$ is asymptotic
with asymptotic couple $(\Gamma,\psi)$. Let $g\in L^{\times}$, $g\not\asymp 1$; 
by Proposition~\ref{CharacterizationAsymptoticFields},~(2), it is enough 
to show that then 
$v(g^\dagger)=\psi(vg)$.

Before doing so, note that if $\phi\in L^\times$, then $K$ is
also asymptotic in $L^{\phi}$
with $(\Gamma, \psi -v\phi)$ as the asymptotic couple of $K$ in $L^{\phi}$, and
with $\phi^{-1}g^\dagger$ as the
logarithmic derivative of $g$ in $L^\phi$.
Thus we may replace $L$ by a compositional conjugate. 

Take $f\in K^\times$ with $f\sim g$, so 
$g=f(1+\varepsilon)$ with $\varepsilon \in \smallo_L$.
Then $g^\dagger=f^\dagger + \frac{\varepsilon'}{1+\varepsilon}$.
Now $v(f^\dagger)=\psi(vf)=\psi(vg)\in \Psi$. Compositional conjugation by 
$\phi:= f^\dagger$  (and renaming) arranges that $v(f^\dagger)=0\in \Psi$, so
$(\Gamma, \psi)$ has small derivation. Then 
$\der \smallo\subseteq \smallo_L$
and $\der\mathcal{O}\subseteq \mathcal{O}_L$ by Lemma~\ref{pa1}, (4), so 
$\der\smallo_L\subseteq \smallo_L$ by Lemma~\ref{key}. This gives 
$f^\dagger \asymp 1\succ  \frac{\varepsilon'}{1+\varepsilon}$, so
$g^\dagger\sim f^\dagger$, and thus $v(g^\dagger)=v(f^\dagger)=\psi(vg)$. 
\end{proof}

\subsection*{Algebraic extensions}
{\em In this subsection we assume that $K$ is an 
asymptotic field
and $L|K$ is an extension of valued differential fields}.  We shall prove:

\begin{prop}\label{Algebraic-Extensions-Asymptotic}
If $L|K$ is algebraic, then $L$ is an asymptotic field.
\end{prop}



\begin{lemma}\label{trace and norm}
Suppose that $K$ is henselian and $L|K$ is of finite degree. 
Assume also that for every $f\preceq 1$ in $L$ there exists 
$a\preceq 1$ in $K$ such that
\begin{enumerate}
\item $f'\preceq a'$, and
\item if $f'\asymp a'$ and $f\prec 1$, then $a\prec 1$.
\end{enumerate}
Then $L$ is an asymptotic field.
\end{lemma}
\begin{proof}
We verify that $L$ satisfies condition (4) of 
Proposition~\ref{CharacterizationAsymptoticFields}. For this, 
let $f,g\in L^\times$ with $f\preceq 1$ and $g\nasymp 1$. Let $a\preceq 1$ in $K$
satisfy (1) and (2). Put $b:=\operatorname{N}_{L|K}(g)\in K^\times$; 
then $b\nasymp 1$ and $b^\dagger\preceq g^\dagger$ by a result at the end of
Section~\ref{Valdifcon}. Hence if $f\asymp 1$, 
then by (1): 
$f'\preceq a'\preceq b^\dagger\preceq g^\dagger$. 
If $f \prec 1$, then we similarly get, using (2), that 
$f' \prec a'\preceq b^\dagger\preceq g^\dagger$, or $a\prec 1$ and 
$f'\asymp a'\prec b^\dagger\preceq g^\dagger$.
\end{proof}

\begin{lemma}\label{Residue-Field-Extension-Asymptotic}
Suppose that $K$ is henselian and $L|K$ is of finite degree, such that
$[L:K]=\bigl[\res(L):\res(K)\bigr]=n>1$. Then $L$ is an asymptotic field.
\end{lemma}
\begin{proof}
Take $y\asymp 1$ in $L$ such that $\res(L)=\res(K)[\bar{y}]$, where
$\bar{y}$ is the residue class of~$y$ in $\res(L)$. Let 
$a_0,\dots,a_{n-1}\preceq 1$ in $K$ be such that
$$P(Y)=Y^n+a_{n-1}Y^{n-1}+\cdots +a_1Y+a_0\in K[Y]$$ is the
minimum polynomial of $y$ over $K$, so its reduction $\bar{P}(Y)$ in
$\res(K)[Y]$ is the minimum polynomial of $\bar{y}$ over $\res(K)$; 
in particular $P'(y)\asymp 1$. Moreover, $P'(y)y'=-\sum_{i=0}^{n-1}a_i'y^i$, 
hence $y' \asymp a_{i_0}'$ with $i_0\in\{0,\dots,n-1\}$. Let 
$f\preceq 1$ in $L$. Then we have $f_0,\dots,f_{n-1}\preceq 1$ in $K$ such that
$$f=f_0+f_1y+\cdots+f_{n-1}y^{n-1}.$$
Then
$$f' = 
\sum_{i=0}^{n-1} f_i'y^i + \left(\sum_{j=1}^{n-1} jf_jy^{j-1}\right)y'$$
and hence 
$$v(f') \geq \gamma := \min\left\{\min_{0\leq i<n} v(f_i'), 
\min_{0<j<n} v(f_j)+v(a_{i_0}')\right\}.$$
We now define an element $a\in  \mathcal{O}$ as follows: If 
$\gamma=\min_{0\leq i<n} v(f_i')$, then $a:=f_{i_1}$ where 
$0\leq i_1<n$ and $v(f_{i_1}')=\gamma$;
if $\gamma<\min_{0\leq i<n} v(f_i')$, then $a:=a_{i_0}$. 
Then $a$ satisfies conditions (1) and (2) of Lemma~\ref{trace and norm}, 
so $L$ is an asymptotic field.
\end{proof}

\noindent
The next lemma is a variant of Lemma~3.3 in \cite{AvdD2}:

\begin{lemma}\label{Lemma34}
Suppose $\res(K) = \res(L)$,
$T\supseteq K^\times$ is a subgroup of
$L^{\times}$ such that $L=K(T)$ \rom{(}as fields\rom{)}, each element of 
$K[T]\setminus \{0\}$ has the
form $t_1+\dots+t_k$ with $k\ge 1$, $t_1,\dots,t_k\in T$ and
$t_1 \succ t_i$ for $2\le i \le k$, and for all 
$a,b\in T$,
\begin{align}
  a,b\prec 1 
&\quad\Longrightarrow\quad a' \prec b^\dagger \label{Eq1} \\
  a\asymp 1,\ b\prec 1 
&\quad\Longrightarrow\quad a' \preceq b^\dagger. \label{Eq2}
\end{align}
Then $L$ is an asymptotic field.
\end{lemma}
\begin{proof}
Let $g\in L^\times$, $g\prec 1$. Then by the assumptions on $T$ we have
$$g=b\cdot\frac{1+\sum_{i=1}^m a_i}{1+\sum_{j=1}^n b_j}$$
where $b\in T$, and $a_i,b_j\in T$ with $a_i,b_j\prec 1$, 
for $1\leq i\leq m$, $1\leq j\leq n$. So $g\asymp b\prec 1$; we claim that 
$g'\asymp b'$. For this, note that $b^\dagger \ne 0$ by \eqref{Eq1}, so
$$g^\dagger = b^\dagger 
\left(1+\frac{\sum_{i=1}^m a_i'/b^\dagger}{1+\sum_{i=1}^m a_i}-
\frac{\sum_{j=1}^n b_j'/b^\dagger}{1+\sum_{j=1}^n b_j}\right).$$
By \eqref{Eq1} we have $a_i'/b^\dagger, b_j'/b^\dagger\prec 1$ for 
$1\leq i\leq m$, $1\leq j\leq n$. Therefore $g^\dagger \asymp b^\dagger$ 
and thus $g'\asymp b'$ as claimed.

Now if $f,g\in L^\times$ satisfy $f,g\prec 1$, then this claim and 
\eqref{Eq1} yield $f' \prec g^\dagger$. Suppose $f,g\in L^\times$ with
$f\asymp 1$ and $g\prec 1$. Take $b\in T$ with $b\asymp g$ and 
$b'\asymp g'$ as above. Since $\res(K)=\res(L)$ we have
$f=a+h$ with $a\in K$, $a\asymp 1$ and
$h\in L$, $h\prec 1$. By
the claim above we find $t\in T\cup\{0\}$ with $h\asymp t$ and $h'\asymp t'$. 
Now $a' \preceq b^\dagger$
by \eqref{Eq2} and $t'\prec b^\dagger$ by \eqref{Eq1}, so
$f'=a'+h'\preceq b^\dagger\asymp g^\dagger$. The implication 
(4)~$\Rightarrow$~(1) of Proposition~\ref{CharacterizationAsymptoticFields} 
now yields that $L$ is an asymptotic field.
\end{proof}

\noindent
The same proof also yields Lemma 3.3 in \cite{AvdD2}:

\begin{lemma}\label{Lemma3.3} 
Suppose $K$ is pre-$\d$-valued, $\res(K) = \res(L)$,
$T\supseteq K^\times$ is a subgroup of
$L^{\times}$ with $L=K(T)$, each element of 
$K[T]\setminus \{0\}$ has the
form $t_1+\dots+t_k$ with $k\ge 1$, $t_1,\dots,t_k\in T$ and
$t_1 \succ t_i$ for $2\le i \le k$, and for all 
$a,b\in T$,
$$ a\preceq 1,\ b\prec 1
\quad\Longrightarrow\quad a' \prec b^\dagger. \label{Eq3}
$$
Then $L$ is a pre-$\d$-valued field. 
\end{lemma}

\noindent
We shall need a version of the above for pre-$H$-fields:

\begin{lemma}\label{lem3.3pre} Assume in addition to the hypotheses of Lemma~\ref{Lemma3.3}
that $K$ and~$L$ are equipped with field orderings making $K$ a pre-$H$-field and $L$ an ordered field extension of $K$, such that $\mathcal{O}_L$ is convex with respect to the ordering of $L$, and for all $a\in T$, if
$a\succ 1$, then $a^\dagger >0$. Then $L$ is a pre-$H$-field.
\end{lemma}
\begin{proof} Let $f\in L$, $f> \mathcal{O}_L$; we need to show that $f'>0$. Take $a\in T$ such that~$a\asymp f$. Then $\frac{f}{a}-\frac{f'}{a'}\prec 1$ by 
Lemma~\ref{lem:char pdv}, and $\frac{f}{a}\asymp 1$. If $a>0$, then 
this gives $\frac{f'}{a'}>0$, so $f'>0$, and if $a<0$, we get likewise
$\frac{f'}{a'}<0$, so again $f'>0$.
\end{proof}




\begin{lemma}\label{Purely ramified-Asymptotic}
Let $p$ be a prime number, and suppose that $L=K\bigl(u^{1/p}\bigr)$
where $u\in K^{\times}$ with $vu\notin p\Gamma$.
Then $L$ is an asymptotic field.
\end{lemma}
\begin{proof}
Let $u^{i/p} := (u^{1/p})^i$ for $i\in\Z$, and put 
$T:=\bigcup_{i=0}^{p-1} K^\times u^{i/p}$. Then $T$ is a multiplicative 
subgroup of $L^\times$. By Lemma~\ref{lem:pth root},  
$\res(K)=\res(L)$, and each element of $L$ has the form $t_1+\cdots+t_k$ with 
$t_1,\dots,t_k\in T$, $t_1\succ \cdots \succ t_k$. Now let $a,b\in T$; 
then $a^p\in K^\times$ and $(a^p)^\dagger=pa^\dagger\asymp a^\dagger$, 
and similarly $b^p\in K^\times$, $(b^p)^\dagger\asymp b^\dagger$. Hence 
if $a,b\prec 1$, then 
$v(a')=va+v\big((a^p)^\dagger\big)=\frac{1}{p}\alpha+\psi(\alpha)$ and 
$v(b^\dagger)=v\big((b^p)^\dagger)=\psi(\beta)$ where 
$\alpha:=pva,\beta:=pvb\in\Gamma$, and in the asymptotic couple 
$(\Q\Gamma,\psi)$ we have $\frac{1}{p}\alpha+\psi(\alpha)=
(\id+\psi)\big(\frac{1}{p}\alpha\big)>\psi(\beta)$, so $a' \prec b^\dagger$. 
If $a\asymp 1 \succ b$, then 
$a'\asymp (a^p)' \preceq (b^p)^\dagger\asymp b^\dagger$. 
Hence $L$ is an asymptotic field by Lemma~\ref{Lemma34}.
\end{proof}

\begin{proof}[Proof of Proposition~\ref{Algebraic-Extensions-Asymptotic}] 
We assume that $L|K$ is algebraic. We need to show that then $L$ is an
asymptotic field. The property of
being an asymptotic field is inherited by valued differential subfields, so
we can assume that $L$ is an algebraic closure of $K$. Next, by  
Lemma~\ref{pa5}, we can arrange that $K$ is henselian. We then reach $L$ in two steps. In the first step we pass from~$K$ to its maximal unramified extension
$K^{\text{unr}}$ inside $L$. Then $K^{\text{unr}}$ is asymptotic by 
Lemma~\ref{Residue-Field-Extension-Asymptotic}. In the second step we obtain $L$ as a
purely ramified extension of~$K^{\text{unr}}$ (Proposition~\ref{prop:ramified}), and now Lemma~\ref{Purely ramified-Asymptotic}  applies. 
\end{proof}

\noindent
%Lemma~\ref{PresInf-Lemma2},~(1), 
Note: if $K$ has small derivation and $L|K$ is algebraic, then 
$L$ has small derivation, by Proposition~\ref{Algebraic-Extensions}. Also, if $K$ is of $H$-type and 
$L|K$ is 
algebraic, then $L$ is of $H$-type. The above material on algebraic 
extensions is a mild generalization of Section~3 in \cite{AvdD2}. That section also contains some easy variants of Proposition~\ref{Algebraic-Extensions-Asymptotic}, which we shall 
use freely when convenient:
\begin{enumerate}
\item if $K$ is pre-$\d$-valued and $L|K$ is algebraic, 
then $L$ is pre-$\d$-valued; 
\item if $K$ is $\d$-valued and $L$ is an algebraic closure of $K$,
then $L$ is $\d$-valued;
\item if $K$ is an $H$-field and $L$ is a real closure of $K$, then the ordered
valued dif\-fer\-en\-tial field $L$ is an $H$-field.
\end{enumerate}

\subsection*{An application} {\em In this subsection $K$ is an ungrounded $H$-asymptotic field, and $\Gamma=v(K^\times)\ne \{0\}$}. For use in Chapter~\ref{evq} we extend slightly some results from 
Section~\ref{Applicationtodifferentialpolynomials} by dropping the assumption that $\Gamma$ is divisible:
 
%\noindent
%For use in Chapter~ \ref{evq} we also observe that some %results from 
%Section~\ref{Applicationtodifferentialpolynomials} go 
%through under a 
%weaker assumption than divisibility of $\Gamma=v(K^\times)$:

\begin{cor}\label{betterdifpol} 
%Assume $K$ is of $H$-type and 
%$\Gamma\ne \{0\}$ has no smallest positive element. 
Let $P\in K\{Y\}^{\ne}$
have order $r$. Then Corollary~\ref{ps6e}
goes through if we drop ``with the intermediate value property''.
Also Corollary~\ref{ps6c} goes through, for a unique tuple
$(\alpha, d, d_0, e_1,\dots, e_{r-1})$. In particular, there exists $\beta\in \Gamma^{<}$ such that $P(y)\ne 0$ for all $y\in K$ with $\beta < vy < 0$.
\end{cor}
\begin{proof} This follows by applying Corollaries~\ref{ps6e} and~\ref{ps6c} to the algebraic closure~$K^{\a}$ of $K$, taking into account
that the value group of $K^{\a}$ is $\Q\Gamma$, that 
$\Gamma^{<}$ is cofinal in $(\Q\Gamma)^{<}$, that $\Psi_{K^{\a}}=\Psi$, and that the $\chi$-map
of the $H$-asymptotic couple~$(\Q\Gamma, \psi)$ extends the
$\chi$-map of $(\Gamma, \psi)$. The ``uniqueness'' uses Lemma~\ref{evtcon}.
\end{proof} 

\noindent
Here is a striking consequence that will not
be needed, since in Chapter~\ref{ch:The Dominant Part and the Newton Polynomial} we prove more precise results for so-called $\upo$-free $K$ (using heavier machinery):



\begin{cor}\label{betterdifpolcor} Suppose $K$ is existentially closed in some grounded $H$-asymp\-to\-tic field extension of $K$. Then
Corollary~\ref{ps6c} holds with all $e_i=0$, for every~$P$ in~$K\{Y\}^{\ne}$ of order $r$. \rm{(See end of \ref{sec:ultra products} for ``existentially closed''.)}
\end{cor}
\begin{proof} The assumption on $K$ 
yields an elementary extension of $K$ with an element~$y\succ 1$ such that $K\<y\>$
has $\Cl(y)$ as its smallest comparability class. Let $P\in K\{Y\}^{\ne}$ have order $r$, let $\beta$ and $(\alpha, d, d_0, e_1,\dots, e_{r-1})$ be as in Corollary~\ref{ps6c}, and
suppose towards a contradiction that some $e_i\ne 0$. 
We have $\beta < vy <0$, and taking $a\in K^\times$ with
$va=\alpha$ we get an element $f=P(y)/ay^{d_0}(y^\dagger)^d$
of $K\<y\>^\times$ such that
$vf=-\sum_{i=1}^{r-1}e_i\chi^i(vy)$,
so $f\not\asymp 1$ and  $\Cl(f) < \Cl(y)$, a contradiction. 
\end{proof} 

\noindent
If $K$ is a directed union of grounded asymptotic subfields, then $K$ is existentially closed in some grounded $H$-asymptotic field extension of $K$; see~\ref{cor:ec in ext}. Note that
$K=\T$ and $K=\T_{\log}$ are such directed unions. 





==> mt-9-7.tex <==




\section{Immediate Extensions of Asymptotic Fields}
\label{ImmExtAs}

\noindent
We begin with recording analogues for asymptotic fields of the
results on maximal immediate extensions 
from Chapter~\ref{ch:valueddifferential}.
Next we prove
some easy technical facts that are often needed. We also show how to construct immediate extensions by (un)coarsening, and we finish
with constructing fluent completions.

\subsection*{Asymptotically maximal immediate extensions} 
{\em In this subsection $K$ is an asympotic field with small derivation and differential residue field $\k$ such that the derivation on $\k$ is nontrivial}.
This is the same condition as in Section~\ref{sec:cimex}. 
Recall that the derivation of any immediate asymptotic extension of
$K$ is small. 
Here are two easy consequences of Section~\ref{sec:cimex} and Lemmas~\ref{ndsupPsi=0} and ~\ref{impreservesas}:

\begin{cor}\label{cor1asdiftrzda} If $K$ is asymptotically maximal, then $K$ is spherically complete.
\end{cor}

\begin{cor}\label{cor2asdiftrzda} $K$ has an immediate asymptotic 
extension that is spherically complete. 
\end{cor}


\subsection*{Easy technical lemmas} {\em In this 
subsection $F$ is a valued differential field with a subfield $K$
that is asymptotic in $F$, and with $L$ as an intermediate field, so that
$K\subseteq L \subseteq F$}. Note that then $L$ is asymptotic in $F$
if for each $f\in L^\times$ with $f\prec 1$ there is $a\in K^\times$ such that
$f\asymp a$ and $f'\asymp a'$.


\begin{lemma}\label{pa3} 
Suppose $L|K$ is immediate and for all $a\in K^\times$ and
$f\in L$,
\begin{equation}\label{ImmediateEq}
\bigl(a\prec 1, f\prec
1\bigr)\quad\Longrightarrow\quad f' \prec a^\dagger.
\end{equation}
Then $L$ is asymptotic in $F$.
\end{lemma}
\begin{proof}
Let $a\in K^\times$, $h\in L^\times$ with $h\prec a\prec 1$; we claim
that $h'\prec a'$. To see this, set $g:= h/a\in L^\times$, so
$g \prec 1$, and by
\eqref{ImmediateEq}, 
$\frac{h}{a}-\frac{h'}{a'}=-\frac{g'a}{a'}\prec 1$, hence $h'/a'\prec
1$ and thus $h'\prec a'$.
Let now $f\in L^\times$, $f\prec 1$. Take $a\in K$
with $f\sim a$, so
$h=f-a \prec a\prec 1$. 
Then $h'\prec a'$, so $f'=a'+h'\asymp a'$ as required.
\end{proof}

\begin{lemma}\label{pa4}
Suppose $L|K$ is immediate, $U\supseteq K$ is a
$K$-linear subspace of $L$ with 
$L=\bigl\{u/w : u,w\in U, w\neq 0\bigr\}$, and for all
$a\in K^\times$ and  $u\in U$,
\begin{align}
\bigl(a\prec 1, u\prec 1\bigr)
\quad\Longrightarrow\quad u'\prec a^\dagger, \label{ImmediateEq1}\\
\bigl(a\prec 1, u\asymp 1\bigr)
\quad\Longrightarrow\quad u' \preceq a^\dagger. \label{ImmediateEq2}
\end{align}
Then $L$ is asymptotic in $F$.
\end{lemma}
\begin{proof}
We shall verify \eqref{ImmediateEq}. Let $f\in L$, $f\prec 1$. Then
$f=u/w$ with $u,w\in U$ and $w\neq 0$. After dividing $u$ and
$w$ by an element of $K$ asymptotic to $w$, we may assume $u\asymp f$
and $w\asymp 1$. We have $f'=u'/w -fw'/w$ with $u'/w \asymp u' \prec
a^\dagger$ and $fw'/w \asymp fw' \prec  a^\dagger$ for all
$a\in K^\times$ with $a\prec 1$, by \eqref{ImmediateEq1} and
\eqref{ImmediateEq2}, respectively; hence $f'\prec a^\dagger$ for all
such $a$. 
\end{proof}



\subsection*{Immediate extensions by coarsening} Let $K$ be an asymptotic field and $\Delta$ a convex subgroup
of $\Gamma=v(K^\times)$, giving rise to the coarsened valuation
$$\dot{v}\colon K^\times \to \dot{\Gamma}=\Gamma/\Delta$$ 
with residue field $\dot{K}=\dot{\cal{O}}/\dot{\smallo}$. 
Let $(L, \dot{v})$ be an immediate valued field
extension of~$(K, \dot{v})$, and denote its residue field by 
$\dot{L}$, so $\dot{L}=\dot{K}$ after the usual identification.
In Section~\ref{sec:decomposition} we extended the 
valuation $v$ on $K$ to a valuation
$v\colon L^\times \to \Gamma$
such that if $f\in L^\times$ and
$f=gu$ with $g\in K^\times$ and $u\in L^\times$, $\dot{v}(u)=0$, then
$v(f)=v(g)+v(\dot{u})$. By Lemma~\ref{immcoarse}, $L$ with $v$ is an immediate
valued field extension of the valued field~$K$, and its coarsening by
$\Delta$ is the $(L,\dot{v})$ we started with. 
Let $L$ also be equipped with a derivation $\der$ making 
$(L, \dot{v})$ an asymptotic extension of
$(K, \dot{v})$. Then:

\begin{lemma} 
\label{Un-coarsen} With the above valuation $v$ on $L$, the 
valued differential field 
$L$ is a $\Delta$-immediate asymptotic extension of $K$. 
\end{lemma}   
\begin{proof} Let $f\in L$ and $\dot{v}f>0$; we claim that 
then $v(f') > \Psi$.
To see this, note that $f=g(1+h)$ with $g\in K$, $h\in L$, and $\dot{v}h>0$,
since $(L, \dot{v})$ is an immediate extension of $(K, \dot{v})$. Then
$vh>0$, so $vg=vf> \Delta$. Now 
$$f'=g'(1+h)+ gh',\ \text{ with }\ v(g'(1+h))=vg' > \Psi.$$ 
Also, $0< \dot{v}f = \dot{v}g$ gives
$\dot{v}(f')=\dot{v}(g')= v(g')+\Delta$,
so $v(f')=v(g') + \delta$ with $\delta\in \Delta$, hence $vf' > \Psi + \delta$.
With $h$ instead of $f$ this gives $vh' > \Psi + \delta$ for some 
$\delta\in \Delta$, so $v(gh')> \Psi$ in view of $vg> \Delta$. Thus
$v(f') > \Psi$, as claimed.

Now $(L,v)$ is an immediate 
valued field extension of $K$ by Lemma~\ref{immcoarse}. Using this fact, 
the claim above, and Lemma~\ref{pa3} we show that $(L,v)$ is an
asymptotic field. 
Let $f\in L$ with $vf>0$; it is enough to show
that then $v(f') > \Psi$. As before, $f=g(1+h)$ with $g\in K$, $h\in L$, and
$\dot{v}h>0$. Then $vg>0$ and $f'=g'(1+h)+ gh'$ with $v(g'(1+h))=vg' > \Psi$.
By the claim above applied to $h$ instead of $f$ we have $v(h')>\Psi$,
so $v(gh') \ge v(h')> \Psi$. Thus $v(f') > \Psi$.
%, as desired.
\end{proof}

\subsection*{Fluency and $\Delta$-immediate extensions} 
Let $K$ be an asymptotic field, $\Delta$ a convex subgroup of $\Gamma$, and 
$\dot{v}=v_{\Delta}$ the coarsening of $v$ by $\Delta$. By 
Lemma~\ref{Un-coarsen} any proper immediate asymptotic extension of the asymptotic field $(K, \dot{v})$ yields by ``uncoarsening'' a proper
$\Delta$-immediate asymptotic extension of $K$.

\begin{lemma}\label{flasy} Assume $\Delta\ne \{0\}$. Then the following are equivalent: \begin{enumerate}
\item $K$ has no proper $\Delta$-immediate asymptotic extension;
\item every $\Delta$-fluent pc-sequence in $K$ pseudoconverges in $K$.
\end{enumerate}
\end{lemma}
\begin{proof} The direction $(2)\Rightarrow (1)$ follows from 
Corollary~\ref{maxdeltafluent}. As to $(1)\Rightarrow (2)$, we prove its 
contrapositive. Assume there exists a divergent $\Delta$-fluent pc-sequence in~$K$.
Take $\delta\in \Delta^{\ne}$ and $\phi\in K^\times$ with $v\phi=\psi(\delta)$. Then $\psi^{\phi}(\delta)=0$, so $0\in \psi^{\phi}(\Delta^{\ne}) \cap \Delta$. 
Replacing $K$ by its compositional conjugate $K^{\phi}$ 
we arrange $0\in \psi(\Delta^{\ne})\cap \Delta$, so $K$ has small derivation
and $\psi(\Delta^{\ne})\subseteq \Delta$. Then
$(K, \dot{v})$ has small derivation, and the derivation of the differential
residue field of $(K, \dot{v})$ is nontrivial. Hence $(K, \dot{v})$ has a proper immediate 
asymptotic extension by Corollary~\ref{cor1asdiftrzda}, and this yields a proper $\Delta$-immediate asymptotic extension of $K$ by Lemma~\ref{Un-coarsen}.
\end{proof}

\noindent
By Zorn there exists a $\Delta$-immediate asymptotic
extension of $K$ that has no proper $\Delta$-immediate asymptotic
extension. Such an extension of $K$ is called
a {\em maximal $\Delta$-immediate asymptotic extension\/} of $K$.
Let $K(\Delta)$ be a maximal $\Delta$-immediate asymptotic extension
of $K$. By Lemma~\ref{flasy}, if $\Delta\ne \{0\}$, then $K(\Delta)$ is also a maximal $\Delta$-immediate extension of $K$ as a valued field, and 
so its $\Delta$-coarsening~$(K, \dot{v})$ is henselian. Here is a weak ``asymptotic'' version of Proposition~\ref{fluentcompletion}:
  

\index{maximal!$\Delta$-immediate asymptotic extension}

\begin{prop}\label{asfl} Let $K$ be an asymptotic field such that $\Gamma\ne \{0\}$ and $[\Gamma^{\ne}]$ has no least element.
Then $K$ has an immediate asymptotic extension which, as a valued field extension of $K$, is a fluent completion of $K$.
\end{prop}
\begin{proof} We follow the construction in the proof of Proposition~\ref{fluentcompletion}. Fix a decreasing coinitial sequence $(\Delta_{\alpha})$
of nontrivial convex subgroups of~$\Gamma$ indexed by the ordinals
$\alpha< \lambda$ for some infinite limit ordinal $\lambda$. For each $\alpha$ we pick a maximal $\Delta_{\alpha}$-immediate
asymptotic extension $K(\Delta_{\alpha})$ of $K$. We arrange this so that
$K(\Delta_{\alpha})$ is a valued differential subfield of 
$K(\Delta_{\beta})$ whenever
$\alpha < \beta < \lambda$. Put 
$$  K^{\operatorname{f}}\ :=\  \bigcup_{\alpha< \lambda} K(\Delta_{\alpha}).$$
Then  $K^{\operatorname{f}}$ is an asymptotic extension of $K$, and $K^{\operatorname{f}}$ as a valued field extension of~$K$ is a semifluent completion of $K$ as defined in the proof of Proposition~\ref{fluentcompletion}. Iterating as in that proof the construction
$K \leadsto K^{\operatorname{f}}$ we eventually arrive at an asymptotic extension of $K$ that is also a fluent completion of $K$.      
\end{proof}



























==> mt-9-8.tex <==

\section{Liouville Extensions}
\label{Solving Homogeneous First-Order Equations}

\noindent
In this section we adjoin integrals (solutions $y=\int s$ of 
equations
$y'=s$) as well as exponential integrals (solutions $y=\exp(\int s)$ of equations 
$y^\dagger =s$).
The expressions~$\int s$ and $\exp(\int s)$ here are purely suggestive and 
we attach no formal meaning to their use.
We begin with mild variants of adjunctions performed in \cite{AvdD2}.

\subsection*{Variants of earlier results on Liouville extensions} For most 
of the lemmas below we try to give the main idea so that the reader can reconstruct the proof. In contrast to Section 4 in \cite{AvdD2} we consider here only asymptotic fields of $H$-type. 

\begin{lemma}\label{extensionpdvfields1}
Let $K$ be an $H$-asymptotic field, and let $s\in K$ be such that $vs$ is
a gap in $K$.
Then $K$ has an $H$-asymptotic extension $K(y)$ with $y\prec 1$ and 
$y'=s$ such that 
for any $H$-asymptotic extension $L$ of $K$ and $z\in L$ with $z\prec 1$
and $z'=s$ there is a unique $K$-embedding $K(y) \to L$ sending
$y$ to $z$.
%Let $L=K(y)$ be a field extension of $K$ 
%with $y$ transcendental over
%$K$. Give $L$ the unique derivation extending that of $K$ 
%with $y'=s$. Then there is exactly one valuation on $L$
%extending the one on $K$ and making $L$ an $H$-asymptotic 
%field with $y \prec 1$.
\end{lemma}
\begin{proof} Suppose $K(y)$ is an $H$-asymptotic extension of $K$
with $y\prec 1$ and $y'=s$.  
Then for $\alpha:= vy$ we have $\alpha>0$ and $\alpha'=vs$, so by Lemma~\ref{extension1} and its proof
we have $0 < n\alpha < \Gamma^{>}$ for all $n\ge 1$. Thus $y$ is transcendental over $K$ and the asymptotic couple
of $K(y)$ is just the $H$-asymptotic couple
$(\Gamma + \Z\alpha, \psi^{\alpha})$ with $\alpha'=\beta$ from 
Lemma~\ref{extension1}, with $\beta:=vs$. Thus $K(y)$ has the universal property
stated in the present lemma. These arguments also indicate how to construct
such an extension $K(y)$. See Lemma~4.1 in \cite{AvdD2}
for details. (In the third line of the proof of that lemma, ``$\Gamma^{<0} < nv(y) < 0$'' should be 
``$0<nv(y) < \Gamma^{>0}$''.)
\end{proof}

\noindent
Let $K$, $s$, and $K(y)$ be as in Lemma~\ref{extensionpdvfields1}. Then $K$ is pre-$\d$-valued, by Lemma~\ref{asy1} and 
Corollary~\ref{asymp-predif}, and $\res\big(K(y)\big)=\res(K)$ by Lemma~\ref{lem:lift value group ext}. The proof of Lemma~4.1 
in~\cite{AvdD2} and subsequent comments also yield
the following: \begin{enumerate}
\item $K(y)$ is pre-$\d$-valued and grounded, by (\ref{eq:Psialpha});
\item if $K$ is $\d$-valued, then so is $K(y)$, and $C_{K(y)}=C$;
\item if $K$ is equipped with an ordering making it a pre-$H$-field, then there is a unique ordering on $K(y)$ making it a pre-$H$-field extension of $K$.  
\end{enumerate}
What if we replace $y\prec 1$ in 
Lemma~\ref{extensionpdvfields1} by $y\succ 1$? For a reasonably concise
answer we need to restrict ourselves to $\d$-valued $K$. This answer is indicated in remark (2) after the proof of Lemma~4.1 in \cite{AvdD2}:  


\begin{lemma}\label{variant41}
Let $K$ be a $\d$-valued field of $H$-type, and let $s\in K$ be such that $vs$ is a gap in $K$.
Then $K$ has a $\d$-valued extension $K(y)$ of $H$-type with $y\succ 1$ and 
$y'=s$ such that 
for any $H$-asymptotic extension $L$ of $K$ and $z\in L$ with $z\succ 1$
and $z'=s$ there is a unique $K$-embedding $K(y) \to L$ sending
$y$ to $z$.
\end{lemma}

\noindent
Let $K$ and $K(y)$ be as in Lemma~\ref{variant41}, and set $\alpha:= vy$.
Then $\alpha< 0$ and $\alpha'=vs$ and so $\Gamma^{<} < n\alpha < 0$ for all $n\ge 1$ by the remark following (\ref{eq:Psialpha}). Thus the value group
of $K(y)$ is $\Gamma + \Z\alpha$. 
Taking into account also remark (7) after the proof of Lemma~4.1 in \cite{AvdD2}, we have: \begin{enumerate}
\item $C_{K(y)}=C$ and $K(y)$ is grounded, by (\ref{eq:Psialpha}); 
\item if $K$ is equipped with an ordering making it an $H$-field, then there is a unique ordering on $K(y)$ making it an $H$-field extension of 
$K$.  
\end{enumerate} 
Next a variant of Lemma~4.2 in \cite{AvdD2}:

\begin{lemma}\label{pre-extas2}
Let $K$ be a pre-$\d$-valued field of $H$-type and let $s\in K$ be such that $vs = \max \Psi$. Then $K$ has a pre-$\d$-valued extension $K(y)$ of $H$-type with $y'=s$ such that 
for any pre-$\d$-valued extension $L$ of $K$ of $H$-type and $z\in L$ with
$z'=s$ there is a unique $K$-embedding $K(y) \to L$ sending
$y$ to $z$.
\end{lemma}
\begin{proof} Suppose $K(y)$ is a pre-$\d$-valued extension of $K$
of $H$-type such that~$y'=s$. The assumption that $K(y)$ is 
pre-$\d$-valued gives $\alpha:=vy< 0$, and then the $H$-type assumption
together with $\alpha^\dagger=vs-\alpha > \Psi$ gives $\Gamma^{<} < n\alpha < 0$ for all 
$n\ge 1$.
Thus~$y$ is transcendental over $K$, and the asymptotic couple
of~$K(y)$ is $(\Gamma + \Z\alpha, \psi^{\alpha})$ with
$\alpha'=vs$, which is just the $H$-asymptotic couple from Lemma~\ref{extas2} for $\beta=vs$. This makes it clear why $K(y)$ has the universal property
stated in the lemma, and it also indicates a way to construct
such an extension~$K(y)$. We refer to Lemma~4.2 in \cite{AvdD2} for further details.    
\end{proof}

\noindent
Let $K(y)$ be as in Lemma~\ref{pre-extas2} and set $\alpha:= vy$. By Lemma~\ref{lem:lift value group ext} we have 
$\res\big( K(y)\big)=\res(K)$. 
In view of the remarks following the proof of Lemma~\ref{extas2} we have 
$\Psi_{K(y)}=\Psi\cup\{\alpha^\dagger\}$ with 
$\Psi < \alpha^\dagger$. By remarks after Lemma 4.2 in
\cite{AvdD2}: \begin{enumerate}
\item if $K$ is $\d$-valued, then so is $K(y)$, and $C_{K(y)}=C$;
\item if $K$ is equipped with an ordering making it a pre-$H$-field, then there is a unique ordering on $K(y)$ making it a pre-$H$-field extension
of $K$.
\end{enumerate}    





\begin{lemma}\label{var43} Let $K$ be a henselian $H$-asymptotic field, 
and suppose
$s\in K$ is such that $vs\in (\Gamma^{>})'$, $s\ne a'$ for all $a\in \smallo$, 
and $$S\ :=\ \big\{v(s-a'):\ a\in \smallo\big\}$$ has no largest element. 
Let $L=K(y)$ be a field extension of
$K$ with $y$ transcendental over $K$, and let $L$ be equipped with the 
unique derivation extending the derivation of $K$ such that $y'=s$. Then there is a unique valuation of $L$ that makes it an asymptotic field
extension of~$K$ with $y\not\asymp 1$. With this valuation $L$ is an
immediate extension of $K$ with $y\prec 1$.
\end{lemma}
\begin{proof} We indicate the changes to be made in the proof 
of Proposition~4.3 in~\cite{AvdD2}. Claim 1 in that proof 
holds by our assumptions. Replace the term ``pre-differential-valued'' 
in that proof by ``asymptotic''. To obtain the analogue of Claim 3
in that proof, verify the hypotheses of Lemma~\ref{pa4} with $F=L$ and $U=K[y]$,
instead of the hypotheses of Lemma 3.1 of \cite{AvdD2}.  
\end{proof}

\noindent
If $K$ is $\d$-valued, then the assumption in 
Lemma~\ref{var43} that $S$ has no largest element is automatically satisfied. 
We shall also use a variant of Lemma~5.1 in \cite{AvdD2}:

\begin{lemma}\label{var51} Let $K$ be a henselian $H$-asymptotic field, and
suppose $s\in K$ is such that $s\ne a'$ and 
$v(s-a')< (\Gamma^{>})'$ for all $a\in K$, 
and 
$$S\ :=\  \big\{v(s-a'):\ a\in K\big\}$$ 
has no largest element. Let $L=K(y)$ be a field extension of
$K$ with $y$ transcendental over $K$, and let $L$ be equipped with the 
unique derivation extending the derivation of $K$ such that $y'=s$.

Then there is a unique valuation of $L$ making it an asymptotic field
extension of $K$. With this valuation $L$ is an
immediate extension of $K$ with $y\succ 1$.
\end{lemma}
\begin{proof} Note that $vs\in S$. Since $S$ has no largest element, each 
$\alpha\in S$ satisfies
$\alpha < \gamma$ for some $\gamma\in \Psi$. Set 
$\kappa= \operatorname{cf}(S)$ and take a sequence $(a_{\lambda})_{\lambda < \kappa}$ in $K$, such that $v(s-a_{\lambda}')$ is strictly increasing and 
cofinal in $S$ as a function of $\lambda$, and $v(s-a_{\lambda}')> vs$ for all
$\lambda$. As in the proof of Lemma 5.1 in \cite{AvdD2} one shows that 
$(a_{\lambda})$ is a divergent pc-sequence in $K$ with $a_{\lambda}-a_{\mu}\succ 1$
for all $\lambda < \mu < \kappa$. It follows that $a_{\lambda} \preceq 1$ for at 
most one $\lambda$, and so we can arrange that $a_{\lambda} \succ 1$
for all $\lambda$. The rest of the proof follows that of
of Lemma 5.1 in \cite{AvdD2}, with the term ``pre-differential-valued'' 
replaced by
``asymptotic'' and with an appeal to Lemma~\ref{pa4} for $F=L$ and $U=K[y]$ 
to verify that the valued differential field $K(y)$ is asymptotic.
\end{proof} 
 
 \noindent
The following observation, a variant of Remark~(2) following \cite[Lemma~5.1]{AvdD2}, is relevant in connection with
Lemma~\ref{var51}, and will be used in Section~\ref{sec:extkx}.

\begin{lemma}\label{lem:remark5.1(2)}
Let $K$ be a pre-$\d$-valued field, $s\in K$, and suppose
$$S\ :=\ \big\{ v(s-a'): a\in K\big\}\ \subseteq\ 
\Gamma_\infty$$
has a largest element $\beta$. Then $\beta\notin (\Gamma^{\neq})'$.
\end{lemma}
\begin{proof}
Take $a\in K$ and $b\in K^\times$, $b\nasymp 1$, such that 
$\beta=v(s-a')=v(b')$. 
Next, take $u\in K$ with $u\asymp 1$ and $s-a'=ub'$. Then 
$u'\prec b^\dagger$ since $K$ is pre-$\d$-valued, hence
$s-(a+ub)'=-u'b\prec b'$, contradicting the maximality of 
$\beta$.
\end{proof}

 
 
\noindent
By alternating the passage to a henselization with the extension procedures 
of Lemmas~\ref{var43} and ~\ref{var51} we obtain the following:

\begin{prop}\label{asintint} Let $K$ be a $\d$-valued field of $H$-type with 
asymptotic integration. Then $K$ has an immediate asymptotic extension
$K(\int)$ such that:  \begin{enumerate}
\item $K(\int)$ is henselian and closed under integration;
\item $K(\int)$ embeds over $K$ into any henselian $\d$-valued 
field extension of $K$ that is closed under integration.
\end{enumerate}
\end{prop}
\begin{proof} Define an {\em integration tower\/} on $K$ to be a strictly 
increasing chain $(K_{\lambda})_{\lambda\le \mu}$ of immediate asymptotic extensions
of $K$, indexed by the ordinals less than or equal to some ordinal $\mu$, such 
that:  $K_0 = K$; if $\lambda$ is a limit ordinal, $0<\lambda \le \mu$, then 
$K_\lambda = \bigcup_{\iota<\lambda} K_\iota$; for $\lambda < \lambda +1 \le \mu$, {\em either\/} $K_{\lambda + 1}$ is a henselization of $K_\lambda$,
{\em or\/} $K_\lambda$ is already henselian,
$K_{\lambda + 1} = K_\lambda(y_{\lambda})$ with $y_\lambda\notin K_\lambda$
(hence $y_\lambda$ is transcendental over~$K_\lambda$), $y_\lambda'= s_\lambda \in K_\lambda$, and  one of
the following holds, with $(\Gamma_\lambda, \psi_\lambda)$
the asymptotic
couple of $K_\lambda$: 
\begin{enumerate}
\item[(i)]
$v(s_\lambda)\in (\Gamma_\lambda^{>})'$, and 
$s_\lambda\neq\varepsilon'$ for all 
$\varepsilon\in K_\lambda^{\prec 1}$;
\item[(ii)] $S_\lambda :=\bigl\{v(s_\lambda - a'): a\in K_\lambda\bigr\} <
(\Gamma_\lambda^{>})'$.
\end{enumerate}
Note that in (i) we can arrange $y_{\lambda} \prec 1$ by subtracting a 
constant from $y_{\lambda}$, and that in (ii) the set
$S_\lambda$ has no largest element and $y_{\lambda} \succ 1$. This is relevant
in connection with the uniqueness of the valuations in 
Lemmas~\ref{var43} and ~\ref{var51}.


Take a maximal integration tower $(K_{\lambda})_{\lambda\le \mu}$ on $K$, where ``maximal'' means that it cannot be extended to an integration tower 
$(K_{\lambda})_{\lambda\le \mu+1}$ on $K$. Then the top~$K_{\mu}$ of the tower 
has the properties stated about $K(\int)$.  
\end{proof}

\nomenclature[Z]{$K(\int)$}{closure of $K$ under integration}

\begin{cor}\label{minint} With $K$ and $K(\int)$ as in 
Proposition~\ref{asintint}, the only henselian asymptotic subfield 
of $K(\int)$ containing $K$ and closed under integration
is $K(\int)$.
\end{cor} 
\begin{proof} Let $F$ be the intersection of all
henselian asymptotic subfields $L\supseteq K$ of~$K(\int)$ that are closed
under integration. Then $F$ itself is among these $L$, and so is the smallest
such $L$. Since $F$ is a
$\d$-valued field extension of $K$ closed under integration,
 $K(\int)$ embeds into $F$ over $K$, and the image of any such an embedding is
also among these $L$, and thus equals $F$. In particular, $K(\int)$ is 
$K$-isomorphic to~$F$, and so inherits the minimality property of $F$.    
\end{proof}

\noindent
Let $K$ be a $\d$-valued field of $H$-type with 
asymptotic integration. A consequence of the minimality property of 
Corollary~\ref{minint} is that an asymptotic extension 
$K(\int)$ as in Proposition~\ref{asintint} is unique
up to isomorphism over $K$: if $L$ is also an asymptotic extension of $K$ with the properties of $K(\int)$
as in that proposition, then there is a $K$-embedding of $L$ into $K(\int)$, 
and the image of this embedding is then $K(\int)$.   

%Next we consider some adjunctions of exponential integrals. 





\subsection*{Adjoining exponential integrals} {\em In this subsection $K$ is an
 $H$-asymptotic field 
with asymptotic couple $(\Gamma, \psi)$, $\Gamma\ne \{0\}$, and $a$, $b$ range over $K^\times$ and $j$, $k$ over $\Z$.
In Proposition~\ref{newprop} and  
Lemmas~\ref{newprop-1} through 
%~\ref{step4}, \ref{newprop0}, \ref{newprop, lemma 1}, 
%\ref{prehexpint} and 
\ref{newprop, lemma 2}
we fix an
$s\in K^\times$ such that $s\ne a^\dagger$ for each~$a$, and
we take a field extension $K(f)$ of~$K$ with $f$ transcendental over~$K$, 
equipped with the unique derivation extending  the derivation of $K$ such 
that $f^\dagger=s$}. If $K$ is algebraically closed,   
then the constant field of $K(f)$ is $C$, by 
Lemma~\ref{lem:exp integration simple} and Corollary~\ref{cor:unit alg}.
%seems to be true also for real closed $K$.

\begin{prop} \label{newprop}
Suppose $K$ is algebraically closed and $\d$-valued. Then there is a valuation of $K(f)$ that 
makes it a $\d$-valued field extension of $H$-type of $K$  
with asymptotic couple $(\Gamma_f,\psi_f)$, and 
for any such valuation,
$$ \Gamma_f=\Gamma\ \Longleftrightarrow\ 
v(s-a^\dagger)\in (\Gamma^{>})'\text{  for some $a$.}$$
\end{prop}

\noindent
The proof consists of several lemmas, which give more precise information.

\begin{lemma}\label{newprop-1} Let $K$ be $\d$-valued. Let
$K(f)$ carry a valuation making it a $\d$-valued field 
extension of $K$ with value group $\Gamma_f=\Gamma$. Then 
$v(s-a^\dagger) \in (\Gamma^{>})'$ for some $a$.
\end{lemma}
\begin{proof} Since $vf\in \Gamma$, we have $a$ and $g$ such that 
$f=ag$, $g\in K(f)$, and $g\asymp 1$. Then 
$s-a^\dagger=g^\dagger\asymp g'$. Thus 
$v(s-a^\dagger)=v(g') \in (\Gamma^{>})'$.
\end{proof}

\begin{lemma}\label{step4}
Assume $K$ is henselian and $\d$-valued,
and $v(s) \in (\Gamma^{>})'$. 
Then there is a unique valuation
of $K(f)$ that makes it an asymptotic field extension of $K$ 
with $f-1\not\asymp 1$. With this valuation $K(f)$ is $\d$-valued of $H$-type, and an immediate extension of $K$ with $f \sim 1$.
\end{lemma}

\noindent
Using that $K$ is of $H$-type, this is a variant of Lemma~5.2 in \cite{AvdD2} with the same proof, and $f=1+y$ in the notations used there. 


\begin{lemma}\label{newprop0} 
Let $K$ be algebraically closed and $\d$-valued, and suppose $a$ satisfies
$v(s-a^\dagger)\in (\Gamma^{>})'$. Then some valuation of $K(f)$ 
makes it a $\d$-valued field extension of $H$-type of $K$; 
any such valuation makes $K(f)$ an immediate extension of $K$.
\end{lemma}
\begin{proof} By Lemma~\ref{step4} with $s-a^\dagger$
and $f/a$ instead of $s$ and $f$ we get a valuation of $K(f)$  
making it a $\d$-valued field extension of $H$-type of $K$. Let~$K(f)$
be equipped with any such valuation.
Then $(f/a)^\dagger = s-a^\dagger$, hence $f\asymp a$, so  $f/a = c(1+z)$ with 
$c\in C^\times$ and $z\prec 1$, and then $(1+z)^\dagger =s-a^\dagger$. 
Thus by Lemma~\ref{step4}, the valued
field $K(f)=K(1+z)$ is an immediate extension of $K$.
\end{proof}

\noindent
This takes care of Proposition~\ref{newprop} in the case that
$v(s-a^\dagger)\in (\Gamma^{>})'$ for some $a$.


\medskip
\noindent
It remains to consider the case 
that $v(s-a^\dagger)< (\Gamma^{>})'$ for all $a$. 
This condition is for $\d$-valued $K$ equivalent to: 
$$s-a^\dagger\ \succ\  u'\quad 
\text{ for all }a \text{ and for all }u\in K^{\preceq 1}.$$ 
The next lemma falls under this case, but deals with a rather special situation. It is not needed for the proof of Proposition~\ref{newprop}.

\begin{lemma}\label{lemma62}
Suppose $K$ is a real closed $H$-field, $s< 0$, and
 $v(s-a^\dagger)\in \Psi^{\downarrow}$ for all $a$.
 Then there is a unique pair 
consisting of a valuation of $K(f)$ and a field ordering on $K(f)$ making it a 
pre-$H$-field extension of $K$ with $f>0$. With this valuation and
ordering we have:
\begin{enumerate}
\item  $K(f)$ is an $H$-field with $v(f)\notin \Gamma$ and $f\prec 1$;
\item $C_{K(f)}=C$, and $\Psi$ is cofinal in $\Psi_{K(f)}$;
\item If $K(f)$ has a gap which is not in $\Gamma$, then $[\Gamma]=[\Gamma_{K(f)}]$.
\end{enumerate} 
\end{lemma}

\noindent
This combines Lemma~5.3 in \cite{AvdD2} with some remarks following its proof. (In that proof, references to Lemmas 3.4 and 3.5 should be to Lemmas 3.3 and 3.4 instead, and 
``$v(d)>v(y)$'' at the end should be $v(d) < v(y)$.)


\medskip\noindent
{\em In the next three lemmas we presuppose that 
$s-a^\dagger \succ u'$ for all $a$ and $u\in K^{\preceq 1}$},
but do {\em not\/} assume that $K$ is algebraically closed or 
$\d$-valued, since the extra
generality will be of some use.
(Of course we keep the assumption that $K$ is an 
$H$-asymptotic field with asymptotic couple 
$(\Gamma, \psi)$, $\Gamma\ne \{0\}$.) Put 
$$ S\ :=\ \big\{ v(s-a^\dagger) :\  a\in K^\times \big\}\ \subseteq\ \Gamma,$$ so
$S<(\Gamma^{>})'$. Taking $a=1$ shows that $vs\in S$. 
The next lemma is the most substantial of this section. 
 

\begin{lemma} \label{newprop, lemma 1}
Suppose $S$ has no maximum and $\Gamma$ is divisible. Then there is 
a unique valuation
on $K(f)$ that makes $K(f)$ an $H$-asymptotic field extension of $K$ with 
asymptotic couple $(\Gamma_f, \psi_f)$. Moreover, for this valuation we have:
\begin{enumerate}
  \item[(i)] $vf\notin \Gamma$, $\Gamma_f=\Gamma\oplus\Z {vf}$, $[\Gamma_f]=[\Gamma]$,  
and $\res K(f) = \res K$; 
\item[(ii)] if $K$ has small derivation, then so does $K(f)$;
\item[(iii)] if $K$ is pre-$\d$-valued, then so is $K(f)$; 
\item[(iv)] if $K$ is $\d$-valued, then so is $K(f)$, with the same constant field.
\end{enumerate}
\end{lemma}
\begin{proof}
Since $S$ has no largest element, Lemma~\ref{have1} and 
Corollary~\ref{trich} yield $S\subseteq (\Gamma^{<})'$.
Let the infinite cardinal $\kappa$ be the cofinality of $S$ and let 
$(a_\lambda)_{\lambda<\kappa}$ be a sequence in $K^\times$ 
such that the sequence $\bigl(v(s-a_\lambda^\dagger)\bigr)$ is strictly
increasing and cofinal in $S$ with $v(s-a_\lambda^\dagger)>vs$ for all
$\lambda$. Then $s\sim a_\lambda^\dagger$ for all $\lambda$. Since $vs\in (\Gamma^{<})'$,
and $b^\dagger \asymp b'$ if $b\asymp 1$, this gives $a_\lambda\not\asymp 1$ for all $\lambda$ by (1) of Corollary~\ref{CharacterizationAsymptoticFields-Corollary}. Also,
$$s-a_\lambda^\dagger\ \asymp\ 
a_\mu^\dagger - a_\lambda^\dagger\ \asymp\ a_\lambda^\dagger - a_\mu^\dagger\qquad\text{for $\lambda<\mu<\kappa$,}$$
since $s$ is a pseudolimit of the pc-sequence $(a_\lambda^\dagger)$. Hence
$$(a_\lambda/a_\mu)^\dagger\ =\ a_\lambda^\dagger-a_\mu^\dagger\ \succ\
a_\mu^\dagger-a_\nu^\dagger\ =\ (a_{\mu}/a_\nu)^\dagger \qquad\text{for $\lambda<\mu<\nu<\kappa$.}$$
We have $v(a_\lambda/a_\mu) \neq 0$ for $\lambda<\mu<\kappa$:
otherwise $s-a_\lambda^\dagger \asymp (a_\lambda/a_\mu)^\dagger \asymp (a_\lambda/a_\mu)'$
and $v\big((a_\lambda/a_\mu)'\big)> (\Gamma^{<})'$
by (1) of Corollary~\ref{CharacterizationAsymptoticFields-Corollary},  
a contradiction. Now we put $\alpha_\lambda:=v(a_\lambda)$, so 
$\alpha_\lambda-\alpha_\mu=v(a_\lambda/a_\mu)$, and thus by the $H$-type
assumption,
$$ [0]\ <\ [\alpha_\nu-\alpha_\mu]\ <\ [\alpha_\mu-\alpha_\lambda]
\qquad\text{for $\lambda<\mu<\nu<\kappa$}.$$
Thus $(\alpha_\lambda)$ is a pc-sequence with respect to the standard valuation of the ordered abelian group~$\Gamma$.

\claim[1]{For no $\alpha\in \Gamma$ is $\bigl([\alpha-\alpha_\lambda]\bigr)_{\lambda}$ 
eventually strictly decreasing.} 


\noindent
Otherwise we have $[\alpha-\alpha_\lambda]=[\alpha_\mu-\alpha_\lambda]$
for $\lambda_0\leq\lambda<\mu<\kappa$, hence with $\alpha=va$ we get,
for $\lambda_0\leq\lambda<\mu<\kappa$:
$$v(a^\dagger-a_\lambda^\dagger)\ =\ \psi(\alpha-\alpha_\lambda)\ =\ 
\psi(\alpha_\mu-\alpha_\lambda)\ =\ v(a_\mu^\dagger-a_\lambda^\dagger)\ =\
v(s-a_\lambda^\dagger)$$
and therefore
$$v(s-a^\dagger)\ =\ v(s-a_\lambda^\dagger+a_\lambda^\dagger-
a^\dagger)\ \geq\ v(s-a_\lambda^\dagger)$$ for  $\lambda_0\leq\lambda 
< \kappa$, contradicting the choice of $(a_\lambda)$.

\medskip\noindent
Claim~1 says that the pc-sequence $(\alpha_\lambda)$ does not have a pseudolimit in $\Gamma$ with respect to the standard valuation; thus by Corollary~\ref{pc4}: 

\claim[2]{For every $\alpha\in\Gamma$, the sequence 
$\big([\alpha-\alpha_\lambda]\big)$ is eventually constant.}

\noindent
Since $(\Gamma,\psi)$ is of $H$-type, Claim~1 also gives:

\claim[3]{For no $a$ is $\bigl(v(a^\dagger-a_\lambda^\dagger)\bigr)_{\lambda}$ eventually strictly increasing.}
%{There is no $a$ and $\lambda_0<\kappa$ such that
%$\bigl(v(a^\dagger-a_\lambda^\dagger)\bigr)_{\lambda_0\leq\lambda<\kappa}$ 
%is strictly in\-creasing.}

\noindent
Suppose now that $K(f)$ is equipped with a valuation that makes it an 
$H$-asymptotic field extension of $K$ with asymptotic couple
$(\Gamma_f,\psi_f)$. Then $\eta:=vf\notin\Gamma$:
otherwise $f=ua$ for some $a$ and $u\in K(f)$ with $u\asymp 1$; for such $a$ and $u$
we have $u^\dagger\asymp u' \prec b'$ for all $b\succ 1$
%>\big(\Gamma_f^{<}\big)'$ 
by (1) of Corollary~\ref{CharacterizationAsymptoticFields-Corollary}, in particular 
$u^\dagger \prec s-a_\lambda^\dagger$ and therefore
$$a^\dagger-a_\lambda^\dagger\ =\ 
f^\dagger -u^\dagger-a_{\lambda}^\dagger\ =\ 
(s-a_\lambda^\dagger) - u^\dagger\ \asymp\  s-a_\lambda^\dagger,$$
for all $\lambda$, contradicting Claim~3. This
yields $\Gamma_f=\Gamma\oplus\Z\eta$. The sequence
$\big([\eta-\alpha_\lambda]\big)$ is strictly decreasing in $[\Gamma_f]$, 
since
$\psi_f(\eta-\alpha_\lambda)=v(s-a_\lambda^\dagger)$ for all $\lambda$,
and $(\Gamma_f,\psi_f)$ is of $H$-type.
Using also Claim~2 it follows that for all $\alpha\in\Gamma$ we have
$[\alpha-\eta] = [\alpha-\alpha_\lambda]$ eventually. Hence 
$[\Gamma_f]=[\Gamma]$. It also follows that 
for all $\alpha\in\Gamma$,
$$\alpha<\eta \Longleftrightarrow \alpha<\alpha_\lambda \text{ eventually}, \qquad 
\alpha>\eta \Longleftrightarrow \alpha>\alpha_\lambda \text{ eventually}.$$
This determines the ordering on $\Gamma_f$. Hence there is at most
one valuation on $K(f)$ making $K(f)$ an $H$-asymptotic field extension of 
$K$.

We now construct such a valuation. By Lemma~\ref{divimm, standard val} we can 
take an element $\eta$ in an ordered abelian group extending $\Gamma$
such that $\eta\notin \Gamma$,
the sequence $\bigl([\eta-\alpha_\lambda]\bigr)$ is eventually strictly
decreasing, and $[\Gamma_f]=[\Gamma]$, where
$\Gamma_f:=\Gamma\oplus\Z\eta$. By Lemma~\ref{extension4} there exists
a unique extension of $\psi\colon\Gamma^{\ne}\to\Gamma$ to a map
$\psi_f\colon\Gamma_f^{\ne}\to\Gamma$ such that $(\Gamma_f,\psi_f)$ is an
asymptotic couple of $H$-type. Now $\Gamma$ is divisible, so $\Gamma^{>}$ is coinitial
in $\Gamma_f^{>}$. Therefore, 
if $(\Gamma, \psi)$ has small derivation, then so does $(\Gamma_f, \psi_f)$.


\claim[4]{$\psi_f\bigl(va +j\eta\bigr)=v(a^\dagger+js)\in S$ for all $a$ and 
all $j\neq 0$.}

\noindent
To prove Claim~4, let $a$ and $j\ne 0$ be given, and take $u,d\in K^{\times}$ such that $a=ud^{-j}$ and $u\asymp 1$ (which is possible since $\Gamma$ is divisible). Then $a^\dagger = -jd^\dagger + u^\dagger$ and $u^\dagger\asymp u'\prec s-d^\dagger$,
so
\begin{align*} v(a^\dagger+js)\ &=\ v(js-jd^\dagger+ u^\dagger)\ =\ v(s-d^\dagger)\in S, \\
\psi_f(va+j\eta)\ &=\ \psi_f\big(j(-vd+\eta)\big)\ =\ \psi_f(\eta-vd),
\end{align*} 
so it only remains
to show that $\psi_f(\eta-vd)=v(s-d^\dagger)$. Since
$\bigl([\eta-\alpha_\lambda]\bigr)$ is strictly decreasing, 
there are arbitrarily large $\lambda<\kappa$ with $[\eta-vd]=
[\alpha_\lambda-vd]$.  For those $\lambda$ we have
$\alpha_\lambda\neq vd$ (since $\eta\neq vd$), and thus
$$\psi_f(\eta-vd)\ =\  \psi(\alpha_\lambda-vd)\ =\ 
v(a_\lambda^\dagger-d^\dagger).$$
By cofinality of 
$\bigl(v(s-a_\lambda^\dagger)\bigr)$ in $S$ we get
$v(a_\lambda^\dagger-d^\dagger)=
v(s-d^\dagger)$
for all sufficiently large $\lambda$. Hence
 $\psi_f(\eta-vd)=v(s-d^\dagger)$ 
as required.


\medskip\noindent
We now equip $K(f)$ with the valuation $v\colon K(f)^\times \to \Gamma_f$
that extends the valuation of $K$ and such that $vf=\eta$. 

\claim[5]{$K(f)$ is an asymptotic field 
with asymptotic couple $(\Gamma_f,\psi_f)$.}

\noindent
By Claim~4 we have:
\begin{equation}\label{psi-f}
v\big((af^j)^\dagger\big)\ =\ \psi_f\big(va+j\eta\big) 
\qquad\text{if $va+j\eta\neq 0$.}
\end{equation} 
Therefore, if $va+j\eta,vb+k\eta>0$, then $$v\big((af^j)'\big)\ =\
(va+j\eta)'\ >\ \psi_f(vb+k\eta)\ =\ v\big((bf^k)^\dagger\big).$$ 
Now suppose $va+j\eta=0$; then $j=0$, so $v\big((af^j)'\big)=v(a')>S$. 
In particular, 
if $k\neq 0$, then $v\big((af^j)'\big)>v\big((bf^k)^\dagger\big)$ by 
\eqref{psi-f} and Claim~4. If $vb\neq 0$, then 
$v\big((af^j)'\big)=v(a')\geq v(b^\dagger)$.
Since $\Gamma_f\neq\Gamma$ we have $\res K(f)=\res K$.
Hence $K$, $L:=K(f)$ and $T:=\bigcup_j K^\times f^j$ satisfy the hypotheses 
of Lemma~\ref{Lemma34}, so $L$ is an asymptotic field. By 
\eqref{psi-f}, its asymptotic couple is $(\Gamma_f,\psi_f)$. If $K$ is pre-$\d$-valued, then so is $K(f)$ by Lemma~\ref{Lemma3.3}.
If~$K$ is $\d$-valued, then so is $K(f)$ by Lemma~\ref{dv}.
\end{proof}

\noindent
The uniqueness part of Lemma~\ref{newprop, lemma 1}
strengthens Proposition~\ref{newprop} significantly 
in the case considered. 
We also need a version for pre-$H$-fields:

\begin{lemma}\label{prehexpint} With the assumptions of Lemma~\ref{newprop, lemma 1}, 
and the valuation on $K(f)$ of that lemma, let $K$ be given a field ordering making it a pre-$H$-field. Then there is a unique field ordering on $K(f)$ making it a pre-$H$-field extension of $K$ with $f>0$.
\end{lemma}
\begin{proof} We can assume $s < 0$. (If $s>0$, replace $s$ and
$f$ by $-s$ and $f^{-1}$.) 

\claim{For all $a\prec 1$ we have:
$f\succ a\Longleftrightarrow s>a^\dagger$.}

\noindent
To prove this claim, let $a\prec 1$ and set $\alpha:=va$. Then
\begin{align*}
f\ \succ\ a\ &\Longleftrightarrow\ \eta\ <\ \alpha\ \Longleftrightarrow\ \alpha_{\lambda}\ <\ \alpha \text{ eventually}\\ 
&\Longleftrightarrow\ a_{\lambda}\ \succ\ a \text{ eventually}\\
&\Longleftrightarrow\ a_{\lambda}^\dagger\ >\ a^\dagger \text{ eventually}\ 
\Longleftrightarrow\ s\ >\  a^\dagger.
\end{align*}
We order $K(f)$ as indicated in Lemma~\ref{extror} with $f$ in the role of
$y$, and show that this makes $K(f)$ a pre-$H$-field extension of $K$.  
Now $K(f)$ is pre-$\d$-valued by item~(iii) of Lemma~\ref{newprop, lemma 1}, and so with $T$ as in the proof of that lemma, it remains to show by Lemma~\ref{lem3.3pre} that
for all $t\in T$ with $t\succ 1$ we have $t^\dagger > 0$. 

Let $t\in T$, $t\succ 1$, so $t=af^j$. Consider first the case $j>0$.
Take $d\in K^\times$ with $ad^j\asymp 1$.  Then $t\asymp (f/d)^j\succ 1$ gives $f \succ d$, so
$s > d^\dagger$ by the Claim, hence $js> jd^\dagger= -a^\dagger + g$ with $g\in K$, $vg> \Psi$, and thus
$a^\dagger + js > g$. Also $v(a^\dagger + js)\in S < vg$
by Claim~4 in the proof of Lemma~\ref{newprop, lemma 1}, and thus
$t^\dagger= a^\dagger + js >0$. In the same way we treat the case that $j < 0$. The case $j=0$ is trivial.   
\end{proof}

\noindent
Since $(-f)^\dagger=f^\dagger=s$, Lemma~\ref{prehexpint} goes through with $f<0$ instead of $f>0$. 




\begin{lemma}\label{newprop, lemma 2}
Suppose $S$ has a maximum and $\Gamma$ is divisible. Then there is a valuation on $K(f)$ 
making it an $H$-asymptotic field extension of $K$ with
$[v(af)] \notin [\Gamma]$ for some $a$.
For any such valuation, with asymptotic couple $(\Gamma_f, \psi_f)$
of $K(f)$,  \begin{enumerate}
\item[(i)] $vf\notin \Gamma$, $\Gamma_f=\Gamma\oplus \Z vf$,  
$\res K(f)=\res K$, and 
$\Psi_f \subseteq \Gamma$;
\item[(ii)] if $K$ has small derivation, then so does $K(f)$;
\item[(iii)] if $K$ is $\d$-valued, then so is $K(f)$, with the same 
constant field.
\end{enumerate}
\end{lemma}
\begin{proof}
Let $vt$ with $t=s-b^\dagger$ be the largest element of $S$. Then 
$v(t-a^\dagger)=v\big(s-(ab)^\dagger\big)\leq vt$ for all $a$. By renaming 
$f/b$ as $f$ and $t$ as $s$ the hypotheses of  
Lemma~\ref{newprop, lemma 2} remain valid; 
then $v(s-a^\dagger)\leq vs$ for all $a$. Also 
\begin{equation}\label{min-formula asymptotic}
v(a^\dagger+js)\ =\ 
\min\big(vs,v(a^\dagger)\big)\in S\qquad\text{for all $a$ and all $j\neq 0$.}
\end{equation}
To see this, let $a$ and $j\ne 0$ be given. Since $\Gamma$ is divisible we can
take $u,d\in K^{\times}$ such that $u\asymp 1$ and $a=ud^{-j}$. 
Then $a^\dagger = -jd^\dagger + u^\dagger$ and $u^\dagger\asymp u'\prec s-d^\dagger$,
so
$$v(a^\dagger+js)\ =\ v(js-jd^\dagger+ u^\dagger)\ =\ v(s-d^\dagger)\
=\ \min\big(vs,v(d^\dagger)\big)\ =\ 
\min\big(vs,v(a^\dagger)\big).$$
(To get the last two equalities, consider the cases $vs = v(d^\dagger)$ and $vs=v(a^\dagger)$ separately.) 
Since $(\Gamma,\psi)$ is of $H$-type, 
$$M:=\bigl\{\gamma\in\Gamma^{<}: \psi(\gamma) \leq vs\bigr\}$$ 
is closed downward in $\Gamma$.
Let $\eta$ be an element of an ordered abelian group extending~$\Gamma$ such that $M<\eta<\Gamma\setminus M$, so $\eta < 0$. Put  
$\Gamma_f:=\Gamma\oplus \Z\eta$. Then $[\eta]\notin [\Gamma]$:
otherwise $n\gamma < \eta < \gamma$ where $\gamma\in \Gamma^{<}$ and $n\geq 2$,
so $\psi(\gamma)= \psi(n\gamma)\le vs$, a contradiction.
Hence $[\Gamma_{f}]=[\Gamma]\cup \bigl\{[\eta]\bigr\}$.
We can now apply Lemma~\ref{extension5} with 
$$C\ :=\ \big\{[\gamma]:\ \gamma\in \Gamma,\ M < \gamma < 0\big\}, \quad \beta: =vs.$$
This gives an $H$-asymptotic couple $(\Gamma_f,\psi_f)$ that extends $(\Gamma, \psi)$
with 
$$\psi_f\colon \Gamma_f^{\ne} \to \Gamma, \qquad
\psi_f(\gamma + j\eta)\ :=\ 
\min\big(\psi(\gamma),vs\big)  \quad
\text{ for $\gamma\in\Gamma$ and  $j\neq 0$.}$$
Equip $K(f)$ with the valuation
$v \colon K(f)^\times \to \Gamma_f$ extending the valuation of $K$ 
such that $vf=\eta$.  Since 
$\Gamma_f\neq\Gamma$ we have $\res K(f)=\res K$. If $va+j\eta\neq 0$, then 
$$v\big((af^j)^\dagger\big)\ =\ v(a^\dagger+js)\ =\ \psi_f(va+j\eta)$$ 
by \eqref{min-formula asymptotic}. Therefore, if $va+j\eta,vb+k\eta>0$, 
then $$v\big((af^j)'\big)=(va+j\eta)'>\psi_f(vb+k\eta)=
v\big((bf^k)^\dagger\big).$$ Next suppose $va+j\eta=0$; then $va=0$, $j=0$, 
so $v\big((af^j)'\big)=v(a')$. Now $v(a')>vs$, 
and if $vb\neq 0$, then $v(a')\geq v(b^\dagger)$; hence 
$v\big((af^j)'\big)\geq v\big((bf^k)^\dagger\big)$ 
if $vb+k\eta\neq 0$. We have now shown that $K$, $L=K(f)$ and 
$T=\bigcup_j K^\times f^j$ 
satisfy the hypotheses of Lemma~\ref{Lemma34}, so $K(f)$ is an 
asymptotic field.

Now let $K(f)$ be equipped with any valuation that makes
it an $H$-asymptotic field extension of $K$ with asymptotic couple 
$(\Gamma_f, \psi_f)$
such that $[v(af)]\notin [\Gamma]$ for some $a$. Fix such $a$. 
Then $vf\notin \Gamma$, so $\Gamma_f=\Gamma\oplus \Z vf$ and 
$\res K(f)=\res K$. Also
$[\Gamma_f]=[\Gamma]
\cup \big\{[v(af)]\big\}$ by Lemma~\ref{archextclass}, and 
$\psi_f\big(v(af)\big)=v(a^\dagger+s)$, hence
$$\Psi_f\ =\ \Psi \cup \big\{v(a^\dagger+s)\big\}\ \subseteq\ \Gamma,$$
which gives (i). To prove (ii), assume that $K$ has small derivation. We 
wish to show that $K(f)$ has small derivation. With $a$ as above we have 
$\psi_f\big(v(af)\big)=v(a^\dagger + s)\in \Psi_f$, so we are done if
$v(a^\dagger + s)\ge 0$. Suppose $v(a^\dagger + s)< 0$. Then
Lemma~\ref{PresInf-Lemma} gives $\gamma\in \Gamma^{<}$ such that 
$v(a^\dagger +s) < \psi(\gamma)$. Then
$v(af) < \gamma <0$ or $-v(af) < \gamma < 0$. Because $[\Gamma_f]=[\Gamma]\cup
\{[v(af)]\}$ it follows that $\Gamma^{<}$ is cofinal in 
$\Gamma_f^{<}$, and we are done by Lemma~\ref{PresInf-Lemma}. 
Lemma~\ref{dv} gives (iii). 
\end{proof} 

\noindent
Lemmas~\ref{newprop-1}, ~\ref{newprop0}, ~\ref{newprop, lemma 1}, ~\ref{newprop, lemma 2} above cover all claims of
Proposition~\ref{newprop}.




\begin{example}
Let $K=\C[[x^{\Q}]]$ with its usual derivation 
($x'=1$ and $C=\C$) and valuation $v\colon K^\times \to \Gamma=\Q$, $vx=-1$, so
$K$ is an algebraically closed $\d$-valued field of $H$-type 
with $\Psi= \{1\}$. Let $s=\imag\in\C$, $\imag^2=-1$, so $s\ne a^\dagger$
for all $a$. Let
$f$ be as in the beginning of this subsection: transcendental over $K$ 
with the derivation on $K(f)$ extending that of $K$ with $f^\dagger=s$.
(One may think of $f$ as $e^{\imag x}$.) 
We have $S=\{0\}=\{vs\}$, and $K(f)$ with the valuation constructed 
in the proof of Lemma~\ref{newprop, lemma 2} is $\d$-valued and
satisfies $vf<\Gamma$ and $\Psi_f=\{0,1\}$.
\end{example}


\begin{cor} \label{newcor}
Suppose that $K$ is algebraically closed, $\d$-valued, and 
has small derivation.
Then there exists a $\d$-valued field extension $L$ of $H$-type
of $K$ with
small derivation and the following properties:
\begin{enumerate}
\item $L$ is algebraically closed with constant field $C$;
\item for each $s\in K$ there exists $f\in L^\times$
with $f^\dagger=s$;
\item $L$ is algebraic over its subfield 
generated over $K$ by the $f\in L^\times$ with $f^\dagger\in K$;
\item there exists a family $(f_i)_{i\in I}$
of elements of $L^\times$ such that $f_i^\dagger\in K$ for all $i\in I$, and
$\Gamma_L=\Gamma\oplus \bigoplus_{i\in I} \Q v(f_i)$ 
\textup{(}internal direct sum of $\Q$-linear subspaces\textup{)}.
\end{enumerate}
Moreover, any such $L$ has the following additional properties:
\begin{enumerate}
\item[(5)] $\Psi_L\subseteq \Gamma$, and if $\Psi$ has a maximum $\alpha$, 
then $\Psi_L=\Gamma^{\leq\alpha}$;
\item[(6)] $L$ has no proper differential field extension $M$ satisfying $(1),\ (2),\ (3)$ with $M$ instead of $L$.
\end{enumerate}
\end{cor}
\begin{proof} 
Iterating the extension steps of Lemmas~\ref{newprop0},
\ref{newprop, lemma 1}, and \ref{newprop, lemma 2}, and alternating these 
steps by taking algebraic closures, we obtain a $\d$-valued 
field extension $L$ of $K$, with small derivation, of $H$-type, and
satisfying (1)--(4).

Let any such $L$ be given. To prove (5), consider any element of $\Psi_L$.
It equals $v(f^\dagger)$ with $f\in L^\times$, $f\nasymp 1$. By (4) we have a
nonzero $k\in \Z$ such that
$$f^k\asymp af_1^{k_1}\cdots f_m^{k_m}, \qquad f_1,\dots,f_m\in L^\times,\ k_1,\dots, k_m\in \Z.$$
Then $kf^\dagger\asymp a^\dagger + k_1f_1^{\dagger} + \cdots + k_mf_m^\dagger \in K$,
so $v(f^\dagger)\in \Gamma$, as claimed. 
Now assume also that $\Psi$ has largest element $\alpha$. Then by 
$\Psi_L\subseteq \Gamma$ and 
Lemma~\ref{asy1} we have 
$\Psi_L\subseteq \Gamma^{\leq\alpha}$. The reverse inclusion is clear from (2).

If $M$ is a 
differential field extension of $L$ satisfying (1), (2), (3), then for 
any $g\in M^\times$ with $g^\dagger\in K$ we have $f\in L^\times$ such that
$f^\dagger=g^\dagger$, hence $g=cf$ for some $c\in C$, and thus $g\in L$.
This proves (6). 
\end{proof}



==> mt-9-9.tex <==

\section{Differential Polynomials of Order One}\label{caseorderone}

\noindent
{\em Throughout this section
$K$ is an $H$-asymptotic field with asymptotic couple
$(\Gamma, \psi)$, $\Gamma\ne \{0\}$. We let $\gamma$ range over $\Gamma$ and $y$ over $K^\times$, and assume 
$P\in K\{Y\}^{\ne}$ has order $\le 1$}. For such $P$ we improve on what earlier sections yield for differential polynomials of arbitrary order. The results here are not used later in this volume. 

\subsection*{Behavior of $v\big(P(y)\big)$} The goal of this
subsection is to show the following:

\begin{prop}\label{prop:vP(y), order 1}
Suppose $P(0)=0$. Then there is a finite set $\Delta(P)\subseteq\Gamma$ and a finite partition of $\Gamma\setminus\Delta(P)$ into  
convex subsets of $\Gamma$ such that for each set $U$ in 
this partition we have a strictly increasing function $i_U\colon U\to\Gamma$ for which
$$v\big(P(y)\big)\ =\ i_U(vy)\  \text{ whenever $vy \in U$.}$$
\end{prop}

\index{map!slowly varying}
\index{slowly varying}

\noindent
We derive this from a more precise result for homogeneous $P$.
We start with some generalities about functions on ordered abelian groups. Let $G$ be an ordered abelian group and $U\subseteq G$. 
A function $\eta\colon U \to G$ is said to be {\bf slowly varying} if
$\eta(\alpha)-\eta(\beta)=o(\alpha - \beta)$
for all distinct $\alpha, \beta \in U$. Note that then the function
$\alpha \mapsto  \alpha + \eta(\alpha)\colon U \to G$ is strictly increasing.
A key example of a slowly varying function is of course
$\psi\colon \Gamma^{\ne} \to \Gamma$. Note that each constant function $U\to G$ is
slowly varying, and that if $\eta_1, \eta_2\colon U\to G$ are slowly 
varying, so
are $\eta_1 + \eta_2, \eta_1 - \eta_2,$ and 
$$\alpha \mapsto \min\big(\eta_1(\alpha), \eta_2(\alpha)\big)\colon\ U\to G.$$


\begin{lemma} \label{slowlyvarying}
Let $s\in K$ be given. Then there is a $\gamma_0\in \Gamma$ and
a slowly varying function 
$\eta\colon \Gamma \setminus \{\gamma_0\} \to \Gamma$
with the following properties: \begin{enumerate}
\item $v(y^\dagger-s)=\eta(vy)$ for all $y$ with $vy\ne \gamma_0$;
\item for each $\alpha\in \Gamma$ the set
$\{\gamma:\ \gamma\ne \gamma_0,\ \eta(\gamma)\le \alpha\}$
is a union of finitely many disjoint convex subsets of $\Gamma$.
\end{enumerate}
\end{lemma}
\begin{proof} Suppose first that $s=a^\dagger$ with $a\in K^\times$.
Then $y^\dagger - s = (y/a)^\dagger$, so $v(y^\dagger - s) = \psi(vy - va)$
if $vy \ne va$. In this case we can take $\gamma_0=va$ and
$\eta(\gamma)= \psi(\gamma - va)$. 

Next assume that $s\ne y^\dagger$ for all $y$. Then we take a nonzero 
$\phi$ in an elementary extension $L$ of $K$ such that
$v(y^\dagger -s)\le v(\phi^\dagger -s)$ for all $y$. (This $\phi$ could be
an element of $K$.) Let $\gamma_1:=v(\phi^\dagger -s)\in \Gamma_L$.  
Then we claim that for all $y$ with $vy\ne v\phi$:
$$ v(y^\dagger - s)\ =\ \begin{cases} \psi_L(vy - v\phi) 
& \text{ if } \psi_L(vy - v\phi)\le \gamma_1\\
\gamma_1 & \text{ if }\psi_L(vy - v\phi)\ge \gamma_1. \end{cases}
$$
To see this, let $vy \ne v\phi$. From 
$v(y^\dagger - s) \le v(\phi^\dagger -s)$ we get
$y^\dagger - \phi^\dagger \not\sim s-\phi^\dagger$. Since
$$y^\dagger - s\ =\ (y^\dagger - \phi^\dagger) - (s-\phi^\dagger)\ \text{ and }\
y^\dagger - \phi^\dagger\  =\ (y/\phi)^\dagger,$$ 
this gives the claim. Note that the claim can also be expressed as:
$$v(y^\dagger-s) = \min\big\{\psi_L(vy-v\phi),\gamma_1\big\} 
\text{ whenever }vy\ne v\phi.$$
If $v\phi\in \Gamma$, then the lemma clearly
holds with $\gamma_0:= v\phi$, and if $v\phi\notin \Gamma$, then
the lemma holds for any $\gamma_0\in \Gamma$. 
\end{proof}

\begin{lemma}\label{lem:vP(y), order 1, homog}
Suppose $P$ is homogeneous of degree $d$. There is a finite set $\Delta(P)\subseteq\Gamma$ and a finite partition of $\Gamma\setminus\Delta(P)$ into  
convex subsets of $\Gamma$ such that for each set $U$ in this partition
we have a slowly varying function $\eta_U\colon U\to\Gamma$ for which
$$v\big(P(y)\big)\ =\ d\,vy+\eta_U(vy)\  \text{ whenever $vy \in U$.}$$
\end{lemma}

\begin{proof}
We have $P=a_0Y^d + a_1Y^{d-1}Y' + \dots +a_d(Y')^d$ with  $a_0,\dots,a_d\in K$,
so $P(y)=y^d(a_0 + a_1z + \dots + a_dz^d)$, where 
$z=y^\dagger$. The henselization of $K$ is still $H$-asymptotic with the same asymptotic couple, so we can
assume $K$ is henselian. Now apply Lemma~\ref{piecewise uniform description} and the surrounding 
remarks to the polynomial 
$a_0+ a_1Z + \dots + a_dZ^d$ to partition $K$ into 
sets $G_1,\dots,G_k$ such that for $i=1,\dots,k$: 
$G_i$ is a special disk in $K$ with holes, and we have  
$b_{i0},\dots, b_{id}, s_i\in K$ with
$$v\big(P(y)\big)\ =\ 
d\,vy + \min\big\{v(b_{ij}) + j\,v(z - s_i):\  0\le j\le d\big\}\qquad\text{if $z\in G_i$.}$$ 
In addition, either $s_i=0$ and the condition
$z\in G_i$ is of the form 
$$v(z- s_{i,1})\ \le\ v(s_{i,1}),\ \dots,\ 
v(z - s_{i,n(i)})\ \le\  v(s_{i,n(i)}),$$
or $s_i\ne 0$ and the condition $z\in G_i$ is of the form
$$v(z - s_i)\ >\  v(s_i),\  v(z- s_{i,1})\ \le\ v(s_{i,1}),\
\dots,\ v(z - s_{i,n(i)})\ \le\  v(s_{i,n(i)})$$
where in both cases $s_{i,1},\dots,s_{i,n(i)}\in K^\times$.
Now use Lemma~\ref{slowlyvarying}.
\end{proof}

\begin{proof}[Proof of Proposition~\ref{prop:vP(y), order 1}]
We have
$$P(Y)\ =\ P_1(Y) + \dots + P_n(Y)\ 
\text{ (decomposition into homogeneous parts)}.$$ 
Let
$d$ below range over the numbers $1,\dots,n$ for which $P_d\ne 0$; 
likewise with $e$. Applying Lemma~\ref{lem:vP(y), order 1, homog} to all $P_d$ simultaneously we
obtain a finite $\Delta(P)\subseteq\Gamma$ and a finite partition of~$\Gamma\setminus\Delta(P)$
into convex subsets of $\Gamma$
such that for each set $U$ in the partition and each $d$ we have a slowly varying function $\eta_{U,d}\colon U\to\Gamma$ 
for which
$$v\big(P_d(y)\big)\ =\ d\,vy+\eta_{U,d}(vy)\ \text{ whenever $vy\in U$.}$$
If $d<e$, then the function 
$$\gamma \mapsto 
\big(e\,\gamma+ \eta_{U,e}(\gamma)\big) -
\big(d\,\gamma+ \eta_{U,d}(\gamma)\big)\colon\ U \to \Gamma$$ is strictly increasing. Hence, after increasing $\Delta(P)$ and refining our 
partition if necessary, we can arrange that for each $U$ in the partition 
there is a $d=d_U$ such that for all $e\ne d$:
$$v\big(P_d(y)\big)< v\big(P_e(y)\big)  \text{ whenever $vy\in U$.}$$
Thus $v\big(P(y)\big) =  v\big(P_d(y)\big)$ for $d=d_U$ and $vy\in U$, and the proposition follows.
\end{proof}


\subsection*{Evaluation at pc-sequences} {\em In this subsection we fix a pc-sequence $(a_{\rho})$ in $K$}. 
Proposition~\ref{pca-extension}
below is an analogue of Kaplansky's theorem (Lemma~\ref{lem:Kaplansky, 2}) about pc-sequences of algebraic type.
It is stronger than Lemma~\ref{zda} in not requiring the derivation of 
$K$ to be small with nontrivial differential
residue field, but weaker in assuming that $K$ is $H$-asymptotic and $P$ has order $\le 1$. Moreover, we never need to replace in our situation $(a_{\rho})$ by an equivalent pc-sequence. 
%In addition to $P\in K\{Y\}^{\ne}$ being of order 
%$\le 1$ we also assume below that $P\notin K$. 


\begin{lemma}\label{psa} Assume $P\notin K$ and 
$a_\rho\leadsto a\in K$. Then $P(a_\rho) \leadsto P(a)$.
\end{lemma}

\begin{proof} 
Replacing $a_\rho$ by $a_\rho -a$ and $P(Y)$ by $P_{+a}(Y)-P(a)$ we can  assume
that $a_\rho \leadsto 0$, $P(0)=0$, and have to show that then
$P(a_\rho) \leadsto 0$. Proposition~\ref{prop:vP(y), order 1} gives a finite subset $\Delta(P)$ of $\Gamma$ and a finite partition of $\Gamma\setminus\Delta(P)$ into finitely
many convex subsets of $\Gamma$ such that for each set~$U$ in this partition,
$v\big(P(y)\big)$ is strictly increasing as a function of $vy\in U$. 
Taking $U$ in the partition such that $v(a_\rho)\in U$  eventually, 
we conclude that $P(a_\rho) \leadsto 0$.
\end{proof}


\begin{cor}\label{pca} If $P\notin K$, then $\big(P(a_\rho)\big)$ 
is a pc-sequence.
\end{cor}
\begin{proof} Use that  $(a_\rho)$ has a pseudolimit in
some elementary extension of $K$. 
\end{proof}

 
\begin{prop} \label{pca-extension} Assume $P\notin K[Y]$, 
$P(a_{\rho})\leadsto 0$, and $Q(a_{\rho})\not\leadsto 0$ for
every $Q\in K\{Y\}$ with $\operatorname{c}(Q) < \operatorname{c}(P)$.
Then $K$ has an immediate asymptotic extension
field $K\langle a \rangle$ with the following properties: \begin{enumerate}
\item $P(a)=0$ and $a_\rho \leadsto a$;
\item for any $H$-asymptotic extension field $L$ of $K$ 
and any $b\in L$ with $P(b)=0$ and $a_\rho \leadsto b$ there is a 
unique embedding
$K\langle a\rangle \to L$ over $K$ that sends $a$ to $b$. 
\end{enumerate}
\end{prop}
\begin{proof} Note first that $P\in K[Y,Y']$ is irreducible.  
Consider the domain 
$$K[y_0, y_1]\ =\ K[Y,Y']/(P), \quad y_0:= Y+(P), \quad y_1:= Y'+(P),$$ and let $K(y_0,y_1)$ be its field of fractions. 
We extend the valuation~$v$ on $K$ to a valuation 
$v\colon K(y_0,y_1)^\times \to \Gamma$ as
follows. Pick a pseudolimit $e$ of $(a_\rho)$ in some $H$-asymptotic field
extension of $K$. Let $\phi\in K(y_0,y_1)$, $\phi\ne 0$, so 
$\phi=f(y_0, y_1)/g(y_0)$ with $f\in K[Y,Y']$ of lower degree in $Y'$ 
than $P$ and $g\in K[Y]^{\neq}$. 

\claim{$v\big(f(e,e')\big), v\big(g(e)\big)\in \Gamma$, and
$v\big(f(e,e')\big)- v\big(g(e)\big)$ depends only on $\phi$ and not on 
the choice of $(f,g)$.}

\noindent
To see why this claim is true, note that 
$f(a_\rho, a_\rho') \not\leadsto 0$ by the minimality of $P$, 
and that $f(a_\rho, a_\rho') \leadsto f(e,e')$ if $f\notin K$, 
by Lemma~\ref{psa}. Hence
$$f(a_{\rho}, a_{\rho}') \sim f(e,e')\ \text{ and }\
v\big(f(a_{\rho}, a_{\rho}')\big)= v\big(f(e,e')\big), 
\quad \text{eventually}.$$
In particular, $v\big(f(e,e')\big) \in \Gamma$, and likewise, 
$v\big(g(e)\big)\in \Gamma$. 
Suppose that also 
$\phi=f_1(y_0, y_1)/g_1(y_0)$ with $f_1\in K[Y,Y']$ of lower degree in $Y'$ 
than $P$ and $g_1\in K[Y]^{\neq}$. Then $fg_1 \equiv f_1g \bmod P$ in 
$K[Y,Y']$, and thus $fg_1=f_1g$ since $fg_1$ and $f_1g$ have lower degree in 
$Y'$ than $P$. Hence 
$v\big(f(e,e')\big)- v\big(g(e)\big)=v\big(f_1(e,e')\big)- v\big(g_1(e)\big)$,
thus establishing the claim.

\medskip\noindent
This allows us to define $v\colon K(y_0,y_1)^\times \to \Gamma$ by
$$v\phi\ :=\  v\big(f(e,e')\big)- v\big(g(e)\big).$$
It is routine to check that this map $v$ is a valuation on the field 
$K(y_0,y_1)$, except maybe for the multiplicative law. 
For this, let $\phi_1,\phi_2\in
K(y_0,y_1)^\times$, so $\phi_1=f_1(y_0,y_1)/g_1(y_0)$, 
$\phi_2=f_2(y_0,y_1)/g_2(y_0)$ with $f_1,f_2\in K[Y,Y']^{\neq}$ 
of lower degree in~$Y'$ than $P$ and $g_1, g_2\in K[Y]^{\neq}$. Then 
$$v(\phi_i)\ =\ v\big(f_i(a_\rho,a_\rho')\big)-v\big(g_i(a_\rho)\big)
\quad\text{eventually ($i=1,2$)}$$
and hence
$$v(\phi_1)+v(\phi_2)\ =\ v\big((f_1f_2)(a_\rho,a_\rho')\big)-
 v\big((g_1g_2)(a_\rho,a_\rho')\big)
 \quad\text{eventually.}$$
We have $f_1f_2=(qP)/h\ +\ r/h$
where $q,r\in K[Y,Y']$, $h\in K[Y]^{\neq}$ and $\deg_{Y'} r<\deg_{Y'} P$.
Then 
$\phi_1\phi_2=r(y_0,y_1)/s(y_0)$ where $s:=g_1g_2h\in K[Y]^{\neq}$, 
and hence $$v(\phi_1\phi_2)\ =\
v\big(r(a_\rho,a_\rho')\big)-v\big(s(a_\rho)\big)
\qquad\text{eventually.}$$
Now $(f_1f_2)(a_\rho,a_\rho')\not\leadsto 0$ since
$f_1(a_\rho,a_\rho')\not\leadsto 0$ and $f_2(a_\rho,a_\rho')\not\leadsto 0$. 
Moreover, $P(a_\rho,a_\rho')\leadsto 0$ 
and $r(a_\rho,a_\rho')\not\leadsto 0$; hence
$$v\big((f_1f_2)(a_\rho,a_\rho')\big)\ =\ 
v\big(r(a_\rho,a_\rho')\big)-v\big(h(a_\rho)\big)
\quad\text{eventually.}$$
Therefore $v(\phi_1\phi_2)=v(\phi_1)+v(\phi_2)$ as desired.
Obviously, the value group of the valuation $v$ on $K(y_0,y_1)$ is $\Gamma$.
Its residue field is that of $K$. To see this, let $\phi\in K(y_0,y_1)^\times$
and $v\phi=0$; we shall find $s\in K$ with $v(\phi -s)>0$. We have
$\phi=f(y_0,y_1)/g(y_0)$ with $f\in K[Y,Y']$ of lower
degree in $Y'$ than $P$ and $g\in K[Y]^{\neq}$. Multiplying
$f$ and $g$ by a suitable element of $K^\times$ we may
assume that $v\big(f(e,e')\big)=v\big(g(e)\big)=0$. By the above we have
$f(e,e')\sim f(a_\rho, a_\rho')$ and $g(e)\sim g(a_\rho)$, eventually, hence
$v\left(\frac{f(e,e')}{g(e)} - s\right) >0$ where 
$s:=\frac{f(a_\rho, a_\rho')}{g(a_\rho)}$ with large enough $\rho$,
so $v(\phi -s)>0$ for such $s$. 

\medskip\noindent
We now equip $K(y_0,y_1)$ with the derivation 
extending the derivation of $K$ such that $y_0'=y_1$. We also set $a:= y_0$, 
so $a'=y_1$ and $K(y_0, y_1)=K\langle a \rangle$. Then $P(a)=0$, trivially, 
and $a_\rho \leadsto a$, as is easily checked.

\medskip\noindent
To show that $K\langle a \rangle$ is an asymptotic field, we use 
Proposition~\ref{pa5} with $K(a)$ in the role of $K$ and 
$L= K\langle a \rangle$. By that proposition it is enough to show
that  $K(a)$ is asymptotic in $K\langle a \rangle$. To do that we apply Lemma~\ref{pa4} with $L=K(a)$, $F= K\langle a \rangle$ 
and $U=K[a]$.
Consider elements $u=g(a)$  with $g\in K[Y]\setminus K$, and 
$b\in K^\times$ such that $b\prec 1$; it suffices to show that then
$u' \prec b^\dagger$ if $u\prec 1$, and
$u' \preceq b^\dagger$ if $u\asymp 1$. If $u\asymp 1$, then we take
$s\in K$ with $u \sim s$ and use $s'\preceq b^\dagger$
to reduce to the case $u \prec 1$. So we assume $u\prec 1$.
Note that 
$v(u)= \text{eventual value of } v\big(g(a_\rho)\big)$,
so $v\big(g(a_\rho)\big)>0$ eventually, hence
$v\big( g(a_\rho)' \big)$ is eventually constant as a function of $\rho$, 
and $v\big( g(a_\rho)' \big)>v(b^\dagger)$ eventually.
Therefore it is enough to show:

\claim{$v(u')= \text{eventual value of $v\big(g(a_\rho)'\big)$}$.}

\noindent
Let $g=c_0 + c_1Y + \dots +c_nY^n$ ($c_i\in K$), and put
$g^*:=c_0' + c_1'Y + \dots +c_n'Y^n$, so
$$ u'\ =\  g(a)'\ =\  g^*(a) + g'(a)a', \qquad 
g(a_\rho)'\ =\  g^*(a_\rho) + g'(a_\rho)a_\rho'.$$
Therefore the claim holds if $P(Y,Y')$ is of degree $>1$ in $Y'$, so we can
assume 
$$P(Y,Y')\ =\ P_0(Y)+P_1(Y)Y'\qquad\text{where $P_0,P_1\in K[Y]$, $P_1\neq 0$.}$$
Put $R:=-P_0/P_1$. Then $P_1(a)\neq 0$ and $a'=R(a)$. 
Also $P_1(a_\rho)\neq 0$ eventually. We may assume that 
$P_1(a_\rho)\neq 0$ for all $\rho$. Then for each $\rho$ we have
\begin{equation}\label{formula for g(a_rho)'}
g(a_\rho)'\ =\  g^*(a_\rho) + g'(a_\rho)R(a_\rho) + 
g'(a_\rho)\big(a_\rho'-R(a_\rho)\big).
\end{equation}
Now $$v\big( g^*(a_\rho) + g'(a_\rho)R(a_\rho) \big)\  =\  
v\big( g^*(a) + g'(a)R(a) \big)$$ eventually. Also
$a_\rho'-R(a_\rho)=P(a_\rho,a_\rho')/P_1(a_\rho)$, hence 
$v\big(g'(a_\rho)\big(a_\rho'-R(a_\rho)\big)\big)$ is eventually 
strictly increasing. We have
$$v\big(g'(a_\rho)\big(a_\rho'-R(a_\rho)\big)\big)\ >\ 
v\big( g^*(a) + g'(a)R(a) \big)$$
eventually: otherwise,
$$v\big(g'(a_\rho)\big(a_\rho'-R(a_\rho)\big)\big)\ <\ 
v\big( g^*(a) + g'(a)R(a) \big)$$
eventually, and then, by \eqref{formula for g(a_rho)'},
$v\big(g(a_\rho)'\big)$ would be both eventually constant and eventually
strictly increasing. Hence
$$v\big(g(a_\rho)')\ =\   v\big( g^*(a) + g'(a)R(a) \big)\ =\  v(u')$$
eventually, proving the claim. Thus $K\langle a \rangle$ is an 
asymptotic field.

\medskip\noindent
It remains to prove item (2). But this follows easily from the above,
since any $b$ as in (2) is transcendental over $K$, and can serve
as $e$ in the arguments above. 
\end{proof}

\subsection*{Notes and comments} Suppose $K$ has small derivation and~$P$ (of order $\le 1$) is homogeneous
of degree $d\geq 1$, with $d\Gamma=\Gamma$. Then the function
$v_P\colon\Gamma\to\Gamma$ is a strictly
increasing bijection, by the Equalizer Theorem. For this case, however, we have a more constructive (unpublished) argument leading to the stronger result that 
the function 
$\gamma\mapsto \textstyle\frac{1}{d}v_P(\gamma)\colon\Gamma\to\Gamma$ is
$\psi$-steady. \marginpar{need to check this is correct}





==> mt-9.tex <==

\chapter{Asymptotic Differential Fields}\label{ch:asymptotic differential fields}

\noindent
The key restriction on valued differential fields in Chapter~\ref{ch:valueddifferential}
was the {\em continuity\/} of the derivation. (Strictly speaking, we assumed
the derivation $\der$ to be {\em small}, but continuity of $\der$
reduces by compositional conjugation to smallness of $\der$.)

In this chapter we introduce asymptotic differential fields:
valued differential
fields with a much stronger interaction of the valuation 
and derivation.
For brevity we just call them {\em asymptotic fields}.
They include Rosenlicht's differential-valued fields~\cite{Rosenlicht2} 
and share 
many of their basic properties. The advantage of
the class of asymptotic fields over its subclass of differential-valued 
fields is that the former is closed under taking 
valued differential subfields,
under coarsening, and even under specialization 
(subject to a mild restriction). 





\medskip\noindent
A key feature of an asymptotic field is its asymptotic couple, which is 
just its value group
with some extra structure induced by the derivation. Asymptotic couples of
differential-valued fields were introduced by Rosenlicht~\cite{Rosenlicht2}. 
In Section~\ref{As-Fields,As-Couples}
we define asymptotic fields and their asymptotic couples. In 
Section~\ref{AbstractAsymptoticCouples} we consider asymptotic couples  
independent of their connection to asymptotic fields. This gets used
in Section~\ref{Applicationtodifferentialpolynomials} to describe 
the behavior of differential polynomials as functions on asymptotic fields.
In Section~\ref{Asymptotic-Fields-Section} we  discuss Hardy fields, $H$-fields, and Liouville closures of $H$-fields, 
and summarize some facts about them from the literature. In Section~\ref{Asymptotic-Fields-Basic-Facts} we
consider asymptotic fields with small derivation
and the operations of coarsening and specialization. 
In Section~\ref{pafae} we show that algebraic extensions of 
asymptotic fields are asymptotic fields. In Section~\ref{ImmExtAs} we 
adapt the results on immediate extensions from Section~\ref{sec:cimex}
to asymptotic fields.
In Section~\ref{Solving Homogeneous First-Order Equations} we show how to 
adjoin integrals and
exponential integrals to asymptotic fields. Section~\ref{caseorderone} treats differential polynomials of order one over so-called $H$-asymptotic fields.
Section~\ref{Miscellaneous Facts about Asymptotic Fields} contains 
miscellaneous facts about asymptotic fields.  

This chapter and the next include some new parts but are mainly based on
\cite{Rosenlicht2, , , , } most of


\input{mt-9-1}
\input{mt-9-2}
\input{mt-9-3}
\input{mt-9-4}
\input{mt-9-5}
\input{mt-9-6}
\input{mt-9-7}
\input{mt-9-8}
\input{mt-9-9}
\input{mt-9-10}


==> mt-modth-old.tex <==

\let\thetheorem\thetheoremold


\chapter{Basic Model Theory} \label{app:modth}\label{app:modeltheory}


\noindent
This appendix is written for readers unfamiliar with model theory.
It provides a full treatment of
the model-theoretic concepts used in our work:
back-and-forth, compactness, types, model completeness, quantifier elimination, and (in a different vein) NIP. 
We adopt a many-sorted setting from the outset. In the first four sections we 
specify the notion of a {\em model-theoretic structure\/} and
build up a formalism for handling these structures
rigorously and efficiently in the rest of the appendix. 
%We have included these matters since we do not like the usual textbook accounts.   
%For more information we refer to the textbooks~\cite{ChangKeisler,Hodges,Marker,Poizat,TentZiegler}. 
%We learnt much about the history of the subject from \cite{Chang,Hodges00,Lascar,Vaught74}.



\section{Structures and their Definable Sets} \label{sec:structures and definable sets}

\noindent
In this section we associate to a {\it structure}\/ 
its category of {\it definable sets and definable maps.}\/ 
The notion of structure introduced below is very general and includes not only
familiar (one-sorted) algebraic objects such as groups and rings, but also two-sorted structures such as group actions and topological spaces. 

In the case of a field,
the definable sets include the solution sets of finite systems of polynomial
equations, but as we shall see, the notion of definable set goes beyond this by allowing boolean operations and  projections. 


 
\subsection*{Model-theoretic structures}
A (model-theoretic) {\bf structure} consists of: 
\begin{list}{}{\leftmargin=2.5em }
\item[(S1)] a family $(M_s)_{s\in S}$ of nonempty sets $M_s$,
\item[(S2)] a family $(R_i)_{i\in I}$ of relations
$R_i\subseteq M_{s_1}\times\cdots \times M_{s_m}$
on these sets, with the tuple $(s_1,\dots,s_m)\in S^m$ determined by the index $i\in I$, and
\item[(S3)] a family $(f_j)_{j\in J}$ of functions 
$f_j\colon M_{s_1}\times\cdots \times M_{s_n}\to M_{s}$
with the tuple $(s_1,\dots,s_n,s)\in S^{n+1}$ determined by the index~$j\in J$. 
\end{list}
Notation:
$$\mathbf M\ =\ \big( (M_s); (R_i), (f_j) \big).$$
The elements of the index set $S$ are called {\bf sorts}, and $M_s$ is the {\bf underlying set} of sort~$s$ of $\mathbf M$. 
Elements of $M_s$ are also called ``elements of $\mathbf M$ of sort~$s$''.
The $R_i$ and~$f_j$ are called the {\bf primitives} of $\mathbf M$. For $m=0$ the set $S^m$ has the empty tuple as its only element, and the product $M_{s_1}\times\cdots \times M_{s_m}$ is then a singleton, that is, a one-element set. For $n=0$ in (S3), the function~$f_j$ is then identified with its unique value in $M_{s}$ and is called a {\bf constant.} The family $M=(M_s)$ is said to {\bf underly} the structure $\mathbf M$, or, abusing language, to be the {\bf underlying set} of $\mathbf M$.


\index{structure} \index{structure!primitives} \index{structure!underlying set} \index{structure!sorts} \index{structure!constant} 
\index{primitives}  \index{sorts} \index{constant}
 
One  calls $\mathbf M$ as above an {\bf $S$-sorted structure}.
If $S$ is finite of size $n$, then we also speak of an {\bf $n$-sorted structure}.
% and if $S$ has
%more than two elements, of a {\bf many-sorted structure.}
Many texts only consider one-sorted structures, so~$S$ doesn't need to be mentioned. But the extra generality adds useful flexibility and is natural, since many mathematical structures are often many-sorted to begin with. In fact, virtually anything that mathematicians consider as a structure can be viewed as a structure in the above sense. We only mention a few examples here; more are discussed in~\ref{ex:L-structures} below. 

In specifying one-sorted structures we often take the liberty of using the same capital letter for the underlying set of the structure as for the structure itself. 

\begin{examplesNumbered}\label{ex:structures}\mbox{}

\begin{enumerate} 
\item Any (additively written) abelian group $M$ is construed naturally as a one-sorted structure 
$(M;0,{-},{+})$ with the constant $0\in M$ and the functions
$$a\mapsto -a\colon M\to M, \quad (a,b)\mapsto a+b\colon M\times M\to M.$$
\item Every ring $R$ is viewed naturally as a one-sorted structure $(R;0,1,{-},{+},{\,\cdot\,})$ with
constants $0$, $1$ and functions 
$$ r\mapsto -r\colon R\to R, \ \ (r,s)\mapsto r+s\colon R\times R\to R,\  \
  (r,s)\mapsto r\cdot s\colon R\times R\to R.\quad $$
\item Let $R$ be a ring  and $M$ an $R$-module. Then $M$ can be viewed as a one-sorted structure, equipped with the functions in (1) 
and for each $r\in R$ the function $a\mapsto ra\colon M\to M$.
\item
Sometimes it is convenient to construe a module~$M$ over a ring $R$ as a {\em two-sorted \/}structure, one sort with underlying set $R$ and the same functions as in~(2),
the other sort with underlying set $M$ and the same functions as in~(1), as well as with a function $(r,a)\mapsto ra\colon R\times M\to M$ for the action of $R$ on~$M$.
\item A nonempty ordered set in the sense of Section~\ref{sec:ordered sets} is the same thing as a one-sorted structure
$(M;{\leq})$ where the binary relation $\leq$ on $M$ is reflexive, antisymmetric, transitive, and total.
\item An incidence geometry is a two-sorted structure consisting of a nonempty set~$P$ whose elements are called points, a nonempty set $L$ whose elements are called lines, and a relation $R\subseteq P\times L$ between points and lines.  
For example, a nonempty topological space can be viewed as an incidence geometry, taking the underlying set of the space for $P$, the collection of open sets for $L$, and the membership relation between points and open sets for $R$.  
\end{enumerate}
\end{examplesNumbered}


\subsection*{Definable sets}
Let $\mathbf M=\big( M; (R_i), (f_j) \big)$  be an $S$-sorted structure as above, where $M=(M_s)$. The main role of the primitives of $\mathbf M$ is to generate the {\it definable sets}\/ of $\mathbf M$. 
Let $\mathbf s=s_1\dots s_m$ and 
$\mathbf t=t_1\dots t_{n}$ be elements of $S^*$, that is, words on the alphabet $S$. 
Then $\mathbf s\mathbf t=s_1\dots s_m t_1\dots t_{n}\in S^*$ is the concatenation of $\mathbf s$ and $\mathbf t$. We set
$M_{\mathbf s}:=M_{s_1}\times\cdots\times M_{s_m}$, and identify $M_{\mathbf s}\times M_{\mathbf t}$ with $M_{\mathbf s\mathbf t}$ in the obvious way. 

\medskip\noindent
There is no need to require $M_s\cap M_{t}=\emptyset$ for distinct $s, t\in S$. (This would be
unnatural in Example (4) above, since $R$ is naturally an
$R$-module.) Instead we impose the convention
that in referring to an element $a\in M_{\mathbf s}$, this is short for a reference to an ordered pair $(a,\mathbf{s})$ such that $a\in M_{\mathbf s}$.
A similar convention is in force when we refer to a set $X\subseteq M_{\mathbf s}$. Given a map $f\colon X\to Y$, where $X\subseteq M_{\mathbf s}$, $Y\subseteq M_{\mathbf t}$, we let
$\Gamma(f)\subseteq M_{\mathbf s\mathbf t}$ be the graph of 
$f$. 

\begin{definition}\label{def:0-definable} \index{structure!definable set} \index{set!$0$-definable} \index{set!absolutely definable}
The {\bf $0$-definable} (or absolutely definable) sets of $\mathbf M$ are the relations $X\subseteq M_{\mathbf s}$
%, with $\mathbf s$ part of the specification 
obtained recursively as follows:
\begin{list}{}{\leftmargin=1em }
\item[(D1)] the relations $R_i\subseteq M_{s_1\dots s_m}$ and the graphs $\Gamma(f_j)\subseteq M_{s_1\dots s_n s}$ are $0$-definable;
\item[(D2)] if $X,Y\subseteq M_{\mathbf s}$ are $0$-definable, then so are $X\cup Y\subseteq M_{\mathbf s}$ and $(M_{\mathbf s}\setminus X)\subseteq M_{\mathbf s}$;
\item[(D3)] if $X\subseteq M_{\mathbf s}$ and $Y\subseteq M_{\mathbf t}$ are $0$-definable, then so is
$X\times Y\subseteq M_{\mathbf s\mathbf t}$;
\item[(D4)] for all distinct $i,j\in \{1,\dots,m\}$ with $s_i=s_j$,  
the diagonal 
$$\Delta_{ij}:=\big\{ (x_1,\dots,x_m)\in M_{\mathbf s}:x_i=x_j\big\}$$ is $0$-definable;
\item[(D5)] if $X\subseteq M_{\mathbf s\mathbf t}$ is $0$-definable, then so is  $\pi(X)\subseteq M_{\mathbf s}$, where $\pi\colon M_{\mathbf s\mathbf t}\to M_{\mathbf s}$ is the obvious projection map.
\end{list}
\end{definition}


\noindent
We extend this notion to {\it $A$-definability.}\/ Here $A$ is a so-called {\bf parameter set} in $\mathbf M$, that is,  a family $A=(A_s)$ with $A_s\subseteq M_s$ for each~$s$ (shorthand: $A\subseteq M$).
Then the structure $\mathbf M_A$ is obtained from $\mathbf M$ by adding for each $a\in A_s$ the constant $a\in M_s$ as a primitive. The {\bf $A$-definable sets} of $\mathbf M$ are just the $0$-definable sets of~$\mathbf M_A$. 
The parameter set $A$ with $A_s=\emptyset$ for each $s$ is also denoted by $0$, so $\mathbf M_0=\mathbf M$
and the terminology ``$0$-definable'' is unambiguous.
Instead of ``$M$-definable'' we just write ``definable''; so all finite sets $X\subseteq M_{\mathbf s}$ are definable. 
%A map $f\colon X\to X'$ ($X\subseteq M_{\mathbf s}$, $X'\subseteq M_{\mathbf s'}$) is said to be $A$-definable if its graph $\Gamma(f)\subseteq M_{\mathbf s\mathbf s'}$  is $A$-definable. (By (D5), the domain $X=\pi(\Gamma(f))\subseteq M_{\mathbf s}$ of $f$ is then automatically $A$-definable.)

For any family $(A_i)_{i\in I}$ of parameter sets in 
$\mathbf M$ we let $\bigcup_i A_i$ be the parameter set $A$ in $\mathbf M$ such that $A_s=\bigcup_i A_{i,s}$ for every $s\in S$.

\index{parameter set} \index{structure!parameter set} \index{set!parameter} \index{set!$A$-definable} \index{set!definable}\index{definable!set}

\subsection*{Describing definable sets}
For constructing new definable sets  from old ones,  it is convenient to systematize the correspondence between sets and the conditions used to define them. Let $x$ be a variable ranging over a set
$X$, and let $\phi(x)$, $\psi(x)$ be formulas (``conditions'' on $x$) defining the subsets  
$$\Phi := \big\{x \in X  : \text{$\phi (x)$ holds} \big\}\quad\text{and}\quad
  \Psi := \big\{x \in X  : \text{$\psi (x)$ holds} \big\}$$
of $X$. (We will make this precise in Section~\ref{sec:formulas} below.)
Various logical operations on formulas
correspond to operations on the sets that these formulas define:
\begin{list}{}{\leftmargin=2.5em } 
\item[(C1)] $\neg \phi (x)$ defines the complement $X\setminus\Phi$;
\item[(C2)] $\phi(x)\vee\psi(x)$ defines the union  $\Phi \cup \Psi$;
\item[(C3)] $\phi(x) \wedge \psi(x)$, also written as $\phi(x) \, \& \, \psi(x)$, defines the intersection $\Phi \cap \Psi$;
this set can also be defined by $\neg(\neg\phi(x)\vee\neg\psi(x))$.
\end{list}
Moreover, if $y$ is a variable ranging over a set $Y$ and $\theta(x,y)$ is a formula defining the subset $\Theta$ of $X\times Y$, then
\begin{list}{}{\leftmargin=2.5em }
\item[(C4)] $\exists  y\,  \theta(x,y)$  defines   $\pi  (\Theta)
\subseteq X$  where $\pi\colon X\times Y\to X$ is the natural projection;
\item[(C5)]
$\forall y \,\theta(x,y)$ defines the set $\big\{  x \in X : \{ x \}
\times Y \subseteq \Theta \big\}$; note that $\neg \exists y\, \neg  \theta(x,y)$ defines the same subset of $X$.
\end{list}
Thus, with $X=M_{\mathbf s}$ and  $Y=M_{\mathbf t}$, if the sets $\Phi$, $\Psi$ defined by $\phi(x)$, $\psi(x)$ are 
$A$-definable, then so are the sets defined by $\neg \phi(x)$,  $\phi(x)\vee\psi(x)$,
$\phi(x) \wedge \psi(x)$, and if
 $\Theta$ is $A$-definable, then so are the
sets defined by $\exists  y \, \theta(x,y)$  and $\forall y\, \theta(x,y)$.
The advantage of the logical formalism is that it is often more suggestive and transparent than
traditional set-theoretic notation, in particular when quantifiers are involved:

\begin{example} Let $A\subseteq \R$, and let $\mathbf M=(\R;\dots)$ be a one-sorted structure  with the usual ordering $\leq$ 
of the real line among the $A$-definable subsets of $\R^2$. Equip $\R^m$ with its usual product topology.
Suppose $X\subseteq \R^m$ is $A$-definable (in $\mathbf M$). Then the interior $\operatorname{int}(X)$
of $X$ in the ambient space $\R^m$ is $A$-definable. To see this, note that, with $\phi  \to  \psi$ short for $(\neg \phi) \vee \psi$, 
we have the equivalence
$$ x \in  \operatorname{int}(X)\quad \Longleftrightarrow \quad
\exists  u\, \exists  v\,  \big[ ( u <  x <  v)\ \&\ \forall  y\, ( u <  y <  v \to  y \in X)\big]$$
where $ u$, $ v$, $ x$, $ y$ range over $\R^m$ and $ u< x< v$ is short for
$$u_1<x_1<v_1 \ \&\ \cdots\ \& \ u_m<x_m<v_m.$$
Likewise, if $f\colon X\to \R$ is $A$-definable (that is, if its graph $\Gamma(f)$ is $A$-definable), then the set 
$\{x\in X:\text{$f$ is continuous at $x$}\}$ is easily seen to be $A$-definable. 
%, thanks to the equivalence
%\begin{multline*}
%\text{$f$ is continuous at $\vec x$} \quad \Longleftrightarrow \quad \\ \forall s \forall t \big[s<f(\vec x)<t \to \exists \vec u \, \exists \vec  v \, \big(\vec u <  \vec x < \vec v  \, \& \, \forall \vec y \, ( \vec u <  \vec y < \vec v \to s < f(\vec y) <t)\big)\big].
%\end{multline*}
\end{example}


\noindent
In general the $0$-definable relations of a structure cannot be described in a way that is significantly more explicit than the  recursive definition in \ref{def:0-definable}. 
For example, this is the case for the ring $\Z$ viewed as  a one-sorted structure as in Example~\ref{ex:structures},~(3);
see \cite[\S{}7.5]{Shoenfield} for details. But in some cases, a more explicit description does exist. One example is the field $\C$ of complex numbers; here we construe~$\C$ as a one-sorted structure as in \ref{ex:structures},~(2 ). (Including also as a primitive, say, $x\mapsto x^{-1}\colon \C^\times\to\C$,
extended to a total function $\C\to\C$ by declaring $0^{-1}:=0$, wouldn't add to the $0$-definable relations of~$\C$.)
Then by the Chevalley-Tarski constructibility theorem the $0$-definable subsets of $\C^n$ are just the
finite unions of sets  
$$\big\{ a\in \C^n:\  P_1(a) = \cdots = P_m(a) = 0,\ Q(a)\neq 0\big\}$$
with $P_1,\dots,P_m,Q\in \Q[X_1,\dots,X_n]$. For a subfield $A$ of $\C$ as a parameter set we get the same description of the $A$-definable subsets of $\C^n$ but now the polynomials have their coefficients in $A$. The above goes through for any algebraically closed field $K$ instead of $\C$, with the prime field of $K$ in place of $\Q$. So in this case the notion of ``$A$-definable'' is akin to Weil's notion of an algebraic variety defined over $A$. (Model-theoretic notions are often similar to foundational items in Weil's algebraic geometry.)
Another prominent example, more relevant to our work, where a concise description of the definable sets is available is the field $\R$ of real numbers.
Here, by the Tarski-Seidenberg Theorem, the $0$-definable subsets of $\R^n$ are the
{\it $\Q$-semialgebraic}\/ subsets of $\R^n$, that is, finite unions of sets
of the form
$$\big\{ a\in \R^n:\  P(a) = 0,\ Q_1(a) > 0, \dots, Q_m(a) > 0 \big\}$$
with $P,Q_1,\dots,Q_m\in \Q[X_1,\dots,X_n]$.
Note that the usual ordering relation on $\R$ is $0$-de\-finable in the field $\R$:
$$x\leq y\quad\Longleftrightarrow\quad \exists z\, [ z^2=y-x ].$$
In this appendix we develop some tools which allow us to 
identify  benign structures, like $\C$ and $\R$, 
whose definable sets allow such explicit descriptions. The theorems of Chevalley-Tarski and Tarski-Seidenberg are proved in Section~\ref{sec:some theories}. 

\index{theorem!Chevalley-Tarski}
\index{theorem!Tarski-Seidenberg}

\subsection*{Conventions and notations} Let $M=(M_s)$ and $M'=(M'_s)$ be families of sets indexed by a set $S$. 
The {\it size}\/ $|M|$ of $M$ is defined to be the sum 
$\sum |M_s|$ of the cardinalities of the sets $M_s$, in other words, it is the cardinality of the disjoint union 
$\bigcup_s M_s\times\{s\}$. 
%So if $\kappa$ is an infinite cardinal, $|S| < \kappa$, 
%and $|M_s| < \kappa$ for all $s$, 
%then $|M| < \kappa$.  
%We say that $M$ is {\it finite}\/ if
%$|M|$ is finite, {\it infinite}\/ if $|M|$ is infinite, and {\it countable}\/ if~$|M| \leq \aleph_0$.  
We set $M\subseteq M'$ iff $M_s\subseteq M'_s$ for all~$s$. 
%We put $M'\setminus M:=(M'_s\setminus M_s)$, and
%if $(A_i)_{i\in I}$ is a family where  $A_i=(A_{i,s})\subseteq M$ for each $i\in I$, then 
%$\bigcap_i A_i := (\bigcap_i A_{i,s})$ and
%$\bigcup_i A_i := (\bigcup_i A_{i,s})$.
%If $(a_i)_{i\in I}$ and $(s_i)_{i\in I}$ are families with $s_i\in S$ and $a_i\in M_{s_i}$ for each $i\in I$, then we denote by $\{a_i:i\in I\}$ the family $A\subseteq M$ with $A_s=\{a_i: s_i=s\}$ for each $s$.
% \marginpar{Reintroduced definition of set-theoretic operations on parameter sets, since these are used freely throughout.}
A map $h\colon M\to M'$ is a family $h=(h_s)$ of maps $h_s\colon M_s\to M'_s$.
Let $h=(h_s)$ be such a map $M\to M'$.
We say that~$h$ is {\it injective}\/ if each $h_s$ is injective, and similarly with ``surjective'' or ``bijective'' in place of ``injective''.
Given $\mathbf s=s_1\dots s_m\in S^*$ and  $a=(a_1,\dots,a_m)\in M_{\mathbf s}$ we put $ha=h_{\mathbf s}a:=(h_{s_1}a_1, \dots , h_{s_m}a_m)\in M'_{\mathbf s}$. For $A=(A_s)\subseteq M$ we put $h(A):=\big(h(A_s)\big)\subseteq M'$.
Given also $M'':= (M''_s)$ and a map $h'\colon M'\to M''$, we let $h'\circ h$ denote the map $M\to M''$ given
by $(h'\circ h)_s=h'_s\circ h_s$ for all~$s$.


\subsection*{Notes and comments}
The idea of ``structure'' emerged in the 19th century in algebra 
(Dedekind) and the foundations of 
mathematics~\cite{Hilbert99,Schroeder}. It led to the structural point of view in algebra, later extended by Bourbaki to other parts of mathematics; see~\cite{Corry}.
In the early literature in mathematical logic, structures were called  systems until 
the current terminology came into widespread use in the 1950s (see for example \cite{Robinson52}), perhaps under the influence of Bourbaki. 

Following de Morgan~\cite{deMorgan46}, the underlying set $M_s$ of sort $s$ of a structure $\mathbf M$ 
is sometimes also called  the {\it universe}\/ of sort $s$ of $\mathbf M$. 
The notion of definable set can be traced back to Weyl~\cite{Weyl}, but became more familiar after Kuratowski and Tarski~\cite{KT31} spelled out the above
correspondence between logical connectives and set-theoretic operations.



\section{Languages}\label{sec:languages}

\noindent
In this section we formalize the idea of {\em structures of the same kind\/} by defining the category of {\it $\mathcal L$-structures\/} for a given (model-theoretic) {\it language $\mathcal L$}. We also discuss various constructions
with $\mathcal L$-structures: products, direct limits.

\subsection*{Languages} \index{language} \index{sorts} \index{language!sorts} \index{language!relation symbols} \index{language!function symbols} \index{language!constant symbols} \index{symbols!function} \index{symbols!relation} 
A {\bf language} $\mathcal L$ is a triple $(S,\mathcal L^{\operatorname{r}},\mathcal L^{\operatorname{f}})$ consisting of
\begin{list}{}{\leftmargin=2.5em}
\item[(L1)] a set $S$ whose elements are the {\bf sorts} of $\mathcal L$,
\item[(L2)] a set $\mathcal L^{\operatorname{r}}$ whose elements are the {\bf relation symbols} of $\mathcal L$, and
\item[(L3)] a set $\mathcal L^{\operatorname{f}}$ whose elements are the {\bf function symbols} of $\mathcal L$,
\end{list}
where $\mathcal L^{\operatorname{r}}$ and $\mathcal L^{\operatorname{f}}$  are disjoint, each $R \in \mathcal L^{\operatorname{r}}$  is equipped with a word $s_1\dots s_m\in S^*$, called its {\bf sort},
and each $f \in \mathcal L^{\operatorname{f}}$ is equipped with a {\bf sort} $s_1\dots s_n s\in S^*$. 
The elements of $\mathcal L^{\operatorname{r}}\cup \mathcal L^{\operatorname{f}}$ are  called {\bf nonlogical symbols} of~$\mathcal L$.  \index{symbols!nonlogical}
We also call~$\mathcal L$ an {\bf $S$-sorted language,} with the same linguistic conventions as for structures if~$S$ is finite.
It is customary in practice to present a  language  
as a disjoint union $\mathcal L=\mathcal L^{\operatorname{r}}\cup\mathcal L^{\operatorname{f}}$ 
of its sets of relation and function symbols,
while separately specifying the set $S$ of sorts as well as the kind (relation symbol or function symbol) and sort of each nonlogical symbol of~$\mathcal L$.
If $R\in \mathcal L^{\operatorname{r}}$ has sort $s_1\dots s_m\in S^*$, then we also call $R$
an {\bf $m$-ary} relation symbol of $\mathcal L$;  similarly  a function symbol of $\mathcal L$ of sort $s_1\dots s_n s$
is called an $n$-ary function symbol of $\mathcal L$.
Instead of ``$0$-ary'', ``1-ary'', ``2-ary'' we say ``nullary'', ``unary'', ``binary'', respectively. A {\bf constant symbol}
is a nullary function symbol.  An $m$-ary relation symbol of sort $s\dots s$ is also said to be of sort $s$;
an $n$-ary function symbol of sort $s\dots ss$  is said to be of sort $s$. \index{symbols!constant}

\index{language!extension}\index{extension!language}\index{sublanguage}\index{language!sublanguage}

A language
$\mathcal L' = (S',\mathcal L'^{\operatorname{r}},\mathcal L'^{\operatorname{f}})$
is called an {\bf extension} of a language
$\mathcal L = (S,\mathcal L^{\operatorname{r}},\mathcal L^{\operatorname{f}})$ 
(and $\mathcal L$ is a {\bf sublanguage} of $\mathcal L$)
if $S \subseteq S'$, $\mathcal L^{\operatorname{r}}\subseteq \mathcal L'^{\operatorname{r}}$,  
 $\mathcal L^{\operatorname{f}}\subseteq \mathcal L'^{\operatorname{f}}$, and each nonlogical symbol of $\mathcal L$  has the same sort in $\mathcal L'$ as it has in $\mathcal L$;
 notation: $\mathcal L\subseteq\mathcal L'$.
%If $\mathcal L=(S,\mathcal L^{\operatorname{r}},\mathcal L^{\operatorname{f}})$ and 
%$\mathcal L'=(S',\mathcal L'^{\operatorname{r}},\mathcal L'^{\operatorname{f}})$ are two   languages with 
%$\mathcal L^{\operatorname{r}}\cap \mathcal L'^{\operatorname{r}}=\emptyset$ and
%$\mathcal L^{\operatorname{f}}\cap \mathcal L'^{\operatorname{f}}=\emptyset$, then we define their
% {\bf union} as the language $$\mathcal L\cup\mathcal L':=(S\cup S', \mathcal L^{\operatorname{r}}\cup \mathcal L'^{\operatorname{r}}, \mathcal L^{\operatorname{f}}\cap \mathcal L'^{\operatorname{f}}),$$ where each nonlogical symbol of $\mathcal L$ is assigned the same sort in $\mathcal L\cup\mathcal L'$ as it is in $\mathcal L$, and similarly for the nonlogical symbols of $\mathcal L'$.

\begin{examplesNumbered}\label{ex:languages}
\mbox{}

\begin{enumerate}
\item The one-sorted language $\mathcal L_{\operatorname{G}}=\{ 1, {\ }^{-1}, {\, \cdot\,} \}$ of 
groups has constant
symbol $1$, unary function symbol ${\ }^{-1}$, and binary function symbol $\cdot\,$. %\nomenclature[Bex1]{$\mathcal L_{\operatorname{Gr}}$}{language of groups}

\item The one-sorted language $\mathcal L_{\operatorname{A}}=\{ 0, {-}, {+} \}$ of 
(additive) abelian groups has constant
symbol $0$, unary function symbol $-$, and binary function symbol $+$. %\nomenclature[Bex2]{$\mathcal L_{\operatorname{Ab}}$}{language of abelian groups}

\item The one-sorted language $\mathcal L_{\operatorname{R}}=\{ 0, 1, {-}, {+}, {\,\cdot\,}\}$ of rings
is the extension of $\mathcal L_{\operatorname{A}}$ by a constant symbol $1$ and a binary function symbol $\cdot\,$. \nomenclature[Bex3]{$\mathcal L_{\operatorname{R}}$}{language of rings}

\item The one-sorted language $\mathcal L_{\operatorname{O}}=\{ {\leq} \}$ of ordered sets has just one binary relation symbol $\leq$. \nomenclature[Bex4]{$\mathcal L_{\operatorname{O}}$}{language of ordered sets}

\item Combining (2) and (4) yields the one-sorted language $\mathcal L_{\operatorname{OA}}=\{{\leq},0, {-}, {+} \}$ of ordered abelian groups. Combining (3) and (4) yields
the one-sorted language $\mathcal L_{\operatorname{OR}}=\{ {\leq}, 0, 1, {-}, {+}, {\,\cdot\,}\}$
of ordered rings. \nomenclature[Bex51]{$\mathcal L_{\operatorname{OA}}$}{language of ordered abelian groups} \nomenclature[Bex52]{$\mathcal L_{\operatorname{OR}}$}{language of ordered rings}
\item Let $R$ be a ring. The language $\mathcal L_{\text{$R$-mod}}=
\mathcal L_{\operatorname{A}}\cup\{ {\lambda_r} \colon r\in R\}$ of $R$-modules is the one-sorted language which
extends $\mathcal L_{\operatorname{A}}$ by unary function symbols $\lambda_r$, one for each $r\in R$.
%\nomenclature[Bex6]{$\mathcal L_{\text{$R$-mod}}$}{language of $R$-modules}

\item The language $$\mathcal L_{\operatorname{Mod}}=\{ 0_{\operatorname{R}},1_{\operatorname{R}},{-_{\operatorname{R}}},{+}_{\operatorname{R}},{\,\cdot\,}_{\operatorname{R}},
0_{\operatorname{M}},{-}_{\operatorname{M}},{+}_{\operatorname{M}},\lambda\}$$ of modules (with unspecified scalar ring)
is a two-sorted language with sorts~$\operatorname{R}$ and~$\operatorname{M}$.
Here the symbols indexed with a subscript $\operatorname{R}$ are of sort $\operatorname{R}$,
and similarly for $\operatorname{M}$. The symbols
$0_{\operatorname{R}}$,~$1_{\operatorname{R}}$, $0_{\operatorname{M}}$ are constant symbols, 
${-_{\operatorname{R}}}$, ${-_{\operatorname{M}}}$ are unary function symbols, and 
${+}_{\operatorname{R}}$, ${\,\cdot\,}_{\operatorname{R}}$, ${+}_{\operatorname{M}}$  are binary function symbols. The symbol $\lambda$ is a function symbol of sort $\operatorname{R}\operatorname{M}\operatorname{M}$. %\nomenclature[Bex7]{$\mathcal L_{\operatorname{Mod}}$}{language of modules}
\end{enumerate}
\end{examplesNumbered}




\noindent
{\it In the rest of this appendix $\mathcal L$ is a language with $S$ as its set of sorts, unless specified
otherwise. We let $s$ \textup{(}possibly subscripted\textup{)} range over $S$ and $\mathbf s=s_1\dots s_m$ over~$S^*$.}\/ 
The {\bf size} of $\mathcal L$ is the cardinal
$$\abs{\mathcal L}\ :=\  \max\big\{\aleph_0, \abs{S}, \abs{\mathcal L^{\operatorname{r}}\cup\mathcal L^{\operatorname{f}}}\big\},$$
and we say that $\mathcal L$ is {\bf countable} if $\abs{\mathcal L} = \aleph_0$, that is, $S$, $\mathcal  L^{\operatorname{r}}$, and $\mathcal L^{\operatorname{f}}$ are countable.  \index{language!size} \index{language!countable}

\subsection*{$\mathcal L$-structures}
An {\bf $\mathcal L$-structure} is an $S$-sorted structure
$$\mathbf M\ =\ \big( M; (R^{\mathbf M})_{R\in \mathcal L^{\operatorname{r}}}, (f^{\mathbf M})_{f\in \mathcal L^{\operatorname{f}}} \big)\qquad \text{where $M=(M_s)$,}$$
such that for every $R\in \mathcal L^{\operatorname{r}}$
of sort $s_1\dots s_m$ its {\bf interpretation $R^{\mathbf M}$} in $\mathbf M$ is a subset of~$M_{s_1\dots s_m}$, and for $f\in \mathcal L^{\operatorname{f}}$ of sort 
$s_1\dots s_n s$ its {\bf interpretation~$f^{\mathbf M}$} in $\mathbf M$ is a function $M_{s_1\dots s_n}\to M_{s}$. For a constant symbol $c$ of $\mathcal L$ of sort $s$ the corresponding $M_s$-valued function $c^{\mathbf M}$ is identified with its unique value in $M_s$, so $c^{\mathbf M}\in M_s$. If~$\mathbf M$ is understood from the context we often omit the superscript $\mathbf M$ in denoting the interpretation in $\mathbf M$ of a nonlogical symbol of $\mathcal L$.  The reader is supposed to keep in mind the distinction between symbols
of $\mathcal L$ and their interpretation in an $\mathcal L$-structure, even if we use the same notation
for both.   \index{structure!$\mathcal L$-structure} \index{$\mathcal L$-structure} \index{interpretation} \index{structure!interpretation}

\begin{examplesNumbered}\label{ex:L-structures}
\mbox{}

\begin{enumerate}
\item Every group is considered as an $\mathcal L_{\operatorname{G}}$-structure by interpreting the symbols $1$, ${\ }^{-1}$, and $\cdot$ as the identity element of the group, its group inverse, and its group multiplication, respectively.
\item Let $\mathbf A=(A; 0,{-},{+})$ be an abelian group; here $0 \in A$ is the zero element
of the group, and ${-}\colon A \to A$ and ${+} \colon A^2 \to A$ denote the group operations
of $\mathbf A$. We consider $\mathbf A$ as an $\mathcal L_{\operatorname{A}}$-structure by taking as interpretations of
the symbols $0$, $-$ and $+$ of $\mathcal L_{\operatorname{A}}$ the group operations $0$, $-$ and $+$ on $A$.
(We took here the liberty of using the same notation for possibly entirely
different things: $+$ is an element of the set $\mathcal L_{\operatorname{A}}^{\operatorname{f}}$, but also denotes in this
context its interpretation as a binary operation on the set $A$. Similarly
with $0$ and $-$.) In fact, any set~$A$ in which we single out an element, a
unary operation on $A$, and a binary operation on $A$, can be construed as
an $\mathcal L_{\operatorname{A}}$-structure if we choose to do so.
\item Likewise, any ring is construed as an $\mathcal L_{\operatorname{R}}$-structure in the obvious way.
\item
$(\N; {\leq})$ is an $\mathcal L_{\operatorname{O}}$-structure where we interpret $\leq$ as the usual ordering
relation on $\N$. Similarly for $(\Z; {\leq})$, $(\Q; {\leq})$ and $(\R; {\leq})$. (Here we take
even more notational liberties, by letting $\leq$ denote five different things: a
symbol of $\mathcal L_{\operatorname{O}}$, and the usual orderings of $\N$, $\Z$, $\Q$, and $\R$ respectively.)
Again, any nonempty set  equipped with a binary relation on it can be
viewed as an $\mathcal L_{\operatorname{O}}$-structure.
\item Any ordered abelian group is an $\mathcal L_{\operatorname{OA}}$-structure.
%\item $(\Z; 0, 1, {-}, {+} , {\,\cdot\,})$, $(\R; 0, 1, {-}, {+} , {\,\cdot\,})$, and $(\C; 0, 1, {-}, {+} , {\,\cdot\,})$ are $\mathcal L_{\operatorname{Ri}}$-structures.
\item The ordered ring of integers and any ordered field are $\mathcal L_{\operatorname{OR}}$-structures.
\item Let $R$ be a ring and $M$ be an $R$-module. Then $M$ becomes an $\mathcal L_{\text{$R$-mod}}$-structure by interpreting the symbols of $\mathcal L_{\operatorname{A}}$ as in (2) and the function symbol~$\lambda_r$~($r\in R$) by the function $x\mapsto rx\colon M\to M$.
We can also construe~$M$ as an $\mathcal L_{\operatorname{Mod}}$-structure 
whose underlying set of sort~$\operatorname{R}$ is $R$ and
whose underlying set of sort~$\operatorname{M}$ is $M$, and where
the symbols $0_{\operatorname{R}}$,~$1_{\operatorname{R}}$,~${-_{\operatorname{R}}}$,~${+}_{\operatorname{R}}$,~${\,\cdot\,}_{\operatorname{R}}$ are interpreted by the ring operations on $R$,
the symbols $0_{\operatorname{M}}$,~${-}_{\operatorname{M}}$,~${+}_{\operatorname{M}}$ by the group
operations on $M$, and $\lambda$ by $(r,x)\mapsto rx\colon R\times M\to M$.
\end{enumerate}
\end{examplesNumbered}

\noindent
Let
$\mathcal L'$ be an $S'$-sorted extension of $\mathcal L$ (so
$S'\supseteq S$). An
$\mathcal L'$-structure $\mathbf M' = \big(M'; \dots\big)$ is said to be an {\bf $\mathcal L'$-expansion} of an $\mathcal L$-structure
 $\mathbf M=(M;\dots)$ (and
$\mathbf M$ is said to be the {\bf $\mathcal L$-reduct} of $\mathbf M'$) if $M_s = M'_s$ for all $s$, and each
nonlogical symbol of $\mathcal L$ has the same interpretation in~$\mathbf M$ as in $\mathbf M'$. 
Given such an $\mathcal L'$-expansion $\mathbf M'$ of $\mathbf M$ we sometimes abuse notation by letting a parameter set $A = (A_s)$ in $\mathbf M$ denote also the parameter set $(A_{s'})_{s'\in S'}$ in~$\mathbf M'$, where $A_{s'} = \emptyset$ 
for~$s' \in S' \setminus S$.  \index{structure!expansion}\index{structure!reduct} \index{expansion}\index{reduct}

\begin{example} The ordered field of reals is an $\mathcal L_{\operatorname{OR}}$-expansion of 
the real line, where ``the real line'' stands for the $\mathcal L_{\operatorname{O}}$-structure $(\R; {\leq})$.
\end{example}

\subsection*{Substructures} Let $\mathbf M=(M;\dots)$ and
$\mathbf N=(N;\dots)$ be $\mathcal L$-structures.
Then $\mathbf M$ is called a {\bf substructure} of $\mathbf N$  (notation: $\mathbf M\subseteq\mathbf N$) if $M_s\subseteq N_s$ for all $s$, and 
\begin{align*}
R^{\mathbf N}\cap M_{s_1\dots s_m}\ 	&=\  R^{\mathbf M}	&	& \text{whenever $R\in\mathcal L^{\operatorname{r}}$ has sort $s_1\dots s_m$},\\
f^{\mathbf N}|_{M_{s_1\dots s_n}}\ 	&=\  f^{\mathbf M}\colon M_{s_1\dots s_n}\to M_{s}	&	& \text{whenever $f\in\mathcal L^{\operatorname{f}}$ has sort $s_1\dots s_n s$.}
\end{align*}
We also say in this case that {$\mathbf N$ \bf is an extension of $\mathbf M$} or that {$\mathbf N$ \bf extends $\mathbf M$}. For groups, this is just the notion of subgroup, and for rings the notion of subring.\index{structure!substructure}\index{substructure}\index{extension!of $\mathcal L$-structures}\index{structure!extension}

\nomenclature[Bj00]{$\mathbf M\subseteq\mathbf N$}{$\mathbf M$ is a substructure of $\mathbf N$}

%\begin{examples} \mbox{}
%\begin{enumerate}
%\item $(\Z; 0, 1, {-}, {+} , {\,\cdot\,})\subseteq (\R; 0, 1, {-}, {+} , {\,\cdot\,}) \subseteq (\C; 0, 1, {-}, {+} , {\,\cdot\,})$;
%\item $(\N;{\leq})\subseteq (\Z;{\leq}) \subseteq (\Q;{\leq}) \subseteq (\R;{\leq})$.
%\end{enumerate}
%\end{examples}

\subsection*{Morphisms}
Let $\mathbf M$ and $\mathbf N$ be $\mathcal L$-structures. \index{morphism} \index{structure!morphism}
A {\bf morphism} $h \colon \mathbf M \to \mathbf N$ is a map $h\colon M\to N$ that respects the primitives of $\mathbf M$,  that is:
\begin{list}{}{\leftmargin=2.5em}
\item[(M1)] for every  $R\in\mathcal L^{\operatorname{r}}$ of sort $s_1\dots s_m$ and all 
$a \in M_{s_1\dots s_m}$,
$$a\in R^{\mathbf M} \quad\Rightarrow\quad h_{s_1\dots s_m}a \in R^{\mathbf N};$$
\item[(M2)] for every $f\in\mathcal L^{\operatorname{f}}$ of sort $s_1\dots s_n s$
and all $a \in M_{s_1\dots s_n}$,
$$h_{s}\big(f^{\mathbf M}(a)\big)\ =\ f^{\mathbf N}(h_{s_1\dots s_n}a).$$
\end{list}
Replacing $\Rightarrow$ in (M1) by $\Longleftrightarrow$ 
and also requiring $h$ to be injective
yields the notion of an {\bf embedding}. 
An {\bf isomorphism} is a bijective
embedding, and an {\bf automorphism} of $\mathbf M$ is an isomorphism $\mathbf M\to\mathbf M$. 
If $\mathbf M \subseteq \mathbf N$, then the inclusions $a\mapsto a \colon M_s \to N_s$ yield an embedding $\mathbf M \to \mathbf N$, called the {\bf natural inclusion} of  $\mathbf M$ into $\mathbf N$.
Conversely, a morphism $h \colon \mathbf M \to \mathbf N$ yields a substructure~$h(\mathbf M)$ of~$\mathbf N$ 
whose 
underlying set of sort~$s$ is  $h_s(M_s)$, and if $h$ is an embedding we have an isomorphism $\mathbf M \to h(\mathbf M)$ given by 
$$a\mapsto h_s(a)\colon M_s\to h(M_s).$$
If $h\colon  \mathbf M\to \mathbf M'$ and $h' \colon \mathbf M' \to\mathbf M''$ are morphisms (embeddings, isomorphisms, respectively), then so is $h'\circ h \colon \mathbf M \to\mathbf M''$.
The automorphisms of $\mathbf M$ form a group~$\Aut(\mathbf M)$ under composition. A parameter set~$A$ in $\mathbf M$
yields the subgroup 
$$\Aut(\mathbf M|A)\ :=\ \big\{f\in\Aut(\mathbf M): \text{$f_s(a) = a$ for every $s$ and $a \in A_s$ } \big\}$$
of $\Aut(\mathbf M)$. We write $\mathbf M\cong\mathbf N$ if there is an isomorphism $\mathbf M\to\mathbf N$.
\index{structure!isomorphism}\index{isomorphism!of $\mathcal L$-structures}\index{automorphism!of an $\mathcal L$-structure}\index{structure!automorphism}\index{embedding!of $\mathcal L$-structures}\index{structure!embedding}
\index{structure!natural inclusion} \index{natural inclusion}

\nomenclature[Bk1]{$\Aut(\mathbf M)$}{group of automorphisms of $\mathbf M$}
\nomenclature[Bk2]{$\Aut(\mathbf M\lvert A)$}{group of automorphisms of $\mathbf M$ over $A$}
\nomenclature[Bj1]{$\mathbf M\cong\mathbf N$}{$\mathbf M$, $\mathbf N$ are isomorphic}


\begin{examples} 
If $\mathbf M$ and $\mathbf N$ are abelian groups, construed as $\mathcal L_{\operatorname{A}}$-structures according to~\ref{ex:L-structures},~(2), then a
morphism $\mathbf M\to\mathbf N$ is exactly what in algebra is called a (homo)morphism
from the group $\mathbf M$ into the group $\mathbf N$. Likewise with rings, and other kinds of
algebraic structures. 
\end{examples}

%\noindent
%Let $\mathcal L'$ be an extension of $\mathcal L$ and $h'=(h'_{s'})_{s'\in S'}\colon\mathbf M'\to\mathbf N'$ be a morphism
%of $\mathcal L'$-structures. Let $\mathbf M$, $\mathbf N$ be the $\mathcal L$-reducts of $\mathbf M$, $\mathbf N$, respectively. Then $h:=(h'_s)_{s\in S}$ is a morphism $\mathbf M\to\mathbf N$, which we call the
%$\mathcal L$-reduct of $h$. Clearly if $h'$ is an embedding (isomorphism, automorphism, respectively), then so is
%$h$.

\subsection*{Products} \index{structure!product}
Now let $(\mathbf N_\lambda)_{\lambda\in\Lambda}$ be a family of $\mathcal L$-structures,
where $\Lambda\neq\emptyset$, and
let $\lambda$ range over $\Lambda$. For each $s$ 
put $N_s:=\prod_{\lambda} (N_\lambda)_s$. (The Axiom of Choice guarantees that $N_s\neq\emptyset$.)
We write the typical element of~$N_s$ as $a=\big(a(\lambda)\big)$.
For  $a=(a_1,\dots,a_m)\in N_{\mathbf s}$,   put 
$$a(\lambda)\ :=\ \big(a_1(\lambda),\dots,a_m(\lambda)\big)\in (N_\lambda)_{\mathbf s}.$$
The {\bf product} $\prod_{\lambda} \mathbf N_\lambda$ of $(\mathbf N_\lambda)$ 
is defined to be the $\mathcal L$-structure $\mathbf N$ whose underlying set of sort $s$ is $N_s$, and where the basic relations and functions are defined coordinatewise:
for $R\in\mathcal L^{\operatorname{r}}$ of sort $s_1\dots s_m$ and $a\in N_{s_1\dots s_m}$
$$a\in R^{\mathbf N} \quad:\Longleftrightarrow\quad \text{$a(\lambda)\in R^{\mathbf N_\lambda}$ for all $\lambda$},$$
and for $f\in\mathcal L^{\operatorname{f}}$ of sort $s_1\dots s_n s$
and $a\in N_{s_1\dots s_n}$,
$$f^{\mathbf N}(a)\  :=\  \big(f^{\mathbf N_\lambda}(a(\lambda)) \big) \in N_s.$$
For each $\lambda$ the projection to the $\lambda$th factor is the morphism $\pi_\lambda=\pi_\lambda^{\mathbf N}\colon\mathbf N\to\mathbf N_\lambda$
given by $(\pi_{\lambda})_s(a)=a(\lambda)$ for $a\in N_s$.
This product construction makes it possible to combine several morphisms
with a common domain into a single one: if for each~$\lambda$ we have a morphism
$h_\lambda \colon \mathbf M \to \mathbf N_\lambda$, then we obtain a morphism $h\colon \mathbf M\to \mathbf N$
with $\pi_\lambda\circ h = h_\lambda$ for each $\lambda$. If each $h_\lambda$ is an embedding, then so is~$h$.
This yields: \index{embedding!diagonal} \index{diagonal!embedding}

\begin{lemma}\label{lem:morphisms on products}
For each $\lambda$, let $h_\lambda\colon\mathbf M_\lambda\to\mathbf N_\lambda$ be a morphism. Then we have a morphism $h\colon \mathbf M:=\prod_\lambda \mathbf M_\lambda\to \mathbf N=\prod_\lambda \mathbf N_\lambda$ such that $\pi_\lambda^{\mathbf N}\circ h = h_\lambda\circ\pi_\lambda^{\mathbf M}$ for all~$\lambda$.
If every $h_\lambda$ is an embedding, then so is $h$.
\end{lemma}

\noindent
If $\mathbf N_\lambda=\mathbf M$ for all~$\lambda$, then $\prod_\lambda \mathbf N_\lambda$ is denoted by $\mathbf M^\Lambda$;
in this case we have an embedding $\Delta\colon\mathbf M\to \mathbf M^\Lambda$ with 
$\big(\Delta_s(a)\big)(\lambda) = a$ for all $a\in M_s$ and $\lambda$, called the 
{\bf diagonal embedding} of~$\mathbf M$ into $\mathbf M^\Lambda$.

%\subsection*{Congruences}
%A {\bf congruence} on the $\mathcal L$-structure $\mathbf M$ is a family $({\sim_s})$ where each~$\sim_s$ is an   equivalence relation on the underlying set $M_s$  of sort $s$, such that
%\begin{list}{}{\leftmargin=2.5em}
%\item[(C1)] if $R\in\mathcal L^{\operatorname{r}}$ has arity $s_1\cdots s_m$  and $a_i,b_i\in M_{s_i}$ ($i=1,\dots,m$) satisfy $a_i\sim_{s_i} b_i$  ($i=1,\dots,m$), then
%$$(a_1, \dots, a_m) \in R^{\mathbf M}\quad\Longleftrightarrow\quad (b_1, \dots , b_m) \in R^{\mathbf M};$$
%\item[(C2)] if $f\in\mathcal L^{\operatorname{f}}$ has arity $s'_1\cdots s'_n s$ and  $a_i,b_i\in M_{s'_i}$ ($i=1,\dots,n$) satisfy  $a_i\sim_{s'_i} b_i$  ($i=1,\dots,n$),
%then $$f^{\mathbf M}(a_1,\dots,a_n) \sim_s f^{\mathbf M}(b_1,\dots,b_n).$$
%\end{list}
%Note that a strong morphism $h\colon\mathbf M \to \mathbf N$ yields a congruence $({\sim_{h,s}})$ on $\mathbf M$  by setting $a \sim_{h,s} b :\Longleftrightarrow  h_s(a) = h_s(b)$ for $a,b\in M_s$.

%Let $\sim$ be a congruence on the $\mathcal L$-structure $\mathbf M$. Denote the equivalence class of $a\in M_s$ with respect to $\sim_s$ by 
%$$a^{\sim}:=\{b\in M_s:b\sim_s a\}.$$
%We obtain an $\mathcal L$-structure~$\mathbf M/{\sim}$ (the {\bf quotient} of $\mathbf M$ by $\sim$) as follows:
%\begin{list}{}{\leftmargin=2.5em}
%\item[(Q1)] the underlying set of  $\mathbf M/{\sim}$ of sort $s$ is the  set $M_s/{\sim_s}:=\{a^\sim:a\in M_s\}$  of equivalence classes of elements of $M_s$;
%\item[(Q2)] the interpretation of an  $R\in\mathcal L^{\operatorname{r}}$ of arity $s_1\cdots s_m$  in $\mathbf M/{\sim}$ is the relation
%$$\big\{ (a_1^{\sim},\dots,a_m^{\sim}:(a_1,\dots,a_m)\in R^{\mathbf M}\big\}\subseteq (M/{\sim})_{s_1\cdots s_m};$$
%\item[(Q3)] the interpretation of an $f\in\mathcal L^{\operatorname{f}}$ of arity $s'_1\cdots s'_n s$ in $\mathbf M/{\sim}$ is the function
%$$(M/{\sim})_{s_1'\cdots s_n'}\to (M/{\sim})_s\colon \ (a_1^{\sim},\dots,a_n^{\sim})  \mapsto f^{\mathbf M}(a_1,\dots,a_n)^{\sim}.$$
%\end{list}
%We then have a strong morphism $h\colon\mathbf M\to \mathbf M/{\sim}$ given by $a\mapsto a^{\sim} \colon M_s \to (M/{\sim})_s$, and $\sim_h$ agrees with $\sim$.


\subsection*{Direct limits}
Let $\Lambda$ be a nonempty partially ordered set, and let $\lambda, \lambda',\lambda_1, \lambda_2,\dots$ range over~$\Lambda$. Suppose that $\Lambda$ is {\bf directed}, that is, for all $\lambda_1$,~$\lambda_2$ there exists~$\lambda$ with $\lambda_1, \lambda_2\leq \lambda$.
A {\bf directed system} of $\mathcal L$-structures indexed by $\Lambda$
consists of a family $(\mathbf M_\lambda)$
of $\mathcal L$-structures together with a family $(h_{\lambda\lambda'})_{\lambda\leq\lambda'}$ of
morphisms $h_{\lambda\lambda'}\colon \mathbf M_\lambda \to \mathbf M_{\lambda'}$ such that
 $h_{\lambda\lambda}=\operatorname{id}_{\mathbf M_{\lambda}}$ for all $\lambda$
and 
 $h_{\lambda\lambda''}=h_{\lambda'\lambda''}\circ h_{\lambda\lambda'}$ whenever $\lambda\leq\lambda'\leq\lambda''$.
Suppose that $\big((\mathbf M_\lambda),(h_{\lambda\lambda'})\big)$ is a directed system 
of $\mathcal L$-structures indexed by $\Lambda$. For this situation we have the following routine lemma. \index{directed system} \index{structure!directed system}

\begin{lemma}
There
exists an $\mathcal L$-structure $\mathbf M$ and a family $(h_\lambda)$ of morphisms $h_\lambda\colon\mathbf M_\lambda\to\mathbf M$ with the following properties:
\begin{enumerate}
\item if $\lambda\leq\lambda'$, then $h_\lambda = h_{\lambda'} \circ h_{\lambda\lambda'}$;
\item if $\mathbf N$ is an $\mathcal L$-structure and $(f_\lambda)$ is a family of morphisms
$f_\lambda\colon \mathbf M_\lambda\to\mathbf N$ such that $f_\lambda=f_{\lambda'}\circ h_{\lambda\lambda'}$ whenever $\lambda\leq\lambda'$, then there is a unique morphism $g\colon \mathbf M\to\mathbf N$ such
that $f_\lambda=g\circ h_\lambda$ for all $\lambda$.
\end{enumerate}
\end{lemma}
%\begin{proof}
%For each $s$ let $U_s$ be the disjoint union of the underlying sets $(M_\lambda)_s$ of sort~$s$ of the
%$\mathbf M_\lambda$. Define a relation $\sim_s$ on $U_s$ by declaring, for $a_i\in (M_{\lambda_i})_s$ 
%($i=1,2$): $a_1\sim_s a_2$ iff there is some $\lambda$ with $\lambda_i\leq\lambda$ ($i=1,2$) and $h_{\lambda_1\lambda}(a_1)=h_{\lambda_2\lambda}(a_2)$.
%One verifies easily that $\sim_s$ is an equivalence relation on $U_s$. 
%Let $a^\sim$ denote the equivalence class of $a\in U_s$ with respect to $\sim_s$, and
%let $M_s:=\{ a^\sim: a\in U_s\}$. For each $\lambda$ and $s$ we let  $(h_\lambda)_s(a):=a^\sim$ for $a\in (M_\lambda)_s$. Set $M:=(M_s)$ and  $h_\lambda:=\big( (h_\lambda)_s \big)\colon M_\lambda \to M$; then $h_\lambda=h_{\lambda'}\circ h_{\lambda\lambda'}$ whenever $\lambda\leq\lambda'$.
%We now turn $M$ into an $\mathcal L$-structure $\mathbf M$  as follows:
%For $R\in\mathcal L^{\operatorname{r}}$ of sort $\mathbf s$ and $b\in M_{\mathbf s}$ put
%$$b\in R^{\mathbf M} \quad:\Longleftrightarrow\quad \text{
%there is some $\lambda$ and $a\in R^{\mathbf M_\lambda}$ such that $(h_\lambda)_{\mathbf s}(a)=b$.}$$
%For $f\in\mathcal L^{\operatorname{f}}$ of sort $\mathbf s' s$ and $b\in M_{\mathbf s'}$,
%take $\lambda$ and $a\in (M_\lambda)_{\mathbf s'}$  such that $(h_\lambda)_{\mathbf s'}(a)=b$; then 
%the element $(h_\lambda)_s(f^{\mathbf M_\lambda}(a))$ of $M_s$ does not depend on $a$,~$\lambda$,
%and we set
%$$f^{\mathbf M}(b) := (h_\lambda)_s(f^{\mathbf M_\lambda}(a)).$$
%One easily checks that then each  $h_\lambda$ is a morphism $\mathbf M_\lambda\to\mathbf M$, and $\mathbf M$ and $(h_\lambda)$ satisfy conditions~(1) and (2).
%\end{proof}
   
\noindent   
We call an $\mathcal L$-structure $\mathbf M$ together with 
a family $(h_\lambda)$ of morphisms $h_\lambda\colon\mathbf M_\lambda\to\mathbf M$
as in the previous lemma a {\bf direct limit} of the directed system
$((\mathbf M_\lambda),(h_{\lambda\lambda'}))$.
If $\mathbf M$,~$(h_\lambda)$ and $\tilde{\mathbf M}$,~$(\tilde h_\lambda)$ are two direct limits of
$((\mathbf M_\lambda),(h_{\lambda\lambda'}))$,  then the unique morphism $h\colon \mathbf M\to \tilde{\mathbf M}$ such that
$\tilde h_\lambda = h\circ h_\lambda$ for all $\lambda$ is actually an isomorphism.
This allows us to speak of {\it the}\/ direct limit of $((\mathbf M_\lambda),(h_{\lambda\lambda'}))$. 
One verifies easily that 
if all $h_{\lambda\lambda'}$ are embeddings, then so are all $h_\lambda$.
 \index{direct!limit} \index{structure!direct limit}


\medskip
\noindent
Now let $(\mathbf M_\lambda)$ be a family of $\mathcal L$-structures such that for $\lambda\leq\lambda'$,
$\mathbf M_\lambda$ is a substructure of~$\mathbf M_{\lambda'}$, with
natural inclusion $h_{\lambda\lambda'}\colon\mathbf M_{\lambda}\hookrightarrow \mathbf M_{\lambda'}$.
Then $\big((\mathbf M_\lambda),(h_{\lambda\lambda'})\big)$ is a  directed system of $\mathcal L$-structures, and its direct limit $\bigcup_{\lambda\in\Lambda} \mathbf M_\lambda$,~$(h_\lambda)$ is called  the {\bf direct union} of $(\mathbf M_\lambda)$.
In the following we always identify each $\mathbf M_\lambda$ with a substructure of $\bigcup_{\lambda\in\Lambda} \mathbf M_\lambda$
via the embedding $h_\lambda$, and we also simply speak of $\bigcup_{\lambda\in\Lambda} \mathbf M_\lambda$ as the direct union of 
$(\mathbf M_\lambda)$. \index{direct!union} \index{structure!direct union}


\begin{exampleNumbered}\label{ex:Fpalg}
View fields as  $\mathcal L_{\operatorname{R}}$-structures in the natural way.
The algebraic closure~$\mathbb F_p^\alg$ of the finite field $\mathbb F_p$ with $p$ elements is the direct union
of the family of finite subfields of $\mathbb F_p^\alg$.
\end{exampleNumbered}

\subsection*{Notes and comments}
What we call here a language is also known as a {\it signature,}\/ or a {\it vocabulary.}\/ 
Uncountable languages first appear explicitly in \cite{Malcev36},
and many-sorted languages and structures were first considered by Herbrand~\cite{Herbrand} and Schmidt~\cite{Schmidt38,Schmidt51}.  Most structures occurring in mathematical practice are one-sorted or two-sorted, but
structures with infinitely many sorts do naturally arise in model theory. For example, even if the structure $\mathbf M$
is one-sorted, the structure~$\mathbf M^{\operatorname{eq}}$ associated to $\mathbf M$ by Shelah~\cite[III.6]{Shelah78} is most naturally viewed as infinitely-sorted; see \cite[Section~4.3]{Hodges}. 

\section{Variables and Terms}

\noindent
{\it In the rest of this appendix $\mathbf M=(M;\dots)$ and $\mathbf N=(N;\dots)$ are $\mathcal L$-structures unless noted otherwise.}\/ In this section and the next we introduce the syntax (variables, terms, formulas) that helps to specify the definable sets of $\mathbf M$ along the lines of~\ref{sec:structures and definable sets},
uniformly for all $\mathcal L$-structures $\mathbf M$.  

\subsection*{Variables}
We assume that for each sort $s$ we have available  infinitely  many symbols, called {\bf variables of sort $s$}, chosen so that if $s$ and $s'$ are different sorts, then no variable of sort $s$ is a variable of sort $s'$. We also assume that no variable of any sort is a nonlogical symbol of any language.
A {\bf variable} of $\mathcal L$ is a variable of some sort~$s$, and a {\bf multivariable} of $\mathcal L$ is a tuple $x=(x_i)_{i\in I}$ of {\it distinct}\/ variables of $\mathcal L$.
The size of the index set $I$ is called the size of $x$, and the $x_i$ are called the variables in $x$.
Often the index set $I$ is finite, say $I=\{1,\dots,n\}$, so that $x=(x_1,\dots,x_n)$;
in this case, if $x_i$ is of sort $s_i$ ($i=1,\dots,n$), we say that $x$ is of sort $s_1\dots s_n$.
Instead of ``$x$ has finite size'' we also say ``$x$ is finite''. Let $x=(x_i)_{i\in I}$ be a multivariable of~$\mathcal L$, with $x_i$ of sort $s_i$ for $i\in I$. We define the {\bf $x$-set} of~$\mathbf M$ as
$$M_x := \prod_{i\in I} M_{s_i},$$
and we think of $x$ as a variable running over $M_x$.  
When $I=\emptyset$, then
$x$ is said to be {\bf trivial}, and
$M_x$ is a 
singleton. If $h\colon \mathbf M\to\mathbf N$ is a morphism, we obtain a map 
$(a_i) \mapsto \big(h_{s_i}(a_i)\big)\colon M_x\to N_x$ between $x$-sets,
which we denote by $h_x$.
For a parameter set $A=(A_s)$ in $\mathbf M$,  we set
$$A_x := \prod_{i\in I} A_{s_i} \subseteq M_x.$$
Multivariables $x=(x_i)_{i\in I}$ and $y=(y_j)_{j\in J}$ of $\mathcal L$ are said to be {\bf disjoint} if $x_i\neq y_j$ for all $i\in I$, $j\in J$, and in that case we put $M_{x,y}:=M_x\times M_y$.
%If in addition $I=J$ and $x_i$ and $y_i$ have the same sort for all $i\in I$ (so that $M_x=M_y$), then we call $x$ {\bf disjoint and similar.} 
From now on $x$ and~$y$ denote multivariables of $\mathcal L$, unless specified otherwise.

\index{variable} \index{multivariable} \index{language!variable} \index{language!multivariable} \index{structure!$x$-set} \index{multivariable!disjoint} \index{multivariable!trivial}

\subsection*{Terms}
We define {\bf $\mathcal L$-terms} to be words on the alphabet consisting of the function
symbols and variables of $\mathcal L$, obtained recursively as follows: 
\begin{list}{}{\leftmargin=2.5em}
\item[(T1)] each variable of
sort~$s$, when viewed as a word of length~$1$, is an $\mathcal L$-term of sort $s$, and
\item[(T2)]
if $f$ is a function symbol of $\mathcal L$ of sort $s_1\cdots s_n s$ and $t_1, \dots , t_n$ are $\mathcal L$-terms of sort $s_1, \dots, s_n$ respectively, then $ft_1 \cdots t_n$ is an $\mathcal L$-term of sort~$s$.
\end{list}
Thus every constant symbol of $\mathcal L$ of sort $s$ is an $\mathcal L$-term of sort $s$.
Usually we write $f(t_1, \dots , t_n)$ to denote $ft_1 \dots t_n$,   
and shun prefix notation if dictated by tradition. \index{language!term} \index{term}

\begin{example}
The word ${\,\cdot\,}{+}x{-}yz$ is an $\mathcal L_{\operatorname{R}}$-term in the official prefix notation. For easier reading we indicate
this term instead by $(x + (-y)) \cdot z$ or even $(x - y)z$.
\end{example}

\noindent
The following allows us to give definitions and proofs by ``induction on terms''.

\begin{lemma}\label{lem:unique readability, terms}
Every $\mathcal L$-term of sort $s$ is either a variable of sort $s$, or equals $ft_1\dots t_n$ for a unique tuple
$(f, t_1,\dots, t_n)$ with $f$ an $n$-ary function symbol of some sort $s_1\dots s_ns$, and $t_i$ an $\mathcal L$-term of sort $s_i$ for $i=1,\dots,n$.
\end{lemma}

\noindent
For now we shall assume this lemma without proof. At the
end of this section we establish more general results which are also needed in the next section.

\medskip
\noindent
Let $x$ be a multivariable. An $(\mathcal L, x)$-term is a pair $(t, x)$ where $t$ is an $\mathcal L$-term such that each variable
in~$t$ is a variable in $x$.  Such an $(\mathcal L, x)$-term is also written more suggestively
as $t(x)$, and referred to as ``the $\mathcal L$-term $t(x)$''. 
(It is not required that each variable in~$x$ actually occurs in $t$; this is like indicating a polynomial in the indeterminates
$X_1, \dots, X_n$ by $P(X_1, \dots , X_n)$, where some of these indeterminates
might not occur in $P$. Note that only finitely many of the variables in $x$ can occur in any $\mathcal L$-term.)
Given an $\mathcal L$-term $t(x)$ of sort $s$, we define a function $$t^{\mathbf M}\colon M_x\to M_s$$ as follows,
with $a=(a_i)$ ranging over $M_x$:
\begin{enumerate}
\item if $t=x_i$, then $t^{\mathbf M}(a):=a_i$;
\item if $t=ft_1\cdots t_n$ where
$f\in\mathcal L^{\operatorname{f}}$ is of sort $s_1\dots s_n s$ and $t_1, \dots , t_n$ are 
$\mathcal L$-terms of sort $s_1, \dots, s_n$ respectively,
then $$t^{\mathbf M}(a):=f^{\mathbf M}\big(t_1^{\mathbf M}(a),\dots,t_n^{\mathbf M}(a)\big)\in M_s.$$
\end{enumerate}
This inductive definition is justified by Lemma~\ref{lem:unique readability, terms}.

\begin{example}
Let $R$ be a commutative ring viewed as an $\mathcal L_{\operatorname{R}}$-structure in the natural way.
Let $t(x, y, z)$ be the $\mathcal L_{\operatorname{R}}$-term 
$(x - y)z$. Then the function $t^{R}  \colon R^3 \to R$ is given by $t^R(a, b, c) = (a - b)c$.
In fact,
for each $\mathcal L_{\operatorname{R}}$-term $t(x_1,\dots,x_n)$
there is a (unique) polynomial $P^t(X_1,\dots,X_n)$ with integer coefficients such that for every commutative ring $R$ we have $t^R(a)=P^t(a)$ for all $a\in R^n$. Conversely, there is for each polynomial $P\in \Z[X_1,\dots, X_n]$ an 
$\mathcal L_{\operatorname{R}}$-term $t(x_1,\dots, x_n)$ such that $t^R(a)=P(a)$ for every commutative ring $R$ and all $a\in R^n$.
\end{example}

\noindent
Let $t(x)$ be an $\mathcal L$-term of sort $s$ and $a\in M_x$.
If $h\colon\mathbf M\to\mathbf N$ is a morphism of $\mathcal L$-structures, then
$h_s(t^{\mathbf M}(a))=t^{\mathbf N}(h_x(a))$; so  if
$\mathbf M\subseteq \mathbf N$, then $t^{\mathbf M}(a) = t^{\mathbf N}(a)$.
If~$\mathcal L'$ is an extension of~$\mathcal L$ and $\mathbf M'$ is an $\mathcal L'$-expansion of $\mathbf M$, then each $\mathcal L$-term $t(x)$ is also an $\mathcal L'$-term and
$t^{\mathbf M}=t^{\mathbf M'}\colon M_x \to M_s$.


\subsection*{Variable-free terms}
A term is said to be {\bf variable-free} if no variables occur in it. Let $t$ be a variable-free
$\mathcal L$-term of sort $s$. Then the above gives a nullary function~$t^{\mathbf M}$ with value in $M_s$, identified as usual with its value, so
$t^{\mathbf M} \in M_s$. In particular, if $t$ is a constant symbol $c$, then $t^{\mathbf M} = c^{\mathbf M} \in M_s$, where
$c^{\mathbf M}$ is as in Section~\ref{sec:languages}, and if $t = ft_1\dots t_n$ with $f\in\mathcal L^{\operatorname{f}}$ of sort $s_1\dots s_n s$ and
variable-free $\mathcal L$-terms $t_1,\dots,t_n$ of sorts $s_1,\dots,s_n$, respectively, then $t^{\mathbf M} = f^{\mathbf M}(t^{\mathbf M}_1, \dots, t^{\mathbf M}_n)\in M_s$.\index{term!variable-free}
%A family $(t_i)$ of $\mathcal L$-terms is said to be variable-free if each $t_i$ is variable-free.

\subsection*{Names} \index{language!name} \index{name}\index{symbols!names} \nomenclature[Bj0]{$\mathbf M_A$}{expansion of $\mathbf M$ by names for the elements of $A$}
Let $A\subseteq M$ be a parameter set.
We extend $\mathcal L$ to
a language $\mathcal L_A$ by adding a constant symbol $\underline{a}$ of sort $s$ for each $a \in A_s$, called the {\bf name}
of~$a$. These names are symbols not in $\mathcal L$. 
Note that $\abs{\mathcal L_A}=\max\{\abs{A},\abs{\mathcal L}\}$.
We make~$\mathbf M$ into an $\mathcal L_A$-structure by interpreting each name $\underline{a}$ as the element $a\in A_s$. The $\mathcal L_A$-structure thus
obtained is indicated by $\mathbf M_A$. (This is consistent with the notation introduced in Section~\ref{sec:structures and definable sets}.) Hence for each variable-free $\mathcal L_A$-term $t$ of sort $s$ we have
a corresponding element~$t^{\mathbf M_A}$ of~$M_s$, which for simplicity of notation we denote
instead by $t^{\mathbf M}$. All this applies  to the case $M = A$, where in $\mathcal L_M$ we
have a name~$\underline{a}$ for each element~$a$ of~$M_s$.
If $\mathbf M\subseteq\mathbf N$, then we consider $\mathcal L_M$ to be a sublanguage of~$\mathcal L_N$ in such a way
that each $a \in M$ has the same name in~$\mathcal L_M$ as in $\mathcal L_N$.
Then for each variable-free $\mathcal L_M$-term~$t$ we have $t^{\mathbf M} = t^{\mathbf N}$.
Given a multivariable $x=(x_i)$ of $\mathcal L$ and $a=(a_i)\in M_x$,  we set $\underline{a}:=(\underline{a_i})$. 

\subsection*{Substitution} \index{term!substitution} \index{substitution!into terms} 
Let $\alpha$ be an $\mathcal L_M$-term, $x=(x_i)_{i\in I}$ a multivariable, and
$t=(t_i)_{i\in I}$ a family of $\mathcal L_M$-terms
such that  $t_i$ is of the same sort as $x_i$, for each $i$. Then~$\alpha(t/x)$ denotes the word obtained by
replacing all occurrences of $x_i$ in $\alpha$ by $t_i$, {\it simultaneously}\/ for all $i$.
If $\alpha$ is given in the form $\alpha(x)$, then $\alpha(t)$ is short
for $\alpha(t/x)$ and for $a\in M_x$ we often write $\alpha(a)$ instead of $\alpha(\underline{a})$.

\begin{lemma}\label{lem:subst lemma, terms}
Let $\alpha(x)$ be an $\mathcal L_M$-term of sort $s$,
and recall that $\alpha$ defines a
map $\alpha^{\mathbf M}\colon M_{x} \to M_s$. Let $t=(t_i)_{i\in I}$ be a family of  $\mathcal L_M$-terms, with each $t_i$
of the same sort as $x_i$. Then $\alpha(t)$ is an $\mathcal L_M$-term of sort $s$.
Moreover, if all $t_i$ are variable-free, then so is~$\alpha(t)$, and 
with $a_i:= t_i^{\mathbf M}$, $a:=(a_i)\in M_x$ %and $\underline{a}:=(\underline{a}_i)$, 
we have
$$\alpha(t)^{\mathbf M}\ =\ \alpha(a)^{\mathbf M}\ =\  \alpha^{\mathbf M}(a).$$
\end{lemma} 

%\begin{lemma}[``Associativity of substitution'']\label{lem:assoc of subst} \marginpar{New lemma, used in the proof of \ref{lem:subst lemma, formulas}.}
%Let $\alpha(x)$ be an $\mathcal L$-term, let $y=(y_j)_{j\in J}$ be a multivariable, and let $t=(t_i)_{i\in I}$ and 
%$t'=(t_j')_{j\in J}$
%be families of $\mathcal L$-terms. Suppose that each
%$t_i(y)$ is of the same sort as $x_i$ and each $t_j'$ is of the same sort as $y_j$. 
%Then $$\alpha(t)(t')=\alpha(t(t')).$$
%\end{lemma}

\noindent
This follows by a straightforward induction on the length of $\alpha$. 
%We often omit the superscript $\mathbf M$ in expressions as in the lemma above when the ambient structure $\mathbf M$ is clear from the context.


\subsection*{Generators} \index{substructure!generators} \index{structure!generators}
Assume $\mathcal L$ has for each~$s$ a constant symbol of sort $s$. Let $A\subseteq M$ be given.
For each~$s$ we set
$$B_s\ :=\ \big\{t^{\mathbf M}(a):\ t(x) \text{ is an $\mathcal L$-term of sort~$s$, and~$a\in A_x$}\big\}\ \subseteq\ M_s .$$
Then $B=(B_s)$ underlies a substructure $\mathbf B=(B;\dots)$
of $\mathbf M$, and clearly $\mathbf B\subseteq \mathbf C$ for all substructures
$\mathbf C$ of $\mathbf M$ with $A\subseteq C$. We call~$\mathbf B$ the
substructure of~$\mathbf M$ {\bf generated} by $A$; notation: $\mathbf B=\<A\>_{\mathbf M}$. 
Note that $\abs{A}\leq \abs{\<A\>_{\mathbf M}}\leq\max\big\{\abs{A},\abs{\mathcal L}\big\}$.
If $\mathbf M = \<A\>_{\mathbf M}$, then we say that $\mathbf M$ is generated
by $A$.
If $\mathbf N$ is an $\mathcal L$-structure, then each map $A\to N$ has clearly at most one extension to a morphism $\<A\>_{\mathbf M}\to\mathbf N$. 
%Given a family $(a_i)_{i\in I}$ of elements   of $M$ and 
%$(s_i)_{i\in I}$ of $S$, if it is understood from the context that $a_i\in M_{s_i}$ for each $i\in I$,
%then we also write $\<a_i:i\in I\>_{\mathbf M}$ instead of~$\<A\>_{\mathbf M}$,
%where $A$ is the parameter set with $A_s=\{a_i:i\in I,\ s=s_i\}$. \marginpar{Changed this sentence.}
%For each morphism $h'\colon \<A\>_{\mathbf M}\to\mathbf N$ extending the map $h$ and each $\mathcal L$-term $t(x)$ of sort $s$ and $a\in A_x$ we have $h'_s(t^{\mathbf M}(a))=t^{\mathbf N}(h'_x(a))=t^{\mathbf N}(h_x(a))$.


\subsection*{Unique readability}
We finish this section with the promised general result on unique readability. 
We let $F$ be a set of symbols with a function $a \colon F \to \N$ (called the
{\bf arity} function). A symbol $f \in F$ is said to have arity $n$ if $a(f) = n$. 
A word on~$F$ is said to be {\bf admissible} if it can be obtained by applying the following rules:
\begin{enumerate}
\item If $f \in F$ has arity $0$, then $f$ viewed as a word of length $1$ is admissible.
\item If $f \in F$ has arity $n\geq 1$ and $t_1, \dots, t_n$ are admissible words on $F$, then
the concatenation $ft_1\dots t_n$ is admissible.
\end{enumerate}
Below we just write ``admissible word'' instead of ``admissible word on $F$''. Note
that the empty word is not admissible, and that the last symbol of an admissible
word cannot be of arity~$\geq 1$. \index{admissible!word}

\begin{example}
The $\mathcal L$-terms are admissible words on the alphabet consisting of the function symbols of $\mathcal L$ and the variables of $\mathcal L$, where each $n$-ary $f\in \mathcal L^{\operatorname{f}}$ has arity $n$ and each variable has arity $0$.  
\end{example}


\begin{lemma}
Let $t_1, \dots , t_m$ and $u_1, \dots, u_n$ be admissible words and $w$ any
word on $F$ such that $t_1 \dots t_mw = u_1 \dots u_n$. Then $m \leq n$, $t_i = u_i$ for $i =
1, \dots ,m$, and $w = u_{m+1} \dots u_n$.
\end{lemma}
\begin{proof}
By induction on the length $\ell$ of $u_1 \dots u_n$. If $\ell=0$, then $m = n = 0$ and~$w$ is the empty word. Suppose $\ell> 0$, and assume the lemma
holds for smaller lengths. Note that $n > 0$. If $m = 0$, then the conclusion of the
lemma holds, so suppose~$m > 0$. The first symbol of $t_1$ equals the first symbol
of $u_1$. Say this first symbol is $h \in F$ with arity $k$. Then $t_1 = ha_1\dots a_k$ and
$u_1 = hb_1  \dots b_k$ where $a_1, \dots, a_k$ and $b_1, \dots, b_k$ are admissible words. Cancelling
the first symbol $h$ gives
$$a_1 \dots a_k t_2 \dots t_m w = b_1 \dots b_k u_2 \dots u_n.$$
(Caution: any of $k$, $m-1$, $n-1$ could be $0$.) We have $\operatorname{length}(b_1\dots b_ku_2 \dots u_n) = \ell-1$, so the induction hypothesis applies. It yields $k + m  -1 \leq k + n - 1$ (so $m \leq n$), $a_1 = b_1, \dots , a_k = b_k$ (so $t_1 = u_1$), $t_2 = u_2$, \dots , $t_m = u_m$,
and $w = u_{m+1} \cdots u_n$.
\end{proof}

\noindent
In particular, if $t_1, \dots, t_m$ and $u_1, \dots , u_n$ are admissible words such that $t_1 \dots t_m =
u_1 \dots u_n$, then $m = n$ and $t_i = u_i$ for $i = 1,\dots ,m$. Thus:

\begin{cor}[Unique Readability]
Each admissible word equals $ft_1 \dots t_n$ for a unique tuple $(f,t_1,\dots,t_n)$ with $f \in F$ of arity
$n$ and $t_1, \dots , t_n$ admissible words.
\end{cor}

 




\section{Formulas}\label{sec:formulas}

\noindent
We now fix once and for all the eight {\bf logical symbols}:
$$\top \qquad \bot \qquad \neg  \qquad \vee \qquad \wedge \qquad = \qquad \exists \qquad \forall$$
to be thought of as {\it true,}\/ {\it false,}\/ {\it not,}\/ {\it or,}\/ {\it and,}\/ {\it equals,}\/ {\it there exists,}\/ and {\it for all,}\/ respectively.
These are assumed to be distinct from all nonlogical symbols
and variables of every language. 
The symbols $\neg$, $\vee$, $\wedge$ are called (logical) {\bf connectives}
and $\exists$,~$\forall$ are called {\bf quantifiers}.
It will be convenient to fix
once and for all a sequence $v_0, v_1, v_2,\dots$ of distinct
symbols, called {\em unsorted\/} variables, and to declare that for each sort 
$s$ the symbols $v_n^s$ are the {\bf quantifiable variables}\/ of sort $s$. For any $S$-sorted language $\mathcal{L}$ and
$s\in S$, these are
among its variables of sort $s$, but $\mathcal{L}$ can have other (unquantifiable) variables of sort $s$. 
A multivariable is called quantifiable if each variable in it is quantifiable. \index{symbols!logical}\index{logical!symbols}\index{symbols!connectives}\index{symbols!quantifiers} \index{variable!quantifiable} \index{multivariable!quantifiable}

\subsection*{Formulas} \index{formula!atomic} \index{atomic formula}
The {\bf atomic $\mathcal L$-formulas} are the following words  on the alphabet $$\mathcal{L}^{\text{r}}\cup\mathcal{L}^{\text{f}}\cup\{\text{variables of $\mathcal L$}\}\cup\{\top, \bot,{=}\}:$$  
\begin{list}{}{\leftmargin=2.5em }
\item[(A1)] $\top$ and $\bot$ (as words of length $1$);
\item[(A2)] the words $Rt_1\dots t_m$ where  $R\in\mathcal L^{\operatorname{r}}$ is of
sort $s_1\dots s_m$ and $t_1,\dots,t_m$ are $\mathcal L$-terms of sort $s_1,\dots,s_m$, respectively; 
\item[(A3)] the words ${=}t_1t_2$ where $t_1$, $t_2$ are $\mathcal L$-terms of the same sort. 
\end{list}
The {\bf $\mathcal L$-formulas} are the words on the alphabet 
$$ \mathcal{L}^{\text{r}}\cup\mathcal{L}^{\text{f}}\cup\{\text{variables of $\mathcal L$}\}\cup\{\top, \bot,{\neg}, {\vee},{\wedge},{=}, {\exists}, {\forall}\}$$ obtained as follows:
\begin{list}{}{\leftmargin=2.5em }
\item[(F1)] atomic $\mathcal L$-formulas are $\mathcal L$-formulas;
\item[(F2)] if $\varphi$, $\psi$ are $\mathcal L$-formulas, then so are $\neg\varphi$, $\vee\varphi\psi$, and
$\wedge\varphi\psi$;
\item[(F3)] if $\varphi$ is an $\mathcal L$-formula and $x$ is a quantifiable variable, then $\exists x\varphi$ and
$\forall x\varphi$ are $\mathcal L$-formulas.
\end{list}

\index{formula}
 
\begin{remarks}\mbox{}

\begin{enumerate}
\item Having the connectives $\vee$ and $\wedge$ in front of the $\mathcal L$-formulas they
``connect'' rather than in between, is called {\it prefix notation}\/ or {\it Polish notation.}\/
This is theoretically elegant, but for the sake of readability we usually write $\varphi\vee\psi$
and $\varphi\wedge\psi$ to denote $\vee \varphi\psi$ and $\wedge \varphi\psi$, respectively, and we also use parentheses and
brackets if this helps to clarify the structure of an $\mathcal L$-formula.  
\item All $\mathcal L$-formulas are admissible words on the alphabet consisting of the nonlogical
symbols of $\mathcal L$,  the variables of $\mathcal L$, and the eight logical symbols,
where~$\top$ and~$\bot$ have arity $0$, 
$\neg$ has arity $1$, 
$\vee$, $\wedge$, $=$, $\exists$ and $\forall$ have arity 2, and the other symbols have the arities
assigned to them earlier. Thus the results on unique readability
are applicable to $\mathcal L$-formulas. (However, not all admissible words on this alphabet
are $\mathcal L$-formulas: the word $\exists xx$ is admissible but not an $\mathcal L$-formula.)
\item  The reader should distinguish between different ways of using the symbol~$=$.
Sometimes it denotes one of the eight formal logical symbols, but we also use it
to indicate equality of mathematical objects in the usual way. The context should always make it clear what our intention is in
this respect without having to spell it out. To increase readability we usually
write an atomic formula ${=} t_1t_2$ as $t_1 = t_2$ and its negation $\neg{=}t_1t_2$ as $t_1 \neq t_2$,
where $t_1$, $t_2$ are $\mathcal L$-terms of the same sort. 
%The logical symbol $=$ is treated just as a binary relation symbol, but its interpretation in a structure will always be the equality relation on its underlying set. This will become clear later.
\end{enumerate}
\end{remarks}
\noindent
We shall use the following notational conventions: $\varphi \to \psi$ denotes $\neg\varphi \vee \psi$, and
$\varphi \leftrightarrow \psi$ denotes $(\varphi \rightarrow \psi) \wedge (\psi \rightarrow \varphi)$.   We sometimes write $\varphi\ \&\ \psi$ instead of~$\varphi \wedge \psi$.

 
\begin{definition}
Let $\varphi$ be an $\mathcal L$-formula. Written as a word on the alphabet introduced above
we have $\varphi = a_1 \dots a_m$. 
A {\bf subformula} of $\varphi$ is a subword of the 
form $a_i\dots a_k$ (where $1 \leq i \leq k \leq m$) which also happens to be an $\mathcal L$-formula.
An occurrence of a variable $x$ in $\varphi$ at the $j$th place (that is, $a_j = x$) is said
to be {\bf bound} if $\varphi$ has a subformula $a_ia_{i+1} \dots a_k$ with $i \leq j \leq k$ that
is of the form $\exists x\psi$ or $\forall x\psi$. An occurrence which is not bound is said to be {\bf free}. A {\bf free variable} of~$\varphi$ is a variable that occurs free in $\varphi$.  \index{variable!free} \index{formula!subformula} \index{subformula} \index{variable!free occurrence} \index{variable!bound occurrence}
\end{definition}

\begin{example}
In the $\mathcal L_{\operatorname{A}}$-formula 
$\big( \exists x(x = y) \big) \wedge x = 0$, where $x$ and $y$ are distinct variables, the first two occurrences of $x$ are bound, the third is free, and the only occurrence of $y$ is free.
(Note: this formula is actually the string $\wedge \exists x = xy = x0$, and the occurrences of $x$ and $y$ are the occurrences in this string.)
\end{example}

\noindent
An $(\mathcal L,x)$-formula is a pair $(\varphi,x)$ with $\varphi$ an $\mathcal L$-formula and $x$ a multivariable such that
all free variables of $\varphi$ are in $x$. Such an $(\mathcal L,x)$-formula is written more suggestively as $\varphi(x)$, and referred to as ``the $\mathcal L$-formula $\varphi(x)$''. Likewise, when referring to an $\mathcal L$-formula $\varphi(x,y)$ we really mean a triple $(\varphi,x,y)$ consisting of an $\mathcal L$-formula~$\varphi$ and disjoint multivariables $x$ and $y$ such that all free variables of $\varphi$ are in $x$ or $y$.
If $\mathcal L$ and $x$ both have size $\le \kappa$,
then the set of $(\mathcal L, x)$-formulas has size $\le \kappa$. 

\medskip
\noindent
An {\bf $\mathcal L$-sentence} is an $\mathcal L$-formula without free variables. 
The set of all $\mathcal L$-sentences has size $|\mathcal L|$.
(That is why we restricted $x$ to be quantifiable in (F3).) \index{sentence} \index{formula!sentence}


\subsection*{Substitution} Let $\varphi$ be an $\mathcal L$-formula, let $x=(x_i)_{i\in I}$ be a multivariable, and
let~$t=(t_i)_{i\in I}$ be a family of $\mathcal L$-terms with $t_i$ of the same sort as $x_i$ for all $i$. Then~$\varphi(t/x)$ denotes the word obtained by
replacing all the free occurrences of $x_i$ in $\varphi$ by~$t_i$, {\it simultaneously}\/ for all $i$.
If $\varphi=\varphi(x)$, then we also write $\varphi(t)$ instead of~$\varphi(t/x)$.
We have the following facts whose routine proofs are left to the reader.

\begin{lemma}
The word $\varphi(t/x)$ is an $\mathcal L$-formula. If
 $t$ is variable-free and $\varphi = \varphi(x)$, then $\varphi(t)$ is an $\mathcal L$-sentence.
\end{lemma}

\noindent
Given an $\mathcal L$-structure $\mathbf M$, an $\mathcal L_M$-formula $\varphi(x)$ and $a\in M_x$, we shall avoid many ugly 
expressions by
writing the $\mathcal L_M$-sentence $\varphi(\underline{a})$ as
just $\varphi(a)$.  \index{substitution!into formulas} \index{formula!substitution}


\subsection*{Truth and definability}
We can now define what it means for an $\mathcal L_M$-sentence~$\sigma$ to be {\bf true}
in the $\mathcal L$-structure $\mathbf M$ (notation: $\mathbf M\models \sigma$, also read as   $\mathbf M$ {\bf satisfies} $\sigma$, or   $\sigma$ {\bf holds} in $\mathbf M$). First we consider atomic $\mathcal L_M$-sentences:
\begin{list}{}{\leftmargin=2.5em}
\item[(T1)] $\mathbf M \models \top$ and $\mathbf M \not\models \bot$;
\item[(T2)]  $\mathbf M \models Rt_1 \dots t_m$ if and only if $(t_1^{\mathbf M} , \dots , t_m^{\mathbf M})
\in R^{\mathbf M}$, for $R \in \mathcal L^{\operatorname{r}}$ of sort $s_1\dots s_m$ and
variable-free $\mathcal L_M$-terms $t_1, \dots , t_m$ of sort $s_1,\dots,s_m$, respectively;
\item[(T3)]  $\mathbf M \models {t_1 = t_2}$ if and only if $t^{\mathbf M}_1 = t^{\mathbf M}_2$, for variable-free $\mathcal L_M$-terms $t_1$, $t_2$ of the same sort.
\end{list}
We extend the definition inductively to arbitrary $\mathcal L_M$-sentences as follows:
\begin{list}{}{\leftmargin=2.5em}
\item[(T4)] Suppose $\sigma = \neg\tau$; then $\mathbf M\models \sigma$ if and only if $\mathbf M\not\models\tau$.
\item[(T5)] Suppose $\sigma = \sigma_1 \vee \sigma_2$; then $\mathbf M\models \sigma$ if and only if $\mathbf M\models \sigma_1$ or $\mathbf M\models \sigma_2$.
\item[(T6)] Suppose $\sigma = \sigma_1 \wedge \sigma_2$; then $\mathbf M\models \sigma$ if and only if $\mathbf M\models \sigma_1$ and $\mathbf M\models \sigma_2$.
\item[(T7)] Suppose $\sigma = \exists x\varphi$ where $x$ is a quantifiable variable and $\varphi(x)$ is an $\mathcal L_M$-formula; then $\mathbf M\models \sigma$ if and only if $\mathbf M\models \varphi(a)$ for some $a \in M_x$.
\item[(T8)] Suppose $\sigma = \forall x\varphi$  where $x$ is a quantifiable variable and $\varphi(x)$ is an $\mathcal L_M$-formula; then $\mathbf M\models \sigma$ if and only if $\mathbf M\models \varphi(a)$ for all $a \in M_x$.
\end{list}
Even if we just want to define $\mathbf M\models \sigma$  for $\mathcal L$-sentences $\sigma$, one can see that if
$\sigma$ has the form considered in (T7) or (T8), the inductive definition above forces us to
consider $\mathcal L_M$-sentences $\varphi(a)$. This is why we introduced names. (``Inductive'' refers here to induction with respect to the number of
logical symbols in $\sigma$.) \index{sentence!truth}

\nomenclature[Bl0]{$\mathbf M\models\sigma$}{$\sigma$ is true in $\mathbf M$}
\nomenclature[Bl9]{$\varphi^{\mathbf M}$}{set defined by $\varphi$ in $\mathbf M$}


\begin{definition} 
Given an $\mathcal L_M$-formula $\varphi(x)$  we let
$$\varphi^{\mathbf M}\ :=\ \big\{ a \in M_x:\  \mathbf M \models  \varphi(a)\big\}\subseteq M_x.$$
The formula $\varphi(x)$ is said to {\bf define} the set $\varphi^{\mathbf M}$ in $\mathbf M$. 
Given a parameter set~$A\subseteq M$, a subset 
of $M_{x}$
is said to be {\bf $A$-definable} in $\mathbf M$ if it is of the form $\varphi^{\mathbf M}$ for some $\mathcal L_A$-formula $\varphi(x)$. 
A map $f\colon X\to M_y$, where $X\subseteq M_x$,  is said to be $A$-definable if its graph $\Gamma(f)\subseteq M_{x,y}$ is.
We use {\bf definable} synonymously with  $M$-de\-finable. \index{set!$A$-definable} \index{set!definable} \index{definable!set}\index{formula!defining a set}\index{map!$A$-definable}\index{definable!map}
\end{definition}

\begin{examples}\mbox{}
Let $\mathbf R=(\R; {\leq}, 0, 1, {+}, {-}, {\cdot})$.
\begin{enumerate}
\item The set $\big\{r \in \R : r \leq \sqrt{2}\big\}$ is $0$-definable in $\mathbf R$: it is defined
by the formula $(x^2 \leq 1+1) \vee (x \le 0)$. (Here $x^2$ abbreviates the term $x\cdot x$.)
\item The set $\{r \in \R : r \leq \pi\}$ is definable in $\mathbf R$: it is defined by
the formula $x \leq \pi$. (It takes more effort to show that it is not $0$-definable, see Example~\ref{ex:RCF QE}.)
\end{enumerate}
\end{examples}

\noindent
It is easy to see that given $A\subseteq M$, a subset of $M_{\mathbf s}$ is $A$-definable in the sense of the previous definition 
if and only if it is $A$-definable in the sense of 
Definition~\ref{def:0-definable}. (Using the correspondences (C1)--(C5) between formulas and sets defined by them
from Section~\ref{sec:structures and definable sets}.)
If $\psi(y)$ is an $\mathcal L_A$-formula, then there is a finite multivariable~$x$ disjoint from $y$, an $\mathcal L$-formula~$\varphi(x,y)$ and an~$a\in A_x$, such that $\varphi(a,y)=\psi(y)$.
Thus a set $Y \subseteq M_y$ is $A$-definable iff for some 
finite $x$ disjoint from $y$, some
$a \in A_x$ and some $0$-definable $Z \subseteq M_{x,y}$ we have $Y = Z(a):=\big\{b\in M_y: (a,b)\in Z\big\}$. In this way {\em $A$-definability} reduces to {\em $0$-definability}.


\medskip
\noindent
We defined what it means for an $\mathcal L$-sentence to hold in~$\mathbf M$. It is convenient to extend this to arbitrary $\mathcal L$-formulas.
First, given $A\subseteq M$ we define an {\bf $A$-instance} of an $\mathcal L_A$-formula $\varphi=\varphi(x)$  to be an 
$\mathcal L_A$-sentence of the form $\varphi(a)$ with $a\in A_x$. Of course~$\varphi$ can also
be written as $\varphi(y)$ for another multivariable $y$. Thus for the above to
count as a definition of ``$A$-instance'', the reader should check that these different
ways of specifying variables (including at least the free variables of $\varphi$) give the same $A$-instances.  \index{formula!$A$-instance}

\begin{definition} An $\mathcal L$-formula $\varphi$ is said to be {\bf valid} in $\mathbf M$ (notation: $\mathbf M\models\varphi$) if all its
$M$-instances are true in $\mathbf M$.  \index{formula!valid in a structure} 
\end{definition}


\noindent
If the multivariable $x=(x_1,\dots,x_m)$ is (finite and) quantifiable, then for an $\mathcal L$-formula $\varphi$ we abbreviate $\forall x_1\cdots\forall x_m \varphi$ by~$\forall x\varphi$, and similarly with $\forall$ replaced by~$\exists$.
The reader should check that if $\varphi=\varphi(x)$ with quantifiable $x=(x_1,\dots,x_m)$, then~$\forall x\varphi$ is an $\mathcal L$-sentence and
$$\mathbf M \models \varphi\quad\Longleftrightarrow\quad \mathbf M \models \forall x\,\varphi.$$
We also write $\models\varphi$ if $\varphi$ is valid in every $\mathcal L$-structure $\mathbf M$. We say that $\mathcal L$-formulas~$\varphi$,~$\psi$ are {\bf equivalent} if $\models \varphi \leftrightarrow \psi$. \index{formula!equivalence} \index{equivalence!of formulas} For example, given an $\mathcal{L}$-formula $\varphi$ and a quantifiable variable $x$,
the formulas $\neg\forall x\varphi$ and $\exists x\neg\varphi$ are equivalent.


\medskip\noindent
Let $\varphi_1,\dots,\varphi_n$ be $\mathcal L$-formulas, where $n\geq 1$.
We inductively define 
$$\varphi_1\wedge\cdots\wedge\varphi_n := \begin{cases}
\varphi_1 													& \text{if $n=1$,} \\
\varphi_1\wedge\varphi_2									& \text{if $n=2$,} \\
(\varphi_1\wedge\cdots\wedge\varphi_{n-1})\wedge\varphi_n	& \text{if $n\geq 3$.}
\end{cases}$$
Similarly define $\varphi_1\vee\cdots\vee\varphi_n$.
For each permutation $i$ of $\{1,\dots,n\}$, the $\mathcal L$-formulas
$\varphi_1\wedge\cdots\wedge\varphi_n$ and $\varphi_{i1}\wedge\cdots\wedge\varphi_{in}$
are equivalent; similarly with $\wedge$ replaced by $\vee$.

\subsection*{Formulas of a special form}
We now single out formulas by certain syntactical conditions. These conditions
have semantic counterparts in terms of the behavior of these formulas under
embeddings, as explained in the next subsection.
An $\mathcal L$-formula is said to be {\bf quantifier-free} if it has no occurrences of $\exists$ and
no occurrences of~$\forall$. An $\mathcal L$-formula is said to be {\bf existential} (or an {\bf $\exists$-formula}) if it has the form~$\exists x\,\rho$ with a finite multivariable $x$ and a quantifier-free $\mathcal L$-formula $\rho$, and  {\bf universal} (or a {\bf $\forall$-formula}) if it has the form $\forall x\,  \rho$ with 
finite  $x$ and quantifier-free~$\rho$.
If~$\varphi$ is a $\forall$-formula, then $\neg\varphi$ is equivalent to an $\exists$-formula, and similarly with ``$\forall$'' and ``$\exists$'' interchanged.
Finally, an $\mathcal L$-formula is said to be   {\bf universal-existential} (or a {\bf $\forall\exists$-formula}) if
it has the form $\forall x \exists y \,\varphi$ with finite disjoint $x$, $y$ and quantifier-free~$\rho$.\index{formula!quantifier-free}\index{formula!existential}\index{formula!universal}\index{formula!universal-existential}\index{existential formula} \index{universal!formula} \index{$\exists$-formula} \index{$\forall$-formula}\index{$\forall\exists$-formula}
 
\begin{lemma}
If $\varphi$, $\psi$ are $\exists$-formulas, then
$\varphi\wedge\psi$ and $\varphi\vee\psi$ are equivalent to $\exists$-formulas;
similarly with $\forall$ or $\forall\exists$ in place of $\exists$. 
\end{lemma}
\begin{proof}
The easy proofs of these facts use the technique of ``renaming variables'' which we often use tacitly below.
Let $\varphi=\exists x\,\rho$, $\psi=\exists y\,\theta$ where  $\rho$, $\theta$ are quantifier-free; 
it is easy to check that if $x$, $y$ are disjoint, then $\varphi\wedge\psi$ and
$\exists x\exists y(\rho\wedge\theta)$ are
 equivalent. 
In the general case, first
choose
disjoint finite quantifiable multivariables $x'$, $y'$ of the same sort as $x$, $y$, respectively,
such that no variable occurring in $\rho$, $\theta$, is in $x'$ or $y'$, 
and replace $\varphi$, $\psi$ by the respective equivalent formulas
 $\exists x'\,\rho(x'/x)$, $\exists y'\,\theta(y'/y)$.
\end{proof}

\subsection*{Maps preserving formulas}
{\it In this subsection $A$ is a parameter set in $\mathbf M$ and 
$h\colon A\to N$ is a map.}\/
For an $\mathcal L_A$-term~$t$, let $h(t)$ be the $\mathcal L_N$-term obtained from~$t$ by replacing every occurrence of a name of an element $a\in A_s$ by the name of $h_s a\in N_s$. For an $\mathcal L_A$-formula~$\varphi$, let $h(\varphi)$ be the $\mathcal L_N$-formula obtained from $\varphi$  by replacing every occurrence of a name of an element
$a\in A_s$ by the name of $h_sa$. If $t$ is variable-free, then so is~$h(t)$, and if $\varphi$ is a sentence, then so is $h(\varphi)$.
If $\varphi(x)$ is an $\mathcal L$-formula and~$a\in A_x$, then $h(\varphi(a))=\varphi(ha)$.
We say that {\bf $h$ preserves atomic formulas} if for all 
atomic $\mathcal{L}$-formulas $\varphi(x)$ and $a\in A_x$ such that
$\mathbf{M}\models \varphi(a)$ we have $\mathbf{N}\models \varphi(ha)$. In the same way we define ``$h$ preserves quantifier-free formulas'' and ``$h$ preserves formulas''.\index{map!preserving formulas}  



%\begin{lemma}\label{lem:persist, 1}
%Let $\varphi$, $\psi$ be $\mathcal L_A$-formulas which persist under $h$. and suppose $x$ is a quantifiable variable. Then
%\begin{enumerate}
%\item $\varphi\vee\psi$ and $\varphi\wedge\psi$ persist under $h$;
%\item if $A=M$, then $\exists x \varphi$ persists under $h$;
%\item if $h$ is surjective, then $\forall x \varphi$ persists under $h$.
%\end{enumerate}
%\end{lemma}

\begin{lemma}\label{lem:persist, 2}
Suppose $A=M$. Then we have the following two equivalences:
\begin{enumerate}
\item $h$ is a morphism $\mathbf M\to\mathbf N$ iff $h$ preserves atomic formulas;
\item $h$ is an embedding $\mathbf M\to\mathbf N$ iff $h$ preserves
quantifier-free formulas.
\end{enumerate}
\end{lemma}

\noindent
We leave the proofs of this routine lemma to the reader.

\begin{cor}\label{cor:persist, 1}
Suppose $\mathbf M\subseteq\mathbf N$, and let $\sigma$ be an $\mathcal L_M$-sentence.
\begin{enumerate}
\item If $\sigma$ is quantifier-free, then $\mathbf M\models\sigma\Longleftrightarrow\mathbf N\models \sigma$.
\item If $\sigma$ is existential, then $\mathbf M\models\sigma \Rightarrow \mathbf N\models \sigma$.
\item If $\sigma$ is universal, then $\mathbf N\models\sigma \Rightarrow \mathbf M\models \sigma$.
\end{enumerate}
\end{cor}
\begin{proof}
Part (1) is immediate from Lemma~\ref{lem:persist, 2},~(2).
Part (2) follows easily from~(1), and~(3) follows from (2).
\end{proof}

\noindent
In the next corollary we assume that 
$\mathcal L$ has for every $s$ a constant symbol of sort $s$. This is to guarantee that $\<A\>_{\mathbf M}$ is defined.

\begin{cor}\label{cor:persist, 2}
The map
$h$ extends to
a morphism $\<A\>_{\mathbf M}\to\mathbf N$ iff $h$ preserves
atomic formulas. The map
$h$ extends to
an embedding $\<A\>_{\mathbf M}\to\mathbf N$ iff $h$ preserves 
quantifier-free formulas.
\end{cor}
\begin{proof}
The forward directions in both statements follow from Lem\-ma~\ref{lem:persist, 2} and
Corollary~\ref{cor:persist, 1},~(1). Suppose for every
atomic $\mathcal L_A$-sentence $\sigma$ true in $\mathbf M$, its image~$h(\sigma)$ is true in $\mathbf N$. Now every element of sort $s$ of $\<A\>_{\mathbf M}$ has the form $t^{\mathbf M}(a)$ for
some $\mathcal L$-term $t(x)$ of sort $s$ and some $a\in A_x$. Moreover, if $t_1(x)$ and $t_2(y)$ are $\mathcal L$-terms of sort $s$ and $t_1(a)=t_2(b)$, where $a\in A_x$ and $b\in A_y$,
then $\mathbf M\models t_1(a) = t_2(b)$, and hence
$\mathbf N\models t_1(h_x(a)) = t_2(h_y(b))$, and thus
$t_1^{\mathbf N}(h_x(a)) = t_2^{\mathbf N}(h_y(b))$. These two facts easily yield the backward directions of the two equivalences.
\end{proof}


\index{map!elementary}\index{elementary!map}\index{embedding!elementary}\index{elementary!embedding}\index{structure!elementary embedding}


\noindent
We say that $h\colon A \to N$ is {\bf elementary} if it preserves formulas, that is, for all $\mathcal L$-formulas $\varphi(x)$ and all $a\in A_x$, 
$$\mathbf M\models\varphi(a)\quad\Longleftrightarrow\quad\mathbf N\models\varphi(ha).$$
By Lemmas~\ref{lem:persist, 2}, 
every elementary map $M\to N$ is an embedding $\mathbf M\to\mathbf N$, and
every isomorphism of $\mathcal L$-structures is elementary.
Suppose the $\mathcal L_A$-formula $\varphi(x)$ defines the set
$X\subseteq M_x$. If $h\in\Aut(\mathbf M)$, then the $\mathcal L_{h(A)}$-formula $h(\varphi)(x)$ defines the set
$h(X)\subseteq M_x$, so if $h\in\Aut(\mathbf M|A)$, then  $X=h(X)$.
This observation can sometimes be used to show that certain relations are not definable:

\begin{example}
The ordering relation $\leq$ on $\R$ is not definable in the  $\mathcal L_{\operatorname{A}}$-structure
$(\R; 0, {-},{+})$: for all $r_1,\dots,r_n\in\R$ there is an automorphism $\sigma$ of this structure which
satisfies $\sigma(r_i)=r_i$ for $i=1,\dots,n$ and $\sigma(r)<0<r$ for some $r\in\R$.
\end{example}


\subsection*{More on substitution}
We finish this section with a technical result used in Sections~\ref{sec:ultra products} and \ref{sec:LS} below.
Let $x=(x_i)_{i\in I}$ and $y=(y_j)_{j\in J}$ be multivariables,
and let $t=(t_i)$ be a family of $\mathcal L$-terms with $t_i=t_i(y)$ of the same sort as $x_i$, for all $i\in I$.
Then for $a\in M_y$ we put $t^{\mathbf M}(a):=\big(t_i^\mathbf M(a)\big)\in M_x$. 
\begin{lemma} \label{lem:subst lemma, formulas} 
Let $\varphi(x)$ be a quantifier-free $\mathcal L_M$-formula.
Then for all $a\in M_y$,
$$\mathbf M \models \varphi(t)(a) \quad\Longleftrightarrow\quad \mathbf M \models \varphi(t^{\mathbf M}(a)).$$
\end{lemma}
\begin{proof}   
Suppose $\varphi$ is atomic, say $\varphi=
R\alpha_1 \cdots \alpha_m$ where $R\in\mathcal L^{\operatorname{r}}$ is $m$-ary and $\alpha_1(x), \dots, \alpha_m(x)$ are $\mathcal L_M$-terms. Let $a\in M_y$. Then
$$\varphi(t) = R\alpha_1(t)\cdots\alpha_m(t),\quad\varphi(t^{\mathbf M}(a)) = R\alpha_1(t^{\mathbf M}(a)) \cdots \alpha_m(t^{\mathbf M}(a)).$$ 
Now $\alpha_i(t)(a)=\alpha_i(t(a))$ for each $i$, as is easy to verify, and so
$$\mathbf M\models \varphi(t)(a)\quad\Longleftrightarrow\quad
\big(\alpha_1(t(a))^{\mathbf M}, \dots, \alpha_m(t(a))^{\mathbf M}\big) \in R^{\mathbf M}.$$ Also 
$$\mathbf M \models \varphi(t^{\mathbf M}(a)) \quad\Longleftrightarrow\quad 
\big(\alpha_1(t^{\mathbf M}(a))^{\mathbf M}, \dots, \alpha_m(t^{\mathbf M}(a))^{\mathbf M}\big) \in R^{\mathbf M}.$$
By  Lemma~\ref{lem:subst lemma, terms} we have for each $i$,
$$\alpha_i(t(a))^{\mathbf M} = \alpha_i(t(a)^{\mathbf M})^{\mathbf M} = 
\alpha_i(t^{\mathbf M}(a))^{\mathbf M}.$$
Thus $\mathbf M \models \varphi(t)(a)$ iff
$\mathbf M \models \varphi(t^{\mathbf M}(a))$. The case that $\varphi$ is $\alpha = \beta$ is handled the same way.
It is clear that the desired property is inherited by disjunctions, conjunctions
and negations of formulas $\varphi(x)$ that have the property. 
\end{proof}




\subsection*{Notes and comments}
The definition (T1)--(T8) of the satisfaction relation goes back to  
Tarski's paper~\cite{Tarski35a}, but in the form above is closer to Tarski-Vaught~\cite{TarskiVaught}. 




\section{Elementary Equivalence and Elementary Substructures}

\noindent
The syntax (terms, formulas, sentences) and semantics (truth, definability) from the previous section will be used in this section to compare $\mathcal L$-structures.

\subsection*{Elementary equivalence}
We say that $\mathbf M$ and $\mathbf N$ {\bf elementarily equivalent} (notation: $\mathbf M\equiv\mathbf N$) if they satisfy the same $\mathcal L$-sentences.
So isomorphic $\mathcal L$-structures 
are elementarily equivalent. By~\ref{ex:DLO} below, however, the non-isomorphic ordered sets $(\Q;{\leq})$ and $(\R;{\leq})$ are elementarily equivalent as well. This uses 
the {\it back-and-forth method}, a general tool that we also relied on in Chapter~\ref{ch:monotonedifferential}. \index{structure!elementary equivalence} \index{equivalence!elementary} \index{elementary!equivalence}

\nomenclature[Bj2]{$\mathbf M\equiv\mathbf N$}{$\mathbf M$, $\mathbf N$ are elementarily equivalent}

\begin{definition} \index{isomorphism!partial}\index{structure!partial isomorphism}
A {\bf partial isomorphism} from $\mathbf M$ to $\mathbf N$ is a bijection $\gamma\colon A\to B$
with $A\subseteq M$, $B\subseteq N$, such that
\begin{enumerate}
\item for each $R\in\mathcal L^{\operatorname{r}}$ of sort $s_1\dots s_m$ and $a\in A_{s_1\dots s_m}$,
$$a\in R^{\mathbf M}\quad\Longleftrightarrow\quad \gamma a \in R^{\mathbf N};$$
\item for each $f\in\mathcal L^{\operatorname{f}}$ of sort $s_1\dots s_n  s$ and $a\in A_{s_1\dots s_n}$, $b\in A_s$,
$$f^{\mathbf M}(a)=b \quad\Longleftrightarrow\quad f^{\mathbf N}(\gamma a)=\gamma b.$$
\end{enumerate}
\end{definition}

\noindent
Note that in this definition we do not assume that $A$ and $B$ are the underlying sets of substructures of   $\mathbf M$ and
$\mathbf N$, respectively. If
$A$ and $B$ {\it are}\/ the underlying sets of substructures $\mathbf A$ of $\mathbf M$ and $\mathbf B$ of
$\mathbf N$, respectively, then  a partial isomorphism~$A\to B$ from $\mathbf M$ to $\mathbf N$
is the same thing as an isomorphism $\mathbf A\to\mathbf B$.

Given a partial isomorphism $\gamma\colon A\to B$ from $\mathbf M$ to $\mathbf N$, we set 
$\operatorname{domain}(\gamma_s):=A_s$ and
$\operatorname{domain}(\gamma):=A$, and likewise $\operatorname{codomain}(\gamma_s):=B_s$ and $\operatorname{codomain}(\gamma):=B$.
If~$(\gamma_\lambda)_{\lambda\in \Lambda}$ is a family of partial isomorphisms indexed by a
directed set $(\Lambda,{\leq})$, such that $\gamma_{\lambda'}$ extends $\gamma_\lambda$ for 
$\lambda\leq\lambda'$ in $\Lambda$, then there is a unique partial isomorphism $\gamma:=\bigcup_{\lambda\in\Lambda} \gamma_\lambda$
from $\mathbf M$ to $\mathbf N$ with domain $\bigcup_{\lambda\in\Lambda} \operatorname{domain}(\gamma_\lambda)$ such that $\gamma(a)=\gamma_\lambda(a)$ for 
all $s\in S$, $\lambda\in\Lambda$, and 
$a\in\operatorname{domain}(\gamma_{\lambda,s})$.

\begin{example}
Let $\mathbf M = (M; {\leq})$ and $\mathbf N = (N; {\leq})$ be   ordered sets, and let
$a_1, \dots , a_n \in M$ and $b_1, \dots , b_n \in N$ with $a_1 < a_2 < \cdots < a_n$ and
$b_1 < b_2 < \cdots < b_n$; then the map $a_i \mapsto b_i \colon \{a_1, \dots , a_n\} \to \{b_1, \dots , b_n\}$ is a
partial isomorphism from~$\mathbf M$ to~$\mathbf N$.
\end{example}


\begin{definition} \index{back-and-forth system}\index{structure!back-and-forth system}
A {\bf back-and-forth system} from $\mathbf M$ to $\mathbf N$ is a collection $\Gamma$ of partial
isomorphisms from $\mathbf M$ to $\mathbf N$ such that $\Gamma\ne \emptyset$ and:
\begin{list}{}{\leftmargin=1em}
\item[(``Forth'')] for each $\gamma \in  \Gamma$, $s\in S$, and $a \in  M_s$ there is a $\gamma' \in  \Gamma$ extending
$\gamma$ such that $a \in  \operatorname{domain}(\gamma'_s)$;
\item[(``Back'')] for each $\gamma \in  \Gamma$, $s\in S$, and $b \in  N_s$ there is a $\gamma' \in  \Gamma$  extending
$\gamma$ such that $b \in  \operatorname{codomain}(\gamma'_s)$.
\end{list}
We say that $\mathbf M$ and $\mathbf N$ are {\bf back-and-forth equivalent} (notation: $\mathbf M \equiv_{\operatorname{bf}} \mathbf N$) if there
exists a back-and-forth system from $\mathbf M$ to $\mathbf N$. \index{structure!back-and-forth equivalent} \index{equivalence!back-and-forth}\nomenclature[Bj3]{$\mathbf M\equiv_{\operatorname{bf}}\mathbf N$}{$\mathbf M$, $\mathbf N$ are back-and-forth equivalent}
\end{definition}

\begin{prop}\label{prop:bf, 1}
If  $\mathbf M$, $\mathbf N$ are countable and $\mathbf M \equiv_{\operatorname{bf}} \mathbf N$, then~$\mathbf M\cong\mathbf N$.
\end{prop}
\begin{proof} 
Suppose $\Gamma$ is a back-and-forth system from $\mathbf M$ to $\mathbf N$. 
Note first that for $\gamma\in\Gamma$ and $s\in S$ we have:
$\operatorname{domain}(\gamma_s)=M_s$ iff $\operatorname{codomain}(\gamma_s)=N_s$.
In view of this fact, and assuming $M$ and $N$ are countable, we can start with any $\gamma_0\in \Gamma$ and build recursively
a sequence $(\gamma_n)$ in $\Gamma$ such that $\gamma_{n+1}$ extends $\gamma_n$ for all $n$ (going forth if $n$ is even, and going back if $n$ is odd) such that 
$\bigcup_n \operatorname{domain}(\gamma_n) = M$ and 
$\bigcup_n \operatorname{codomain}(\gamma_n) = N$.  
Then we have an isomorphism $\bigcup_n \gamma_n\colon \mathbf M\to\mathbf N$.
\end{proof}

\noindent
In applying this proposition and the next one in a concrete situation, the
key is to guess a back-and-forth system. That is where insight and imagination
(and experience) come in. In the following result we do not assume
countability.

\begin{prop}\label{prop:bf, 2}
If $\mathbf M \equiv_{\operatorname{bf}} \mathbf N$, then $\mathbf M \equiv  \mathbf N$.
\end{prop}


\noindent
Towards the proof, define an $\mathcal L$-formula to be {\bf unnested} if every atomic subformula of it is either $\top$, or $\bot$, or has one of the following forms: 
\begin{enumerate}
\item $Rx_1 \dots x_m$; here $R \in \mathcal L^{\operatorname{r}}$  and $x_1,\dots, x_m$ are distinct variables;
\item $x=y$; here $x$ and $y$ are distinct variables; 
\item $fx_1\dots x_n=y$; here $f \in \mathcal L^{\operatorname{f}}$ and $x_1,\dots, x_n,y$ are distinct
variables.
\end{enumerate}

\begin{lemma}\label{unnested}
Each atomic $\mathcal L$-formula $\varphi(x)$ is equivalent to an unnested existential $\mathcal L$-formula $\varphi_\exists(x)$,
and also to an unnested universal $\mathcal L$-formula $\varphi_\forall(x)$. Each $\mathcal L$-formula $\varphi(x)$ is equivalent
to an unnested $\mathcal L$-formula $\varphi_{\operatorname{u}}(x)$. 
\end{lemma}

\noindent
We leave the proof of this lemma to the reader.
\index{formula!unnested} \index{unnested formula}



\begin{proof}[Proof of Proposition~\ref{prop:bf, 2}]
Suppose $\Gamma$ is a back-and-forth system from $\mathbf M$ to~$\mathbf N$. Let $\varphi(x)$ be an unnested $\mathcal L$-formula. By induction on the
number of logical symbols in $\varphi$ we show that
for all $\gamma\in\Gamma$ with domain $A$ and $a \in A_x$,
$$\mathbf M\models \varphi(a) \quad\Longleftrightarrow\quad \mathbf N \models\varphi(\gamma a).$$
This yields $\mathbf M \equiv  \mathbf N$, using Lemma~\ref{unnested} for sentences.
The stated equivalence follows from the definitions if $\varphi$ is atomic, and its validity is
preserved under~$\wedge$,~$\vee$,~$\neg$. Suppose $\varphi=\exists y\psi$ where $y$ is a quantifiable
variable of sort $s$ not occurring in $x$ and $\psi(x,y)$ is unnested, and let $\gamma\in\Gamma$ with domain $A$
and $a\in A_x$. If $\mathbf M\models \varphi(a)$, then we
take $b\in M_s$ such that $\mathbf M\models\psi(a,b)$,
and then $\gamma'\in\Gamma$ extending~$\gamma$ with $b\in\operatorname{domain}(\gamma'_s)$;
by inductive hypothesis $\mathbf N\models\psi(\gamma a,\gamma' b)$
and hence $\mathbf N\models\varphi(\gamma a)$.
Similarly one shows that $\mathbf N\models\varphi(\gamma a)\Rightarrow\mathbf M\models \varphi(a)$.
\end{proof}

\begin{exampleNumbered}\label{ex:DLO}
Let $\mathbf M=(M;{\leq})$ and $\mathbf N=(N;{\leq})$ be dense ordered sets without endpoints.
Then the collection of all strictly increasing bijections $A\to B$, where $A\subseteq M$
and $B\subseteq N$ are finite, is a back-and-forth system from $\mathbf M$ to $\mathbf N$.
Hence $\mathbf M\equiv\mathbf N$, and if $M$, $N$ are countable, then $\mathbf M\cong\mathbf N$.
\end{exampleNumbered}



\subsection*{Elementary substructures} \index{substructure!elementary} \index{elementary!substructure} \index{extension!elementary} \index{elementary!extension} Let $\mathbf M\subseteq\mathbf N$.
One says that $\mathbf M$ is an {\bf elementary substructure} of $\mathbf N$ (and that the extension $\mathbf M\subseteq\mathbf N$ is {\bf elementary}) if the natural inclusion
$\mathbf M\hookrightarrow\mathbf N$ is elementary; notation: $\mathbf M\preceq\mathbf N$.
We have  
$$\mathbf M\preceq\mathbf N\quad\Longleftrightarrow\quad \text{$\varphi^{\mathbf M}=\varphi^{\mathbf N}\cap M_x$
for each $\mathcal L_M$-formula $\varphi(x)$}.$$ 
Also, $\mathbf M\preceq\mathbf N \Longleftrightarrow \mathbf M_M\equiv\mathbf N_M$, so  $\mathbf M\preceq\mathbf N\Rightarrow\mathbf M\equiv\mathbf N$.
\nomenclature[Bj01]{$\mathbf M\preceq\mathbf N$}{$\mathbf M$ is an elementary substructure of $\mathbf N$}


\begin{exampleNumbered}\label{ex:simple gps}
View groups as $\mathcal L_{\operatorname{G}}$-structures  as in~\ref{ex:L-structures},~(1).
Let  $G$, $H$ be groups with $G\preceq H$, and suppose that $H$ is simple. Then $G$ is also simple: to see this, let 
$g,g'\in G$, $g\neq 1$; it suffices to show that $g'$ is in the normal subgroup of~$G$ generated by $g$.
Now $g'=h_1 g^{k_1} h_1^{-1}\cdots h_n g^{k_n} h_n^{-1}$
where $n\ge 1$, $h_1,\dots,h_n\in H$, $k_1,\dots,k_n\in\Z$. Therefore
$H$ satisfies the $\mathcal L_G$-sentence 
$$\exists x_1\cdots \exists x_n \big( g' = x_1 g^{k_1} x_1^{-1} \cdots x_n g^{k_n} x_n^{-1}\big),$$
and so does $G$, since $G\preceq H$.
\end{exampleNumbered}

\noindent
We have the following useful criterion for a substructure to be elementary: \index{test!Tarski-Vaught}

\begin{prop}[Tarski-Vaught Test]\label{prop:TV}
Let $A\subseteq N$. Suppose that for every $\mathcal L_A$-formula~$\varphi(x)$ with $x$
a quantifiable variable, if $\mathbf N\models\exists x\varphi(x)$, then
$\mathbf N\models\varphi(a)$ for some $a\in A_x$.
Then $A$ underlies an elementary substructure of $\mathbf N$.
\end{prop}

\begin{proof} Note first that $N_s\ne \emptyset$ gives 
$A_s\neq\emptyset$, for all $s$.
If $f$ is a function symbol of $\mathcal L$ of sort $s_1\dots s_n s$ and $a\in A_{s_1\dots s_n}$,
consider the $\mathcal L_A$-formula $\varphi(x)$ given by $f(a)=x$, with $x$ a quantifiable variable of sort~$s$;
then $\mathbf N\models\exists x\varphi$ and hence 
$f^{\mathbf N}(a)\in A_x$. Thus $A$ is the underlying set of a substructure $\mathbf A$ of $\mathbf N$.
We show that for each $\mathcal L_A$-sentence $\sigma$ we have
$\mathbf A\models\sigma\Longleftrightarrow\mathbf N\models\sigma$ by induction on the construction of $\sigma$.
If~$\sigma$ is atomic, then this holds by Corollary~\ref{cor:persist, 1},~(1), and it is clear that the desired property is preserved under taking negations, conjunctions, and disjunctions.
It remains to treat the case where $\sigma=\exists x\varphi$ with
 an $\mathcal L_A$-formula $\varphi(x)$. Then
\begin{align*}
\mathbf A \models \sigma 	& \quad\Longleftrightarrow\quad \text{$\mathbf A\models\varphi(a)$
for some $a\in A_x$} \\
							& \quad\Longleftrightarrow\quad \text{$\mathbf N\models\varphi(a)$
for some $a\in A_x$}\\
							& \quad\Longleftrightarrow\quad \text{$\mathbf N\models\sigma$,}
\end{align*}
using the hypothesis in the proposition for the third equivalence.
\end{proof}

\begin{cor}
If $\mathbf M\subseteq \mathbf N$ and for all finite $A\subseteq M$ and all $b\in N_s$ there exists $h\in\Aut(\mathbf N|A)$
with $h(b)\in M_s$, then $\mathbf M\preceq\mathbf N$.
\end{cor}

\begin{example}
The previous corollary easily yields $(\Q;{\leq})\preceq (\R;{\leq})$.
\end{example}


\noindent
The Tarski-Vaught test can be used to construct small elementary substructures: \index{theorem!L\"owenheim-Skolem}

 
\begin{prop}[L\"owenheim-Skolem ``downwards'']\label{prop:LS downwards}
Let $A\subseteq N$ and suppose~$\kappa$ is a cardinal such that
$\max\big\{ |A|,|\mathcal L|\big\} \leq \kappa \leq |N|$.
Then $\mathbf N$ has an elementary substructure~$\mathbf M$ of 
size $\kappa$ with $A\subseteq M$.
\end{prop}
\begin{proof}
After enlarging $A$ to a parameter set in $\mathbf N$ of size $\kappa$,
we may assume that $|A|=\kappa$. For every $B\subseteq N$ and $s$, let $\Phi_{B,s}$ be the set of all $\mathcal L_B$-formulas~$\varphi(x)$ with~$x$ a quantifiable variable of sort $s$ such that $\mathbf N\models \exists x\varphi$.
For every  $\varphi\in\Phi_{B,s}$ choose a $b_\varphi\in N_s$ with $\mathbf N\models\varphi(b_\varphi)$, and let $B'_s:=\{b_\varphi:\varphi\in\Phi_{B,s}\}$. 
For each~$b\in B_s$ and quantifiable variable $x$ of sort $s$ the $\mathcal L_B$-formula $x=b$ is in~$\Phi_{B,s}$,
so $b=b_{x=b}\in B'_s$, hence $B_s\subseteq B_s'$. 
Setting $B':=(B'_s)$, we have $|B|\leq |B'| \leq \max\big\{ |B|, |\mathcal L| \big\}$. We now
inductively define an increasing sequence $A_0\subseteq A_1\subseteq\cdots$ of parameter sets in~$\mathbf M$
by $A_0:=A$ and $A_{n+1}:=A_n'$, and put $M:=\bigcup_n A_n$. Then $|A_n|=\kappa$ for each $n$, hence also 
$|M|=\kappa$. By Proposition~\ref{prop:TV}, $M$ is the underlying set of an elementary substructure of~$\mathbf N$.
\end{proof}



\begin{exampleNumbered}\label{ex:LS downwards}
Any infinite simple group $H$ has a simple subgroup
of any given infinite size $\leq |H|$, by Example~\ref{ex:simple gps} and Proposition~\ref{prop:LS downwards}.
\end{exampleNumbered}




\subsection*{Direct unions}
Suppose $\mathbf M$ is the direct union of the family $(\mathbf M_\lambda)_{\lambda\in\Lambda}$  of substructures of $\mathbf M$. Let $\lambda$, $\lambda'$ range over $\Lambda$.
By (1) and (2) of  Corollary~\ref{cor:persist, 1}, if $\sigma$ is a $\forall\exists$-sentence such that
$\mathbf M_\lambda\models\sigma$ for all~$\lambda$, then $\mathbf M\models\sigma$.
 
\begin{exampleNumbered}\label{ex:forallexists Fpalg}
If the universal-existential $\mathcal L_{\operatorname{R}}$-sentence $\sigma$ holds in
all sufficiently large finite fields of characteristic $p$, then $\sigma$ holds in the algebraic closure 
$\mathbb F_p^{\alg}$
of $\mathbb F_p$. (See also Example~\ref{ex:Fpalg}.)
\end{exampleNumbered}

\begin{lemma}\label{lem:elementary chains}
Suppose  $\mathbf M_\lambda\preceq \mathbf M_{\lambda'}$ for all $\lambda\leq\lambda'$. Then $\mathbf M_\lambda\preceq\mathbf M$ for all $\lambda$.
\end{lemma} 
\begin{proof}
By induction on $n$ we show that for each $\lambda$ and each $\mathcal L_{M_\lambda}$-sentence $\sigma$ of length $n$ we have $\mathbf M_\lambda\models\sigma\Longleftrightarrow \mathbf M\models\sigma$.
This is clear if~$\sigma$ is atomic by Corollary~\ref{cor:persist, 1},~(1), and  the desired property is preserved under taking negations, conjunctions, and disjunctions.
So let $\varphi(x)$ be an $\mathcal L_{M_\lambda}$-formula, where~$x$ is a single quantifiable variable,
and $\sigma=\exists x\varphi$. 
Suppose first that $\mathbf M\models\sigma$, and take $a\in M_x$ with
$\mathbf M\models\varphi(a)$.
Then we can take some $\lambda'\geq\lambda$ such that  $a\in (M_{\lambda'})_x$.
By inductive hypothesis $\mathbf M_{\lambda'}\models\varphi(a)$ and so
$\mathbf M_{\lambda'}\models\sigma$, hence $\mathbf M_\lambda\models \sigma$ since
$\mathbf M_\lambda\preceq \mathbf M_{\lambda'}$. Conversely, suppose 
 $\mathbf M_\lambda\models \sigma$, and take $a\in (M_\lambda)_x$ with
 $\mathbf M_\lambda\models\varphi(a)$; then $\mathbf M\models\varphi(a)$ by inductive
 hypothesis, hence $\mathbf M\models\sigma$.
 \end{proof}




\subsection*{Algebraic closure and definable closure} 
Let $A$ be a parameter set in $\mathbf M$ and~$b \in M_{\mathbf s}$. The tuple $b$ is said to be {\bf $A$-definable} in $\mathbf M$ (or {\bf definable over~$A$}
in~$\mathbf M$) if $\{b\}\subseteq M_{\mathbf s}$ is $A$-definable, and is said to be {\bf $A$-algebraic}
in $\mathbf M$ (or {\bf algebraic over $A$} in $\mathbf M$) if $b\in X$ for some finite $A$-definable set
$X\subseteq M_{\mathbf s}$. If $\mathbf M\preceq\mathbf N$, then $b$ is definable over $A$ in $\mathbf M$
iff $b$ is definable over $A$ in $\mathbf N$, and similarly with ``algebraic'' in place of ``definable''.
In the above we omit ``in $\mathbf M$'' if $\mathbf M$ is clear from the context.
Clearly ``$A$-definable'' implies ``$A$-algebraic''. \index{element!definable}\index{element!algebraic} \index{definable!tuple}\index{algebraic!tuple}

\begin{lemma}\label{lem:dcl and def fns} 
The tuple $b$ is $A$-definable if and only if $f(a)=b$ for some 
finite multivariable $x$, $0$-definable $X\subseteq M_x$, $a\in X\cap A_x$, and $0$-definable $f\colon X\to M_{\mathbf s}$. 
\end{lemma}
\begin{proof}
The ``if'' direction is obvious. 
For the ``only if'' direction, suppose $b$ is $A$-definable. Take a finite multivariable $x$, a $0$-definable set
$Y\subseteq M_x\times M_{\mathbf s}$, and an $a\in A_x$ such that $Y(a)=\{b\}$. Then the set 
$$X\ :=\ \big\{a'\in M_x:\ |Y(a')|=1\big\}\ \subseteq\ M_x$$
is $0$-definable, and
$f\colon X \to M_{\mathbf s}$ given by $Y(a')=\big\{f(a')\big\}$ does the job.
\end{proof}

\noindent
Let 
$\operatorname{dcl}(A)$
be the parameter set in $\mathbf M$ such that for every $s$,
$$\operatorname{dcl}(A)_s\ =\ \{b \in M_s:\  \text{$b$ is definable over $A$}\},$$ 
and define   $\operatorname{acl}(A)$ likewise, with ``algebraic''
instead of ``definable''.\nomenclature[Bm1]{$\operatorname{acl}(A)$}{algebraic closure of $A$}\nomenclature[Bm2]{$\operatorname{dcl}(A)$}{definable closure of $A$} Call $\operatorname{dcl}(A)$ (respectively, $\operatorname{acl}(A)$) the 
{\bf definable
closure} of $A$ in $\mathbf M$ (respectively, the {\bf algebraic closure} of $A$ in $\mathbf M$). We say
that $A$ is {\bf definably closed} in $\mathbf M$ (respectively, {\bf algebraically closed} in $\mathbf M$) if
$\operatorname{dcl}(A) = A$ (respectively, $\operatorname{acl}(A) = A$). 
It is easy to check that 
$\operatorname{dcl}(A)$ is
definably closed in $\mathbf M$, and that $\operatorname{acl}(A)$ is algebraically closed in $\mathbf M$.
Both $\operatorname{dcl}(A)$ and $\operatorname{acl}(A)$ do not change if we pass from $\mathbf M$
to an elementary extension.
Clearly $\operatorname{dcl}(A)\subseteq\operatorname{acl}(A)$, and
if $A$ is algebraically closed in~$\mathbf M$, then $A$ is definably closed in~$\mathbf M$. Note that if $\mathbf M$ is
one-sorted and there exists an $A$-definable total ordering
on the underlying set $M$ of $\mathbf M$, then $\operatorname{dcl}(A)=\operatorname{acl}(A)$.


\index{closure!definable} \index{closed!definably}  \index{closure!algebraic} \index{closed!algebraically} \index{definable!closure}\index{algebraically!closed}\index{algebraic!closure}


\noindent
Suppose $\mathcal L$ has for each $s$ a constant symbol of sort~$s$.
%that for each $s$ we have $A_s\neq\emptyset$ or .
If $A$ is definably closed in~$\mathbf M$, then
$A$ underlies a substructure of $\mathbf M$. Hence both  
$\operatorname{dcl}(A)$ and
$\operatorname{acl}(A)$ underlie substructures of~$\mathbf M$, also denoted by
$\operatorname{dcl}(A)$ and $\operatorname{acl}(A)$, respectively, with $\<A\>_{\mathbf M}\subseteq \operatorname{dcl}(A)\subseteq\operatorname{acl}(A)$.

\medskip
\noindent
If $a\in M_{\mathbf s}$ is $A$-definable, then $a$ is $A_0$-definable for some finite subset $A_0$ of $A$, and similarly with ``algebraic'' in place of ``definable''.
%Hence for all $a\in\operatorname{dcl}(A)$ there is a finite $A_0\subseteq A$ with
%$a\in\operatorname{dcl}(A_0)$; similarly with $\operatorname{acl}$ in place of $\operatorname{dcl}$.
If $A\subseteq B\subseteq M$, then $\operatorname{dcl}(A)\subseteq\operatorname{dcl}(B)$ and
$\operatorname{acl}(A)\subseteq\operatorname{acl}(B)$.

\begin{lemma}\label{lem:dcl, acl}
Let $b\in M_s$ and set $X:=\big\{\sigma(b):\sigma\in\Aut(\mathbf M|A)\big\}\subseteq M_s$.
If $b\in\operatorname{dcl}(A)_s$, then $X=\{b\}$, and if
$b\in\operatorname{acl}(A)_s$, then $X$ is finite.
\end{lemma}

\begin{example}
Let $K$ be a field  and
$V$ an infinite $K$-linear space viewed as an $\mathcal L_{\text{$K$-mod}}$-structure
as in Example~\ref{ex:L-structures},~(7), and $A\subseteq V$. Then  $$\operatorname{dcl}(A)\ =\ \operatorname{acl}(A)\ =\ \text{the subspace of $V$ generated by $A$.}$$ To see this, let $W$ be the subspace of~$V$ generated by $A$.
Then $V\setminus W$ is infinite and is an orbit
for the action of $\Aut(V|A)$ on $V$. Now use 
Lemma~\ref {lem:dcl, acl}.
\end{example}


\subsection*{Notes and comments}
The notion of elementary equivalence is from~\cite{Tarski36}.
The fact about countable dense ordered sets without endpoints from~\ref{ex:DLO} is due to Cantor~\cite{Cantor}, with the back-and-forth proof found by Huntington~\cite{Huntington} and Hausdorff~\cite{Hausdorff14}. Proposition~\ref{prop:bf, 2} goes back to Ehrenfeucht~\cite{Ehrenfeucht} and Fra\"\i{}ss\'e~\cite{Fraisse}. (See \cite{Felgner02, Plotkin} for the history of ``back-and-forth''.)
Elementary extensions as well as Propositions~\ref{prop:TV} and~\ref{prop:LS downwards}  and Lemma~\ref{lem:elementary chains} are from \cite{TarskiVaught}. 
 L\"owenheim~\cite{Loewenheim} and Skolem~\cite{Skolem20} had shown 
Proposition~\ref{prop:LS downwards} in the case where $\mathcal L$ is countable; in the stated form it appears in \cite{TarskiVaught}.
Example~\ref{ex:LS downwards} is from \cite[Section~3.1]{Hodges}.
Model-theoretic algebraic closure was introduced by A.~Robinson~\cite[p.~157]{Robinson65} and gained prominence through the work of
Morley~\cite{Morley} and Baldwin-Lachlan~\cite{BaldwinLachlan}.


\section{Models and the Compactness Theorem}\label{sec:compactness}

\noindent
{\it In the rest of this appendix, unless indicated otherwise, $t$ is an $\mathcal L$-term, $\varphi$, $\psi$, and~$\theta$ are $\mathcal L$-formulas,
$\sigma$ is an $\mathcal L$-sentence, and $\Sigma$ is a set of $\mathcal L$-sentences.}\/ We drop the prefix
$\mathcal L$ in ``$\mathcal L$-term'', ``$\mathcal L$-formula'' and so on, unless this would cause confusion. 

\subsection*{Models}
We say that $\mathbf M$ is a {\bf model of $\Sigma$} or {\bf $\Sigma$ holds in $\mathbf M$} (notation: $\mathbf M\models\Sigma$)
if $\mathbf M\models\sigma$ for all $\sigma\in\Sigma$. \index{model} \index{structure!model}
%A class $\mathfrak K$ of $\mathcal L$-structures is said to be {\bf elementary} if there is a set of $\mathcal L$-sentences whose models are exactly the $\mathcal L$-structures in $\mathfrak K$.

\nomenclature[Bl1]{$\mathbf M\models\Sigma$}{$\mathbf M$ is a model of $\Sigma$}


To discuss examples it is convenient to introduce some notation. Suppose $\mathcal L$
contains (at least) the constant symbol $0$ and the binary function symbol $+$.
Given any terms~$t_1,\dots,t_n$ we define the term $t_1+\cdots+t_n$ inductively as follows:
it is the term~$0$ if $n = 0$, the term $t_1$ if $n = 1$, and the term $(t_1 + \cdots + t_{n-1})+t_n$
for~$n \geq 2$. We write $nt$ for the term $t+\cdots+t$ with $n$ summands, in particular, $0t$
and $1t$ denote the terms $0$ and $t$ respectively. Suppose $\mathcal L$ contains the constant
symbol~$1$ and the binary function symbol $\cdot$ (the multiplication sign). Then we
have similar notational conventions for $t_1 \cdot \ldots \cdot t_n$ and $t^n$; in particular, for $n = 0$
both stand for the term~$1$, and $t^1$ is just $t$.

\begin{examplesNumbered}\label{ex:theories}
Fix three distinct quantifiable variables $x$, $y$, $z$.  
\begin{enumerate}
\item {\it Groups}\/ are the  $\mathcal L_{\operatorname{G}}$-structures that are models of
\begin{align*}
\qquad\operatorname{Gr}\ :=\ \big\{\, & \forall x(x \cdot 1 = x),\ \forall x\big(x \cdot x^{-1} = 1\big),  \\
&\, \forall x \forall y \forall z\big((x \cdot y) \cdot z = x \cdot (y \cdot z)\big)\big\}.
\end{align*}
\item {\it Abelian groups}\/ are the $\mathcal L_{\operatorname{A}}$-structures that are models of
\begin{align*}
\qquad\operatorname{Ab}\ :=\ \big\{\, & \forall x(x + 0 = x),\ \forall x\big(x + (-x) = 0\big),\ \forall x \forall y(x + y = y + x), \\
&\, \forall x \forall y \forall z\big((x + y) + z = x + (y + z)\big)\big\}.
\end{align*}
\item {\it Torsion-free abelian groups}\/ are the $\mathcal L_{\operatorname{A}}$-structures that are models of
$$\operatorname{Tf}\ :=\ \operatorname{Ab}\ \cup\ \big\{ \forall x(nx = 0 \to x = 0) : n = 1, 2, 3, \dots \big\},$$
and {\it divisible abelian groups}\/ are the $\mathcal L_{\operatorname{A}}$-structures that are models of
$$\operatorname{Div}\ :=\ \operatorname{Ab}\ \cup\ \big\{ \forall x\exists y(ny = x) : n = 1, 2, 3, \dots \big\}.$$
\item {\it Ordered sets}\/ are the $\mathcal L_{\operatorname{O}}$-structures that are models of
\begin{align*}
 \operatorname{Or}\ :=\ \big\{\, &
\forall x(x\leq x), \ 
\forall x\forall y\forall z \big( (x\leq y \wedge y \leq z) \to x\leq z\big), \\
&\, \forall x\forall y \big( (x\leq y \wedge y\leq x) \to x=y\big) \big\}.
\end{align*}
Abbreviating $x\leq y\ \wedge \neg x = y$ by $x<y$, {\it dense ordered sets without endpoints}\/ are the $\mathcal L_{\operatorname{O}}$-structures that are models of
$$\qquad\operatorname{DLO}\ :=\ \operatorname{Or}\ \cup\ \big\{\forall x\forall y\exists z(x<y\to x<z \wedge z<y), \
\forall x\exists y\exists z ( y<x \wedge x<z) \big\}.$$
\item {\it Ordered abelian groups}\/ are the $\mathcal L_{\operatorname{OA}}$-structures that are models of
$$\operatorname{OAb}\ :=\ \operatorname{Or}\cup\operatorname{Ab}\cup\big\{\forall x \forall y \forall z
(x\leq y \to x+z\leq y+z) \big\}.$$
\item {\it Rings}\/ are the $\mathcal L_{\operatorname{R}}$-structures that are models of
\begin{align*}
\hskip2.5em  \operatorname{Ri}\ :=\ \operatorname{Ab} \cup \big\{\, & \forall x\forall y\forall z
\big( (x \cdot  y) \cdot  z = x \cdot  (y \cdot  z) \big), \forall x ( x \cdot  1 = x \wedge 1 \cdot  x = x), \\
&\, \forall x\forall y\forall z \big(
x \cdot  (y + z) = x \cdot  y + x \cdot  z \wedge (x + y) \cdot  z = x \cdot  z + y \cdot  z\big)\big\}.
\end{align*}
\item {\it Fields}\/ are the $\mathcal L_{\operatorname{R}}$-structures that are models of
$$\operatorname{Fl}\ :=\ \operatorname{Ri}\ \cup\ \big\{\,\forall x\forall y(x \cdot  y = y \cdot  x),\ 1 \neq 0,\ \forall x\big(x \neq 0 \to \exists y (x \cdot  y = 1)\big) \big\}.$$
\item {\it Ordered rings}\/ are the $\mathcal L_{\operatorname{OR}}$-structures that are models of
$$\operatorname{ORi}\ :=\ \operatorname{OAb}\cup\operatorname{Ri}\cup\big\{\forall x\forall y( 0 \leq x \wedge 0 \leq y \to 0\leq x\cdot y)\big\},$$
and {\it ordered fields}\/ are the $\mathcal L_{\operatorname{OR}}$-structures that are models of
$\operatorname{OFl}:=\operatorname{ORi}\cup\operatorname{Fl}$.
\item {\it Fields of characteristic $0$}\/ are the $\mathcal L_{\operatorname{R}}$-structures that are models of
$$\operatorname{Fl}(0)\ :=\  \operatorname{Fl}\ \cup\ \{n1 \neq 0 : n = 2, 3, 5, 7, 11, \dots \},$$
and given a prime number $p$, {\it fields of characteristic $p$}\/ are the $\mathcal L_{\operatorname{R}}$-structures that are models of $\operatorname{Fl}(p) := \operatorname{Fl}\ \cup\ \{p1=0\}$.
\item {\it Algebraically closed fields}\/ are the $\mathcal L_{\operatorname{R}}$-structures that are models of
$$\operatorname{ACF}\ :=\ \operatorname{Fl}\ \cup\ \big\{\forall u_1 \cdots \forall u_n \exists x(x^n+u_1x^{n-1}+\cdots+u_n = 0) : n \geq 2\big\}.$$
Here $u_1, u_2, u_3, \dots$ is some fixed infinite sequence of distinct quantifiable variables, distinct
also from $x$, and $u_ix^{n-i}$ abbreviates $u_i \cdot  x^{n-i}$, for $i = 1, \dots , n$.
\item Given a prime number $p$ or $p=0$, {\it algebraically closed fields of characteristic~$p$}\/ are the $\mathcal L_{\operatorname{R}}$-structures that are
models of $\operatorname{ACF}(p)\ :=\  \operatorname{ACF} \cup \operatorname{Fl}(p)$.
\end{enumerate}
\end{examplesNumbered}


\nomenclature[Bi11]{$\operatorname{ACF}$}{theory of algebraically closed fields in the language $\mathcal L_{\operatorname{Ri}}$}
\nomenclature[Bi12]{$\operatorname{ACF(p)}$}{theory of algebraically closed fields of characteristic $p$ in the language $\mathcal L_{\operatorname{Ri}}$}

\noindent
Here is the important Compactness Theorem: \index{theorem!Compactness Theorem}

\begin{theorem}\label{thm:compactness, 1}
If every finite subset of~$\Sigma$ has a model, then $\Sigma$ has a model.
\end{theorem}

\noindent
We give the proof of this theorem in the next section. The rest of this section contains some
reformulations and 
simple but instructive applications of this theorem.


\subsection*{Logical consequence}
We say that $\sigma$ is a {\bf logical consequence} of $\Sigma$ (writ\-ten~${\Sigma\models\sigma}$) if $\sigma$
is true in every model of $\Sigma$. More generally, we say that a formula~$\varphi$ is 
a {\bf logical consequence} of~$\Sigma$ (notation: $\Sigma\models\varphi$) if $\mathbf M\models\varphi$ for all models $\mathbf M$ of~$\Sigma$.
%Thus $\models\varphi$ iff $\emptyset\models\varphi$.
We also write $\sigma\models\varphi$ instead of $\{\sigma\}\models\varphi$.
Note that $\Sigma\cup\{\sigma_1,\dots,\sigma_n\}\models\varphi$
iff $\Sigma\models (\sigma_1\wedge\cdots\wedge\sigma_n)\to\varphi$. \index{logical!consequence} 

\nomenclature[Bl2]{$\Sigma\models\sigma$}{$\sigma$ is a logical consequence of $\Sigma$}

 
\begin{example}
It is well-known that in any ring $R$ we have $r \cdot 0 = 0$ for all $r\in R$.
This can now be expressed as $\operatorname{Ri}\models  x \cdot 0 = 0$.
\end{example}

\noindent
Here is a version of the Compactness Theorem in terms of {\em logical consequence}:

\begin{theorem} \label{thm:compactness, 2}
If $\Sigma\models\sigma$, then $\Sigma_0\models\sigma$
for some finite $\Sigma_0\subseteq \Sigma$.
\end{theorem}
\begin{proof} Suppose $\Sigma_0\not\models \sigma$ for all finite $\Sigma_0\subseteq\Sigma$. Then every finite subset of
$\Sigma\cup\{\neg\sigma\}$ has a model, so by Theorem~\ref{thm:compactness, 1}, $\Sigma\cup\{\neg\sigma\}$ has a model, and thus $\Sigma\not\models\sigma$.
\end{proof}

\noindent
A similar argument as in the proof of Theorem~\ref{thm:compactness, 2} shows:

\begin{cor}\label{cor:compactness, 2}
Let $(\sigma_i)_{i\in I}$ and $(\tau_j)_{j\in J}$ be families of sentences such that $$\textup{``}\bigwedge_{i\in I}\sigma_i \models\bigvee_{j\in J} \tau_j\textup{''},$$
that is, each structure which is a model of each sentence $\sigma_i$ is a model of one of the sentences $\tau_j$. Then there are
$i_1,\dots,i_m\in I$ and $j_1,\dots,j_n\in J$ such that $\sigma_{i_1}\wedge\cdots\wedge\sigma_{i_m}\models \tau_{j_1}\vee\cdots\vee\tau_{j_n}$.
\end{cor}
\begin{proof}
The hypothesis expresses that $\{\sigma_i:i\in I\}\cup\{\neg\tau_j:j\in J\}$ has no model. By the Compactness Theorem 
there are $i_1,\dots,i_m\in I$ and $j_1,\dots,j_n\in J$  such that $\{\sigma_{i_1},\cdots,\sigma_{i_m},\neg \tau_{j_1},\dots,\neg \tau_{j_n}\}$ has no model.
Thus $\sigma_{i_1}\wedge\cdots\wedge\sigma_{i_m}\models \tau_{j_1}\vee\cdots\vee\tau_{j_n}$.
\end{proof}


\noindent
Here is one of many applications of the Compactness Theorem:

\begin{cor}\label{cor:Robinson}
If the $\mathcal L_{\operatorname{R}}$-sentence $\sigma$ is true in all fields of characteristic $0$, then~$\sigma$ is true in all
fields of sufficiently high prime characteristic.
\end{cor}
\begin{proof} If $\operatorname{Fl} \cup \{n1 \neq 0 : n \geq 1\} \models \sigma$, then 
Compactness yields $N \in \N$ such that $\operatorname{Fl} \cup \{n1 \neq 0 : n = 1, \dots,N\} \models\sigma$, so
$\sigma$ holds in all fields of characteristic $p > N$.
\end{proof}

\noindent
%The converse of the implication in the previous corollary fails.
Note that $\operatorname{Fl}(0)$ is
infinite; the previous corollary implies that there is no finite set of $\mathcal L_{\operatorname{R}}$-sentences whose models are
exactly the fields of characteristic $0$.
Here is a typical application of Compactness (via Corollary~\ref{cor:Robinson}) in algebra:

\begin{exampleNumbered}[Noether-Ostrowski]\label{ex:NO}
Let $T=(T_1,\dots,T_n)$ and $P\in \Z[T]$.
Given a prime number $p$, let $P\bmod p$ denote the image of $P$
under the ring mor\-phism $\Z[T]\to\mathbb F_p[T]$ which extends
$a\mapsto a+p\Z\colon \Z\to\Z/p\Z=\mathbb F_p$ and sends~$T_i$ to~$T_i$~($i=1,\dots,n$).
{\it Suppose $P$ is irreducible over $\C$. Then there is some $N\in\N$
such that for all primes~$p>N$ and every field $F$ of characteristic $p$,
the polynomial~${P\bmod p}$ 
is irreducible over $F$.}\/
To see this note that every finitely generated field of characteristic $0$ can be embedded in $\C$,
so the hypothesis implies that $P$ is irreducible over every field of characteristic $0$,
and irreducibility of $P$ over a given field  can be expressed by a sentence: there exists an $\mathcal L_{\operatorname{Ri}}$-sentence $\sigma_P$ such that for each field~$F$, if $F$ has characteristic $0$ then
$F\models\sigma_P\Longleftrightarrow$ $P$ is irreducible over $F$, and if~$F$ has characteristic $p>0$ then
$F\models\sigma_P\Longleftrightarrow$ $P\bmod p$ is irreducible over~$F$.
\end{exampleNumbered}

\subsection*{Completeness and compactness}
We call $\Sigma$ {\bf complete} if $\Sigma$ has a model and for all $\sigma$, 
either $\Sigma\models\sigma$ or $\Sigma\models\neg\sigma$;
equivalently, $\Sigma$ has a model and $\mathbf M\equiv\mathbf N$ for all models $\mathbf M$, $\mathbf N$
of $\Sigma$.
Completeness is a strong property and it can be hard to show that a given
set $\Sigma$ is complete. \index{complete!set of sentences}

\begin{examples}
The set of $\mathcal L_{\operatorname{A}}$-sentences $\operatorname{Ab}$ (the set of axioms for abelian groups)
is not complete: consider $\exists x(x\neq 0)$.
The set of $\mathcal L_{\operatorname{O}}$-sentences~$\operatorname{DLO}$ (the set of axioms for dense ordered
sets without endpoints) is complete; see Example~\ref{ex:DLO}.
%Clearly, $\operatorname{ACF}$ is also not complete, since it says nothing about the characteristic. However, the set $\operatorname{ACF}(p)$ of axioms for algebraically closed fields of characteristic $p$ (where $p$ is a prime number or $p=0$) is complete; see Theorem~\ref{thm:ACFp} below.
\end{examples}

\nomenclature[Bm3]{$\operatorname{Th}(\mathbf M)$}{theory of $\mathbf M$}
\nomenclature[Bm31]{$\operatorname{Th}(\mathcal C)$}{theory of a class $\mathcal C$ of $\mathcal L$-structures}
\nomenclature[Bm32]{$\operatorname{Th}(\Sigma)$}{set of logical consequences of $\Sigma$}


\noindent
An {\bf $\mathcal L$-theory} is a set $T$ of 
$\mathcal L$-sentences such that for all
$\sigma$, if $T \models \sigma$, then $\sigma \in T$.\index{theory}
In particular, we have for any $\Sigma$ the $\mathcal{L}$-theory
$$\operatorname{Th}(\Sigma)\ :=\ \{\sigma:\ \Sigma\models\sigma\}$$
An {\bf axiomatization\/} of an $\mathcal L$-theory $T$ is a set $\Sigma$ such that $\operatorname{Th}(\Sigma)=T$. We use the symbol
$\operatorname{Th}$ also in another way: for any $\mathbf M$, the set 
$$\operatorname{Th}(\mathbf M)\ :=\ \{\sigma:\mathbf M\models\sigma\}$$ is a complete $\mathcal L$-theory,
called the {\bf theory of~$\mathbf M$}.\index{theory!of a structure}  (Thus if $\Sigma$ has a model, then $\Sigma\subseteq T$ for some complete $\mathcal{L}$-theory $T$.)\index{axiomatization}\index{theory!axiomatization} Given a class $\mathcal C$ of $\mathcal L$-structures, we set
$$\operatorname{Th}(\mathcal C)\ :=\ \bigcap_{\mathbf M\in\mathcal C} \operatorname{Th}(\mathbf M)\ =\ \{\sigma:\ \sigma \text{ is true in every $\mathbf M\in \mathcal C$}\}.$$
This is an $\mathcal L$-theory (not necessarily complete), called the {\bf theory of $\mathcal C$}. Thus $\operatorname{Th}(\Sigma)=\operatorname{Th}(\mathcal C)$,
where $\mathcal C$ is the class of models of $\Sigma$.\index{theory!of a class of structures} 

\medskip
\noindent
A complete $\mathcal L$-theory that contains $\Sigma$ is called a {\bf completion} of $\Sigma$. 
Let $\operatorname{S}(\Sigma)$ be the set of completions of $\Sigma$, and set
$\<\sigma\>:=\{ T \in \operatorname{S}(\Sigma): \sigma\in T\}$.
One verifies easily that for sentences $\sigma$, $\tau$ we have
$\<\sigma\>=\<\tau\>$ iff $\Sigma\models\sigma\leftrightarrow\tau$, and
$$\<\sigma\wedge\tau\>=\<\sigma\>\cap\<\tau\>,\quad \<\sigma\vee\tau\>=\<\sigma\>\cup\<\tau\>,\quad
\<\neg\sigma\>= \operatorname{S}(\Sigma)\setminus\<\sigma\>.$$
The topology on $\operatorname{S}(\Sigma)$ with
the sets $\<\sigma\>$ as a basis is called the {\bf Stone topology}. 
Its open sets are the unions
$\bigcup_{\sigma\in\Delta} \<\sigma\>$ with $\Delta$ a set
of sentences. Note that the basic open sets $\<\sigma\>$ are also
closed, and so the Stone topology on~$\operatorname{S}(\Sigma)$  is hausdorff.  
%if $T,T'\in \operatorname{S}(\Sigma)$  and  $\sigma\in T$, $\sigma\notin T'$, then $\neg\sigma\in T'$ by completeness of $T$, so $T\in\<\sigma\>$, $T'\in\<\neg\sigma\>$, and $\<\sigma\>\cap\<\neg\sigma\>=\emptyset$.
We have $\operatorname{S}(\Sigma)\neq
\bigcup_{\sigma\in\Delta} \<\sigma\>$ iff $\Sigma\cup\{\neg\sigma:\sigma\in\Delta\}$ has a model; 
hence Theorem~\ref{thm:compactness, 1} also has the following reformulation, explaining the name ``Compactness Theorem''.  \index{completion!of a set of sentences}\index{topology!Stone}

\begin{theorem}\label{thm:compactness, 3}
The topological space $\operatorname{S}(\Sigma)$ is compact.
\end{theorem}

\noindent
Let $\Sigma'$ also be a set of $\mathcal{L}$-sentences.
Then $\Sigma$ and $\Sigma'$ are said to be {\bf equivalent} if
they have the same logical consequences. Thus $\Sigma$ and $\Sigma'$ are equivalent iff they  have the same models, iff $\operatorname{S}(\Sigma)=\operatorname{S}(\Sigma')$.  Note that $\Sigma$ and
$\operatorname{Th}(\Sigma)$ are equivalent. 

\index{equivalence!of sets of sentences}

\subsection*{Completeness and decidability} This subsection concerns the relation between completeness and (algorithmic) decidability, a logical issue that is hardly model-theoretic in nature. We just give
an outline and refer to the literature for details.

First, one should distinguish the notion of ``logical consequence of'' from that of
``provable from''. To make the latter concept precise requires a {\em proof system}, which specifies logical axioms and
inference rules for generating certain finite sequences of formulas, called (formal) proofs:
a {\it proof of $\varphi$ from $\Sigma$\/} is a sequence $\varphi_1,\dots,\varphi_n$
of formulas with~$n \geq 1$ and $\varphi_n = \varphi$, such that for $k = 1, \dots, n$,
either $\varphi_k\in\Sigma$, or $\varphi_k$ is a logical axiom, or $\varphi_k$ is ``inferred'' from some of the earlier formulas
$\varphi_1,\dots,\varphi_{k-1}$ by applying an inference rule. (For example, among the logical axioms might be all formulas of the form $\varphi\vee \neg \varphi$, and among the inference rules is usually {\em Modus Ponens}, which allows
one to infer $\psi$ from $\phi$ and $\phi\to \psi$; 
see for example \cite[Section~2.6]{Shoenfield} for an explicit proof system.)
We call $\varphi$ {\it provable from $\Sigma$}  (in symbols: $\Sigma\vdash \varphi$)
if there exists a proof of $\varphi$
from~$\Sigma$.
The logical axioms and inference rules are chosen so that the logical axioms are valid in all $\mathcal L$-structures, and 
if $\varphi$ is inferred from $\varphi_1,\dots,\varphi_{k}$ by an inference rule, then $\varphi$ is valid in all 
$\mathcal{L}$-structures where
$\varphi_1,\dots,\varphi_{k}$ are valid. Hence $\Sigma\vdash\varphi\Rightarrow \Sigma\models\varphi$. We now fix
some traditional proof system for classical predicate logic.
Then the converse also holds: \index{theorem!Completeness Theorem}

\begin{theorem}[G\"odel's Completeness Theorem]\label{thm:Completeness}
If $\Sigma\models\varphi$, then $\Sigma\vdash\varphi$.
\end{theorem}

\noindent
See \cite[Chapter~4]{Shoenfield} for a proof. 
``Completeness'' here refers to the proof system, not to $\Sigma$.
Theorem~\ref{thm:Completeness} and its converse immediately yield version \ref{thm:compactness, 2}
of the Compactness Theorem (of which we give
an independent proof in the next section).

\medskip
\noindent
Suppose now that the language $\mathcal L$ has only finitely many nonlogical symbols. Then formulas can be made
into inputs of computer programs, and the logical axioms and inference rules of the proof system hiding behind the notation $\vdash$ can also be effectively given.  
One says that $\Sigma$ is {\it effectively enumerable}\/ if there is an effective procedure that enumerates all elements of $\Sigma$. 
We say that an $\mathcal{L}$-theory $T$ is {\it decidable}\/ if there is 
an algorithm (program) that takes any sentence $\sigma$ as input and decides whether or not~$\sigma\in T$.
If $\Sigma$ is effectively enumerable,
then so is the set $\operatorname{Th}(\Sigma)$ of all sentences provable from~$\Sigma$, and we obtain:

\begin{cor}\label{cor:Completeness}
If $\mathcal L$ has only finitely many nonlogical symbols and $\Sigma$ is complete and effectively enumerable, then $\operatorname{Th}(\Sigma)$ is decidable.
\end{cor}
 
\subsection*{Notes and comments}
The notion of ``model'' goes back to the Hilbert school. (But it was Tarski~\cite{Tarski54} who first spoke of ``model theory'' as a subject in its own right.)
Theorem~\ref{thm:Completeness} was  proved by  G\"odel~\cite{Goedel30} (1930)
for countable languages and by Hen\-kin~\cite{Henkin49} (1949) in general.
The Compactness Theorem  was shown independently by Mal$'$cev~\cite{Malcev36}~(1936). The formulation in Theorem~\ref{thm:compactness, 3} is due to Tarski~\cite{Tarski52}.
%Deligne~\cite[p.~336]{SGA4-2} rediscovered the Completeness Theorem in a topos-theoretic context; see~\cite{MakkaiReyes}. 
Corollary~\ref{cor:Robinson} is due to A.~Robinson~\cite{Robinson65}.
Algebraic proofs of the statement in Example~\ref{ex:NO} were given by Noether~\cite{Noether22} and Ostrowski~\cite{Ostrowski19}. 




\section{Ultraproducts and Proof of the Compactness Theorem}\label{sec:ultra products}

\noindent
%In this section we use ultraproducts to prove the Compactness Theorem.
In this section $\Lambda$ is a nonempty (index) set and
$\lambda$, $\lambda'$ range over $\Lambda$.


\subsection*{Filters and ultrafilters}
A {\bf proper filter} on $\Lambda$ is a nonempty collection $\mathcal F$ of subsets of $\Lambda$ such that:
\begin{list}{}{\leftmargin=2.5em}
\item[(F1)] $\emptyset\notin\mathcal F$,
\item[(F2)] if $A,B\in\mathcal F$, then $A\cap B\in\mathcal F$; and
\item[(F3)] if $A\subseteq B\subseteq \Lambda$ and $A\in\mathcal F$, then $B\in\mathcal F$.
\end{list}
Note that then $\Lambda\in\mathcal F$ by (F3), and
that for all $A\subseteq \Lambda$, either $A\notin\mathcal F$ or $\Lambda\setminus A\notin\mathcal F$, by (F1) and (F2).  
%Also, if $A,B\subseteq \Lambda$ with $A\cap B\in\mathcal F$, then $A\in\mathcal F$ and $B\in\mathcal F$ by (F3).

\begin{example}
If $\Lambda$ is infinite, then the set of all cofinite subsets of $\Lambda$ is a proper filter on $\Lambda$, called the {\bf Fr\'echet filter} on $\Lambda$. \index{filter!proper}\index{filter!Fr\'echet}
\end{example}

\noindent
A  proper filter on $\Lambda$ that is maximal with respect to inclusion is called an {\bf ultrafilter} on $\Lambda$. By Zorn, every proper filter on $\Lambda$ is included in an ultrafilter on $\Lambda$. \index{filter!ultrafilter}\index{ultrafilter}

%\begin{lemma}\label{lem:maximal F1 F2}
%Suppose $\mathcal F$ satisfies \textup{(F1)} and \textup{(F2)},
%and  is maximal with respect to this property. Then $\mathcal F$ satisfies \textup{(F3)}, hence
%is an ultrafilter on $\Lambda$.
%\end{lemma}
%\begin{proof}
%Let $A\in\mathcal F$ and put $\mathcal E:=\mathcal F\cup \{B\subseteq \Lambda: A\subseteq B\}$. One verifies easily that~$\mathcal E$ satisfies (F1) and (F2). Hence  $\mathcal E=\mathcal F$ by maximality of $\mathcal F$, so
%$A\in\mathcal F$. Hence $\mathcal F$ satisfies (F3).
%Let $A\in\mathcal F$ and put $\mathcal E:=\mathcal F\cup \{B\subseteq \Lambda: A\subseteq B\}$. We claim that $\mathcal E$ satisfies (F1) and (F2). Since (F1) holds trivially, let $B,C\in\mathcal E$; we need to show that $B\cap C\in\mathcal E$. This is clear if $B,C\in\mathcal F$ or $B,C\supseteq A$, so suppose $B\in\mathcal F$ and $C\supseteq A$ (say); then $B\cap C\supseteq B\cap A$ and hence $B\cap C\in\mathcal E$ by (F2). This shows the claim; hence  $\mathcal E$ satisfies (F3) by maximality of $\mathcal E$.
%\end{proof}

\begin{lemma}\label{lem:char ultrafilters}
Suppose $\mathcal F$ is a proper filter on $\Lambda$. Then the following are equivalent:
\begin{enumerate}
\item $\mathcal F$ is an ultrafilter on $\Lambda$;
\item for all $A,B\subseteq \Lambda$ with $A\cup B\in\mathcal F$ we have $A\in\mathcal F$ or $B\in\mathcal F$;
\item for all $A\subseteq \Lambda$
we have $A\in\mathcal F$ or $\Lambda\setminus A\in\mathcal F$.
\end{enumerate}
\end{lemma}
\begin{proof}  
Suppose $\mathcal F$ is an ultrafilter on $\Lambda$ and $A,B\subseteq \Lambda$, $A\cup B\in\mathcal F$. Then $A\cap F\neq\emptyset$ for all
$F\in\mathcal F$, or $B\cap F\neq\emptyset$ for all
$F\in\mathcal F$; we may assume that the first alternative holds. Then
$\{C\subseteq \Lambda:\  C\supseteq A\cap F \text{ for some }F\in \mathcal F\}$ is a proper filter on $\Lambda$ which includes
$\mathcal F\cup \{A\}$, so $A\in\mathcal F$. This shows (1)~$\Rightarrow$~(2), and
(2)~$\Rightarrow$~(3) follows by taking $B=\Lambda\setminus A$. The direction  (3)~$\Rightarrow$~(1) is obvious.
\end{proof}

\noindent
A nonempty collection $\mathcal F$ of subsets of $\Lambda$ has the {\bf finite intersection property}~(FIP) if for all $A_1,\dots,A_n\in\mathcal F$ with $n\geq 1$ we have $A_1\cap\cdots\cap A_n\neq\emptyset$. In particular, any proper filter
on $\Lambda$ has the FIP. \index{finite intersection property}

\begin{lemma}\label{lem:extend to uf}
Suppose the nonempty collection $\mathcal F$ of subsets of $\Lambda$ has the \textup{FIP}.
Then there exits an ultrafilter $\mathcal U\supseteq\mathcal F$ on~$\Lambda$.
\end{lemma}
\begin{proof}
Let $\mathcal F^*$ be the collection of all sets $A\subseteq \Lambda$ that contain an intersection $A_1\cap\cdots\cap A_n$
with $A_1,\dots,A_n\in\mathcal F$, $n\ge 1$. Then~$\mathcal F^*$ is a proper filter and $\mathcal F^*\supseteq \mathcal F$. By Zorn there exists an ultrafilter $\mathcal U\supseteq \mathcal F^*$.
\end{proof}


\subsection*{Ultraproducts}
Let  $(\mathbf M_\lambda)$ be a family of $\mathcal L$-structures and $\mathbf M:=\prod_\lambda \mathbf M_\lambda$ be its product.  (See Section~\ref{sec:languages}.)
Let $\sigma$ be an $\mathcal L_M$-sentence. Take
an $\mathcal L$-formula $\varphi(x)$ and $a\in M_{x}$ such that $\sigma=\varphi(a)$, and set
$$\| \sigma \| := \big\{ \lambda: \mathbf M_\lambda \models \varphi(a(\lambda)) \big\}.$$
This does not depend on the choice of $\varphi(x)$,~$a$.
If  $\sigma$, $\tau$ are $\mathcal L_M$-sentences, then
\begin{equation}\label{eq:boolean extension}
\|\sigma\ \&\ \tau\| = \|\sigma\|\cap\|\tau\|,\quad \|\sigma \vee \tau\| = \|\sigma\|\cup\|\tau\|, \quad
\|\neg\sigma\| = \Lambda \setminus\|\sigma\|,
\end{equation}
\begin{equation}\label{eq:implication-inclusion}
\models \sigma\to\tau\quad\Rightarrow\quad\|\sigma\|\subseteq\|\tau\|.
\end{equation}
Moreover:

\begin{lemma}\label{lem:witnesses}
Let $\psi(y)$ be an $\mathcal L_M$-formula, where $y$ is a quantifiable variable of sort~$s$. Then
for all $b\in M_s$ we have
$\|\psi(b)\| \subseteq \| \exists y\psi\|$,
and there exists $b\in M$ such that equality holds.
\end{lemma}
\begin{proof}
For each $b\in M_s$ we have
$\|\psi(b)\| \subseteq \| \exists y\psi\|$ by \eqref{eq:implication-inclusion}.
To obtain equality,  choose $b=(b(\lambda))\in M_s$ as follows:
Take an $\mathcal L$-formula $\varphi(x,y)$
and $a\in M_{x}$
such that $\psi(y)=\varphi(a,y)$. 
Then 
$$
\|\psi(b)\| = \big\{\lambda: 
\mathbf M_\lambda \models \varphi(a(\lambda),b(\lambda)) \big\}, \quad
\|  \exists y\psi\|=\big\{\lambda: 
\mathbf M_\lambda \models (\exists y \varphi)(a(\lambda))\big\}.$$
For $\lambda\in \|  \exists y\psi\|$ we pick $b(\lambda)\in (M_\lambda)_s$ such that
$\mathbf M_\lambda\models \varphi(a(\lambda),b(\lambda))$, and for $\lambda\notin \|  \exists y\psi\|$ we let $b(\lambda)\in (M_\lambda)_s$ be arbitrary.
Then 
$\|\psi(b)\|\supseteq \|  \exists y\psi\|$
as required.
\end{proof}

\noindent
Let $\mathcal F$ be a proper filter on $\Lambda$.
For  $s\in S$ we define a binary relation $\sim_s$ on $M_s$ by
$$a \sim_s b \quad :\Longleftrightarrow \quad \|a = b \| \in \mathcal F
\quad \Longleftrightarrow \quad \big\{\lambda:a(\lambda)=b(\lambda)\big\}\in\mathcal F.$$
For $a=(a_1,\dots,a_m),b=(b_1,\dots,b_m)\in M_{s_1\dots s_m}$
we set
$$a \sim_{s_1\dots s_m} b \quad :\Longleftrightarrow \quad a_1\sim_{s_1} b_1\ \&\ \cdots \ \&\ a_m\sim_{s_m} b_m.$$
Using \eqref{eq:implication-inclusion} one easily shows:

\begin{lemma} \mbox{}
\begin{enumerate}
\item The relation $\sim_{s_1\dots s_m}$ is an equivalence relation on $M_{s_1\dots s_m}$.
\item If $R \in \mathcal L^{\operatorname{r}}$ has
sort $s_1\dots s_m$, and $a,b\in M_{s_1\dots s_m}$, 
$a\sim_{s_1\dots s_m} b$, then $$\|R\,a\|\in\mathcal F\quad\Longleftrightarrow\quad\|R\,b\|\in\mathcal F.$$
\item If $f \in \mathcal L^{\operatorname{f}}$ has sort $s_1\dots s_n s$ and $a,b\in M_{s_1\dots s_n}$, $a\sim_{s_1\dots s_n} b$, then 
$$f^{\mathbf M}(a)\ \sim_s\  f^{\mathbf M}(b).$$
\end{enumerate}
\end{lemma}

\noindent
For $a\in M_{s_1\dots s_m}$ we let $a^{\sim}$ denote the equivalence class of $a$ with respect to $\sim_{s_1\dots s_m}$, and 
we let~$M^\sim_{s_1\dots s_m}$ be the set of equivalence classes of $\sim_{\mathbf s}$.
We identify $M^\sim_{s_1\dots s_m}$ with $M^\sim_{s_1}\times\cdots\times M^\sim_{s_m}$ in the natural way.
We now define an $\mathcal L$-structure $\mathbf M^{\sim}$ whose underlying set of sort~$s$ is $M^\sim_s$: 
for $R\in\mathcal L^{\operatorname{r}}$ of sort $s_1\dots s_m$ and $a\in M_{s_1\dots s_m}$ we set
$$a^\sim\in R^{\mathbf M^\sim}\quad:\Longleftrightarrow\quad \| R\,a\|\in\mathcal F,$$
and for $f \in \mathcal L^{\operatorname{f}}$ of sort $s_1\dots s_n s$ and $a\in M_{s_1\dots s_n}$ we put
$$f^{\mathbf M^\sim}(a^\sim)\ :=\ \big(f^{\mathbf M}(a)\big)^\sim\in M_s.$$
The $\mathcal L$-structure $\mathbf M^{\sim}$ is called the {\bf reduced product} of
$(\mathbf M_\lambda)$ with respect to $\mathcal F$, and is also denoted by
$\mathbf M/\mathcal F=\left(\prod_{\lambda} \mathbf M_\lambda\right)/\mathcal F$.
If $\mathbf M_\lambda=\mathbf N$ for all $\lambda$, then $\mathbf N^\Lambda/\mathcal F$ is also called the
{\bf reduced power} of $\mathbf N$ with respect to $\mathcal F$. 
If   $\mathcal F$ is an ultrafilter on~$\Lambda$, then we speak of the {\bf ultraproduct~$\mathbf M/\mathcal F$}
of $(\mathbf M_\lambda)$ with respect to $\mathcal F$
and of the {\bf ultrapower~$\mathbf N^\Lambda/\mathcal F$} of $\mathbf N$ with respect to $\mathcal F$.
The maps $a\mapsto a^\sim\colon M_s\to M_s^\sim$ combine to a morphism $\pi\colon\mathbf M\to \mathbf M^{\sim}$.
\index{structure!reduced product}\index{reduced product}\index{structure!ultraproduct}\index{ultraproduct}\index{structure!ultrapower}\index{ultrapower}


\begin{lemma}\label{lem:Los}
Let $\varphi(x)$ be an atomic $\mathcal L$-formula and   $a\in M_{x}$. Then
$$\mathbf M/\mathcal F\models \varphi(a^\sim) \quad\Longleftrightarrow\quad \| \varphi(a) \|\in\mathcal F.$$
\end{lemma}
\begin{proof}
Suppose first that $\varphi=Rt_1\dots t_m$ where  $R\in\mathcal L^{\operatorname{r}}$ has sort $s_1\dots s_m$
and $t_1,\dots,t_m$ are $\mathcal L$-terms of sort $s_1,\dots,s_m$, respectively. 
For notational simplicity we assume $m=1$ and set $t_1=t$.
We have $t(a^\sim)^{\mathbf M/\mathcal F} = t^{\mathbf M/\mathcal F}(a^\sim) =
{t^{\mathbf M}(a)}^\sim$,
using Lemma~\ref{lem:subst lemma, terms} for the first equality, hence
$$\mathbf M/\mathcal F\models\varphi(a^\sim)	\ \Longleftrightarrow\ 
t(a^\sim)^{\mathbf M/\mathcal F}={t^{\mathbf M}(a)}^\sim\in
R^{\mathbf M/\mathcal F} 
\ \Longleftrightarrow\  \big\| R\, t^{\mathbf M}(a)\big\|\in\mathcal F.$$
Also, by Lemma~\ref{lem:subst lemma, formulas}:
$$\big\| R\, t^{\mathbf M}(a)\big\|	=
\left\{ \lambda: \mathbf M_\lambda \models R\,t^{\mathbf M_\lambda}(a(\lambda)) \right\}
= \left\{ \lambda: \mathbf M_\lambda \models (R\,t)(a(\lambda)) \right\} =  \| \varphi(a) \|.$$
If $\varphi$ is of the form $t_1=t_2$ with $\mathcal L$-terms $t_1$, $t_2$,
then one argues similarly.
\end{proof}
 
 \begin{cor}
Let  $\Delta\colon\mathbf N\to\mathbf N^\Lambda$ be the diagonal embedding.
Then the morphism $\pi\circ\Delta\colon \mathbf N\to\mathbf N^\Lambda/\mathcal F$ is an  embedding, called the
{\bf diagonal embedding} of~$\mathbf N$ into its reduced power $\mathbf N^\Lambda/\mathcal F$. \index{embedding!diagonal}\index{diagonal!embedding}
\end{cor}

\noindent
We now come to the main theorem about ultraproducts: 

\begin{theorem}[{\L}o\'{s}]\label{thm:Los}
Suppose $\mathcal F$ is an ultrafilter on $\Lambda$.
Let $\varphi(x)$ be a formula and $a\in M_{x}$. Then
$\mathbf M/\mathcal F\models \varphi(a^\sim) \Longleftrightarrow \| \varphi(a) \|\in\mathcal F$.
\end{theorem}
\begin{proof}
We proceed by induction on the construction of $\varphi$. The case where $\varphi$ is atomic is covered by Lemma~\ref{lem:Los}. The cases where $\varphi=\neg\psi$, $\varphi=\psi_1\ \&\ \psi_2$, or $\varphi=\psi_1\vee\psi_2$ 
with formulas $\psi$, $\psi_1$, $\psi_2$
follow by induction, \eqref{eq:boolean extension}, and Lemma~\ref{lem:char ultrafilters}.
Suppose $\varphi=\exists y\psi$ where $\psi(x,y)$ is a formula and $y$ is  of sort $s$; then
\begin{align*}
\mathbf M/\mathcal F\models \varphi(a^\sim)	&\quad\Longleftrightarrow\quad
\text{$\mathbf M/\mathcal F\models \psi(a^\sim,b^\sim)$ for some $b\in M_s$}  \\
&\quad\Longleftrightarrow\quad \text{$\| \psi(a,b) \| \in\mathcal F$ for some $b\in M_s$,}
\end{align*}
by inductive hypothesis, and by Lemma~\ref{lem:witnesses} the latter statement is equivalent to 
$\| \varphi(a) \|\in\mathcal F$. The case where 
$\varphi=\forall y\psi$ follows,
since $\models \forall y\psi \leftrightarrow \neg\exists y\neg\psi$.
\end{proof}

\noindent
In particular, if $\mathcal F$ is an ultrafilter on $\Lambda$ and $\mathbf M_\lambda\models\Sigma$ for all $\lambda$, then $\mathbf M/\mathcal F\models\Sigma$.

\begin{example}
View abelian groups as $\mathcal L_{\operatorname{A}}$-structures in the natural way.
Let $\mathcal U$ be an ultrafilter on $\N^{\geq 1}$ containing the Fr\'echet filter,
$G:=\prod_{n\geq 1} \left(\Z/n\Z\right)/\mathcal U$, and $g:=(1+n\Z)^\sim\in G$.
Then by Theorem~\ref{thm:Los}, for each $m\geq 1$ we have $G\not\models m g=0$ since
$\| m g=0 \|$ is finite, hence not in $\mathcal U$. So $g$ has infinite order in $G$.
Thus there is no set of $\mathcal L_{\operatorname{A}}$-sentences whose models are the abelian torsion groups.
\end{example}



\begin{cor} If $\mathcal F$ is an ultrafilter on $\Lambda$, then the diagonal embedding  $\Delta$ of~$\mathbf N$ into $\mathbf N^\Lambda/\mathcal F$ is elementary.
\end{cor}
\begin{proof}
Let $\varphi(x)$ be a formula and $a\in N_x$ such that $\mathbf N \models
\varphi(a)$. Then $\| \varphi(\Delta(a)) \| = \Lambda\in\mathcal F$,
hence 
$\mathbf N^\Lambda/\mathcal F\models \varphi(\Delta(a)^\sim)$
by Theorem~\ref{thm:Los}.
\end{proof}

\subsection*{Proof of the Compactness Theorem}
We mean here Theorem~\ref{thm:compactness, 1}.
Thus, suppose every finite subset of $\Sigma$ has a model; we want to show that $\Sigma$ has a model.
For $\Lambda$ we take the set of all  finite subsets of $\Sigma$,
and for each $\lambda$  let~$\mathbf M_\lambda$ be a model of~$\lambda$.
For each $\lambda$ set
$\lambda^*:=\{\lambda' : \lambda\subseteq\lambda'\}$.
Then $\lambda_1^*\cap\lambda_2^*=(\lambda_1\cup\lambda_2)^*$ for all $\lambda_1,\lambda_2\in\Lambda$,
so $\Lambda^*:=\{ \lambda^* : \lambda\in\Lambda\}$ has the finite intersection property.
By Lemma~\ref{lem:extend to uf} take an ultrafilter $\mathcal U$ on $\Lambda$ containing $\Lambda^*$ and
put $\mathbf M:=\left(\prod_{\lambda} \mathbf M_{\lambda}\right)/\mathcal U$;
we claim that~$\mathbf M\models\Sigma$.
Let $\sigma\in\Sigma$. Then $\{ \sigma\}\in \Lambda$ and
$$\{\sigma\}^*  \subseteq
\{ \lambda  : \mathbf M_{\lambda}\models \sigma\} = \|\sigma\|.$$
We have $\{\sigma\}^*\in\mathcal U$, hence also
$\|\sigma\|\in\mathcal U$, so   
$\mathbf M\models \sigma$ by the theorem of {\L}o\'{s}. \qed


\subsection*{Functoriality of  ultraproducts}
Let $(\mathbf M_\lambda)$ and $(\mathbf N_\lambda)$ be families of $\mathcal L$-structures, and for each $\lambda$ let $h_\lambda\colon \mathbf M_\lambda\to\mathbf N_\lambda$ be a morphism. By Lemma~\ref{lem:morphisms on products} we have a morphism $h\colon \mathbf M:=\prod_\lambda \mathbf M_\lambda\to \mathbf N:=\prod_\lambda\mathbf N_\lambda$ such that $\pi_\lambda^{\mathbf N}\circ h=h_\lambda\circ \pi_\lambda^{\mathbf M}$ for each $\lambda$.  
Let $\mathcal F$ be a proper filter on $\Lambda$.
Then for all $a,b\in M_s$ we have $a\sim_s b \Rightarrow h_s a \sim_s h_s b$, hence we obtain
a map $h/{\mathcal F}\colon \mathbf M/{\mathcal F}\to\mathbf N/{\mathcal F}$ making the diagram 
$$\xymatrix{\mathbf M/{\mathcal F} \ar[r]^{h/{\mathcal F}} & \mathbf N/{\mathcal F}  \\
\mathbf M \ar[u] \ar[r]^h & \mathbf N \ar[u]
}$$
commute. Here the vertical arrows are the morphisms $\mathbf M\to\mathbf M/{\mathcal F}$ and  $\mathbf N\to\mathbf N/{\mathcal F}$ defined before Lemma~\ref{lem:Los}. One verifies easily that $h/{\mathcal F}$ is a morphism. If each~$h_\lambda$ is an
embedding and $\mathcal F$ is an ultrafilter on $\Lambda$, then $h/{\mathcal F}$ is an embedding.

We illustrate this functoriality of ultraproducts by proving a statement used in Section~\ref{pafae}.
If $\mathbf M\subseteq\mathbf N$, then we say that~$\mathbf M$ is
{\bf existentially closed in $\mathbf N$} if every existential $\mathcal L_M$-sentence true in $\mathbf N$ is true in
$\mathbf M$; equivalently, every universal $\mathcal L_M$-sentence true in $\mathbf M$ is true in
$\mathbf N$; notation:
$\mathbf M\preceq_\exists\mathbf N$. Note that if $\mathbf M\preceq_\exists\mathbf N$, then also each universal-existential $\mathcal L_M$-sentence true in $\mathbf N$ is true in
$\mathbf M$.
Clearly $\mathbf M\preceq \mathbf N\Rightarrow \mathbf M\preceq_\exists\mathbf N$.\index{closed!existentially} \index{structure!existentially closed}
\nomenclature[Bj02]{$\mathbf M\preceq_\exists\mathbf N$}{$\mathbf M$ is existentially closed in $\mathbf N$}

\begin{cor}\label{cor:ec in ext} Suppose $\mathbf M$ is the direct union of a directed family $(\mathbf M_\lambda)$ of substructures of $\mathbf M$ such that $\mathbf M_\lambda\models\Sigma$ for all $\lambda$. Then $\mathbf M$ is existentially closed in some model of~$\Sigma$.
\end{cor} 
\begin{proof}
Let $\mathcal F$ be the collection of all nonempty  
$A\subseteq\Lambda$ with the property that  for all $\lambda$, $\lambda'$, if $\lambda\in A$ and $\lambda\leq\lambda'$, then $\lambda'\in A$. Since $(\Lambda,{\leq})$ is directed, $\mathcal F$ has the FIP. Then Lemma~\ref{lem:extend to uf} yields an ultrafilter $\mathcal U$ on~$\Lambda$ which contains~$\mathcal F$, and so $\mathbf M^*:=\prod_\lambda \mathbf M_\lambda/{\mathcal U}$ is a model of $\Sigma$ by Theorem~\ref{thm:Los}. Let $\iota_\lambda\colon \mathbf M_\lambda\to\mathbf M$ be the natural inclusion, let
$\iota/{\mathcal U}\colon \mathbf M^* \to \mathbf M^\Lambda/{\mathcal U}$ be the embedding
obtained from the family of embeddings~$(\iota_\lambda)$ as described before the corollary, and
let $\Delta\colon \mathbf M\to \mathbf M^\Lambda/{\mathcal U}$ be the diagonal embedding.
Then $\Delta(\mathbf M)\subseteq (\iota/{\mathcal U})(\mathbf M^*)\subseteq \mathbf M^\Lambda/{\mathcal U}$ and $\Delta(\mathbf M)\preceq \mathbf M^\Lambda/{\mathcal U}$, hence
$\Delta(\mathbf M)$ is existentially closed in $(\iota/{\mathcal U})(\mathbf M^*)$.
\end{proof}

\subsection*{Notes and comments}
Ultrafilters were introduced by H.~Cartan~\cite{Cartan1,Cartan2}, and also appear in Stone~\cite{Stone36}.
%Lemma~\ref{lem:extend to uf} is due to Tarski~\cite{Tarski30}.
The definition of the ultraproduct and Theorem~\ref{thm:Los} are from~\cite{Los55a}, but
versions of ultraproducts had been used already by Skolem~\cite{Skolem31}, Hewitt~\cite{Hewitt},
and Arrow~\cite{Arrow}. Reduced products and the proof of the Compactness Theorem via ultraproducts given above are due to Frayne, Morel and Scott~\cite{FMS}.




\section{Some Applications of Compactness}\label{sec:LS}

\noindent
We first introduce  {\it diagrams,} which provide 
a way to construct embeddings using Compactness.
Next we study the relationship between {\it substructures}\/ and {\it universal sentences}. We also prove the ``upward'' version of the L\"owenheim-Skolem Theorem.
 
\subsection*{Diagrams}
In this subsection we assume $A\subseteq M$.
Let
$\operatorname{Diag}(\mathbf M)$ be the set of all quantifier-free sentences $\sigma$ such that  $\mathbf M\models\sigma$, and set $\operatorname{Diag}_A(\mathbf M):=\operatorname{Diag}(\mathbf M_A)$.
We call  $\operatorname{Diag}_M(\mathbf M)$ the (quantifier-free) {\bf diagram} of $\mathbf M$. \index{structure!diagram}\index{diagram}
\nomenclature[Bm4]{$\operatorname{Diag}_M(\mathbf M)$}{diagram of $\mathbf M$}

\begin{lemma}
Let  $h\colon A\to N$, and
$\mathbf N_h$ the expansion of $\mathbf N$ to an $\mathcal L_A$-structure
given by $\underline{a}^{\mathbf N_h}:=h_s(a)$ for $a\in A_s$. 
Then 
\begin{enumerate}
\item $h$ preserves quantifier-free formulas iff $\mathbf N_h\models \operatorname{Diag}_A(\mathbf M)$;
\item $h$ is elementary iff $\mathbf N_h\models\operatorname{Th}(\mathbf M_A)$.
\end{enumerate}
\end{lemma}

\noindent
This is rather obvious from the definitions, and yields:

\begin{lemma}[Diagram Lemma]\label{lem:diagram}
\mbox{}

\begin{enumerate}
\item There exists a map $A\to N$ preserving quantifier-free formulas if and only if some $\mathcal L_A$-expansion of
 $\mathbf N$ is a model of $\operatorname{Diag}_A(\mathbf M)$;
\item there exists an elementary map $A\to N$ if and only if some $\mathcal L_A$-expansion of
 $\mathbf N$ is elementarily equivalent to $\mathbf M_A$.
\end{enumerate}
\end{lemma}

 

\noindent
In particular,  there exists an embedding $\mathbf M\to\mathbf N$ iff $\mathbf N$ can be expanded to a model of 
the diagram of $\mathbf M$, and  there exists an elementary embedding $\mathbf M\to\mathbf N$ iff
$\mathbf N$ can be expanded to a model of $\operatorname{Th}(\mathbf M_M)$.
The Diagram Lemma   acquires its power through the Compactness Theorem:

\begin{cor}\label{cor:Henkin}
The following conditions on $\mathbf M$ are equivalent:
\begin{enumerate}
\item The structure $\mathbf M$ can be embedded into a model of $\Sigma$; 
\item every finite subset of $\Sigma\cup\operatorname{Diag}_M(\mathbf M)$ has a model.
\end{enumerate} 
For one-sorted $\mathbf M$, these conditons are also equivalent to: \begin{enumerate}
\item[(3)] every finitely generated substructure of $\mathbf M$ can be embedded into a model of $\Sigma$.
\end{enumerate}
Likewise, $\mathbf M$ has an elementary extension that is a model of $\Sigma$ iff
every finite subset of $\Sigma\cup\operatorname{Th}(\mathbf M_M)$ has a model.
\end{cor}
\begin{proof}
Use the Diagram Lemma, Compactness, and the observation that
every finite subset of $\Sigma\cup\operatorname{Diag}_M(\mathbf M)$ is contained in a set of the form
$\Sigma\cup\operatorname{Diag}_N(\mathbf N)$ where $\mathbf N$ is a finitely generated
substructure of~$\mathbf M$.
\end{proof}

%\begin{example}
%Every finite ordered set embeds into $(\Q,{\leq})$; hence by Corollary~\ref{cor:Henkin},
%every ordered set embeds into a dense ordered set without endpoints. 
%\marginpar{Need definition of ``dense without endpoints'' in Section~2.1.}
%\end{example}

\begin{cor}\label{cor:elem equivalence and elem embeddings}
$\mathbf M\equiv\mathbf N$ iff there exists an 
$\mathcal{L}$-structure into which both~$\mathbf M$ and~$\mathbf N$ can be ele\-men\-ta\-ri\-ly embedded.
\end{cor}
\begin{proof}
The ``if'' direction is obvious. For the ``only if'' direction, assume $\mathbf M\equiv\mathbf N$. Let $\mathcal L'$ extend $\mathcal L$ by names for the elements of the $M_s$ and $N_s$,
such that no name of any $a\in M_s$ is the name of any $b\in N_{s'}$;
thus $\mathcal L_M,\mathcal L_N\subseteq\mathcal L'$.
It suffices to show that every finite subset of the set $\operatorname{Th}(\mathbf M_M)\cup
\operatorname{Th}(\mathbf N_N)$ of $\mathcal L'$-sentences has a model. If not, then we can take a formula $\varphi(x)$ and some $a\in M_x$ such that $\{\varphi(a)\}\cup\operatorname{Th}(\mathbf N_N)$ has no model. Thus
no expansion of $\mathbf{N}_N$ to an $\mathcal L'$-structure  satisfies $\varphi(a)$; this yields $\mathbf N\models\forall x\,\neg\varphi$.
Since $\mathbf M\equiv\mathbf N$, we obtain $\mathbf M\models\forall x\,\neg\varphi$,
contradicting $\mathbf M\models\varphi(a)$.
\end{proof}

\noindent
In a similar way one shows:

\begin{cor}\label{cor:ex closed and embeddings} Let $\mathbf M \subseteq \mathbf N$. Then $\mathbf M\preceq_\exists\mathbf N$ if and only if $\mathbf N$ embeds over~$\mathbf M$ into some elementary extension of $\mathbf M$.
\end{cor}

\subsection*{Substructures and  universal sentences} 
Call $\Sigma$   {\bf universal} if all sentences in $\Sigma$ are universal. 
{\it In this subsection we assume that $\mathcal L$ has for each $s$ a constant symbol of sort~$s$}. Thus
$\<A\>_{\mathbf M}$ is defined for any parameter set $A$ in~$\mathbf M$.\index{universal!set of sentences}

\begin{prop}\label{prop:Herbrand}
Suppose $\Sigma$ is universal, $x=(x_1,\dots,x_m)$, $y=(y_1,\dots,y_n)$ are disjoint, and $\varphi(x,y)$ is quantifier-free
such that $\Sigma\models\forall x\exists y\, \varphi(x,y)$. Then there are $n$-tuples
$t_1=(t_{11},\dots,t_{1n}),\dots,t_k=(t_{k1},\dots,t_{kn})$  of terms $t_{ij}(x)$, $k\geq 1$,
with
$$\Sigma\models  \varphi(x,t_1(x))\vee\cdots\vee\varphi(x,t_k(x)).$$
\end{prop}

\noindent
The maneuver used in proving this will also be useful later: 
we extend the language~$\mathcal L$ by new constant symbols and let
them play the role of parameters. Let $x_1,\dots, x_m$ have sort $s_1,\dots, s_m$, respectively. Let  $\mathcal L_c:=\mathcal L\cup \{c_1,\dots,c_m\}$ where
$c_1,\dots,c_m$ are distinct new constant symbols of sort $s_1,\dots,s_m$, respectively. 
An $\mathcal L_c$-structure $(\mathbf M,a)$ is just an $\mathcal L$-structure $\mathbf M$ together with any $m$-tuple $a=(a_1,\dots,a_m)\in M_{x}$.
Thus, given any $\mathcal L$-formula
$\psi(x_1,\dots,x_m)$, 
$$\Sigma\models\psi(c_1,\dots,c_m)
\text{ (relative to $\mathcal L_c$)}\ \Longleftrightarrow\ \Sigma\models\psi(x_1,\dots, x_m) \text{ (relative to $\mathcal L$)}.$$ 

\begin{proof}[Proof of Proposition~\ref{prop:Herbrand}]  
Let 
$\mathbf M\models\Sigma$ and $a=(a_1,\dots,a_m)\in M_x$.
Since~$\Sigma$ is universal, $\mathbf N:=\<a_1,\dots,a_m\>_{\mathbf M}$ is also a model
of $\Sigma$. Hence $\mathbf N\models \forall x\exists y\, \varphi$ and so
$\mathbf N\models\exists y\, \varphi(a,y)$. The elements of $\mathbf N$ of sort~$s$
are of the form $t(a)$ where $t(x)$ is an $\mathcal L$-term of sort~$s$. Hence there
is an $n$-tuple $t=(t_1,\dots,t_n)$ of $\mathcal L$-terms $t_i(x)$ of the same sort as~$y_i$ such that $\mathbf N\models\varphi(a,t(a))$, and 
thus $\mathbf M\models\varphi(a,t(a))$. 
Hence every model of $\Sigma$, viewed as a set of
$\mathcal L_c$-sentences, satisfies some $\mathcal L_c$-sentence
$\varphi(c,t(c))$  with $t=(t_1,\dots,t_n)$ an $n$-tuple of $\mathcal L$-terms $t_i(x)$ of the
same sort as $y_i$ and $c=(c_1,\dots,c_m)$. Now use~\ref{cor:compactness, 2}.
\end{proof}

\noindent
The substructures of fields viewed as $\mathcal L_{\operatorname{R}}$-structures are exactly the integral domains,
that is, the models of the set of universal $\mathcal L_{\operatorname{R}}$-sentences
$$\operatorname{Ri}\cup\big\{ 0\neq 1,\ \forall x\forall y\, (x  y=y  x),\ \forall x\forall y\,
(xy=0 \to x=0 \vee y=0) \big\}.$$
This is an instance of the following general fact:

\begin{prop}\label{prop:LT}
Let 
$$\Sigma_\forall\ :=\ \big\{ \sigma : \text{$\sigma$ is a universal sentence with $\Sigma\models\sigma$} \big\}$$
be the set of universal logical consequences of $\Sigma$. Then $\mathbf M\models\Sigma_\forall$ iff
$\mathbf M$ is a substructure of some model of $\Sigma$.
\end{prop}
\begin{proof}
Suppose $\mathbf M\models\Sigma_\forall$.
To show that $\mathbf M$ is a substructure of a model of $\Sigma$,  let~$\Delta$ be a finite
subset of $\operatorname{Diag}_M(\mathbf M)$; by Corollary~\ref{cor:Henkin} it suffices to show that the set
$\Sigma\cup\Delta$ of $\mathcal L_M$-sentences has a model.
After replacing $\Delta$ by the singleton consisting of the conjunction of the elements of $\Delta$,
we may assume $\Delta=\{\varphi(a)\}$ where $\varphi(x)$ is a quantifier-free $\mathcal L$-formula,
$x=(x_1,\dots,x_n)$, and $a=(a_1,\dots,a_n)\in M_x$ with distinct $a_1,\dots,a_n$,
such that $\mathbf M\models\varphi(a)$. If $\Sigma\cup\Delta$ has no model, then
$\Sigma\models\neg\varphi(a)$ and hence $\Sigma\models\forall x\,\neg\varphi$.
Now the $\mathcal L$-sentence $\forall x\,\neg\varphi$ appears in $\Sigma_\forall$, thus is satisfied
by $\mathbf M$. Hence $\mathbf M\models\neg\varphi(a)$, a contradiction. This shows the forward direction;
the backward direction follows from Corollary~\ref{cor:persist, 1},~(3).
\end{proof}

\begin{cor}\label{cor:LT}
The following are equivalent:
\begin{enumerate}
\item Every substructure of every model of $\Sigma$ is a model of $\Sigma$; 
\item $\Sigma$ and $\Sigma_\forall$ are equivalent;
\item $\Sigma$ is equivalent to some set of universal sentences.
\end{enumerate}
\end{cor}
\begin{proof}
Suppose (1) holds. Clearly every model of $\Sigma$ is also a model of $\Sigma_\forall$;
conversely, if $\mathbf M\models\Sigma_\forall$, then by the preceding proposition,
$\mathbf M\subseteq\mathbf N$ for some model~$\mathbf N$ of $\Sigma$, and so $\mathbf M\models\Sigma$ by (1).
This shows (1)~$\Rightarrow$~(2);
the implication (2)~$\Rightarrow$~(3) is trivial, and
(3)~$\Rightarrow$~(1) is obvious from Corollary~\ref{cor:persist, 1},~(3).
\end{proof}

\noindent
We say that $\varphi$, $\psi$ are {\bf $\Sigma$-equivalent} if $\Sigma\models\varphi\leftrightarrow\psi$. (So  ``$\emptyset$-equivalent'' is the same as ``equivalent'' in the sense of Section~\ref{sec:formulas}.)
Note that $\Sigma$-equivalence is an equivalence relation on the collection of $\mathcal L$-formulas.
If $\varphi(x)$, $\psi(x)$ are $(\mathcal L,x)$-formulas, then~$\varphi$,~$\psi$ are $\Sigma$-equivalent  iff $\varphi^{\mathbf M}=\psi^{\mathbf M}$ for all $\mathbf M\models\Sigma$. \index{equivalence!of formulas}

\begin{cor}\label{cor:equivalent to universal}
The following are equivalent, for a formula $\varphi(x)$:
\begin{enumerate}
\item for all $\mathbf M\subseteq\mathbf N$ and $a\in M_x$, if $\mathbf M,\mathbf N\models\Sigma$ and
$\mathbf N\models\varphi(a)$, then $\mathbf M\models\varphi(a)$;
\item $\varphi(x)$ is $\Sigma$-equivalent to a universal formula $\psi(x)$.
\end{enumerate}
\end{cor}
\begin{proof}
Suppose (1) holds, and consider the set $\Sigma':=\Sigma\cup\{\varphi(c)\}$
of $\mathcal L_c$-sentences. By~\ref{prop:LT} and (1)
we have $(\Sigma')_\forall\cup\Sigma\models\varphi(c)$.
By Compactness, we can take a universal $\mathcal L$-formula $\psi(x)$ such that 
$\psi(c)\in (\Sigma')_\forall$ and
$\{\psi(c)\}\cup\Sigma\models\varphi(c)$. Then $\Sigma\models\varphi\leftrightarrow\psi$.
This shows (1)~$\Rightarrow$~(2). The reverse implication follows from~\ref{cor:persist, 1},~(3). 
\end{proof}

 


\subsection*{The L\"owenheim-Skolem Theorem}
As a consequence of Compactness, first-order logic cannot pin down the size of an infinite structure: \index{theorem!L\"owenheim-Skolem}

\begin{theorem}[L\"owenheim-Skolem ``upwards'']\label{thm:LS}
Suppose that some underlying set~$M_s$ of~$\mathbf M$ is infinite and let $\kappa$ be a cardinal with $\kappa\geq\max\big\{|\mathcal L|,|M|\big\}$. Then~$\mathbf M$ has an elementary extension of size $\kappa$.
\end{theorem}
\begin{proof}
Take $s$ such that $M_s$ is infinite, and let $C$ be a set of new constant symbols of sort $s$
with $|C|=\kappa$ and $\mathcal L':=\mathcal L\cup C$. Every finite subset of the set
$$\Sigma':=\operatorname{Th}(\mathbf M_M)\cup \{ \neg c = d : c,d\in C,\ c\neq d\}$$
of $\mathcal L'_M$-sentences has a model; in fact, as $M_s$ is infinite, $\mathbf M_M$ itself can be expanded to a model by
suitably interpreting the constants in $C$. By Compactness, we obtain a model $\mathbf N'$ of $\Sigma'$;
by the Diagram Lemma, there exists an elementary embedding of~$\mathbf M$ into the $\mathcal L$-reduct of $\mathbf N'$.
Thus we obtain an elementary extension~$\mathbf N$ of $\mathbf M$ of size~$\geq\kappa$.
By Proposition~\ref{prop:LS downwards} take an elementary substructure $\mathbf N_1$
of~$\mathbf N$ with $M\subseteq N_1$ and $|N_1|=\kappa$. Then $\mathbf M\preceq\mathbf N_1$ since both $\mathbf M$ and $\mathbf N_1$ are elementary
substructures of $\mathbf N$
and $M\subseteq N_1$.
\end{proof}

\noindent
The L\"owenheim-Skolem Theorems (\ref{prop:LS downwards} and \ref{thm:LS}) yield:

\begin{cor}
If $\Sigma$ has a model, then it has a model of size at most $|\mathcal L|$. If~$\Sigma$ has a model $\mathbf M$ such that $M_s$ is infinite for some $s$, then for each $\kappa\geq |\mathcal L|$, $\Sigma$ has a model of size $\kappa$.
\end{cor}
%\begin{proof}
%If $\Sigma$ has a model $\mathbf M$ such that $M_s$ is finite for each $s$, then $|M|\leq |\mathcal L|$. If~$\mathbf M$ is a model of $\Sigma$ such that $M_s$ is infinite for some $s$, then we first choose, using Theorem~\ref{thm:LS}, a model $\mathbf N$ of $\Sigma$ of size $\max\{|M|,|\mathcal L|\}$ and then, using Proposition~\ref{prop:LS downwards}, an elementary substructure of $\mathbf N$ of size $|\mathcal L|$. This yields the first statement, which implies the second one using Theorem~\ref{thm:LS}.
%\end{proof}

\noindent
In the following corollary we assume for simplicity that $\mathcal L$ is one-sorted. \index{test!Vaught}

\begin{cor}[Vaught's Test]\label{cor:Vaught's Test}
Suppose $\mathcal L$ has size at most $\kappa$, $\Sigma$ has a model and all models
of $\Sigma$ are infinite. Suppose also that any two models of $\Sigma$ of cardinality~$\kappa$ are
isomorphic. Then $\Sigma$ is complete.
\end{cor}
\begin{proof}
Let $\sigma$ be an $\mathcal L$-sentence and suppose that $\Sigma\not\models\sigma$ and $\Sigma\not\models\neg\sigma$. We
will derive a contradiction. First $\Sigma\not\models\sigma$ means that $\Sigma\cup \{\neg \sigma\}$ has a model.
Similarly $\Sigma\not\models\neg\sigma$ means that $\Sigma\cup \{  \sigma\}$ has a model.
These models must be
infinite since they are models of $\Sigma$, so by the L\"owenheim-Skolem
Theorem $\Sigma\cup \{\neg \sigma\}$  has a model~$\mathbf M$ of cardinality $\kappa$, and $\Sigma\cup \{  \sigma\}$  has a model
$\mathbf N$ of cardinality $\kappa$. By assumption $\mathbf M\cong\mathbf N$, contradicting that $\mathbf M \models \neg\sigma$ and
$\mathbf N \models \sigma$.
\end{proof}

\noindent
Here is an application of Vaught's Test.  

 
\begin{theorem}\label{thm:ACFp}
Let $p$ be a prime number or $p=0$.
The set $\operatorname{ACF}(p)$ of axioms for algebraically closed fields of characteristic $p$ is complete.
\end{theorem}
\begin{proof}
We use some basic facts about transcendence bases (see, e.g., \cite[Chapter~VIII]{Lang}).  Let $K$ be an infinite field of characteristic $p$ with subfield $\k$, and let~$B$ be a transcendence basis of $K$ over $\k$. Then 
$K$ is algebraic over $\k(B)$, hence $|K|=\max\{\aleph_0,|B|,|\k|\}$.
Suppose now that $K$, $L$ are algebraically closed fields of characteristic $p$ of the same
uncountable cardinality, and let $\k=\mathbb F_p$ if $p$ is a prime  and $\k=\Q$ if $p=0$. View $\k$
as a subfield of $K$ and of~$L$ as usual, and note that $|\k|\leq\aleph_0$. Let $B$ be a transcendence basis of $K$ 
over~$\k$ and~$C$ be a transcendence basis of $L$ over $\k$. Then $|B|=|K|=|L|=|C|$, hence there exists a bijection $B\to C$, and this bijection extends to a field isomorphism $K\to L$.
So by Vaught's Test for $\kappa=\aleph_1$,  $\operatorname{ACF}(p)$ is complete.
\end{proof}

\noindent
Theorem~\ref{thm:ACFp} and Corollary~\ref{cor:Completeness} imply that  $\operatorname{ACF}(p)$ is decidable. Some applications of Theorem~\ref{thm:ACFp} and another proof of this theorem are given in Section~\ref{sec:some theories}.


\subsection*{Notes and comments}
Lemma~\ref{lem:diagram} was first systematically used by A.~Robinson~\cite{Robinson52}.
Corollary~\ref{cor:Henkin} is due to Henkin~\cite{Henkin53}.
Corollary~\ref{cor:elem equivalence and elem embeddings} was strengthened by
Keisler~\cite{Keisler61} and Shelah~\cite{Shelah71a}: if $\mathbf M\equiv\mathbf N$ then there is an ultrafilter $\mathcal U$
on some set~$\Lambda$ with $\mathbf M^\Lambda/{\mathcal U}\cong \mathbf N^\Lambda/{\mathcal U}$.
Proposition~\ref{prop:Herbrand} is a weak version of a theorem of Herbrand~\cite{Herbrand}.
Corollary~\ref{cor:LT} is due to {\L}o\'{s}~\cite{Los55b} and Tarski~\cite{Tarski54}, and
Corollary~\ref{cor:Vaught's Test} to {\L}o\'{s}~\cite{Los54} and Vaught~\cite{Vaught54}. 

\section{Types and Saturated Structures}\label{sec:sat}

\noindent
Roughly speaking, a {\it type\/} is a set of formulas specifying a potential property of a tuple of elements in a structure. 
A {\it saturated structure} realizes many types. 


\subsection*{Types}
Let $\Phi=\Phi(x)$ be a set of $(\mathcal L,x)$-formulas. \index{element!realizing a set of formulas}
We say that $a\in M_x$ {\bf realizes~$\Phi$ in~$\mathbf M$} if $\mathbf M\models\varphi(a)$ for all
$\varphi\in\Phi$. Clearly if $\mathbf M\preceq\mathbf N$ and $a\in M_x$, then $a$ realizes~$\Phi$ in~$\mathbf M$ iff $a$ realizes $\Phi$ in~$\mathbf N$.
We say that {\bf $\Phi$ is realized in $\mathbf M$} if some $a\in M_x$ realizes~$\Phi$ in~$\mathbf M$.
Assume $x=(x_i)_{i\in I}$ and take a tuple $c=(c_i)_{i\in I}$ of distinct new constant symbols
with each $c_i$ of the same sort as $x_i$.
Let $\mathcal L_c$ be $\mathcal L$ augmented by these new constant symbols $c_i$.
Then $\Phi$ is realized in some structure iff the set 
$$\Phi(c)\ :=\ \big\{\varphi(c):\varphi\in\Phi\big\}$$ 
of $\mathcal L_c$-sentences
has a model. Hence by Compactness,
$\Phi$ is realized in some structure iff every finite subset of $\Phi$ is realized in some structure.
If this happens we call $\Phi$ an {\bf $x$-type}. 
An $x$-type $\Phi$ is said to be {\bf complete} if for each $\varphi(x)$, either $\varphi \in \Phi$
or $\neg\varphi  \in \Phi$, equivalently, $\Phi(c)$ is a complete $\mathcal{L}_c$-theory. 
For $a \in M_x$ we let 
$\operatorname{tp}^{\mathbf M}_x(a)$ be  the complete $x$-type in $\mathbf M$ realized by~$a$
 (and we leave out the superscript $\mathbf M$ or subscript $x$ if $\mathbf M$ or
$x$ are clear from context); that is, for each $\mathcal L$-formula $\varphi(x)$, we have 
$\varphi\in \operatorname{tp}^{\mathbf M}_x(a)$ iff $\mathbf M\models\varphi(a)$.
%Moreover, if $b\in N_x$ then $(\mathbf M,a)\equiv (\mathbf N,b)$ iff $\operatorname{tp}^{\mathbf M}_x(a)=\operatorname{tp}^{\mathbf N}_x(b)$.
Every $x$-type is contained in a complete one (namely one of the form $\operatorname{tp}^{\mathbf M}_x(a)$). 
If $\mathbf M\preceq\mathbf N$ and $a\in M_x$, then 
$\operatorname{tp}^{\mathbf M}_x(a)=\operatorname{tp}^{\mathbf N}_x(a)$. \index{type}\index{type!complete}\index{type!consistent with a set of sentences}
\nomenclature[Bn1]{$\operatorname{tp}^{\mathbf M}_x(b)$}{complete $x$-type in $\mathbf M$ realized by~$b\in M_x$}



\begin{definition}
We say that $\Phi$ is {\bf $\Sigma$-realizable} if $\Phi$ is realized in some model of~$\Sigma$;
that is, if $\Sigma\cup\Phi(c)$ has a model. The set of all complete $\Sigma$-realizable $x$-types
is denoted by $\operatorname{S}_x(\Sigma)$. 
\end{definition}

\noindent
Thus for
a {\em complete\/} $x$-type $\Phi$, we have: 
$\Phi$ is $\Sigma$-realizable iff $\Sigma\subseteq \Phi(c)$.
A complete $x$-type is usually denoted by a letter like $p$ or $q$. 


Let $\Sigma_c$ be  $\Sigma$ viewed as set of $\mathcal L_c$-sentences. Then
for $p\in \operatorname{S}_x(\Sigma)$ we have $p(c)\in\operatorname{S}(\Sigma_c)$, and 
the map $p\mapsto p(c)\colon \operatorname{S}_x(\Sigma)\to \operatorname{S}(\Sigma_c)$
is a bijection. The {\bf Stone topology} on~$\operatorname{S}_x(\Sigma)$ is the topology
making this bijection a homeomorphism. That is, its basic open sets are the sets 
$\<\varphi\>:=\big\{p\in \operatorname{S}_x(\Sigma):\varphi\in p\big\}$, with
$\varphi=\varphi(x)$. Two formulas $\varphi(x)$ and $\psi(x)$ are $\Sigma$-equivalent iff $\<\varphi\>=\<\psi\>$.
By Theorem~\ref{thm:compactness, 3}, the Stone topology makes 
$\operatorname{S}_x(\Sigma)$ a compact hausdorff space.

%\medskip
%\noindent
%Suppose $x=(x_i)_{i\in I}$ and $y=(y_i)_{i\in I}$, where 
%$x_i$ is of the same sort as $y_i$, for each $i\in I$.
%Then $\Phi$ is an $x$-type iff $\Phi(y):=\big\{\varphi(y/x):\varphi\in\Phi\big\}$ is a $y$-type,  and 
%$p\mapsto p(y)\colon\operatorname{S}_x(\Sigma)\to
%\operatorname{S}_y(\Sigma)$ is a homeomorphism. 
%An {\bf $n$-type} is an $x$-type where $x$ has size $n$. If $\mathcal L$ is one-sorted,
%then we also write $\operatorname{S}_n(\Sigma):=\operatorname{S}_x(\Sigma)$, 
%where $x$ is any multivariable of size $n$, for the space of $n$-types consistent with $\Sigma$.

\subsection*{Separating types}
In this subsection we fix a set $\Theta$ of $(\mathcal L,x)$-formulas such that $\top, \bot\in \Theta$, and 
for all $\phi, \psi\in \Theta$, also 
$\phi\wedge \psi\in \Theta$ and
$\phi\vee \psi\in \Theta$.
%which is closed under conjunction and disjunction, up to $\Sigma$-equivalence.
In the next sections we shall use the following fact:

\begin{lemma}\label{lem:separation}
Let a formula $\psi(x)$ be given. Then the following are equivalent:
\begin{enumerate}
\item $\psi$ is 
$\Sigma$-equivalent to some formula from $\Theta$;
\item for all $p,q\in \operatorname{S}_x(\Sigma)$ with
$\psi\in p$ and $\neg\psi\in q$ there exists $\varphi\in\Theta$ such that $\varphi\in p$ and $\neg\varphi\in q$.
\end{enumerate}
\end{lemma}
\begin{proof}
Suppose (1) holds. Then we have $\varphi\in\Theta$ such that $\<\varphi\>=\<\psi\>$. Let $p,q\in \operatorname{S}_x(\Sigma)$ with 
$\psi\in p$ and $\neg\psi\in q$. Then $\varphi\in p$ and~$\neg\varphi\in q$.
This shows (1)~$\Rightarrow$~(2).
Conversely, suppose (2) holds. Then 
$P:=\<\psi\>$ and its complement $P^{\c}=\<\neg\psi\>$ in~$\operatorname{S}_x(\Sigma)$ are both nonempty.
Let $p\in P$ be given. Then 
$P^{\c}\subseteq\bigcup_{\varphi\in\Theta\cap p} \<\neg\varphi\>$ by~(2).
By compactness of $\operatorname{S}_x(\Sigma)$ and $\Theta\cap p$ being closed under conjunction,
we get $\varphi\in\Theta\cap p$ such that $P^{\c}\subseteq\<\neg\varphi\>$ and
hence $p\in\<\varphi\>\subseteq P$.
Since $p$ was arbitrary, this yields $P=\bigcup_{\phi\in\Delta} \<\varphi\>$ for some $\Delta\subseteq\Theta$.
By compactness of $\operatorname{S}_x(\Sigma)$ again and $\Theta$ being closed under disjunction,
we obtain $\varphi\in\Theta$ with $P=\<\varphi\>$.
\end{proof}


\begin{cor}\label{cor:separation}
Every $(\mathcal L,x)$-formula is 
$\Sigma$-equivalent to some formula from $\Theta$ if and only if
for all $p\neq q$ in~$\operatorname{S}_x(\Sigma)$ we have
$p\cap\Theta\neq q\cap\Theta$.
\end{cor}

\subsection*{Types over a parameter set}
{\it In the rest of this section $A$ is a parameter set in~$\mathbf M$.}\/
An {\bf $x$-type over~$A$ in $\mathbf M$}
is an $x$-type in the language $\mathcal L_A$ that is $\operatorname{Th}(\mathbf M_A)$-realizable.
Equivalently, a set of $(\mathcal L_A,x)$-formulas is an $x$-type over $A$ in $\mathbf M$
if every finite subset of it is realized in $\mathbf M_A$.
For $b \in M_x$ we let $\operatorname{tp}^{\mathbf M}_x(b|A):=\operatorname{tp}^{\mathbf M_A}_x(b)$ 
be the (complete) $x$-type over $A$ in $\mathbf M$
realized by $b$ (and we leave out the superscript~$\mathbf M$ or subscript $x$ if $\mathbf M$ or
$x$ are clear from context).
If $\mathbf M\preceq\mathbf N$ and $b\in M_x$, then $\operatorname{tp}^{\mathbf M}_x(b|A)=\operatorname{tp}^{\mathbf N}_x(b|A)$.
Let $\operatorname{S}^{\mathbf M}_x(A)$ (or  $\operatorname{S}_x(A)$ if $\mathbf M$ is clear from context)
denote the space $\operatorname{S}_x(\operatorname{Th}(\mathbf M_A))$ of complete
$x$-types over $A$ in $\mathbf M$. A basis for the Stone topology on $\operatorname{S}_x(A)$ is given by
the sets~$\<\varphi\>=\{p\in \operatorname{S}_x(A):\varphi\in p\}$ as~$\varphi(x)$ ranges over all $\mathcal L_A$-formulas. \index{type}\index{type!complete}\index{topology!Stone}
\nomenclature[Bn2]{$\operatorname{tp}^{\mathbf M}_x(b\vert A)$}{complete $x$-type in $\mathbf M$ realized by~$b\in M_x$ over $A$}
\nomenclature[Bn3]{$\operatorname{S}^{\mathbf M}_x(A)$}{space of complete $x$-types in $\mathbf M$ over $A$}




\subsection*{Saturated structures}
In this subsection $\kappa$ is an infinite cardinal. 
We declare~$\mathbf M$ to be {\bf $\kappa$-saturated} if for all $A$ of size
$< \kappa$ and every variable $v$ of $\mathcal L$, each complete $v$-type over~$A$ in $\mathbf M$ is realized in
$\mathbf M$; equivalently, if $|A|<\kappa$ and $s\in S$, then each collection of $A$-definable subsets of $M_s$ with the finite intersection property has a nonempty intersection. The definition of ``$\kappa$-saturated'' ostensibly only concerns
families of subsets of $M_s$ for $s\in S$. It is a pleasant feature of model theory, however, that a one-variable property often yields a many-variable analogue, with some effort. This is also the case here: \index{structure!$\kappa$-saturated} \index{saturation}
% but this extends to 
%families of subsets of $M_x$ for $x$ a suitable multivariable:

\begin{lemma}\label{lem:sat}
Suppose $\mathbf M$ is $\kappa$-saturated, $A$ is of size $<\kappa$ and $x$ of
size $\leq \kappa$. Then each $x$-type over $A$ in $\mathbf M$ is realized in $\mathbf M$.
\end{lemma}
\begin{proof} Let $x=(x_i)_{i\in I}$, and let $i$, $j$ range over $I$. Let 
$p\in \operatorname{S}^{\mathbf M}_x(A)$;
it suffices to show that $p$ is realized in $\mathbf M$.
Take a well-ordering $\leq$ of $I$ such that $\operatorname{ot}(I,{\leq})=|I|$.
Then each proper downward closed subset of $I$ has cardinality~$<|I|$.
For each $j$ let $x_{\leq j}:=(x_i)_{i\leq j}$ and let $p_{\leq j}$
be the set of all formulas in $p$ with free variables in~$x_{\leq j}$;
then $p_{\leq j}$ is a complete $x_{\leq j}$-type over $A$ in $\mathbf M$.
Similarly, for each $j\in I$ we define $x_{<j}$ and the complete $x_{<j}$-type $p_{<j}$ over $A$ in $\mathbf M$;
then for each $\varphi\in p_{\leq j}$ we have $\exists x_j\varphi\in p_{<j}$.
By recursion on $i$ we construct a family $(b_i)$ in $M_x$ such that for each~$j$, $(b_i)_{i\leq j}$ realizes $p_{\leq j}$.
Suppose for some $j$ we have already constructed $b=(b_i)_{i<j}$ in $M_{x_{<j}}$ realizing $p_{<j}$.
Then $p_j:=\big\{\varphi(b/x_{<j}):\varphi\in p_{\leq j}\big\}$ is an $x_j$-type
over $A\cup\{b_i:i<j\}$ in $\mathbf M$. Since $A\cup\{b_i:i<j\}$ has cardinality $<\kappa$ and
$\mathbf M$ is $\kappa$-saturated, there exists $b_j\in M_{x_j}$ realizing $p_j$.
Then $(b_i)_{i\leq j}$ realizes~$p_{\leq j}$.
\end{proof}

\begin{example}
View ordered abelian groups as $\mathcal L_{\operatorname{OA}}$-structures.
Every $\aleph_0$-saturated ordered abelian group $(A;{+},{-},0,{\leq})$ with $A\neq \{0\}$ is 
non-archimedean: let $a\in A^>$ and consider the $v$-type $\{v>na:n=0,1,2,\dots\}$
over $\{a\}$.
In particular, the ordered abelian group $(\R;{+},{-},0,{\leq})$ is not $\aleph_0$-saturated.
\end{example}

\noindent
In $\kappa$-saturated structures one can do things that otherwise would require passing to an elementary extension.
As an example, here is a variant of Corollary~\ref{cor:elem equivalence and elem embeddings}:

\begin{cor}\label{cor:sat elem embedd}
Suppose $\mathbf M\equiv\mathbf N$ and $\mathbf N$ is $\kappa$-saturated for some $\kappa\ge\abs{M}$. Then there exists an elementary embedding
$\mathbf M\to\mathbf N$.
\end{cor}
\begin{proof} For simplicity, assume $\mathcal{L}$ is one-sorted. Take a multivariable $x=(x_a)_{a\in M}$, and let $\vec a:=(a)_{a\in M}$. Since $\mathbf M\equiv\mathbf N$, 
$\Phi:=\big\{\varphi(x):\mathbf M\models\varphi(\vec a)\big\}$
is an $x$-type over~$\emptyset$ in $\mathbf N$.
By Lemma~\ref{lem:sat}, $\Phi$ is realized in $\mathbf N$.
If $(a')_{a\in M}$ realizes~$\Phi$ in $\mathbf N$, then $a\mapsto a'$ ($a\in M$) is an elementary
embedding $\mathbf M\to\mathbf N$.
\end{proof}

\noindent
Note that if $M_s$ is finite for all $s$, then
$\mathbf M$ is $\kappa$-saturated  for every $\kappa$.
If $M_s$ is infinite and $\mathbf M$ is $\kappa$-saturated, then $|M_s|\ge \kappa$:
consider the type $\{v\neq a:\ a\in M_s\}$.
If $\mathbf M$ is $\kappa$-saturated and $\abs{A}<\kappa$, then $\mathbf M_A$ is also
$\kappa$-saturated.
Also note that if $\kappa'$ is an infinite cardinal $\leq\kappa$ and $\mathbf M$ is 
$\kappa$-saturated, then $\mathbf M$ is also $\kappa'$-saturated.
Thus by the next proposition, every structure has a $\kappa$-saturated elementary extension:

\begin{prop}\label{prop:saturated elemext}
Suppose $\kappa\geq|\mathcal L|$ and $2^\kappa\geq |M|$. Then $\mathbf M$ has a $\kappa^+$-saturated elementary
extension $\mathbf N$  with $|N| \leq 2^\kappa$.
\end{prop}

\noindent
We first establish the following lemma, with the same assumptions on $\kappa$
as in Proposition~\ref{prop:saturated elemext}.

\begin{lemma}
There exists $\mathbf M'\succeq\mathbf M$ with
$|M'| \leq 2^\kappa$ such that for all $A\subseteq M$
with $|A|\leq\kappa$ and any variable $v$ of $\mathcal L$,  each type in~$\operatorname{S}_v^{\mathbf M}(A)$ is realized in $\mathbf M'$.  
\end{lemma}
\begin{proof}
Let $\mathcal P$ be the union of all $\operatorname{S}_v^{\mathbf M}(A)$ with
$\abs{A}\leq\kappa$ and $v$ a quantifiable variable of $\mathcal L$;
then $\abs{\mathcal P}\leq 2^\kappa$.
For each $v$-type $p\in\mathcal P$ let $c_p$ be a new constant symbol of the same sort as $v$, and let
$\mathcal L'$ be $\mathcal L$ augmented by the $c_p$.
By Compactness and Proposition~\ref{prop:LS downwards} applied to the
set 
$\operatorname{Th}(\mathbf M_M)\cup\bigcup\big\{p(c_p):p\in \mathcal P\big\}$
of $\mathcal L'_{M}$-sentences we obtain an elementary extension $\mathbf M'$ of $\mathbf M$ as desired.
\end{proof}

\noindent
In what follows we use the fact that the least cardinal $\kappa^{+}$ that is greater than $\kappa$ is a regular ordinal as defined in Section~\ref{sec:ordered sets}.  


\begin{proof}[Proof of Proposition~\ref{prop:saturated elemext}] 
%We can assume that $\abs{M}=2^\kappa$.
Let $\alpha$, $\beta$ range over ordinals $<\kappa^+$. By recursion on $\alpha$ we construct a sequence $(\mathbf M_\alpha)$ of
structures of size $\leq 2^\kappa$ such that:
\begin{enumerate}
\item $\mathbf M_0=\mathbf M$ and $\mathbf M_\alpha\preceq\mathbf M_\beta$ if $\alpha<\beta$,
\item if $\alpha$ is a limit ordinal, then $\mathbf M_\alpha=\bigcup_{\beta<\alpha}\mathbf M_\beta$; and
\item if $\alpha=\beta+1$ is a successor ordinal, then
$\mathbf M_{\beta}$ is obtained from $\mathbf M_\alpha$ as $\mathbf M'$ is from $\mathbf M$
in the previous lemma. 
\end{enumerate}
Then $\mathbf N:=\bigcup_{\alpha} \mathbf M_\alpha$  is an elementary extension
of $\mathbf M$ with $|N|\leq 2^\kappa$. Since the ordinal $\kappa^+$ is regular, if $B\subseteq N$ with $\abs{B} \leq \kappa$,
then there is some $\beta$ such that $B\subseteq M_\beta$, 
so every  $p\in\operatorname{S}_v^{\mathbf N}(B)=\operatorname{S}_v^{\mathbf M_\beta}(B)$ is realized in
$\mathbf M_{\beta+1}$ and thus in~$\mathbf N$.
\end{proof}

\subsection*{Notes and comments}
The notion of $\kappa$-saturated structure goes back to the $\eta_\alpha$-sets of
Hausdorff~\cite[p.~181]{Hausdorff14}, but only appeared in model theory in the late 1950s
in the work of Morley and Vaught~\cite{Morley,MorleyVaught,Vaught61}, who also introduced types.
See~\cite{Felgner02} for the history. A motivation for
Hausdorff was du~Bois-Reymond's ``infinitary pantachy''~\cite{dBR71,dBR72} (the partially ordered set of germs at $+\infty$ of continuous real-valued
functions): see~\cite{Steprans}. 



\section{Model Completeness}

\noindent 
If the primitives of an
$\mathcal{L}$-structure $\mathbf M$ are computationally or topologically well-behaved, then the 
sets defined in~$\mathbf M$ by quantifier-free formulas are
often fairly tame as well.  For example, the
subsets of $\R$ definable by quantifier-free formulas in the
ordered field of real numbers (viewed as an $\mathcal L_{\operatorname{OR}}$-structure) are finite unions of open intervals 
and singletons. In the ordered ring of integers,
the subsets of $\Z$ definable by quantifier-free formulas are just the traces of the preceding sets in $\Z$. But taking arbitrary $\mathcal L_{\operatorname{OR}}$-formulas, one can define much more complicated sets in the ordered ring of integers: for example, the formula $\pi(x)$ given by
$$1+1\leq x \ \& \ \forall u\forall v\big((1\le u\ \&\ 1\le v\ \&\ u\cdot v = x)\ \rightarrow\ u= 1 \ \vee \ v = 1 )$$
defines the set of prime numbers. In general, the more quantifiers that occur in a formula $\varphi(x)$, the more complicated the set $\varphi^{\mathbf M}$ defined by $\varphi(x)$ in $\mathbf M$ can be. When this typical behaviour does {\em not\/} occur, it is worth noting!

This is why in this section we consider
{\em model completeness}. In the next section we study a sharper version of this, called
%A structure~{\bf $\mathbf M$
{\em quantifier elimination}. 
%if for each formula~$\varphi(x)$ there exists a quantifier-free formula~$\psi(x)$ such that $\varphi^{\mathbf M}=\psi^{\mathbf M}$. 
%The next section treats quantifier elimination; the present section is devoted to {\it model completeness,}\/ which is weaker but sometimes easier to establish: 
A structure $\mathbf M$ is said to be {\bf model complete} if
for each formula~$\varphi(x)$ there exists an existential formula~$\psi(x)$ such that $\varphi^{\mathbf M}=\psi^{\mathbf M}$. For one-sorted model complete $\mathbf M$, every definable subset of $M^m$ is, for some $n$, the image of a quantifier-free definable
set in $M^{m+n}$ under the natural projection $M^{m+n}\to M^m$. These projections often preserve many desirable 
topological properties, for example, having only finitely many connected components (in a suitable topological environment). 


\medskip
\noindent
Model completeness also makes sense for a set of sentences:


\begin{definition}\index{theory!model complete} \index{model completeness} $\Sigma$ is said to be {\bf model complete} if every formula  is $\Sigma$-equivalent to an existential formula. (Note that then every formula $\varphi(x)$ is actually $\Sigma$-equivalent to an $\exists$-formula $\varphi'(x)$ with no more free variables than those of $\varphi$.) 
\end{definition}

\noindent
Thus $\mathbf M$ is model complete iff  $\operatorname{Th}(\mathbf M)$ is model complete. The following lemma slightly reduces the job of proving model completeness:\index{structure!model complete}


\begin{lemma} Suppose every universal formula is $\Sigma$-equivalent to an existential formula. Then $\Sigma$ is model complete.  \end{lemma}
\begin{proof}
We show by induction that 
every formula $\varphi$ is $\Sigma$-equivalent to
an $\exists$-formula. This is clear if $\varphi$ is quantifier-free,
and the conclusion is preserved under $\wedge$, $\vee$, and $\exists$.
Suppose $\varphi=\neg\psi$. Assuming inductively that 
$\psi$ is $\Sigma$-equivalent to an $\exists$-formula,
 $\varphi$ is $\Sigma$-equivalent to a $\forall$-formula, and thus by hypothesis, $\varphi$ is  $\Sigma$-equivalent to an $\exists$-formula.
The case where $\varphi=\forall y\psi$ with a single quantifiable variable $y$ follows, since then $\varphi$
is equivalent to $\neg\exists y\neg\psi$.
\end{proof}

\noindent
Here is Robinson's model completeness test:\index{model completeness!test}\index{test!for model completeness}

\begin{prop} \label{thm:Robinson test} The following are equivalent:
\begin{enumerate}
\item $\Sigma$ is model complete;
\item for all models $\mathbf M$, $\mathbf N$ of $\Sigma$, if $\mathbf M\subseteq\mathbf N$, then 
$\mathbf M\preceq\mathbf N$;
\item for all models $\mathbf M$, $\mathbf N$ of $\Sigma$, if $\mathbf M\subseteq\mathbf N$, then 
$\mathbf M\preceq_\exists\mathbf N$.
\end{enumerate}
\end{prop}
\begin{proof}
Clearly (1)~$\Rightarrow$~(2)~$\Rightarrow$~(3).
Assume (3), and let~$\varphi(x)$ be universal. 
Then for $\mathbf M,\mathbf N\models\Sigma$ with $\mathbf M\subseteq\mathbf N$ and $a\in M_x$ we have $\mathbf M\models\varphi(a)\Rightarrow \mathbf N\models\varphi(a)$.
Thus by Corollary~\ref{cor:equivalent to universal}, $\varphi$ is $\Sigma$-equivalent to
an $\exists$-formula. Thus by the previous lemma,
$\Sigma$ is model complete. 
\end{proof}

\noindent
Condition (2) in Proposition~\ref{thm:Robinson test} means that
$\Sigma\cup\operatorname{Diag}_M(\mathbf M)$ is complete, for all $\mathbf M\models\Sigma$;
this explains the terminology ``model complete''. %(Compare with Corollary~\ref{cor:substructure completeness}.)
Model completeness often entails completeness:
A {\bf prime model} of $\Sigma$ is a model of $\Sigma$ that embeds elementarily into every model of $\Sigma$. Note that if $\Sigma$ has a prime model, then $\Sigma$ is complete.
If $\Sigma$ is model complete and $\mathbf M$ is a model of $\Sigma$ that embeds into every model
of $\Sigma$, then $\mathbf M$ is a prime model of $\Sigma$.\index{model!prime}\index{prime model}\index{theory!prime model}


\medskip
\noindent
Here is a variant of the above test for model completeness:  

\begin{cor}\label{cor:modelcomplete test}
The following are equivalent:
\begin{enumerate}
\item $\Sigma$ is model complete;
%\item for all models $\mathbf M$, $\mathbf N$ of $\Sigma$ with $\mathbf M\subseteq\mathbf N$ there is an elementary extension $\mathbf M^*$ of $\mathbf M$ and an embedding $\mathbf N\to\mathbf M^*$ extending the natural inclusion $\mathbf M\to\mathbf M^*$;
\item for all models $\mathbf M$, $\mathbf N$ of $\Sigma$ with $\mathbf M\subseteq\mathbf N$ and every elementary extension $\mathbf M^*$ of $\mathbf M$ that is $\kappa$-saturated for some $\kappa>\abs{N}$, there is an embedding $\mathbf N\to\mathbf M^*$
that extends the natural inclusion $\mathbf M\to\mathbf M^*$.
\end{enumerate}
\end{cor}
\begin{proof}
Suppose $\Sigma$ is model complete, and $\mathbf M$, $\mathbf N$, $\mathbf M^*$ are as in the hypothesis of~(2).
Then $\Sigma\cup\operatorname{Diag}_M(\mathbf M)$ is complete, with models
$\mathbf M^*_M$, $\mathbf N_M$. Since $\mathbf M^*_M$ is $|N|$-saturated,
Corollary~\ref{cor:sat elem embedd} yields an embedding $\mathbf N_M\to\mathbf M^*_M$.
This shows (1)~$\Rightarrow$~(2).
The implication (2)~$\Rightarrow$~(1) follows from Corollary~\ref{cor:ex closed and embeddings}, Proposition~\ref{prop:saturated elemext} and the equivalence of (1) and (3) in Theorem~\ref{thm:Robinson test}.
\end{proof}

\begin{exampleNumbered}\label{ex:TfDiv, 1}
Let $\mathcal L:=\mathcal L_{\operatorname{A}}$ be the language of  additive groups and
$$\Sigma\ :=\ \operatorname{Tf}\cup\operatorname{Div}\cup\operatorname{Ab}\cup\{\exists x\,(x\neq 0)\}.$$ 
Then the models of $\Sigma$ are the  nontrivial divisible torsion-free abelian groups: see Example~\ref{ex:theories},~(2),~(3). 
A model of $\Sigma$ may be viewed as a $\Q$-linear space in the natural way,
and if the model is $\kappa$-saturated, then it has dimension
$\geq\kappa$. Together with Corollary~\ref{cor:modelcomplete test} this yields model completeness of $\Sigma$.
\end{exampleNumbered}

\noindent
%Every structure has an expansion which has the same definable sets and is model complete; see Example~\ref{ex:morleyization} below. 
Before showing that a certain theory is model complete, one better checks that it has an axiomatization by
$\forall\exists$-sentences:
%The following fact is a useful necessary a useful yardstick for finding a {\it natural}\/ model complete expansion of a given structure:

\begin{prop}\label{prop:forallexists}
Suppose $\Sigma$ is model complete. Then $\Sigma$ is equivalent to a set of $\forall\exists$-sentences.
\end{prop}
\begin{proof}
Let $\Sigma_\forall$ be as in Proposition~\ref{prop:LT} (so the models of $\Sigma_\forall$ are the substructures of models of $\Sigma$). 
Every sentence of the form $\forall x(\varphi\to\psi)$, where $\varphi(x)$ is universal and $\psi(x)$ is existential, is equivalent to a $\forall\exists$-sentence.
Let $\Sigma_{\forall\exists}$ be the set of all $\forall\exists$-sentences  
equivalent to  a sentence $\forall x(\varphi\to\psi)$, where $\varphi(x)$ is universal, $\psi(x)$ is existential, and $\varphi$, $\psi$  are $\Sigma$-equivalent. We claim that $\Sigma$ and $\Sigma':=\Sigma_\forall\cup \Sigma_{\forall\exists}$ are equivalent.
Note first that $\Sigma'$ is also model complete: Let  $\varphi(x)$ be universal, and
take  an $\exists$-formula $\psi(x)$ which is $\Sigma$-equivalent to $\varphi$; then 
$\varphi$ is also $\Sigma'$-equivalent to $\psi$, since  up to equivalence
$\forall x(\psi\to\varphi)$ lies in $\Sigma_\forall$ and
$\forall x(\varphi\to\psi)$  in~$\Sigma_{\forall\exists}$. Let $\mathbf M\models\Sigma'$; we need to show $\mathbf M\models \Sigma$. Now $\mathbf M\models \Sigma_\forall$ yields  some $\mathbf N\models \Sigma$ with $\mathbf M\subseteq\mathbf N$. 
Then $\mathbf N\models\Sigma'$ and so $\mathbf M\preceq\mathbf N$ by model completeness of~$\Sigma'$, thus $\mathbf M\models\Sigma$.
\end{proof}

\noindent
Call $\Sigma$ {\bf inductive} if the
direct union of any directed family
of models of $\Sigma$ is a model of $\Sigma$. If $\Sigma$ is a set of $\forall\exists$-sentences, then $\Sigma$ is inductive. Hence by \ref{prop:forallexists}:\index{inductive}\index{theory!inductive}
 
\begin{cor}\label{cor:model complete=>inductive}
If $\Sigma$ is model complete, then $\Sigma$ is inductive.
\end{cor}

\subsection*{Existentially closed models} 
An {\bf existentially closed model of $\Sigma$} is a
mo\-del~$\mathbf M$ of $\Sigma$ that is existentially closed
in every extension $\mathbf N\models\Sigma$ of $\mathbf M$.
Thus by Robinson's test, $\Sigma$ is model complete iff every model of $\Sigma$ is an existentially closed model of $\Sigma$.
Inductive theories have existentially closed models: \index{model!existentially closed} \index{closed!existentially}

\begin{lemma}\label{lem:ec models}
Suppose $\Sigma$ is inductive and $\mathbf M\models\Sigma$. Then $\mathbf M$ extends to an existentially closed model of $\Sigma$.
\end{lemma}
\begin{proof}
We first show that $\mathbf M$ has an extension $\mathbf M^*\models\Sigma$ which 
satisfies each existential $\mathcal L_M$-sentence holding in some model of $\Sigma$ extending~$\mathbf M^*$.

Let $(\sigma_\lambda)_{\lambda<\kappa}$ be an enumeration of all $\mathcal L_M$-sentences,
where $\kappa$ is the cardinality of the set of $\mathcal L_M$-sentences.
By recursion on $\mu<\kappa$ we construct a sequence $(\mathbf M_\mu)_{\mu\leq\kappa}$ of
extensions of $\mathbf M$ to models of $\Sigma$ 
such that $\mathbf M_\lambda\subseteq\mathbf M_{\lambda'}$ for all $\lambda\leq\lambda'\leq\kappa$
as follows:
Set $\mathbf M_0:=\mathbf M$. Suppose $0<\mu\leq\kappa$ and
$(\mathbf M_\lambda)_{\lambda<\mu}$ is a sequence
of extensions of  $\mathbf M$ to models of $\Sigma$ 
such that $\mathbf M_\lambda\subseteq\mathbf M_{\lambda'}$ for all $\lambda\leq\lambda'<\mu$. If $\mu$ is a limit ordinal, then set $\mathbf M_\mu:=\bigcup_{\lambda<\mu}\mathbf M_\lambda$; since $\Sigma$ is inductive, we have $\mathbf M_\mu\models\Sigma$.
Suppose $\mu=\mu'+1$; if some
extension of $\mathbf M_{\mu'}$ is a model of $\Sigma\cup\{\sigma_{\mu'}\}$, then we let $\mathbf M_{\mu}$ be such an extension, and otherwise $\mathbf M_\mu:=\mathbf M_{\mu'}$.
Finally, put $\mathbf M^*:=\mathbf M_\kappa$. It is routine to
check that $\mathbf M^*$ has the desired property.

Now inductively define $\mathbf M^0:=\mathbf M$ and $\mathbf M^{n+1}:=(\mathbf M^n)^*$. Then
$\bigcup_n \mathbf M^n$ is an existentially closed model of $\Sigma$ which extends $\mathbf M$.
\end{proof}

\subsection*{Model companions and model completions}
{\it In this subsection we assume that $T$ is an inductive 
$\mathcal{L}$-theory $T$.}\/
Even though $T$ may not be model complete, we may hope for the existence of a theory whose
models are exactly the existentially closed models of $T$. This suggests the following notion:

\begin{definition}\index{model companion}\index{theory!model companion} A {\bf model companion} of $T$ is a
model complete $\mathcal{L}$-theory $T^*\supseteq T$ such that every model of $T$ embeds into
a model of $T^*$.
\end{definition}

\begin{lemma} Let $T^*$ be a $\mathcal{L}$-theory. Then
$T^*$ is a model companion of $T$ iff the models of $T^*$ are exactly the  existentially closed models of $T$. 
\end{lemma}
\begin{proof}
Suppose $T^*$ is a model companion of $T$. Then every model $\mathbf M^*$ of $T^*$ 
is an existentially closed model of $T$: if $\mathbf N\models T$ extends $\mathbf M^*$, extend
$\mathbf N$ to a model~$\mathbf N^*$ of $T^*$; then $\mathbf M^*\preceq\mathbf N^*$ by model completeness of $T^*$ and thus $\mathbf M^*\preceq_\exists\mathbf N$ by Corollary~\ref{cor:persist, 1},~(2). Conversely, suppose $\mathbf M$ is an
existentially closed model of~$T$. Take $\mathbf M^*\models T^*$ with $\mathbf M\subseteq\mathbf M^*$;
then $\mathbf M\preceq_\exists \mathbf M^*$ and thus $\mathbf M\models T^*$ by
Proposition~\ref{prop:forallexists}.
This shows the ``only if'' direction of the lemma; the ``if'' direction follows from Theorem~\ref{thm:Robinson test} and Lemma~\ref{lem:ec models}.\end{proof}

\begin{cor}
There is at most one model companion of $T$.
\end{cor}

\noindent
Thus if a model companion of $T$ exists, we may speak of {\it the}\/ model companion of~$T$.
Clearly $T$ is model complete iff it is its own model companion.\index{model companion}\index{theory!model companion}\index{companion!model}


\begin{exampleNumbered}\label{ex:TfDiv, 2}
The $\mathcal L_{\operatorname{A}}$-theory $T$ of torsion-free abelian groups is inductive. Let~$T^*$ be the 
$\mathcal L_{\operatorname{A}}$-theory of nontrivial divisible torsion-free abelian groups. 
Then $T^*$ is model complete (Example~\ref{ex:TfDiv, 1}), and every $A\models T$
extends to some $A^*\models T^*$: if $A=\{0\}$, take $A^*:=\Q$, and if $A\neq\{0\}$, let
$A^*:=A\otimes_\Z\Q$ be the divisible hull of~$A$. Hence $T^*$ is the model companion of $T$.
\end{exampleNumbered}

\begin{definition}
A {\bf model completion} of $T$ is a model companion $T^*$ of $T$ such that in addition
$T^*\cup\operatorname{Diag}_A(\mathbf A)$ is complete, for all  
$\mathbf A\models T$.
%If it exists, we may speak of {\it the}\/ model completion of $T$. 
\index{model completion} \index{theory!model completion}\index{completion!model}
\end{definition}


\noindent
We say that {\bf $\Sigma$ has AP\/} (short for: {\bf $\Sigma$ has
the amalgamation property}) if for all $\mathbf A,\mathbf M_1,\mathbf M_2\models\Sigma$ and embeddings
$f_i\colon \mathbf A\to \mathbf M_i$ ($i=1,2$) there exist $\mathbf N\models\Sigma$ and embeddings
$g_i\colon \mathbf M_i\to\mathbf N$ ($i=1,2$) making the diagram
$$\xymatrix{ 
& \mathbf N&  \\
\mathbf M_1 \ar@{-->}[ru]^{g_1} & & \mathbf M_2 \ar@{-->}[lu]_{g_2}   \\
& \mathbf A \ar@{->}[lu]^{f_1} \ar@{->}[ru]_{f_2} & }$$
commute. Using the definitions and Corollary~\ref{cor:elem equivalence and elem embeddings}
one easily shows: \index{amalgamation property} \index{theory!amalgamation property}
 
\begin{lemma}\label{lem:amalg prop}
Let $T^*$ be an $\mathcal{L}$-theory. Then
$T^*$ is a model completion of $T$ iff~$T^*$ is a model companion of~$T$ and $T$ has \textup{AP}.
\end{lemma}

\begin{exampleNumbered}
Let $T$, $T^*$ be as in Example~\ref{ex:TfDiv, 2}.
Then $T$ has AP. To see why, let embeddings $f_i\colon A\to M_i$ ($i=1,2$) of abelian groups be given. Set
$$F\ :=\ \big\{(b,c)\in M_1\times M_2:\ nb=f_1(a),\ nc=-f_2(a) \text{ for some $n\ge 1$ and $a\in A$}\big\},$$ 
a subgroup of the direct sum $M_1\oplus M_2$ of
$M_1$ and $M_2$. Put $N:=(M_1\oplus M_2)/F$; it is easy to check that $N$ is torsion-free and that the natural morphisms $g_i\colon M_i\to N$ ($i=1,2$) are embeddings.
Hence $T^*$ is the model completion of $T$.
\end{exampleNumbered}



\subsection*{Notes and comments}
The notion of model completeness and Proposition~\ref{thm:Robinson test} are due to A.~Robinson
\cite{Robinson53,Robinson55c,Robinson56,Robinson65}. 
See~\cite{Macintyre77} for a survey of
classical model completeness results.
In connection with~\ref{prop:forallexists} and~\ref{cor:model complete=>inductive} we should mention that  
$\Sigma$ is inductive iff $\Sigma$ is equivalent to 
a set of $\forall\exists$-sentences;
this is due to Chang~\cite{Chang59} and {\L}o\'{s}-Suszko~\cite{Los-Suszko}; see \cite[Theorem~6.5.9]{Hodges} for a proof. Existentially closed models were introduced by Rabin~\cite{Rabin62}, 
model companions by Barwise and Robinson~\cite{BarwiseRobinson}, and the connection between the two
notions is from~\cite{EklofSabbagh}.
By Cherlin~\cite{Cherlin73}, the $\mathcal L_{\operatorname{R}}$-theory of
commutative rings has no model companion.



\section{Quantifier Elimination}\label{sec:qe}

\noindent  
To avoid certain trivial exceptions {\it we assume in this section that our language~$\mathcal L$ has for each~$s$ a constant symbol of sort $s$.}\/ \index{structure!quantifier elimination} \index{quantifier elimination}
\index{theory!quantifier elimination}
Quantifier elimination is often the first key step to understanding the category of definable sets of a structure.

\begin{definition}
We say that {\bf $\Sigma$ admits quantifier elimination} (QE) if  each formula $\varphi(x)$ is $\Sigma$-equivalent to a quantifier-free formula $\varphi'(x)$.
We also express this by saying that ``$\Sigma$ has QE'' or ``$\Sigma$ eliminates quantifiers''.
We say that $\mathbf M$ admits~QE if $\operatorname{Th}(\mathbf M)$ admits QE.
\end{definition}

\noindent
Note that if $\Sigma$ has QE, then $\Sigma$ is model complete.  
In this section we give criteria for~$\Sigma$ to have QE.
%if the criterion in question is satisfied, 
%then all models of $\Sigma$ are model complete. 
For a given structure $\mathbf M$ of interest, one tries to find a~$\Sigma$ that has~$\mathbf M$ as a model and passes such a test.
By Corollary~\ref{cor:separation}, $\Sigma$ admits QE iff for every multivariable $x$, each type
in $\operatorname{S}_x(\Sigma)$ is determined by its subset of quantifier-free formulas; this fact underlies the tests.
To verify that $\Sigma$ admits QE, it suffices to show that  formulas of a   special
form are $\Sigma$-equivalent to quantifier-free formulas:

\begin{lemma}\label{lem:QE simplified}
Suppose each formula $\exists y\, \theta(x,y)$ with
quantifier-free $\theta$, finite $x$, and a single variable 
$y$, is $\Sigma$-equivalent to a quantifier-free formula.
Then $\Sigma$ has \textup{QE}.
\end{lemma}
\begin{proof} We proceed by induction on the
number of logical symbols in a formula.
To show that any formula $\varphi(x)$ is $\Sigma$-equivalent to a quantifier-free formula $\varphi'(x)$, we first note that
this is obvious for quantifier-free $\varphi$, and that this property is
preserved when taking disjunctions, conjunctions and negations.
Suppose $\varphi=\exists y\psi$. We can assume inductively that
$\psi(x,y)$ is $\Sigma$-equivalent to a quantifier-free formula $\psi'(x,y)$.
The hypothesis of the lemma then yields a quantifier-free formula $\varphi'(x)$ that is
$\Sigma$-equivalent to $\exists y\psi'(x,y)$, and hence to $\varphi(x)$.
The case $\varphi=\forall y\psi$ reduces to the previous cases, since 
$\varphi$ is equivalent to $\neg\exists y\neg\psi$.
\end{proof}

\noindent
Here is a cheap way of obtaining QE that is nevertheless useful later:  


\begin{exampleNumbered}[Morleyization]\label{ex:morleyization}
Let $\varphi(x)$ be a formula where $x=(x_1,\dots, x_m)$ is a quantifiable multivariable of sort $s_1\dots s_m$.
Let $R_{\varphi(x)}$ be a new relation symbol of sort $s_1\dots s_m$, and declare the
{\it defining axiom for $R_{\varphi(x)}$\/} to be the sentence    
$$\forall x\big(R_{\varphi(x)}x_1\cdots x_m\leftrightarrow \varphi(x)\big).$$
Let $\mathcal L_{\operatorname{Mo}}$ be $\mathcal{L}$ augmented by these new relation symbols, one for each $\varphi(x)$ as above, and let 
$\operatorname{Mo}$ be the set of defining axioms for these new relation symbols, considered as a set of $\mathcal L_{\operatorname{Mo}}$-sentences. Then every $\mathcal L_{\operatorname{Mo}}$-formula is $\operatorname{Mo}$-equivalent to an $\mathcal{L}$-formula, and so $\operatorname{Mo}$ has QE.
Each $\mathcal{L}$-structure $\mathbf M$ has a unique expansion to a model of $\operatorname{Mo}$, and this expansion has the same $0$-definable sets as $\mathbf M$.
\end{exampleNumbered}



\subsection*{A general elimination theorem}
Suppose $\mathcal L$ is a sublanguage of
the language~${\mathcal L}^*$. Let $S^*\supseteq S$ be the set of sorts for $\mathcal{L}^*$; assume that $\mathcal{L}^*$ has for each $s^*\in S^*$ a constant symbol of sort $s^*$. 
Let ${\mathbf M}^*$ and ${\mathbf N}^*$
range over ${\mathcal L}^*$-structures, and let~${\mathbf M}$ and~${\mathbf N}$
be their $\mathcal L$-reducts. Let $\Sigma^*$ be a set of ${\mathcal L}^*$-sentences.   
Here is a criterion for an $\mathcal L^*$-formula to be $\Sigma^*$-equivalent to a quantifier-free $\mathcal L$-formula:

\begin{lemma}\label{lem:key lemma} Let $x$ be a multivariable of $\mathcal{L}$. Let $\varphi^*(x)$ be an 
${\mathcal L}^*$-formula. Then $\varphi^*(x)$ is $\Sigma^*$-equivalent to a
quantifier-free ${\mathcal L}$-formula~$\varphi(x)$ iff for all ${\mathbf M}^*,{\mathbf N}^*\models \Sigma^*$ and every
common $\mathcal L$-sub\-struc\-ture ${\mathbf A}=(A;\dots)$ of~${\mathbf M}$ and~${\mathbf N}$, and all~$a\in A_x$:
\begin{equation}\label{eq:key lemma}
{\mathbf M}^*\models \varphi^*(a) \quad\Longleftrightarrow\quad {\mathbf N}^*\models \varphi^*(a).
\end{equation}
\end{lemma}
\begin{proof}
Forward direction: use Corollary~\ref{cor:persist, 1},~(1), and $\mathbf M^*\models\sigma$ iff $\mathbf M\models\sigma$, when $\sigma$ is an $\mathcal L_M$-sentence.
%Suppose $\varphi^*(x)$ is $\Sigma^*$-equivalent to a  quantifier-free ${\mathcal L}$-formula $\varphi(x)$, and let  ${\mathbf M}^*$,~${\mathbf N}^*$, $\mathbf A$ be as in the statement of the lemma, and $a\in A_x$. Then
%$${\mathbf M}^*\models \varphi^*(\underline{a})\quad\Longleftrightarrow\quad {\mathbf M}^*\models \varphi(\underline{a})\quad\Longleftrightarrow\quad \mathbf M\models\varphi(\underline{a})\quad\Longleftrightarrow\quad \mathbf A\models\varphi(\underline{a}), $$
%where the first equivalence holds since $\varphi$ and $\varphi^*$ are $\Sigma^*$-equivalent,  the second equivalence holds since $\varphi(\underline{a})$ is an $\mathcal L_M$-sentence and $\mathbf M$ is the $\mathcal L$-reduct of $\mathbf M^*$, and the third equivalence holds since   $\varphi$ is    quantifier-free  and $\mathbf A\subseteq\mathbf M$. Symmetrically we also have ${\mathbf N}^*\models \varphi^*(\underline{a}) \Longleftrightarrow \mathbf A\models\varphi(\underline{a})$, hence \eqref{eq:key lemma} holds. 
Conversely, suppose \eqref{eq:key lemma} holds for all $\mathbf M^*$, $\mathbf N^*$, $\mathbf A$ and~$a$ as specified in the lemma. 
Let $p,q\in\operatorname{S}_x(\Sigma^*)$ contain the same quantifier-free $\mathcal L$-formulas.
By Lemma~\ref{lem:separation} it is enough to show that then $\varphi^*\in p$ iff $\varphi^*\in q$.
Take $\mathbf M^*,\mathbf N^*\models\Sigma^*$ and $a\in M_x$ realizing $p$ in $\mathbf M^*$ and $b\in N_x$ realizing $q$ in $\mathbf N^*$. Put $\mathbf A:=\<a\>_{\mathbf M}$
and $\mathbf B:=\<b\>_{\mathbf N}$. Since $a$ and $b$ realize the same quantifier-free $\mathcal L$-formulas
in $\mathbf M$ and $\mathbf N$, respectively, we get an isomorphism $\mathbf A\to\mathbf B$ sending $a$ to $b$. Then ${\mathbf M}^*\models \varphi^*(a)$ iff ${\mathbf N}^*\models \varphi^*(b)$, by
\eqref{eq:key lemma}, so $\varphi^*\in p$ iff $\varphi^*\in q$.
\end{proof}


\noindent
Typically,  for $\mathcal L^*\neq\mathcal L$, the criterion in the lemma above gets used via its corollary below. To state that corollary, we
define $\Sigma^*$ to have
{\bf closures of $\mathcal L$-substructures} if 
for all ${\mathbf M}^*,{\mathbf N}^*\models \Sigma^*$ with a common 
${\mathcal L}$-substructure $\mathbf A=(A;\dots)$ of
${\mathbf M}$ and~${\mathbf N}$, there is a (necessarily unique) 
isomorphism over $A$ from the $\mathcal L^*$-substructure of ${\mathbf M}^*$ generated by~$A$ onto the $\mathcal L^*$-substructure of ${\mathbf N}^*$ generated by $A$.  \index{closure!of $\mathcal L$-substructures}

\begin{cor}\label{closureprop}
If $\Sigma^*$ has closures of $\mathcal L$-substructures, then every
quan\-ti\-fier-free ${\mathcal L}^*$-formula is $\Sigma^*$-equivalent to a quantifier-free
$\mathcal L$-formula.
\end{cor}

\begin{example}
Let $\mathcal L=\mathcal L_{\operatorname{R}}$ be the language of rings
and let $\mathcal L^*$ be $\mathcal L$ augmented by a unary function symbol $\iota$.
Any field is naturally an $\mathcal{L}$-structure and
expands to an $\mathcal L^*$-structure by $\iota(0):=0$ and $\iota(a):= a^{-1}$ for nonzero $a$ in the field. Note that
$$\Sigma^*\ :=\ \operatorname{Fl}\cup \big\{ \iota(0)=0,\ \forall x \big( x\neq 0 \rightarrow x\cdot \iota(x)=1 \big) \big\}$$
has closures of $\mathcal L$-substructures, by the universal property of the fraction field of an integral domain. Hence every quantifier-free $\mathcal L^*$-formula is
$\Sigma^*$-equivalent to a quantifier-free $\mathcal L$-formula. (This also follows easily
by a simple direct argument; Corollaries~\ref{lem:L vs L'} and \ref{lem:L vs L^a} are more substantial applications.)
\end{example}



\subsection*{Application to QE} The expression 
$\mathbf{M}\equiv_A \mathbf{N}$ is short for $\mathbf M_A\equiv\mathbf N_A$; 
here $A$ is a parameter set in both $\mathbf{M}$ and
$\mathbf{N}$, that is, $A\subseteq M$ and $A\subseteq N$. Typically we use
this notation when $A$ underlies a common substructure 
$\mathbf{A}$ of
$\mathbf{M}$ and $\mathbf{N}$.
Taking $\mathcal L^*=\mathcal L$ in Lemma~\ref{lem:key lemma} yields:

\nomenclature[Bj4]{$\mathbf M \equiv_A\mathbf N$}{$\mathbf M_A$, 
$\mathbf N_A$ are elementarily equivalent}


\begin{cor}\label{cor:substructure completeness} Given $\Sigma$, the following conditions are equivalent: \begin{enumerate}
\item \text{$\Sigma$ has \textup{QE}}; 
\item \text{$\mathbf M\equiv_A\mathbf N$,
for all $\mathbf M,\mathbf N\models\Sigma$ and any common substructure $\mathbf A$ of $\mathbf M$, $\mathbf N$};
\item \text{$\Sigma\cup\operatorname{Diag}_A(\mathbf A)$ is complete,
for all $\mathbf A\models\Sigma_\forall$.}
\end{enumerate}
\end{cor}

 

\begin{cor}\label{cor:QE and sentences}
Suppose $\Sigma$ admits \textup{QE} and has a model. Then 
 $\Sigma$ is complete iff some $\mathcal{L}$-structure  \textup{(}not necessarily a model of $\Sigma$\textup{)} embeds into every model of $\Sigma$. 
\end{cor}



\subsection*{A test for quantifier elimination} We now come to our first QE test: \index{test!for QE}
\index{quantifier elimination!test}

\begin{prop} \label{prop:QE test} Let $\Sigma$ be given. Then the following are equivalent: \begin{enumerate}
\item $\Sigma$ has \textup{QE};
\item whenever $\mathbf A$ is a substructure of a model $\mathbf M$ of $\Sigma$, any
embedding of $\mathbf A$ into any model $\mathbf N$ of $\Sigma$ extends to an embedding of $\mathbf M$ into some $\mathbf N^*\succeq\mathbf N$.
$$\xymatrix{ 
& \mathbf N^* \\
\mathbf M \ar@{-->}[ur] & \mathbf N  \ar@{-->}[u]_{\preceq} \\
\mathbf A \ar[u]^{\subseteq} \ar[ur] }$$
\end{enumerate}
\end{prop}
\begin{proof}
Suppose $\Sigma$ has QE,  let $\mathbf M,\mathbf N\models\Sigma$,
$\mathbf A\subseteq\mathbf M$, and let $i\colon\mathbf A\to\mathbf N$ be an embedding;
we need to show that $i$ extends to an embedding of $\mathbf M$ into some elementary extension of $\mathbf N$. Replacing $\mathbf N$ by an isomorphic structure we can assume that $\mathbf A\subseteq\mathbf N$ and
$i$ is the natural inclusion $\mathbf A\to\mathbf N$. Then by Corollary~\ref{cor:substructure completeness} we have
$\mathbf M\equiv_A\mathbf N$. Now use
Corollary~\ref{cor:elem equivalence and elem embeddings} to obtain an extension of $i$ to an (elementary) embedding of
$\mathbf M$ into some elementary extension of $\mathbf N$.

For the converse, suppose (2) holds.  
Let $\varphi(x)$ be an existential formula; by Lemma~\ref{lem:QE simplified}
it suffices to show that $\varphi(x)$ is $\Sigma$-equivalent to a quantifier-free formula $\varphi'(x)$. For this we use Lemma~\ref{lem:key lemma} in the case $\mathcal L^*=\mathcal L$.
So let $\mathbf M,\mathbf N\models\Sigma$, let $\mathbf A$ be a common substructure of $\mathbf M$ and $\mathbf N$,
and $a\in A_x$; by symmetry it is enough to show: $\mathbf M\models\varphi(a)\Longrightarrow \mathbf N\models\varphi(a)$. Extend the natural inclusion $\mathbf A\to\mathbf N$ to an embedding of $\mathbf M$ into an elementary extension $\mathbf N^*$ of $\mathbf N$. Then
$$\mathbf M\models\varphi(a)\quad\Rightarrow\quad \mathbf N^*\models\varphi(a)
\quad\Rightarrow\quad \mathbf N\models\varphi(a),$$ 
where we used Corollary~\ref{cor:persist, 1},~(2) for the first implication.
\end{proof}

\subsection*{QE tests using saturation}
Using saturated structures yields QE-tests that are in some cases
easier to use:

\begin{prop}[QE Test, first variant]\label{prop:QE test, 3}\index{test!for QE}\index{quantifier elimination!test}
Let $\Sigma$ be given. Suppose that for every $\mathbf{M}\models \Sigma$ 
and substructure~$\mathbf A$ of $\mathbf M$ with
$A\neq M$ and every embedding $i$ of~$\mathbf A$ into an $\abs{A}^+$-saturated model $\mathbf N$ of $\Sigma$ there exist $s\in S$ and $b\in M_s\setminus A_s$
such that $i$ extends to an embedding $\mathbf A\<b\>\to \mathbf N$. Then $\Sigma$ has \textup{QE}.
\end{prop}
\begin{proof}
Let $\mathbf{A}_0\subseteq\mathbf M\models \Sigma$, 
and let $i\colon\mathbf{A}_0\to\mathbf N\models\Sigma$ be an
embedding. Proposition~\ref{prop:saturated elemext} yields a 
$\kappa^+$-saturated
elementary extension $\mathbf N^*$ of $\mathbf N$, with 
$\kappa:=\max\{\abs{\mathcal L},\abs{M}\}$. By ~\ref{prop:QE test} it is 
enough to extend $i$ to an embedding $\mathbf{M}\to \mathbf{N}^*$.
By Zorn we have a maximal embedding $j: \mathbf{A}\to \mathbf{N}^*$ extending
$i$, that is,
$\mathbf{A}_0\subseteq \mathbf{A}\subseteq \mathbf{M}$, $j$ is an embedding 
extending $i$, and $j$ does not extend to any embedding 
$\mathbf{B}\to \mathbf{N}^*$ with $\mathbf{A}\subseteq \mathbf{B}\subseteq \mathbf{M}$ and $\mathbf{A}\ne \mathbf{B}$. 
Then  $\mathbf{A}=\mathbf{M}$ by the hypothesis of ~\ref{prop:QE test, 3}. 
\end{proof}

\noindent
The freedom to choose $b$ in this test is sometimes convenient.

A {\bf $\Sigma$-closure} of an $\mathcal{L}$-structure $\mathbf A$ is a model $\mathbf A_\Sigma$ of $\Sigma$ with
$\mathbf A\subseteq\mathbf A_\Sigma$ such that every embedding of $\mathbf A$ into a model $\mathbf M$ of $\Sigma$ extends (not necessarily uniquely) to an embedding $\mathbf A_\Sigma\to\mathbf M$. \index{closure!$\Sigma$-closure}
%If every substructure of a model of $\Sigma$  has a $\Sigma$-closure {\it and}\/
%$\Sigma$ is model complete then $\Sigma$ admits QE. 
%However, sometimes it is not much harder to test for QE directly, and then 
%the following test can come in handy:

\begin{prop}[QE Test, second variant]\label{prop:QE test, 2} \index{test!for QE}\index{quantifier elimination!test} Let
$\Sigma$ be given. Assume:
\begin{enumerate}
\item every substructure of every  model of $\Sigma$ has a $\Sigma$-closure; and
\item for all models $\mathbf M$, $\mathbf N$ of $\Sigma$ with $\mathbf M\subseteq\mathbf N$ and
$M\neq N$,  and any $\abs{M}^+$-saturated elementary extension $\mathbf M^*$ of $\mathbf M$
there exist $s\in S$, $a\in M_s\setminus N_s$, and an embedding of $\mathbf M\<a\>$ into $\mathbf M^*$ over $\mathbf M$.
$$\xymatrix{ 
\mathbf N&  \\
\mathbf M\<a\> \ar[u]^{\subseteq} \ar@{-->}[r] & \mathbf M^*   \\
\mathbf M \ar@{-}[u]^{\subseteq} \ar@{-}[ur]_\preceq }$$
\end{enumerate}
Then $\Sigma$ has \textup{QE}.
\end{prop}
\begin{proof} Check that the hypothesis of \ref{prop:QE test, 3} is satisfied.
\end{proof}

\begin{exampleNumbered}\label{ex:DOAb}
Suppose $\mathcal L=\mathcal L_{\operatorname{OA}}$ is the language of ordered abelian groups and
$\Sigma=\operatorname{Div}\cup\operatorname{OAb}\cup\{\exists x\,x\neq 0\}$, so the models of $\Sigma$ are the  nontrivial divisible ordered abelian groups; see Example~\ref{ex:theories},~(3),~(5). 
Substructures of models of~$\Sigma$
are ordered abelian groups. Each ordered abelian group $A$ has a $\Sigma$-closure $A_\Sigma$: 
if $A=\{0\}$,  let $A_\Sigma$ be the ordered additive group~$\Q$; 
if $A\neq\{0\}$, let  $A_\Sigma:=\Q\otimes_\Z A$ be the ordered divisible hull  of~$A$; see Section~\ref{sec:oag}. 

Let $M,N\models\Sigma$ with $M\subseteq N$, let $M^*$ be an $|M|^+$-saturated elementary extension of $M$, and let $a\in N\setminus M$. Take an element $a^*\in M^*$ realizing the same cut in $M$ as $a$. We have
$M\<a\>=M+\Z a=M\oplus\Z a$ and $M+\Z a^*=M\oplus\Z a^*$ (internal direct sums), so we get an embedding $M\<a\>\to M^*$ over $M$ sending $a$ to $a^*$. 
Thus $\Sigma$ has QE by~\ref{prop:QE test, 2}.
\end{exampleNumbered}


\subsection*{Relative quantifier elimination}\index{quantifier elimination!relative}
In this subsection $\mathcal L$ is a sublanguage of
the language~${\mathcal L}^*$. Let $S^*\supseteq S$ be the set of sorts for $\mathcal{L}^*$, and assume that $\mathcal{L}^*$ has for each $s^*\in S^*$ a constant symbol of sort~$s^*$. Let $\Sigma^*$ be a set of ${\mathcal L}^*$-sentences.   

We consider here the property of $\Sigma^*$ having QE 
{\em relative to $\mathcal L$}. To make this notion precise we say that an 
$\mathcal L^*$-formula  is {\bf $\mathcal L$-simple} if it is a boolean 
combination of atomic $\mathcal L^*$-formulas
and formulas $\varphi(t^*)$ where $\varphi(y)$ is an $\mathcal L$-formula
and $t^*$ is a tuple of $\mathcal L^*$-terms. The main ``relative'' QE-test
is Proposition~\ref{prop:relative QE} below. 
\index{formula!simple} \index{simple!formula}
  We let ${\mathbf A}^*$, ${\mathbf M}^*$, ${\mathbf N}^*$, 
range over ${\mathcal L}^*$-structures, with $\mathcal L$-reducts ${\mathbf A}$, ${\mathbf M}$,~${\mathbf N}$.


\begin{lemma}\label{lem:relative QE}
Let $\varphi^*(x)$  be an 
${\mathcal L}^*$-formula. Then $\varphi^*(x)$ is $\Sigma^*$-equivalent to some $\mathcal L$-simple 
$\mathcal L^*$-formula~$\psi^*(x)$ iff for all 
${\mathbf M}^*,{\mathbf N}^*\models\Sigma^*$ and every
common $\mathcal L^*$-sub\-struc\-ture ${\mathbf A^*}$ of ${\mathbf M}^*$ and~${\mathbf N}^*$
such that $\mathbf M\equiv_A\mathbf N$,
and~all $a\in A^*_x$:
\begin{equation}\label{eq:partial qe}
{\mathbf M}^*\models \varphi^*(a) \quad\Longleftrightarrow\quad {\mathbf N}^*\models \varphi^*(a).
\end{equation}
\end{lemma}
\begin{proof}
Suppose $\varphi^*(x)$ is $\mathcal L$-simple, and let 
${\mathbf M}^*,{\mathbf N}^*\models \Sigma^*$ with
common $\mathcal L^*$-sub\-struc\-ture ${\mathbf A^*}$ such that 
$\mathbf M\equiv_A\mathbf N$, and $a\in A^*_x$; we claim that \eqref{eq:partial qe} holds. 
This is clear if $\varphi^*$ is atomic. Suppose $\varphi^*$ has the form
$\varphi(t^*)$ where~$\varphi(y)$ is an $\mathcal L$-formula
and $t^*(x)$ is a tuple of $\mathcal L^*$-terms.
Then $b:=(t^*)^{\mathbf M^*}(a)=(t^*)^{\mathbf A^*}(a)\in A^*_y=A_y$, so
$${\mathbf M}^*\models \varphi^*(a) \ \Longleftrightarrow\ 
{\mathbf M}^*\models \varphi(b)
\ \Longleftrightarrow\ 
{\mathbf M}\models \varphi(b).$$
Similarly ${\mathbf N}^*\models \varphi^*(a)\Longleftrightarrow
{\mathbf N}\models \varphi(b)$.
Together with $\mathbf M\equiv_A\mathbf N$, this yields the claim.
This proves the ``only if'' direction of the lemma.
For the ``if'' direction, suppose \eqref{eq:partial qe} holds for all
$\mathbf A^*$,~${\mathbf M}^*$,~${\mathbf N}^*$ and $a$ as in the statement of the lemma. 
Let $\mathcal L_{\operatorname{Mo}}$ and $\operatorname{Mo}$ be as in~\ref{ex:morleyization}.
Set
$\mathcal L^*_1:=\mathcal L^*\cup\mathcal L_{\operatorname{Mo}}$ and $\Sigma^*_1 := \Sigma^*\cup\operatorname{Mo}$. It suffices to show that $\varphi^*(x)$ is $\Sigma_1^*$-equivalent to a quantifier-free $\mathcal L^*_1$-formula, and
towards this goal we use the case $\mathcal{L}=\mathcal{L}^*$ of 
Lemma~\ref{lem:key lemma}, with $\mathcal L_1^*$
and $\Sigma_1^*$ in the role of $\mathcal L^*$ and~$\Sigma^*$. Accordingly,
let $\mathbf M_1^*, \mathbf N_1^*\models \Sigma_1^*$, and let $\mathbf A^*_1$
be a common substructure of $\mathbf M_1^*$ and $\mathbf N_1^*$. 
Let $\mathbf M^*$, $\mathbf N^*$, $\mathbf{A}^*$ be the $\mathcal{L}^*$-reducts 
of $\mathbf M_1^*, \mathbf N_1^*,\mathbf A^*_1$. Then 
$\mathbf{M}\equiv_A \mathbf{N}$ by the definition of $\operatorname{Mo}$.
Thus by  \eqref{eq:partial qe} we have  $\mathbf M^*\models\varphi^*(a)\ \Leftrightarrow\ \mathbf N^*\models\varphi^*(a)$, for all $a\in A^*_x $, and thus
 $\mathbf M_1^*\models\varphi^*(a)\ \Leftrightarrow\ \mathbf N_1^*\models\varphi^*(a)$, for all $a\in A^*_x $. 
\end{proof}


\begin{cor}\label{cor:relative QE}
The following are equivalent: 
\begin{enumerate}
\item every ${\mathcal L}^*$-formula $\varphi^*(x)$ is $\Sigma^*$-equivalent to some 
$\mathcal L$-simple $\mathcal L^*$-for\-mu\-la~$\psi^*(x)$;
\item 
for all ${\mathbf M}^*,{\mathbf N}^*\models \Sigma^*$ with
common $\mathcal L^*$-sub\-struc\-ture ${\mathbf A^*}$, we have
$$\mathbf M\equiv_A\mathbf N\ \Longrightarrow\ 
\mathbf M^*\equiv_{A^*} \mathbf N^*.$$
\item if $p,q\in\operatorname{S}_x(\Sigma^*)$ 
contain the same $\mathcal L$-simple $\mathcal L^*$-formulas, then $p=q$.
\end{enumerate}
\end{cor}
\begin{proof} Lemma~\ref{lem:relative QE} yields $(1)\Leftrightarrow(2)$ and
Corollary~\ref{cor:separation} gives  $(1)\Leftrightarrow(3)$. \end{proof}


\index{quantifier elimination!relative}

\begin{prop}\label{prop:relative QE}
Suppose that for all models $\mathbf M^*$, $\mathbf N^*$ of $\Sigma^*$, where $\mathbf N^*$ is
$\kappa^+$-sa\-tu\-rated for $\kappa=\abs{M^*}$, every substructure $\mathbf A^*$ of $\mathbf M^*$, every
embedding ${i^*\colon \mathbf A^*\to\mathbf N^*}$, and every embedding $e\colon \mathbf M\to\mathbf N$
extending the $\mathcal L$-reduct of $i^*$, there exists an embedding $\mathbf M^*\to\mathbf N^*$ whose $\mathcal L$-reduct is $e$.
Then every ${\mathcal L}^*$-formula $\varphi^*(x)$ is $\Sigma^*$-equivalent to some 
$\mathcal L$-simple $\mathcal L^*$-for\-mu\-la~$\psi^*(x)$. 
\end{prop}

\noindent
Before proving this, we first establish a lemma, under
 the same assumptions as in Proposition~\ref{prop:relative QE}.

\begin{lemma}
Let $\mathbf M^*,\mathbf N^*\models\Sigma^*$ with $\mathbf M^*\subseteq\mathbf N^*$. Then $\mathbf M\preceq\mathbf N$ iff $\mathbf M^*\preceq\mathbf N^*$.
\end{lemma}
\begin{proof}
The backward direction being obvious, let $\varphi^*(x)$ be an $\mathcal L^*$-formula. By induction on the construction of $\varphi^*$ we show
that for all $\mathbf M^*$, $\mathbf N^*$ as in the hypothesis of the lemma 
with  $\mathbf M\preceq\mathbf N$
and all $a^*\in M^*_x$ we have
$$\mathbf M^*\models\varphi^*(a^*)\quad\Longleftrightarrow\quad \mathbf N^*\models\varphi^*(a^*).$$
For the inductive step, let $\varphi^* = \exists y\theta^*$, where $\theta^*(x, y)$ is an $\mathcal L^*$-formula and $y$ a
single variable of $\mathcal L^*$. Since $\theta^*$ is of lower complexity
than $\varphi^*$ the direction ``$\Rightarrow$'' follows from the induction hypothesis.
So suppose $\mathbf N^*\models\varphi^*(a^*)$. Choose an $|M^*|^+$-saturated elementary extension $\mathbf M_1^*$ of
$\mathbf M^*$, with $\mathcal L$-reduct $\mathbf M_1$. By Corollary~\ref{cor:sat elem embedd} take an elementary embedding
$e\colon \mathbf N\to\mathbf M_1$ extending the natural inclusion $\mathbf M\to\mathbf M_1$, and
by the assumption in Proposition~\ref{prop:relative QE} then take an embedding $\mathbf N^*\to\mathbf M_1^*$
with $\mathcal L$-reduct $e$ extending the natural inclusion $\mathbf M^*\to\mathbf M_1^*$.
Using the inductive hypothesis on $\theta^*$ we get $\mathbf M_1^*\models\varphi^*(a^*)$,
and hence $\mathbf M^*\models\varphi^*(a^*)$.
\end{proof}

\begin{proof}[Proof of Proposition~\ref{prop:relative QE}]
Let $\mathbf M^*,\mathbf N^*\models\Sigma^*$ with a common substructure~$\mathbf A^*$
such that $\mathbf M \equiv_A \mathbf N$; by Corollary~\ref{cor:relative QE} it is enough
to show that then $\mathbf M^*\equiv_{A^*}\mathbf N^*$. 
By Proposition~\ref{prop:saturated elemext}, after replacing $\mathbf N^*$ by an elementary extension we can assume that $\mathbf N^*$ is $\abs{M^*}^+$-saturated.
By Corollary~\ref{cor:sat elem embedd} and the assumption of the proposition there exists
an embedding $\mathbf M^*\to\mathbf N^*$ whose $\mathcal L$-reduct is an elementary embedding $\mathbf M\to\mathbf N$ and which extends the natural inclusion $\mathbf A^*\to\mathbf N^*$.
Now the lemma yields $\mathbf M^*\equiv_{A^*}\mathbf N^*$.
\end{proof}


\begin{exampleNumbered}\label{ex:vs} 
Let $\mathcal L_{\operatorname{Mod}}$ be the two-sorted language of modules as in~\ref{ex:languages},~(7), let $d\in\N\cup\{\infty\}$, and 
let $\operatorname{Vec}_d$ be a set of $\mathcal L_{\operatorname{Mod}}$-sentences whose models are the
$d$-dimensional vector spaces over fields, viewed as $\mathcal L_{\operatorname{Mod}}$-structures in the natural way.
Then every $\mathcal L_{\operatorname{Mod}}$-formula is $\operatorname{Vec}_d$-equivalent to one
without quantifiers over the module sort.
This  follows from Proposition~\ref{prop:relative QE} where $\mathcal L^*=\mathcal L_{\operatorname{Mod}}$,
 $\mathcal L= \{ 0_{\operatorname{R}}, 1_{\operatorname{R}}, {-_{\operatorname{R}}}, {+}_{\operatorname{R}}, {\,\cdot\,}_{\operatorname{R}}\}$ is the copy of the language of rings in the sort $\operatorname{R}$, and
 $\Sigma^*=\operatorname{Vec}_d$. To see this
let $V$, $W$ be $d$-dimensional vector spaces over fields $K$, $L$, respectively, where $W$ is $|V|^+$-saturated, and
let $A$ be a substructure of $V$. Then $A$ is a module over a subring $R$ of $K$.
Let $i=(i_{\operatorname{R}},i_{\operatorname{M}})\colon A\to W$ be an embedding and let $e\colon K\to L$ be a field embedding
which restricts to the ring embedding $i_{\operatorname{R}}\colon R\to L$.
The  $K$-linear map $K\otimes_R A\to V$ with $1\otimes a\mapsto a$ is injective
\cite[\S\S{}3, 4]{Lang}.
Hence $i$ extends to an embedding~$j$ of the $K$-linear subspace of $V$ generated by $A$ into $W$ with $j_{\operatorname{R}}=e$. Now viewing $W$ as $K$-vector space via $e$, we have $\dim_K V\leq \dim_K W$;
hence $j$ extends to an embedding $V\to W$ as required. 
\end{exampleNumbered}

\subsection*{QE and definable closure}
{\it In this subsection we assume that $\Sigma$ is universal, and has \textup{QE}, and $\mathbf M\models\Sigma$.}\/
This has several useful consequences:

\begin{cor} Let $A\subseteq M$. Denoting the underlying set of the substructure~$\<A\>_{\mathbf M}$ of $\mathbf M$ by $\<A\>$,
we have $\<A\>= \operatorname{dcl}(A)$. 
\end{cor}
\begin{proof} This is because $\<A\>\subseteq \operatorname{dcl}(A)$, and 
$\<A\>_{\mathbf M}\preceq \mathbf M$. 
\end{proof}    

\noindent
The next result is known as: $\mathbf M$ has definable Skolem functions.

\begin{cor} Let $x=(x_1,\dots, x_m)$ and $y=(y_1,\dots, y_n)$
be disjoint finite multivariables, and suppose the relation $Z\subseteq M_{x}\times M_{y}$ is $0$-definable in $\mathbf M$.
Let $\pi\colon M_x\times M_y \to M_x$ be the natural projection map.
Then there is a $0$-definable map $f\colon M_x\to M_y$
such that $\big(a,f(a)\big)\in Z$ for all $a\in \pi(Z)$.
\end{cor}
\begin{proof} Replacing $Z$ by $Z\cup \big((M_x\setminus \pi(Z))\times M_y\big)$ we arrange that $\pi(Z)=M_x$. Take a quantifier-free formula $\varphi(x,y)$ that defines $Z$ in~$\mathbf M$. Set 
$$\Sigma(\mathbf M)\ :=\ \Sigma\cup\{\sigma:\ \sigma \text{ is quantifier-free and }\mathbf{M}\models \sigma\}.$$
Then $\Sigma(\mathbf M)$ is complete, so
$\Sigma(\mathbf M)\models\forall x\exists y\, \varphi(x,y)$. Now use Proposition~\ref{prop:Herbrand}.
\end{proof}
 

\noindent
The proof above also shows that
definable functions are piecewise given by terms:

\begin{cor} \label{lem:def fns piecewise as terms}
Suppose $f \colon X \to M_s$ with $X\subseteq M_x$ is $0$-definable. Then there are
terms $t_1(x),\dots,t_k(x)$ of sort $s$, $k\in \N^{\ge 1}$, such that for every $a\in X$
we have $f(a)=t_i^{\mathbf M}(a)$ for some $i\in\{1,\dots,k\}$.
\end{cor}


\subsection*{QE and model completeness} Let $T$ be an $\mathcal{L}$-theory. By Corollary~\ref{cor:substructure completeness}, 
$T$ has~\textup{QE} iff
it is the model completion of $T_\forall$. Thus:

\begin{lemma}\label{lem:model completion with QE} If $T$ has a
universal axiomatization and has a model completion, then this model completion has \textup{QE}.
\end{lemma}

\begin{example}
Let $\mathcal L=\mathcal L_{\operatorname{OA}}$
and $\Sigma$ be as in Example~\ref{ex:DOAb}: the models of $\Sigma$ are the nontrivial divisible 
ordered abelian groups viewed as $\mathcal L$-structures.
Then~$\text{Th}(\Sigma)$ is the model completion of the theory
$\text{Th}(\operatorname{OAb})$ of ordered abelian groups. 
\end{example}


 
\begin{cor}\label{cor:ES}
$T$ has \textup{QE} $\Longleftrightarrow$
$T$ is model complete and $T_\forall$ has \textup{AP}.
\end{cor}


\subsection*{Notes and comments}
%The method of quantifier elimination as a tool for understanding the definable sets in a structure
%was first championed by Tarski starting in the 1920s.
Pioneering work on QE was done by Skolem~\cite{Skolem19,Skolem20}, Langford~\cite{Langford1,Langford2}, Presburger~\cite{Presburger}, and Tarski~\cite{Tarski31,Tarski35b,Ta}. 
%``Morleyization'' as in Example~\ref{ex:morleyization} is actually due to Skolem~\cite{Skolem20}.
Co\-rol\-la\-ry~\ref{cor:substructure completeness} is from Sacks~\cite{Sacks}.
Example~\ref{ex:DOAb} may be seen as the model-theoretic content of ``Fourier-Motzkin elimination''~\cite[III, pp.~209--223]{Schrijver}.
For a survey of  QE results in algebra until the mid-1980s see \cite{Weispfenning84}.
Propositions~\ref{prop:QE test, 3} and \ref{prop:QE test, 4} go back to Shoenfield~\cite{Shoenfield71,Shoenfield77}, and
Proposition~\ref{prop:relative QE} is abstracted from \cite[Section~4]{AvdD}.
In connection with Example~\ref{ex:vs}, see \cite{Pierce} for a way to treat vector spaces over an unspecified field in a one-sorted setting.
For an application of Lemma~\ref{lem:def fns piecewise as terms} see \cite{DMM0}.
Lemma~\ref{lem:model completion with QE} is from~\cite{Robinson58} and
Corollary~\ref{cor:ES} from \cite{EklofSabbagh}.
 
\section{Application to Algebraically Closed and Real Closed Fields}\label{sec:some theories}

\noindent
To demonstrate how the material of the previous sections is used in practice, we now apply it to some basic mathematical structures,
namely  {\it algebraically closed fields}\/ and
{\it real closed fields.}\/  %In particular, we show the theorems of Chevalley-Tarski and Tarski-Seidenberg mentioned in Section~\ref{sec:structures and definable sets}.

\subsection*{Algebraically closed fields}
We establish here the basic model-theoretic facts about algebraically closed
fields: elimination of quantifiers, the Nullstellensatz, strong minimality, definably closed = perfect subfield, and definable functions.

Throughout this subsection $K$, $E$, and $F$ are fields, and %until further notice 
``algebraic over'', ``algebraically closed'', and ``algebraic closure'' are
taken in the sense of field theory; as we shall see, these notions agree in the
context of algebraically closed fields with the model-theoretic notions. By
$\operatorname{ACF}$ we mean here the theory of algebraically closed fields in the language
of rings, and for $p$ a prime number or $p = 0$ we let $\operatorname{ACF}(p)$ be the theory of
algebraically closed fields of characteristic~$p$, as in Examples~\ref{ex:theories},~(10),~(11). Below $p$ ranges over
the set $\{0, 2, 3, 5, \dots \}$ of possible characteristics.

\begin{theorem}\label{thm:ACF QE}
$\operatorname{ACF}$ has \textup{QE.}
\end{theorem}
\begin{proof}
Every integral domain has an $\operatorname{ACF}$-closure, namely the algebraic closure of its fraction field. 
Let $E$  be algebraically closed, let $K$ be  a proper 
algebraically closed subfield of $E$, and let $F$ be algebraically closed, $\abs{K}^+$-saturated, also with~$K$ as a subfield.
Take 
any $a \in E \setminus K$. Then $P(a) \neq 0$ for all  $P(T) \in K[T]^{\neq}$,
that is,~$a$ is transcendental over $K$. By saturation we can take $b \in F\setminus K$, so $b$ is transcendental over $K$. Then the natural inclusion $K\to F$ extends to an embedding
$K[a] \to F$ sending~$a$ to~$b$. Thus $\operatorname{ACF}$ has QE by Proposition~\ref{prop:QE test, 4}.
\end{proof}

\noindent
The substructures of algebraically closed fields are exactly the integral domains, so
by the above, $\operatorname{Th}(\operatorname{ACF})$ is the model completion of the theory of integral domains. 
Here is a well-known manifestation (but not a special case) of Theorem~\ref{thm:ACF QE}:

\begin{example}
Let $X_1,\dots,X_n,Y$ be distinct indeterminates, $X=(X_1,\dots,X_n)$, and
$P,Q\in \Z[X,Y]^{\neq}$ be monic in $Y$. Then there is a polynomial $R\in\Z[X]$ (the {\it resultant}\/ of $P$ and~$Q$)
such that for every algebraically closed $E$ and $a\in E^n$: $R(a)=0$ iff $P(a,Y),Q(a,Y)\in E[Y]$
have a common zero in $E$; see \cite[Chapter~IV, \S{}8]{Lang}.
\end{example}

\noindent
The following consequences of QE make up the Constructibility Theorem
(Che\-val\-ley-Tarski) and the Nullstellensatz (Hilbert).
Let $T=(T_1,\dots,T_n)$ be an $n$-tuple of distinct indeterminates. \index{theorem!Chevalley-Tarski}\index{theorem!Nullstellensatz}

\begin{cor}\label{cor:ACF QE}
Let $E$ be algebraically closed with subfield $K$.
\begin{enumerate}
\item A subset of $E^n$ is $K$-definable in $E$ if and only if it is a boolean
combination of zero sets
$\big\{a \in  E^n : P(a) = 0\big\}$ of polynomials $P \in  K[T]$.
\item If $P_1, \dots , P_k, Q_1, \dots,Q_l \in  K[T]$ and there is an overfield $F$ of
$K$ with a point $a \in  F^n$ such that
$$P_1(a) = \cdots = P_k(a) = 0,\ Q_1(a) \neq 0, \dots , Q_l(a) \neq 0,$$
then there is such a point $a \in  E^n$.
\item Let $P_1, \dots, P_m \in  K[T]$. Then $P_1, \dots , P_m$ have no common
zero in $E$ if and only if there are $Q_1, \dots , Q_m \in  K[T]$ such
that $$P_1Q_1 + \cdots + P_mQ_m = 1\qquad\text{ \textup{(}in $K[T]$\textup{)}.}$$
%\item The maximal ideals of $E[T]$ are exactly the ideals
%$$(T_1 - a_1, \dots , T_n - a_n)E[T]\qquad  (a_1, \dots , a_n \in  E).$$ 
\end{enumerate}
\end{cor}
\begin{proof}
Item (1) is immediate from QE. In (2), extend $F$ to be algebraically
closed, and use that then $E \equiv_K F$  by QE. In (3), suppose there
are no $Q_1,\dots, Q_m\in K[T]$ such that $P_1Q_1 + \cdots + P_mQ_m = 1$. Then
the ideal of $K[T]$ generated by $P_1,\dots,P_m$ is a proper ideal, and thus
contained in a maximal ideal $\m$ of $K[T]$. 
Put $t_i := T_i + \m$ for $i = 1,\dots, n$ and $t:=(t_1,\dots,t_n)$.
Then $\m \cap K = \{0\}$, so
$K[T]/\m = K[t]$
is a field extension of $K$, and $P(t) = P(T) + \m$ for each
$P\in K[T]$; in particular, $P_1,\dots, P_m$ have $t$ as a common
zero in an extension field of~$K$, and thus $P_1,\dots, P_m$ have a common zero in
$E$ by (2).
%As to (4), let $R$ be a ring and $a = (a_1,\dots,a_n)\in R^n$. We claim that the kernel of the ring morphism $P \mapsto P(a) \colon R[T]\to R$  is $(T_1 - a_1, \dots , T_n - a_n)R[T]$. The latter ideal %is certainly part of the kernel. Let $P\in R[T]$ and rewrite $P$ as a polynomial in $T_1 - a_1, \dots , T_n - a_n$, so $P = P^*(T_1 - a_1, \dots , T_n - a_n)$ with $P^*\in R[T]$. If $P$ is in the kernel, then $P(a) = P^*(0) = 0$, so $P^*$ has constant term zero, that is, $P^*\in (T_1,\dots, T_n)R[T]$, and thus $P\in (T_1 - a_1, \dots , T_n - a_n)R[T]$.  If $R$ is a field, the surjectivity of this substitution morphism  shows that its kernel is a maximal ideal of $R[T]$. It remains to show that for $R = E$ this gives all maximal ideals of~$E[T]$. Let $\m$ be a maximal ideal of $E[T]$ and let $P_1,\dots, P_m$ generate this ideal. (By Hilbert's Basis Theorem there is a finite set of generators, see Proposition~\ref{prop:HBT}.) By (3) we have a common zero $a = (a_1,\dots,a_n)\in E^n$ of $P_1,\dots,P_m$ and then~$a$ is a zero of all polynomials in $\m$, so by our earlier consideration we have $\m \subseteq (T_1-a_1,\dots, T_n-a_n)E[T]$. By the maximality of $\m$ this inclusion is an equality.
\end{proof}

\noindent
The following is known as the {\em strong minimality\/} of algebraically closed fields. (This property alone has already many consequences.) 

\begin{cor}\label{cor:ACF sm} Let $E$ be algebraically closed. Then a set $X\subseteq E$ is definable in $E$ iff $X$ is finite or cofinite.
\end{cor}
\begin{proof} For a single indeterminate $T$ and $P\in E[T]^{\ne}$ the set $\big\{a\in E:\ P(a)=0\big\}$ is finite. Now use Corollary~\ref{cor:ACF QE}, (1), for $n=1$.
\end{proof} 




%\noindent
%A typical application  of Compactness yields uniform bounds in (3) above:

%\begin{cor}\label{cor:ACF QE, uniform}
%For all $d,n\in\N$ there is some $B(d,n)\in\N$ such that if $P_1, \dots, P_m \in  K[T]=K[T_1,\dots,T_n]$ all have \textup{(}total\textup{)} degree at most $d$ and no common zero in $E$, then there are $Q_1, \dots , Q_m \in  K[T]$ of degree at most $B(d,n)$ such that $P_1Q_1 + \cdots + P_mQ_m = 1$.
%\end{cor}
%\begin{proof}
%First note that the polynomials of degree $\leq d$ form a $K$-linear subspace $K[T]_{\leq d}$  of $K[T]$ having dimension $M=M(n,d):={n+d\choose d}$. Thus it suffices to prove the existence of $B(d,n)$ such that if $P_1, \dots, P_M \in  K[T]_{\leq d}$ have no common zero in $E$, then there are $Q_1, \dots , Q_M \in  K[T]$ of degree at most $B(d,n)$ such that $\sum_i P_iQ_i = 1$. Fix a $K$-linear bijection $c\colon K[T]_{\leq d}\to K^{M}$. Using Theorem~\ref{thm:ACF QE}, for each $D\in\N$ take an  $\mathcal L_{\operatorname{Ri}}$-formula $\varphi_D(x_1,\dots,x_M)$, where each $x_i$ is a multivariable of length $M$, such that for all $P_1, \dots, P_M \in  K[T]_{\leq d}$: $K\models\varphi_D(c(P_1),\dots,c(P_M))$ iff $P_1, \dots, P_M$   have a common zero in $E$ or there are $Q_1, \dots , Q_M \in  K[T]$ of degree at most $B(d,n)$ such that $\sum_i P_iQ_i = 1$. (One may choose $\varphi_D$ to be existential.)  Let  $\mathcal L=\mathcal L_{\operatorname{Ri}}\cup\{c_{ij}:i,j=1,\dots,M\}$ where the $c_{ij}$ are new distinct constant symbols, and put $c_i=(c_{ij})$ for $i=1,\dots,M$. The set
%$$\operatorname{Fl}\cup\big\{\neg\varphi_D(\underline{c_1},\dots,\underline{c_M}):D\in\N\big\}$$
%of $\mathcal L$-sentences has no model by Corollary~\ref{cor:ACF QE},~(3); hence by Compactness, there is some $B\in N$ such that 
%$$\operatorname{Fl}\cup\big\{\neg\varphi_D(\underline{c_1},\dots,\underline{c_M}):D\leq B\big\}$$
%has no model. Then $B=B(d,n)$ has the desired property.
%\end{proof}

\noindent
In Section~\ref{sec:LS} we showed that 
$\operatorname{ACF}(p)$ is complete. This follows also from Corollary~\ref{cor:QE and sentences},~(2) and Theorem~\ref{thm:ACF QE}, since for $p > 0$ the field $\mathbb F_p$ embeds into every
model of $\operatorname{ACF}(p)$, and the ring $\Z$ embeds into every model of $\operatorname{ACF}(0)$.
Thus an $\mathcal L_{\operatorname{R}}$-sentence holds in {\it some}\/
algebraically closed field of characteristic $p$ iff it holds in {\it every}\/ 
algebraically closed field of characteristic $p$. Moreover:

\begin{cor}\label{cor:Lefschetz}
Let $\sigma$ be an $\mathcal L_{\operatorname{R}}$-sentence.  Then the following are equivalent:
\begin{enumerate}
\item $\sigma$ holds in all algebraically closed fields of characteristic $0$;
\item for all but finitely many prime numbers $p$, $\sigma$ holds in all algebraically closed fields of characteristic $p$.
\end{enumerate}
\end{cor}
\begin{proof}
The direction (1)~$\Rightarrow$~(2) is clear from the Compactness Theorem~\ref{thm:compactness, 2}.
Suppose conversely that $n_0\in\N$ is such that  $\sigma$ holds in all algebraically closed fields of characteristic $p>n_0$. To get (1), it suffices by completeness of $\operatorname{ACF}(0)$ to show that
the set
$\Sigma := \{\sigma\} \cup \operatorname{ACF}(0)$ 
of $\mathcal L_{\operatorname{R}}$-sentences has a model.
Every finite  $\Sigma_0\subseteq\Sigma$  contains only finitely many  sentences $p_1 1\neq 0,\dots,p_n 1\neq 0$
from $\operatorname{Fl}(0)\subseteq \operatorname{ACF}(0)$; since $\sigma$ holds in every algebraically closed
field of characteristic $p>\max\{n_0,p_1,\dots,p_n\}$, every such algebraically closed field 
is a model of $\Sigma_0$. Hence $\Sigma$ has a model by Compactness. This shows (2)~$\Rightarrow$~(1).
\end{proof}



\noindent
Combining Example~\ref{ex:forallexists Fpalg} and Corollary~\ref{cor:Lefschetz} yields:

\begin{cor}\label{cor:forallexists FpAlg}
Let $\sigma$ be a universal-existential $\mathcal L_{\operatorname{R}}$-sentence, and
suppose that for all but finitely many prime numbers $p$, $\sigma$ holds in all finite fields of characteristic~$p$.
Then $\sigma$ holds in every algebraically closed field of characteristic $0$.
\end{cor}


\begin{exampleNumbered}[Serre]\label{ex:Serre}
Suppose $E$ is algebraically closed and $\operatorname{char}(E)\neq 2$.
For $P= (P_1,\dots,P_n )\in E[T]^n$ and $a\in E^n$  set
$P(a):=\big(P_1(a),\dots,P_n(a)\big)\in E^n$.
Then {\it for any $P\in E[T]^n$ such that $P(P(a))=a$ for all $a\in E^n$, there exists an $a\in E^n$ with $P(a)=a$.}\/
To see this note that for fixed $n$ and a bound $d$ on the total degree of the~$P_i$,
the claim can be expressed as a universal-existential $\mathcal L_{\operatorname{R}}$-sentence~$\sigma_{n,d}$. 
Obviously $\sigma_{n,d}$  holds in all finite fields of characteristic $> 2$, and so it 
holds in all algebraically closed
fields of characteristic~$0$ by Corollary~\ref{cor:forallexists FpAlg}, and  in all
algebraically closed
fields of characteristic~$> 2$ by   Example~\ref{ex:forallexists Fpalg} and   completeness of $\operatorname{ACF}(p)$, $p>2$.
\end{exampleNumbered}

%\noindent
%Suppose $x=(x_1,\dots,x_n)$.
%By QE, if $E$, $F$ are algebraically closed with common subfield $K$, then $\operatorname{S}^E_x(K)=\operatorname{S}^F_x(K)$;
%we set $\operatorname{S}_x(K):=\operatorname{S}^{E}_x(K)$ where $E=K^\alg$. One can relate $\operatorname{S}_x(K)$ to the spectrum of the polynomial ring $K[T]=K[T_1,\dots,T_n]$. See Section~\ref{sec:ztn} for the spectrum of a commutative ring.
%In the next corollary, $\operatorname{S}_x(K)$ is equipped with the Stone topology, and $\Spec K[T]$ with the Zariski topology.

%\begin{cor}
%For each $p\in \operatorname{S}_x(K)$,
%$$I_p := \big\{ P\in K[T]: \textup{``$P(x)=0$''}\in p \big\}$$
%is a prime ideal of $K[T]$. The map $p\mapsto I_p\colon \operatorname{S}_x(K) \to \Spec K[T]$
%is a continuous bijection. \textup{(}In particular, $\Spec K[T]$ is compact.\textup{)}
%\end{cor}
%\begin{proof}
%The first statement is easy to see. By QE, if $p,q\in \operatorname{S}_x(K)$ satisfy $I_p=I_q$, then $p=q$; this
%shows that $p\mapsto I_p$ is injective. To show surjectivity, 
%let $\mathfrak p \in\Spec K[T]$. Let $F$ be an algebraic closure of $\Frac(K[T]/\mathfrak p)$ and  
%$t_i=T_i+\mathfrak p\in F$ for $i=1,\dots,n$, and let $p\in \operatorname{S}_x(K)$ be the $x$-type over $K$ realized by $t=(t_1,\dots,t_n)$;
%then $I_p=\mathfrak p$. For $S\subseteq K[T]$,  the preimage of
%the closed set $\Zero(S)$ under $p\mapsto I_p$ is the closed set $\bigcap_{P\in S} \<\textup{``$P(x)=0$''}\>$ of $\operatorname{S}_x(K)$; this shows continuity of $p\mapsto I_p$.
%\end{proof}

\noindent
If $E$ is algebraically closed
with subset $A$, then the (model-theoretic) algebraic closure $\operatorname{acl}(A)$ of $A$ in $E$
contains obviously the field-theoretic algebraic closure in~$E$ of the subfield
of $E$ generated by $A$, and is in fact equal to (the underlying set of) this
field-theoretic algebraic closure:

\begin{lemma} Let $E$ be algebraically closed with algebraically closed subfield
$K$. Then $K$ is algebraically closed in $E$ in the model theory sense.
\end{lemma}
\begin{proof}
Obvious from $K\preceq E$.
\end{proof}

\noindent
If $E$ is algebraically closed and $A\subseteq E$, then the
definable closure $\operatorname{dcl}(A)$ of $A$ in~$E$ contains at least the subfield of $E$ generated by $A$, and equals (the underlying set of) this subfield when $E$ has
characteristic zero:

\begin{prop} \label{prop:ACF(0) dcl} Let $E$ be algebraically closed of characteristic zero, with
subfield $K$. Then $K$ is definably closed in $E$.
\end{prop}
\begin{proof}
Let $a \in E\setminus K$; we claim that then $\sigma a \neq a$ for some $\sigma \in\Aut(E|K)$. (By Lemma~\ref{lem:dcl, acl} the proposition follows from this claim.) If $a$ is transcendental
over~$K$, take a transcendence basis $B$ of $E$ over $K$ with $a \in B$, take the
automorphism of~$K(B)$ over $K$ that sends each $b \in B$ to $b + 1$, and then
extend it to an automorphism of the algebraic closure $E$
of $K(B)$. Suppose $a$ is algebraic over~$K$. Since $a \notin K$, the minimum
polynomial of $a$ over $K$ is of degree $> 1$, so has a zero $b \in E$ with $b \neq a$
(here we use that $E$ has characteristic zero). Take an automorphism $\sigma$ of the
algebraic closure $K^\alg$ of $K$ in $E$ over $K$ that sends $a$ to~$b$, take a transcendence
basis $B$ of $E$ over $K^\alg$, and extend $\sigma$ to the automorphism of~$K^\alg(B)$ that is
the identity on $B$, and then extend further to an automorphism of $E$.
\end{proof}

\noindent
Characterizations of definable closures of this type lead to corresponding
descriptions of definable functions. In this case definable functions are piecewise rational:

\begin{cor}
Let $E$ be algebraically closed of characteristic zero, with
subfield $K$, and let $X \subseteq E^n$ and $f \colon X \to E$ be $K$-definable in $E$. Then
there are $P_1, \dots , P_k, Q_1, \dots , Q_k \in K[T]$ such that for each $x \in X$
there is $i \in \{1, \dots , k\}$ with $Q_i(x) \neq 0$ and $f(x) = P_i(x)/Q_i(x)$.
\end{cor}
\begin{proof}
Extending $E$ if necessary we can assume $E$ is $|K|^+$-saturated. Let
$x \in X$. Then $f(x) \in \operatorname{dcl}(K \cup \{x\}) = K(x)$ by the proposition above, that
is, $f(x) = P(x)/Q(x)$ with polynomials $P, Q \in K[T]$, $Q(x) \neq 0$. Now
use saturation.
\end{proof}

\noindent
Suppose $E$ is algebraically closed of characteristic $p > 0$. Then we have a
$0$-definable automorphism $x \mapsto x^p$ of $E$, the {\it Frobenius map,}\/ and the inverse
$y \mapsto y^{1/p}$
of this map is not given piecewise by rational functions. The $n$th iterate
$x \mapsto x^{p^n}$
of the Frobenius map has inverse $y \mapsto y^{1/p^n}$, and as we shall
see, these inverse maps are the only obstructions in getting an analogue in
positive characteristic of the above. Recall that a field $K$ of characteristic
$p > 0$ is said to be {\it perfect}\/ if every element of~$K$ is a $p$th power $x^p$ of some
$x \in K$. So every finite field is perfect. For any subfield $K$ of $E$
there is a smallest perfect subfield of $E$ containing $K$, namely
$$K^{1/p^\infty} := \bigcup_n K^{1/p^n} \quad\text{ where $K^{1/p^n}:= \big\{x^{1/p^n}: x \in K\big\} \subseteq E$,}$$
and by the next result $K^{1/p^\infty}$
is the definable closure of $K$ in $E$.

\begin{prop} Let $E$ be algebraically closed of characteristic $p > 0$, with
perfect subfield $K$. Then $K$ is definably closed in $E$.
\end{prop}

\noindent
The proof is identical to that of Proposition~\ref{prop:ACF(0) dcl}, using the fact that an
irreducible polynomial in one variable over a perfect field is separable.


\begin{cor}\label{cor:def fn ACF(p)}
Let $E$ be algebraically closed of characteristic $p > 0$, with
perfect subfield $K$, and let $X \subseteq E^n$ and $f \colon X \to E$ be $K$-definable in
$E$. Then there are  $P_1, \dots , P_k, Q_1, \dots , Q_k \in K[T]$ and an $m$ with the
following property: 
for each $x \in X$   there is $i \in \{1, \dots , k\}$ such that
$$Q_i(x^{1/p^m}) \neq 0\ \text{ and }\ f(x) = P_i(x^{1/p^m})/Q_i(x^{1/p^m}),$$
where $x^{1/p^m} := \big(x_1^{1/p^m},\dots,x_n^{1/p^m}\big)$ for $x = (x_1, \dots, x_n) \in E^n$.
\end{cor}

\noindent
Here is an application, usually stated only for injective endomorphisms of
algebraic varieties as a theorem of Ax: \index{theorem!Ax}

\begin{cor} \label{cor:Ax}
Let $E$ be algebraically closed, and suppose $X \subseteq E^n$ and
$f \colon X \to X$ are definable in $E$ and $f$ is injective. Then $f$ is surjective.
\end{cor}
\begin{proof} Consider first the case that $E$ is an algebraic closure of a finite field $K$
of characteristic $p > 0$. After increasing $K$ we can assume that $X$ and $f$ are
definable over $K$. Now $E$ is the union of the intermediate finite fields $F$ with
$K \subseteq F \subseteq E$, and all such $F$ being perfect, it follows from Corollary~\ref{cor:def fn ACF(p)} that~$f$ maps $X(F) := X \cap F^n$ into $X(F)$, so $f(X(F)) = X(F)$ by injectivity of $f$ and finiteness of $F$.
Taking the union over all these $F$ we get $f(X) = X$, so we are done for
this particular $E$. The corollary is equivalent to certain $\mathcal L_{\operatorname{Ri}}$-sentences  holding in all algebraically closed fields; we have shown
these sentences hold in all algebraic closures of finite fields. Therefore they
hold in all algebraically closed fields.
\end{proof}


 
\subsection*{Real closed fields}
In this subsection we view ordered fields as structures in the language $\mathcal L_{\operatorname{OR}}$, and we let $K$, $E$ and $F$ denote ordered fields.
We assume here that the reader is familiar with the basic 
{\em algebraic\/} facts concerning real closed fields as exposed in Section~\ref{sec:valued ordered fields}, partly
based on \cite[Chapter~XI]{Lang}.
The models of 
\begin{align*}
\operatorname{RCF}  := \operatorname{OFl}\ \cup\ \big\{ &\, \forall x \exists y\, ( x\geq 0 \to x=y^2 ), \\
& \,\forall u_1\cdots \forall u_{2n+1} \exists x \,( x^{2n+1} + u_{1} x^{2n} + \cdots + u_{2n+1} = 0 ) : n\geq 1 \big\},
\end{align*}
are the real closed ordered fields.
We have an analogue of Theorem~\ref{thm:ACF QE}: 

\nomenclature[Bi12]{$\operatorname{RCF}$}{theory of real closed ordered fields in the language $\mathcal L_{\operatorname{ORi}}$}


\begin{theorem}\label{thm:RCF QE}
$\operatorname{RCF}$ has \textup{QE.}
\end{theorem}
\begin{proof}
We use Proposition~\ref{prop:QE test, 3}.
Every ordered integral domain has an $\operatorname{RCF}$-closure, namely the
real closure of its ordered fraction field.
Let $E$ and $F$ be real closed and $K$ be a real closed
ordered subfield of both $E$ and $F$. Suppose  $E\neq K$  and~$F$ is $|K|^+$-saturated. It is enough to show that some ordered subfield of $E$ properly containing $K$ embeds
over $K$ into $F$.
Take any $a\in E\setminus K$. Then $a$ is transcendental over $K$ by Corollary~\ref{cor:AS}, and realizes a certain cut $A$
in $K$. Saturation gives an element $b\in F$ realizing the same
cut $A$. Then $b$ is transcendental over $K$, so we have a
field embedding $K(a)\to F$  over $K$ sending $a$ to $b$. This embedding is also order-preserving by Corollary~\ref{cor:propAS}. 
\end{proof}

\begin{example}
Let $\varphi(x_1,x_2)=\exists y\,( y^2+x_1y+x_2=0)$.
Then $\varphi$ is $\operatorname{RCF}$-equivalent to the quantifier-free
$\mathcal L_{\operatorname{OR}}$-formula $4x_2 \leq x_1^2$.
\end{example}

\noindent
The substructures of real closed ordered fields are exactly the ordered integral domains, so
$\operatorname{Th}(\operatorname{RCF})$ is the model completion of the theory of ordered integral domains.
The ordered integral domain $\Z$ embeds into every model of $\operatorname{RCF}$,
hence $\operatorname{RCF}$ is complete and thus decidable. %, by Theorem~\ref{thm:RCF QE} and Corollary~\ref{cor:QE and sentences},~(2), and thus decidable, by Corollary~\ref{cor:Completeness}.  

\begin{remark}
If $E$ is real closed, then $E\models x\geq 0 \leftrightarrow \exists y(y^2=x)$, so
the ordering of~$E$ is  definable by an existential $\mathcal L_{\operatorname{R}}$-formula.
Let $\operatorname{RCF}'$ be a set of $\mathcal L_{\operatorname{R}}$-sentences whose models are the real closed fields.
Then $\operatorname{RCF}'$ is model complete, but
does not have QE. 
(We have two field embeddings $\Q(\sqrt{2})\to\R$, one with $\sqrt{2}\mapsto \sqrt{2}$
and one with $\sqrt{2}\mapsto -\sqrt{2}$,
hence the ordering of $\R$ is not quantifier-free definable in the field $\R$.)
\end{remark}


\begin{cor}\label{cor:Tarski Principle}
The following are equivalent, for an $\mathcal L_{\operatorname{OR}}$-sentence $\sigma$:
\begin{enumerate}
\item $\sigma$ holds in the ordered field $\mathbb R$;
\item $\sigma$ holds in some real closed ordered field;
\item $\sigma$ holds in every real closed ordered field.
\end{enumerate}
\end{cor}

%\noindent
%Here is a sample application of the preceding corollary.

%\begin{exampleNumbered}\label{ex:division algebras}
%Let $K$ be real closed. A {\it division algebra}\/ over $K$ is
%a $K$-linear space $D\neq \{0\}$ equipped with a $K$-bilinear %map $(a,b)\mapsto ab\colon D\times D\to D$
%such that for all $a,b\in D$ with $b\neq 0$ there is unique pair $(x,y) \in D^2$ with $a = bx = yb$.
%{\it If $D$ is a division algebra over $K$ with $\dim_K D<\infty$,
%then $\dim_K D \in \{1,2,4,8\}$.}\/ This fact was shown for $K=\R$ by Bott-Milnor~\cite{BottMilnor} and Kervaire~\cite{Kervaire}. By Corollary~\ref{cor:Tarski Principle} it hence holds for every real closed $R$.
%(No other proof seems to be known.)
%\end{exampleNumbered}


\noindent
In the next three corollaries of Theorem~\ref{thm:RCF QE}, $E$ is real closed with ordered subfield $K$, and
$T=(T_1,\dots,T_n)$ is an $n$-tuple of distinct indeterminates.
First an analogue of part (1) of Corollary~\ref{cor:ACF QE}
for $\operatorname{RCF}$: \index{theorem!Tarski-Seidenberg}


\begin{cor}\label{cor:RCF QE}
A set $X\subseteq E^n$ is $K$-definable in $E$ iff $X$ is a 
boolean
combination  of   sets of the form
$\big\{a \in  E^n : P(a) \geq 0\big\}$ where $P \in  K[T]$.
\textup{(}In particular, if~$K$ is real closed, then the $K$-definable subsets of $E$ are exactly the finite unions
of singletons and intervals $(a,b)$ where $a<b$ are in $K\cup\{-\infty,\infty\}$.\textup{)}
\end{cor}



\begin{exampleNumbered}\label{ex:RCF QE}
The set $X=\{r\in\R:r\leq \pi\}$ is $\R$-definable in $\R$ but not $0$-definable in~$\R$.
(Take $E=\R$ and $K=\Q^{\operatorname{rc}}\subseteq\R$ in the previous corollary.) 
\end{exampleNumbered}

%\noindent
%For $A\subseteq E$ the
%definable closure~$\operatorname{dcl}(A)$ of $A$ in~$E$ agrees with the algebraic closure $\operatorname{acl}(A)$ of
%$A$ in $E$, by Lemma~\ref{lem:dcl=acl}.

\begin{prop}\label{prop:dcl RCF} The definably closed subsets of $E$ are exactly \textup{(}the underlying sets of\textup{)} the real closed subfields of $E$.
%The subset $K$ is definably closed in $E$ 
%iff the subfield $K$ of~$E$ is real closed.
\end{prop}
\begin{proof}
If $K$ is real closed, then $K\preceq E$ by QE, hence $K$ is definably closed in~$E$.
Conversely, suppose $K$ is definably closed in $E$. Then 
$K$ is (the underlying set of) a subfield of $E$. The $0$-definable ordering on $E$ guarantees that $K$ is algebraically closed in~$E$ in the field-theoretic sense. Hence $K$ is real closed by Corollary~\ref{cor:AS}.
\end{proof}

\noindent
In the next corollary $U$ is an indeterminate different from $T_1,\dots,T_n$.

\begin{cor}
Let $X \subseteq E^n$ and $f \colon X \to E$ be $K$-definable in $E$. Then
there exists $P\in K[T,U]^{\neq}$  such that $P\big(x,f(x)\big)=0$ for all $x \in X$.
\end{cor}
\begin{proof}
We can assume $E$ is $|K|^+$-saturated. Let
$x \in X$. Then $\operatorname{dcl}(K \cup \{x\})$ equals the real closure of $K(x)$ in $E$, by
Proposition~\ref{prop:dcl RCF}, and contains
$f(x)$. So $Q\big(x,f(x)\big)=0$ for some  $Q\in K[T,U]^{\neq}$.  By saturation we get $Q_1,\dots,Q_m\in K[T,U]^{\neq}$ such that for each $x\in X$ we have $Q_i(x,f(x))=0$ for some $i\in\{1,\dots,m\}$; now put $P:=Q_1\cdots Q_m$.
\end{proof}

\noindent
In the proof of the corollary above
we tacitly used that for a real closed ordered field extension $F$ of $E$, and $X\subseteq E^n$ and $f\colon X \to E$ that are $K$-definable in $E$, we have a $K$-definable
set $X_F\subseteq F^n$ with $X_F\cap E^n=X$, and an extension
of $f$ to a $K$-definable function $f_F\colon X_F\to F$:
define $X_F$ in $F$ by any formula defining~$X$ in $E$, and likewise with $f_F$, and note that $X_F$, $f_F$ do not
depend on the choice of these formulas.
We finish this section with an application to the 
asymptotics of functions definable in the ordered field~$\R$; in the proof we employ some facts about Hahn fields from Section~\ref{sec:valued ordered fields}. 

\begin{cor}
Let  $f\colon (a,\infty)\to \R$ \textup{(}$a\in\R$\textup{)} be definable in the ordered field~$\R$.
Then $f(r)\to 0$ as $r\to\infty$, or there are 
$c\in \R^\times$, $q\in\Q$ with $f(r)/cr^q \to 1$ as $r\to\infty$.
\end{cor}
\begin{proof}
Consider the real closed ordered field extension $E=\R[[ x^{\Q} ]] $ (so $x>\R$). Suppose $f(r)\not\to 0$ as $r\to\infty$. Then we have $\varepsilon\in\R^>$ such that $|f(r)| \geq \varepsilon$ for arbitrarily large real $r>a$, and thus for all sufficiently large real $r>a$.
Hence $|f_E(x)|\ge \varepsilon$, so $f_E(x)\ne 0$, and
thus $f_E(x)=cx^q(1+\delta)$ with $c\in\R^\times$, $q\in\Q$, and some infinitesimal $\delta$ in $E$. Hence for every
$\varepsilon\in \R^{>}$ we have 
$\left|\frac{f_E(x)}{cx^q} - 1\right|<\varepsilon$, and thus
$\left|\frac{f(r)}{cr^q} - 1\right|<\varepsilon$ for all sufficiently large real $r>a$.
\end{proof}

\begin{exampleNumbered}[H\"ormander]\label{ex:Hormander}
Let $P\in \R[T]$ and define $f\colon \R^>\to\R$ by
$$f(r) := \min \big\{ |P(a)| : a=(a_1,\dots,a_n)\in\R^n,\ |a_1|+\cdots+|a_n|=r \big\}.$$
Then   $f(r)\to 0$ as $r\to\infty$, or there are 
$c\in \R^\times$, $q\in\Q$ with $f(r)/cr^q \to 1$ as $r\to\infty$. 
\end{exampleNumbered}

%\noindent
%Let $x=(x_1,\dots,x_n)$. By QE, if $E$, $F$ are real closed with common ordered subfield~$K$, then $\operatorname{S}^E_x(K)=\operatorname{S}^F_x(K)$; we set $\operatorname{S}_x(K):=\operatorname{S}^{E}_x(K)$ where $E$ is a real closure of~$K$. Let $\operatorname{C}(K)$ be the set of cuts in the ordered set $K$. Then $\operatorname{C}(K)$  is totally ordered by inclusion; we equip $\operatorname{C}(K)$  with the corresponding order topology.  For each $p\in \operatorname{S}_v(K)$ the set $C_p:=\{a\in K:\textup{``$a < v$''}\in p\}$ is a cut in $K$. As a consequence of Corollary~\ref{cor:RCF QE} we obtain a description of $v$-types:
 
%\begin{cor}
%Suppose $K$ is real closed. If $p$ is not realized in $K$, then an element $b$ in a real closed ordered field extension of $K$ realizes $p$ iff $b$ realizes~$C_p$. The map $p\mapsto C_p$ is a continuous bijection from the closed subset of types in~$\operatorname{S}_v(K)$ which are not realized in $K$ onto $\operatorname{C}(K)$.
%\end{cor}
 
\subsection*{Notes and comments}
Theorem~\ref{thm:ACF QE} was known to Tarski (see \cite[p.~54, Note~16]{Ta}), but
the first published proof was given by Seidenberg \cite[p.~373]{Se}.
Part~(1) of Corollary~\ref{cor:ACF QE} is also due independently to Chevalley~\cite[Th\'eo\-r\`eme~3, Corollaire]{Chevalley55}; see also \cite{Seidenberg69}. A. Robinson~\cite{Robinson57} saw
model-theoretic significance in Hilbert's Nullstellensatz~\cite{Hilbert93}. 
%was realized by Abraham Robinson~\cite{Robinson57}, 
This led him to
the notion of model completeness. 
%realized its model-theoretic significance. %  and also showed  Cor\-ol\-lary~\ref{cor:ACF QE, uniform}
Corollary~\ref{cor:Lefschetz} may be seen as a model-theoretic formulation of a heuristic principle in algebraic geometry named after Lefschetz~\cite[p.~242f]{Weil}. See~\cite{Seidenberg58} for a discussion of this principle and \cite{BarwiseEklof, Eklof} for other attempts to make it
precise.
Example~\ref{ex:Serre} is from~\cite{Serre09}. Corollary~\ref{cor:Ax} for endomorphisms of algebraic varieties $X$ is due to Ax~\cite{Ax68,Ax69}, and, independently,
to Grothendieck \cite[\S{}10.4.11]{EGAIV}; 
Borel~\cite{Borel69} gave a different proof of this result for $K=\C$. 

Theorem~\ref{thm:RCF QE} is due to Tarski~\cite{Tarski31,Ta}. The proof above was given by A.~Robinson~\cite{Robinson56}, who also used this theorem to derive in a few lines a solution of
Hilbert's 17th Problem, originally solved by Artin~\cite{Artin27}; see \cite{Robinson55a,Robinson55b}. Other proofs of Theorem~\ref{thm:RCF QE}
were given by {\L}ojasiewicz~\cite{Lojasiewicz} and Seidenberg~\cite{Se}. See \cite{vdDries88} for the history of Tarski's theorem and some applications.
A real Nullstellensatz (analogue of part (3) of Corollary~\ref{cor:ACF QE}) was proved  by Dubois~\cite{Dubois},
Krivine~\cite{Krivine}, and Risler~\cite{Risler}; see \cite[Section~4.1]{BCR}.
Corollary~\ref{cor:Tarski Principle} is sometimes called the ``Tarski Principle''.
%Example~\ref{ex:division algebras} is from~\cite{Robinson73}, and
Example~\ref{ex:Hormander} is from~\cite[Lemma~3.9]{Hormander}.
  




\section{Structures without the Independence Property}
\label{sec:structures having NIP}

\noindent
In the previous sections we assembled a toolbox that 
 helps in finding an intelligible description of  
 the sets and maps definable in a structure $\mathbf M$. Such a description often leads to useful geometric invariants (dimensions, Euler characteristics, \dots) of these objects. 
 But in this final section of the appendix we take another path by considering a robust dividing line in the realm of all structures discovered by Shelah. The tame side of this dividing line is called:  {\it not having the independence property}\/~(NIP).
%Other related notions are {\it  o-minimality}\/ and {\it stability.}\/ (See the notes and comments at the end of this section.)
The NIP condition forbids certain combinatorial patterns in the definable binary relations of a structure. (As is often the case in this subject, a ``tame'' property is introduced here as the negation of a ``wild'' one.) 
Motivating NIP is a striking combinatorial dichotomy (Theorem~\ref{thm:SS}), which we prove first.
This dichotomy leads to the definition of a measure of complexity for families of sets called
{\it VC dimension}\/ and a dual quantity known as {\it independence dimension.}\/
After discussing these quantities we introduce the NIP property, and show that real closed fields have NIP.
(This fact is used in our proof that $\mathbb T$ has NIP in Section~\ref{sec:embth}.) \index{NIP} \index{structure!independence property}

\subsection*{VC dimension} Given a set $A$ we let $2^A$ be the power set of $A$ and
${A\choose n}$ the set of $n$-element subsets of $A$.
{\it Throughout this subsection $X$ is an infinite set and $\mathcal S$ a collection of subsets of $X$.}\/ 
For $A\subseteq X$ we set $\mathcal S\cap A:=\{S\cap A:S\in\mathcal S\}$, and we say that~$A$ is {\bf shattered} by~$\mathcal S$ if $\mathcal S\cap A=2^A$. \index{shattering}
We have a function $\pi_{\mathcal S}: \N \to \N$ given by
$$\pi_{\mathcal S}(n)\ :=\ \max\left\{\abs{\mathcal S\cap A}:\ A\in{X\choose n}\right\}.$$
Thus $0\leq\pi_{\mathcal S}(n)\leq 2^n$, and
$\pi_{\mathcal S}(n)=2^n$ means: some $A\in {X\choose n}$ is shattered by $\mathcal S$.
If $\pi_{\mathcal S}(n)=2^n$, then $\pi_{\mathcal S}(m)=2^m$ for all $m\leq n$. Here is the promised dichotomy:

\begin{theorem}[Sauer, Shelah]\label{thm:SS} \index{theorem!Sauer-Shelah}
Either $\pi_{\mathcal S}(n)=2^n$ for all $n$, or else there exists $d\in\N$ such that $\pi_{\mathcal S}(n)\le n^d$ for all sufficiently large $n$. 
\end{theorem}

\noindent 
%We prove the theorem in the stronger form: Theorem~\ref{ }. 
Here is the result from finite combinatorics that underlies
our dichotomy:


\begin{lemma}\label{lem:SS} Suppose $|A|=n$, and $\mathcal C\subseteq 2^A$ and $d\in \{0,\dots,n\}$ are such that $|\mathcal C| > \sum_{i<d} {n\choose i}$. Then $A$ has a subset $B$ with $|B|=d$ that is shattered by $\mathcal C$.
\end{lemma}

\noindent
The hypothesis is sharp since the collection of subsets of $A$ of size $<d$ has cardinality equal to the indicated sum of binomial coefficients, and this particular collection violates the conclusion of the lemma.
Let us denote the indicated sum of binomial coefficients by $p_d(n)$. There is clearly a unique polynomial $p_d(X)\in \Q[X]$ (of degree~${d-1}$ if $d\ge 1$, and
$p_0(X)=0$), whose value at $n$ is $p_d(n)$ for $n\ge d$. Note that
$$p_{d-1}(X-1)+p_d(X-1)\ =\ p_d(X) \qquad (d\ge 1).$$

\begin{proof}[Proof of Lemma~\ref{lem:SS}] 
By induction on $n$. The desired result holds trivially for
$d=0$ and $d=n$, so let $0 < d < n$. Pick a point $a\in A$ and set $A':= A\setminus \{a\}$. Also put $C':= C\setminus \{a\}$
for $C\in \mathcal C$, and set $\mathcal{C}':=\{C': C\in \mathcal{C}\}$. Under the map $C\mapsto C'\colon \mathcal{C} \to \mathcal{C}'$ a set $D\in \mathcal{C}'$ has either exactly one preimage or exactly two preimages; in the latter case these two preimages are $D$ and $D\cup\{a\}$. So $\mathcal{C}'=\mathcal{C}_1\cup \mathcal{C}_2$ (disjoint union) where $\mathcal{C}_1$ contains those $D\in \mathcal{C}'$ having one preimage in $\mathcal{C}$, and $\mathcal{C}_2$ those with two preimages. If $|\mathcal{C}'|>p_d(n-1)$, then by the inductive
assumption applied to $A'$ and $\mathcal{C}'$ there exists
$B\subseteq A'$ of size $d$ that is shattered by $\mathcal{C}'$
and thus by $\mathcal{C}$. 
So assume $|\mathcal{C}'|\leq p_d(n-1)$. Then
\begin{align*} 
p_d(n-1)+p_{d-1}(n-1)\  =\  p_d(n)\ &<\ |\mathcal{C}|\ =\ |\mathcal{C}_1| + 2|\mathcal{C}_2|\ =\ \big(|\mathcal{C}_1| + |\mathcal{C}_2|\big) + |\mathcal{C}_2|\\ 
&=\ |\mathcal{C}'| + |\mathcal{C}_2|,
\end{align*}
hence $|\mathcal{C}_2|>p_{d-1}(n-1)$, so again by the inductive assumption applied to $A'$ and~$\mathcal{C}_2$ we get 
$B'\subseteq A'$ of size $d-1$ that is shattered by $\mathcal{C}_2$. Since for each $D\in \mathcal{C}_2$ we have
$D\in \mathcal{C}$ and $D\cup\{a\}\in \mathcal{C}$, the set
$B:= B'\cup\{a\}$ is shattered by $\mathcal{C}$.
\end{proof}

\noindent
This yields Theorem~\ref{thm:SS} in a slightly stronger form:

\begin{theorem}\label{thm:SS+} If $d\in \N$ and $\pi_{\mathcal{S}}(d)< 2^d$, then
$\pi_{\mathcal{S}}(n)\le p_d(n)$ for all $n$.
\end{theorem}
\begin{proof} Assume $\pi_{\mathcal{S}}(d)< 2^d$. Then the desired inequality holds for $n<d$, since $p_d(n)=2^n$ for such $n$. Let $n\ge d$ and $A\in {X \choose n}$. If 
$|\mathcal{S}\cap A|>p_d(n)$, then the above lemma would give a set $B\subseteq A$ of size $d$ shattered by $\mathcal{S}$, a contradiction. 
\end{proof}  


\noindent 
We define $$\operatorname{VC}(\mathcal S)\ :=\ \sup\big\{n:\pi_{\mathcal S}(n)=2^n\big\}\in\N\cup\{-\infty, \infty\},$$
so $\operatorname{VC}(\mathcal{S}):=-\infty$ iff $\mathcal{S}=\emptyset$, and $\operatorname{VC}(\mathcal S)=\infty$ iff subsets of~$X$ of arbitrarily large finite size are shattered by~$\mathcal S$.
We call $\operatorname{VC}(\mathcal S)$
 the {\bf VC dimension}  of $\mathcal S$ and say that $\mathcal S$ is a {\bf VC class} if 
$\operatorname{VC}(\mathcal S)<\infty$.
\index{VC!dimension}\index{VC!class}\index{dimension!VC}





\subsection*{Independence dimension}
Let $X$ be a nonempty set.
Given $A_1,\dots,A_n\subseteq X$ we let $S(A_1,\dots,A_n)$ be the set of atoms of the boolean algebra of subsets of $X$ that is generated by the $A_j$: the ``nonempty fields in the Venn diagram of $A_1,\dots,A_n$''; that is, the elements of
$S(A_1,\dots,A_n)\subseteq 2^X$ are the nonempty sets 
$$\bigcap_{i\in I} A_i \cap \bigcap_{i\in [n]\setminus I} X\setminus A_i\qquad\text{where $I\subseteq [n]:=\{1,\dots,n\}$.}$$ 
Thus $S(A_1,\dots, A_n)=\{X\}$ when $n=0$, and always $S(A_1,\dots, A_n)\ne \emptyset$. 
%Note that $S(A_1,\dots,A_n)$ does not depend on the particular order of the $A_i$.

\begin{lemma}\label{lem:atoms BC}
Let $A_1,\dots,A_m,B_1,\dots,B_n\subseteq X$. Then
\begin{enumerate}
\item $|S(A_1,\dots,A_m,B_1,\dots,B_n)| \leq |S(A_1,\dots,A_m)|\cdot |S(B_1,\dots,B_n)|$, and
\item if $A_1,\dots,A_m$ are boolean combinations of $B_1,\dots,B_n$, then
$$|S(A_1,\dots,A_m)|\ \leq\ |S(B_1,\dots,B_n)|.$$
\end{enumerate}
\end{lemma}
\begin{proof}
Part (1) is clear. For (2) note that under the hypothesis of (2),
 the boolean algebra of subsets of $X$ generated by the $B_j$ contains that generated by the $A_i$ as a subalgebra, so every atom of the latter is a disjoint union
of atoms of the former. 
\end{proof}


\noindent
We have $1\leq \abs{S(A_1,\dots,A_n)}\leq 2^n$, and we say that the sequence $A_1,\dots,A_n$ is {\bf independent}~(in~$X$) if $\abs{S(A_1,\dots,A_n)}=2^n$, and call $A_1,\dots,A_n$ {\bf dependent}~(in~$X$) otherwise. Next, let $\mathcal S\subseteq 2^X$, $\mathcal S \ne \emptyset$. Define  
$$\pi^{\mathcal S}(n)\ :=\ \max\big\{\abs{S(A_1,\dots,A_n)}:A_1,\dots,A_n\in\mathcal S \big\}.$$
Note that 
$1\leq \pi^{\mathcal S}(n)\leq 2^n$ for each $n$. 
We say that $\mathcal S$ is {\bf independent} (in $X$) if $\pi^{\mathcal S}(n)=2^n$ for every $n$, that is, if for every $n$ there is an independent sequence of elements of $\mathcal S$ of length $n$. Otherwise, we say that $\mathcal S$ is {\bf dependent} (in $X$). If $\mathcal S$ is dependent, we define the {\bf independence dimension}  of $\mathcal S$ as the largest $n$ such that $\pi^{\mathcal S}(n)=2^n$; notation: $n=\operatorname{IND}(\mathcal S)$. If $\mathcal S$ is independent, we set $\operatorname{IND}(\mathcal S)=\infty$.
If $\mathcal S$ is finite, then clearly $\operatorname{IND}(\mathcal S)\leq \abs{\mathcal S}$. 
\index{dimension!independence}\index{independent}\index{dependent}

\subsection*{VC duality} \index{VC!duality}
Often our collection $\mathcal S$ will be indexed by elements of a parameter
space or index set, and then the set $X$ and this index set play dual roles. To
make this duality explicit, let $X$ and $Y$ be infinite sets and $\Phi\subseteq X\times Y$. For $x\in X$,~$y\in Y$,
\begin{align*} \Phi_x\   &:=\ \big\{ y\in Y:\ (x,y) \in\Phi \big\},  \qquad  \Phi_X\ :=\ \{\Phi_x:\ x\in X\}\subseteq 2^Y\\
\Phi^y\   &:=\ \big\{ x\in X:\ (x,y) \in\Phi \big\},  \qquad  \Phi^Y\ :=\ \{\Phi^y:\ y\in Y\}\subseteq 2^X.
\end{align*} 
One verifies easily that, given a finite set $A=\{x_1,\dots, x_n\}\subseteq X$, the map
$$B \mapsto \bigcap_{x\in B} \Phi_x \cap \bigcap_{x\in A\setminus B} Y\setminus \Phi_x\ \colon\ \Phi^Y\cap A \to S(\Phi_{x_1},\dots, \Phi_{x_n})$$
is a bijection. It follows that $\pi_{\Phi^Y} = \pi^{\Phi_X}$.
%We set $\operatorname{VC}(\Phi):=\operatorname{VC}(\Phi^Y)$.
Thus $\operatorname{VC}(\Phi^Y)=\operatorname{IND}(\Phi_X)$. %, hence $\mathcal S_\Phi$ is a VC class iff $\mathcal S_{\Phi^*}$ is dependent.
Reversing the role of $X$ and $Y$ also yields $\operatorname{VC}(\Phi_X)=\operatorname{IND}(\Phi^Y)$.
 %, and $\mathcal S_{\Phi^*}$ is a VC class iff $\mathcal S_{\Phi}$ is dependent. 
 
\begin{lemma}\label{lem:dual shatter, 2} If 
$\operatorname{VC}(\Phi^Y)< \infty$, then
$\operatorname{VC}(\Phi_X)<2^{1+\operatorname{VC}(\Phi^Y)}$. %\textup{(}In particular $\mathcal S_{\Phi^*}$ is a VC class iff $\mathcal S_{\Phi}$ is a VC class.\textup{)}
\end{lemma} 
\begin{proof}
Let $\varepsilon$ range over the  set of functions $[n]\to \{-1,+1\}$.
Suppose $\operatorname{VC}(\Phi_X)=\operatorname{IND}(\Phi^Y)\geq 2^n$. This yields an independent family 
$\big(\Phi^{y_{\varepsilon}}\big)_\varepsilon$ of $2^n$ subsets of $X$ (with $y_\varepsilon\in Y$ for all $\varepsilon$). So for each $m\in [n]$
 we have 
 $$\bigcap_{\varepsilon(m)=+1} \Phi^{y_\varepsilon} \cap \bigcap_{\varepsilon(m)=-1} (X\setminus\Phi^{y_\varepsilon})\ \neq\ \emptyset,$$ so we can take an element $x(m)$ of the intersection
 on the left. Then
 for each $\varepsilon$ and $m\in [n]$ we have: $x(m)\in\Phi_{y_\varepsilon}\Longleftrightarrow \varepsilon(m)=+1$,
 so $x(1),\dots, x(n)$ are distinct and the set
 $\{x(1),\dots,x(n)\}$ is shattered by $\Phi^Y$. Hence
 $\operatorname{VC}(\Phi^Y)\geq n$.
 \end{proof}

\noindent
We therefore have the equivalences
$$\text{$\Phi^Y$ is dependent}\ \Leftrightarrow\ 
\text{$\Phi_X$ is a VC class}\ \Leftrightarrow\ 
\text{$\Phi^Y$ is a VC class}\ \Leftrightarrow\ 
\text{$\Phi_X$ is dependent}.$$
We say that $\Phi$ is {\bf dependent} if $\Phi^Y$ is dependent. \index{dependent}
We also set $\pi^\Phi:=\pi^{\Phi^Y}$.

\medskip\noindent
Let $\neg\Phi$ be the relative complement $(X\times Y)\setminus \Phi$ of $\Phi$ in~$X\times Y$. It is clear that $\pi^{\neg\Phi}=\pi^{\Phi}$. 
For
 $\Phi,\Psi\subseteq X\times Y$ we have $\pi^{\Phi\cup\Psi},\pi^{\Phi\cap\Psi} \leq \pi^{\Phi}\cdot\pi^{\Psi}$, by Lemma~\ref{lem:atoms BC}. By Theorem~\ref{thm:SS},
this yields:

\begin{lemma} \label{lem:VC for boolean combinations}
If $\Phi,\Psi\subseteq X\times Y$ are dependent, then so are $\neg\Phi$, $\Phi\cup\Psi$, and $\Phi\cap\Psi$.
\end{lemma}

\subsection*{NIP} Let $\mathbf M$ be an $\mathcal L$-structure 
each of whose underlying sets $M_s$ is infinite. Then we define
$\mathbf M$ to have NIP (short for:
 the non-independence property) if every $0$-definable
relation $\Phi\subseteq M_x\times M_y$ with 
finite nonempty multivariables $x,y$ 
is dependent.
Note that if $\mathbf M$ has NIP, then so does $\mathbf M_A$ for each parameter set $A$ in~$\mathbf M$, and so does
every reduct of $\mathbf M$. If
$\mathbf M$ has NIP and  $\mathbf M\equiv\mathbf N$, then
$\mathbf N$ has~NIP. Thus $\mathbf M$ having NIP is really a property of its theory $\operatorname{Th}(\mathbf M)$.

\index{NIP} \index{structure!independence property}\index{structure!NIP} \index{theory!NIP}

Our goal in this subsection is to show that real closed fields have NIP. We obtain this as a consequence of the following:

\begin{prop}\label{prop:Dudley}
Let $\mathcal F$ be an $m$-dimensional real vector space of real-valued functions on an infinite set $X$, and for
each $f\in \mathcal F$, put $$\operatorname{pos}(f):=\big\{x\in X:f(x)>0\big\}.$$ 
Then $\operatorname{pos}(\mathcal F):=\big\{\operatorname{pos}(f):f\in\mathcal F\}$ is a VC class 
of VC dimension $m$.
\end{prop}
\begin{proof}
Let $A\in {X\choose m+1}$. The restriction map
$f\mapsto f|A\colon\mathcal F\to\R^A$ is not surjective, 
since
$\dim\R^A=m+1>\dim\mathcal F$. Therefore we can take
a nonzero $w\in\R^A$ that is orthogonal to all restrictions
$f|A$ ($f\in\mathcal F$) with respect to the standard
inner product $\<u,v\>:=\sum_{a\in A} u(a)\cdot v(a)$ on $\R^A$.
Replacing $w$ by $-w$ if necessary we can assume that
$A^+:=\{a\in A:w(a)>0\}$ is nonempty. 
If there were $f\in\mathcal F$ with $A^+=A\cap\operatorname{pos}(f)$,
then we would have $0=\<w,f|A\>=\sum_{a\in A} w(a)\cdot f(a)>0$,
a contradiction. Hence $A$ is not shattered by $\operatorname{pos}(\mathcal F)$.
Thus $\operatorname{VC}(\operatorname{pos}(\mathcal F))\leq m$,
and we leave the proof that equality holds as an exercise.
\end{proof}

\noindent
The proposition applies to the vector space of all real polynomial functions on ${X=\R^n}$~(${n\geq 1}$) of degree $\leq d$. 
Together with Theorem~\ref{thm:RCF QE} and Lemma~\ref{lem:VC for boolean combinations} this yields at once:

\begin{cor}\label{cor:RCF NIP}
Real closed fields have \textup{NIP}.
\end{cor}

\subsection*{Notes and comments}
Theorem~\ref{thm:SS} was found independently by Sauer~\cite{Sauer} and Shelah~\cite{Shelah72b}.
The notion of VC class first arose in probability theory in the work of Vapnik and Chervonenkis~\cite{VC}. The independence property was introduced into model theory by Shelah~\cite{Shelah71a}, who also proved in \cite{Shelah71b}
by a curious set-theoretic argument the very useful fact that in the above definition of NIP
it suffices to consider the case that $x$ is a single variable.
Laskowski~\cite{Laskowski} realized the connection between  VC classes  and NIP and 
 gave a more elementary proof of the reduction to a single variable;  see \cite[Chapter~5]{vdDries98} for an exposition.
Proposition~\ref{prop:Dudley} was shown in \cite[Theorem~7.2]{Dudley78} and used in~ 
\cite{StengleYukich} to prove that the ordered field $\R$ has NIP.
More generally, all {\it o-minimal}\/ structures have NIP \cite{PillaySteinhorn},
and so do many other structures: for example,    {\it stable}\/ structures 
(such as algebraically closed fields); ordered abelian groups \cite{GurevichSchmitt},
and the field $\Q_p$ of $p$-adic numbers~\cite{Belair}. 
For more about the significance of NIP in model theory, see~\cite{SimonNIP}.


